Introduction into Geometry over Division Ring

Theory of representations of F-algebra is a natural development of the theory of F-algebra. Exploring of morphisms of the representation leads to the concepts of generating set and basis of representation. In the book I considered the notion of tower of representations of F_i-algebras, i=1, ..., n, as the set of coordinated representations of F_i-algebras. I explore the geometry of affine space as example of tower of representations. Exploration of curvilinear coordinates allows us to see how look at the main structures of the manifold with affine connection. I explore Euclidean space over division ring.

==> Abstract.0906.0135.English.tex <==
%auto-ignore

\begin{abstract}
Theory of representations of universal algebra
is a natural development of the theory of universal algebra.
Exploring of morphisms of the representation leads to the concepts 
of generating set and basis of representation.
In the book I considered the notion of tower of left\Hyph side representations of
$\Omega_i$\Hyph algebras, $i=1$, ..., $n$,
as the set of coordinated left\Hyph side representations of
$\Omega_i$\Hyph algebras.

I explore the geometry of affine space as example of tower of representations.
Exploration of curvilinear coordinates allows us to see how look
at the main structures of the manifold with affine connection.
I explore Euclidean space over division ring.
\end{abstract}



==> Abstract.0906.0135.Russian.tex <==
%auto-ignore

\begin{abstract}
Теория представлений универсальной алгебры
является естественным развитием теории универсальной алгебры.
Изучение морфизмов представлений ведёт к понятиям
множества образующих и базиса представления.
В книге рассмотрено понятие башни левосторонних представлений
$\Omega_i$\Hyph алгебр, $i=1$, ..., $n$,
как множество согласованных левосторонних представлений
$\Omega_i$\Hyph алгебр.

Рассматривается геометрия аффинного пространства как пример башни представлений.
Изучение криволинейных координат позволяет понять как
выглядят основные структуры в многообразии аффинной связности.
Рассматривается геометрия эвклидова пространства над телом.
\end{abstract}


==> Affine.Calculus.Russian.tex <==
%auto-ignore
\input{Affine.Calculus.Eq}
\chapter{Математический анализ в \texorpdfstring{$A$}{A}-аффинном пространстве}
\labelChapter{Calculus in Affine Space}

\section{Криволинейные координаты в
\texorpdfstring{$A$}{A}-аффинном пространстве}

\ifx\texFuture\Defined
Все векторы, которые имеют общее начало $A$ порождают векторное пространство,
которое мы будем называть касательным векторным пространством $T_A\mathcal{A}_n$.
Топология, которую $\mathcal{A}_n$ наследует из отображения $\mathcal{A}_n\rightarrow R^n$,
позволяет нам изучать непрерывные преобразования пространства $\mathcal{A}_n$
и их производные. Более точно, производная
преобразования $f$ отображает векторное пространство $T_A\mathcal{A}_n$ в $T_{f(A)}\mathcal{A}_n$.
Если $f$ линейно, то его производная одна и та же в каждой точке.
\fi

Пусть $\overset{\rightarrow}{V}$ -
аффинное пространство над банаховой алгеброй $A$ с делением.\,\footnote{В этом
разделе я изучаю криволинейные координаты аналогично тому,
как это сделано в \citeBib{Rashevsky}, глава V.}
Пусть
\ShowEq{basis 1 n D affine space} -
базис аффинного пространства и
\ShowEq{OM=viei}

Рассмотрим отображение
\ShowEq{set of maps O+fe}
Мы можем отождествить множество производных
\ShowEq{derivative O+fe}
и базис \eV правого $A$\Hyph векторного пространства $V$.

Рассматрим гомеоморфизм
\ShowEq{map and coordinates, D affine space}
как множество отображений
\ShowEq{coordinates V->A}
таких, что
\ShowEq{map and vector of affine basis}
Равенство
\ShowEq{v=f(x1n)}
является следствием равенств
\EqRef{OM=viei},
\EqRef{map and vector of affine basis}.
Мы будем говорить, что образ точки $A$ при отображении $f$
является
\AddIndex{криволинейными координатами точки}
{curvilinear coordinates of point in affine space}
$A$,
а отображение $f$ будем называть системой координат.

\ifx\texFuture\Defined
Если даны две системы координат, $f_1$ и $f_2$,
то отображение $g=f_1f_2^{-1}$ является гомеоморфизмом
\ShowEq{map and coordinates, 1, D affine space}
и называется преобразованием координат.
Преобразование координат, порождённое аффинным преобразованием,
можно рассматривать как частный случай.
\fi

\begin{Remark}
\labelRemark{surface in D affine space}
Рассмотрим поверхность $S$ в аффинном пространстве, определённую уравнением
\ShowEq{line in affine space, 1}
Пусть $M(\aU xi)$ - произвольная точка.
Малое изменение координат точки
\ShowEq{line in affine space, 2}
приводит к малому изменению функции
\ShowEq{line in affine space, 3}
В частности, если бесконечно близкие точки
$M(\aU xi)$ и $L(\aU xi+\Delta\aU xi)$
лежат на одной поверхности, то вектор приращения
$\overset{\longrightarrow}{ML}=\Delta x$
удовлетворяет дифференциальному уравнению
\ShowEq{line in affine space, 4}
и называется вектором, касательным к поверхности $S$.
\end{Remark}

\ifx\texFuture\Defined
Так как производная Гато отображения $f$ в точке $X$
является линейным отображением, то эта производная является
$1$\Hyph$D$\Hyph формой.
Рассмотрим множество $1$\Hyph$D$\Hyph форм
\ShowEq{basis 1 d form, affine space}
Очевидно, что
\ShowEq{basis 1 d form, 1, affine space}
Производную Гато произвольной функции можно представить
в виде
\ShowEq{basis 1 d form, 2, affine space}
Следовательно, производная Гато функции $f$ является линейной комбинацией
$1$\Hyph$D$\Hyph форм $dx^i$.
Пусть
\ShowEq{map and coordinates, 1, D affine space}
преобразование координат аффинного пространства.
Из правила дифференцирования сложной функции
(теорема
\xRef[0812.4763]{theorem: composite map, differential, D vector space})
следует
\ShowEq{basis 1 d form, 3, affine space}
\fi

Координатная линия - это кривая, вдоль которой изменяется только
одна координата $\aU xi$.
%Координатную кривую можно рассматривать либо как
%пересечение поверхностей $x^j=\const$, $j\ne i$, либо как кривую,
Мы будем рассматривать координатную кривую как кривую,
имеющую касательный вектор
\ShowEq{local basis of affine space}
\ShowEq{map and coordinates, 3, D affine space}
%В обоих случаях координаты вектора $\aD xi$
%имеют вид $x^k_i=\delta^k_i$.
Пусть точка $O$ имеет координаты $x$.
Базис аффинного пространства имеет вид
\ShowEq{map and coordinates, 2, D affine space}
%В частности, если точки
%$M(x^i)$ и $L(x^i+\Delta x^i)$ бесконечно
%близки, то вектор $\overset{\longrightarrow}{ML}$
%можно представить в виде
%\ShowEq{map and coordinates, 4, D affine space}

\ifx\texFuture\Defined
Пусть
\ShowEq{map and coordinates, 1, D affine space}
преобразование координат аффинного пространства.
Из правила дифференцирования сложной функции
(теорема
\xRef[0812.4763]{theorem: composite map, differential, D vector space})
следует
\ShowEq{map and coordinates, 5, D affine space}
Из сравнения равенств
\EqRef{map and coordinates, 2, D affine space},
\EqRef{map and coordinates, 5, D affine space}
следует закон преобразования координат вектора
\ShowEq{map and coordinates, 6, D affine space}
\fi

\ifx\texFuture\Defined
\begin{example}
Рассмотрим линейное преобразование координат
\ShowEq{D affine space, example, 1, 1}
Тогда
\ShowEq{D affine space, example, 1, 2}
Из равенств
\EqRef{D affine space, example, 1, 2, x1},
\EqRef{D affine space, example, 1, 2, x2}
следует обратное преобразование
\ShowEq{D affine space, example, 1, 3}
Из равенств \EqRef{D affine space, example, 1, 1}
следует закон преобразования $1$\Hyph$D$\Hyph форм
\ShowEq{D affine space, example, 1, 4}
Из равенств
\EqRef{map and coordinates, 6, D affine space},
\EqRef{D affine space, example, 1, 3}
следует закон преобразования координат вектора
\ShowEq{D affine space, example, 1, 5}
\qed
\end{example}
\fi

\ifx\texFuture\Defined
\begin{example}
Рассмотрим линейное преобразование координат
\ShowEq{D affine space, example, 2, 1}
Тогда
\ShowEq{D affine space, example, 1, 2}
Из равенств
\EqRef{D affine space, example, 1, 2, x1},
\EqRef{D affine space, example, 1, 2, x2}
следует обратное преобразование
\ShowEq{D affine space, example, 1, 3}
Из равенств \EqRef{D affine space, example, 1, 1}
следует закон преобразования $1$\Hyph$D$\Hyph форм
\ShowEq{D affine space, example, 1, 4}
Из равенств
\EqRef{map and coordinates, 6, D affine space},
\EqRef{D affine space, example, 1, 3}
следует закон преобразования координат вектора
\ShowEq{D affine space, example, 1, 5}
\qed
\end{example}
\fi

\section{Параллельный перенос}

Пусть в точке $M_0$ вектор $v$ имеет координаты $\aU{v_0}i$.
Пусть вектор $\overset{\longrightarrow}{M_0M_1}$
является вектором бесконечно малого смещения.
Пусть $N_0=M_0+v$, $N_1=M_1+v$.
Согласно аксиоме \ref{axiom: 3, drc affine space}
координаты векторов $\overset{\longrightarrow}{M_0N_0}$
и $\overset{\longrightarrow}{M_1N_1}$
равны.
Как это построение будет выглядеть в криволинейных координатах?

Мы полагаем функции $\aU fi(x)$
непрерывно дифференцируемыми.
Следовательно, векторы локального репера $\aD xi$ и
координаты вектора $\aU vi$ являются
непрерывно дифференцируемыми функциями.
В точке $M(x)$
справедливо равенство
\ShowEq{Paralel Transfer, affine space, 2}

Рассмотрим кривую
\ShowEq{x=xi(t)}
Тогда равенство
\EqRef{Paralel Transfer, affine space, 2}
gets form
\ShowEq{Paralel Transfer, affine space, 2t}
Так как $v=\const$, то равенство
\ShowEq{Paralel Transfer, affine space, 2 dt}
является следствием равенства
\EqRef{Paralel Transfer, affine space, 2t}.
Согласно определению производной
\ShowEq{dxi=d/d}
Так как
\DrawEq{dxi=d/d 1}{}
линейные отображения,
то это выражение имеет разложение
\ShowEq{def connection coefficients, D affine space, 2}
\ShowEq{connection coefficients, D affine space, 2}
где $\ShowSymbol{connection coefficients, D affine space}{}$ -
линейные отображения, называемые
\AddIndex{коэффициентами связности в $D$\Hyph аффинном пространстве}
{connection coefficients, affine space}.
Из равенств
\EqRef{Paralel Transfer, affine space, 2 dt},
\EqRef{connection coefficients, D affine space, 2},
следует
\ShowEq{connection coefficients, D affine space, 4}
Так как $\aD xk(x)$ - локальный базис,
то из равенства \EqRef{connection coefficients, D affine space, 4}
следует
\ShowEq{parallel transfer, affine space, 1}
%Так как $a$ - произвольный вектор,
%то равенство
%\EqRef{parallel transfer, affine space, 1}
%можно записать в виде
\ShowEq{parallel transfer, affine space, 2}

\ifx\texFuture\Defined
\begin{theorem}
\labelTheorem{symmetry of connection coefficients, D affine space}
В аффинном пространстве
\ShowEq{symmetry of connection coefficients, D affine space}
\end{theorem}
\begin{proof}
Согласно равенству
\EqRef{map and coordinates, 3, D affine space}
\ShowEq{Paralel Transfer, affine space, 5}
Согласно теореме
\xRef[0812.4763]
{theorem: Gateaux partial derivative of Second Order, D vector space}
\ShowEq{connection coefficients, D affine space, 3}
Равенство \EqRef{symmetry of connection coefficients, D affine space}
следует
из равенств
\EqRef{connection coefficients, D affine space, 2},
\EqRef{connection coefficients, D affine space, 3}.
\end{proof}

Пусть
\ShowEq{map and coordinates, 1, D affine space}
преобразование координат аффинного пространства.
Продифференцируем равенство
\EqRef{map and coordinates, 5, D affine space}
по $x'^j$
\ShowEq{connection coefficients, D affine space, 5}
Из равенств
\EqRef{connection coefficients, D affine space, 2},
\EqRef{connection coefficients, D affine space, 5}
следует
\ShowEq{connection coefficients, D affine space, 6}
Из равенств
\EqRef{map and coordinates, 5, D affine space},
\EqRef{connection coefficients, D affine space, 6}
следует
\ShowEq{connection coefficients, D affine space, 7}
Из равенства
\EqRef{connection coefficients, D affine space, 7}
следует
\ShowEq{connection coefficients, D affine space, 8}
\fi


==> Affine.Manifold.Russian.tex <==
%auto-ignore
\input{Affine.Manifold.Eq}
\chapter{Многообразие аффинной связности}
\labelChapter{D Affine Manifold}

Основная задача этой главы - дать общее представление
о тех задачах, которые необходимо будет решать в
процессе изучения дифференциальной геометрии.

\section{Дифференцируемое многообразие над алгеброй}

\ShowText{Manifold over Algebra}

\section{Многообразие аффинной связности}
\labelSection{Manifolds with D-Affine Connections}

\begin{definition}
\labelDefinition{D Affine Manifold}
Расслоенное центральное $D$\Hyph аффинное пространство
называется \AddIndex{многообразием $D$\Hyph аффинной связности}
{manifold with D- affine connections}.
\qed
\end{definition}

Мы полагаем, что размерность базы равна размерности слоя.
Это позволяет отождествить слой с касательным пространством к базе.
Рассмотрим область $U$ многообразия,
в которой определён гомеоморфизм
\ShowEq{homeomorphism affine manifold to Dn}
Так же как и в случае аффинного пространства
мы в каждом слое
определим локальный базис
\ShowEq{local basis, affine manifold}

Мы полагаем, что отображение между слоями является морфизмом
центрального $D$\Hyph аффинного пространства.
Бесконечно малое смещение
\ShowEq{x->x+dx}
на базе порождает пассивное преобразование в слое с матрицей
\ShowEq{-Gamma o dx}
где множество отображений
\ShowEq{connection}
называется
\AddIndex{связностью}{connection}.
Поскольку пассивное преобразование бесконечно мало,
координаты вектора изменяются согласно равенству
\ShowEq{change of coordinates of vector}
\ShowEq{change of coordinates of vector 1}
Равенства
\EqRef{change of coordinates of vector}
\EqRef{change of coordinates of vector 1}
называются параллельным переносом.
Если слой является правым $A$\Hyph модулем,
то параллельный перенос имеет вид
\ShowEq{change of coordinates of vector r}
\ShowEq{change of coordinates of vector 1 r}

\ifx\texFuture\Defined
Ковариантная производная
векторного поля $v$ имеет вид
\ShowEq{covariant derivative, D affine manifold}
Векторное поле $v$ параллельно переносится в
данном направлении, если
\ShowEq{covariant derivative, 1, D affine manifold}
Если $x=x(t)$ - отображение поля действительных
чисел в рассматриваемое пространство, то это отображение определяет
геодезическую, если касательный вектор параллельно переносится
вдоль геодезической
\ShowEq{covariant derivative, 2, D affine manifold}
Уравнение \EqRef{covariant derivative, 2, D affine manifold}
эквивалентно уравнению
\ShowEq{covariant derivative, 3, D affine manifold}
\fi


==> Affine.Space.Russian.tex <==
%auto-ignore
\input{Affine.Space.Eq}
\chapter{\texorpdfstring{$D$}{D}-аффинное пространство}
\labelChapter{Affine Space}

\section{\texorpdfstring{$D$}{D}-аффинное пространство}
\labelSection{D-Affine Space}

\begin{\DefinitionStyle}
\labelDefinition{drc affine space, 1}
Рассмотрим множество точек $\Vcirc$
и множество свободных векторов $\Vector V$.\,\footnotemark
Множество $\Vcirc$ удовлетворяет
следующим аксиомам
\StartLabelItem
\begin{enumerate}
\item
\label{axiom: 1, drc affine space}
Существует по крайней мере одна точка
\item
\label{axiom: 2, drc affine space}
Каждой паре точек $(A, B)$ поставлен в соответствие один и
только один вектор. Этот вектор мы будем обозначать $\Vect AB$.
Вектор $\Vect AB$ имеет начало в точке $A$ и конец в точке B.
\item
\label{axiom: 3, drc affine space}
Для каждой точки $A$ и любого вектора $\Vector a$ существует одна
и только одна точка $B$ такая, что
\ShowEq{axiom: 3, drc affine space, 1}.
Мы будем также пользоваться записью\,\footnotemark
\DrawEq{axiom: 3, drc affine space}1
\item
\label{axiom: 4, drc affine space}
(Аксиома параллелограмма.) Если
\ShowEq{axiom: 4, drc affine space, 11}
то
\ShowEq{axiom: 4, drc affine space, 12}
\end{enumerate}
\end{\DefinitionStyle}

\ShowPrevFootnote{\,
Я написал определения и теоремы
в этом разделе согласно определению аффинного пространства в
\citeBib{Rashevsky}, с. 86 - 93.
}

\ShowNextFootnote{\,
\citeBib{Bamberg Sternberg},
с. 9.
}

\begin{\DefinitionStyle}
\labelDefinition{drc affine space, 2}
Пусть даны векторы $\Vector a$ и $\Vector b$. 
Пусть $A\in\Vcirc$ - произвольная точка.
Пусть $B\in\Vcirc$,
$B=A+\Vector a$.
Пусть $C\in\Vcirc$,
$C=B+\Vector b$.
Вектор $\Vect AC$ называется суммой векторов
$\Vector a$ и $\Vector b$
\ShowEq{sum of vectors, affine space}
\end{\DefinitionStyle}

\begin{\TheoremStyle}
\labelTheorem{vectors of affine space, zero vector}
Вектор $\Vect AA$
является нулём по отношению к операции сложения
и не зависит от выбора точки $A$.
Вектор $\Vect AA$ называется нуль\Hyph вектором
и мы полагаем $\Vect AA=\Vector 0$.
\end{\TheoremStyle}
\begin{proof}
Мы можем записать правило сложения
\EqRef{sum of vectors, affine space} в виде
\ShowEq{sum of vectors, affine space, 1}
Если $B=C$, то из равенства
\EqRef{sum of vectors, affine space, 1} следует
\ShowEq{sum of vectors, affine space, 2}
Если $C=A$, $B=D$, то
из аксиомы
\ref{axiom: 4, drc affine space}
следует
\ShowEq{sum of vectors, affine space, 3}
Утверждение теоремы следует из равенств \EqRef{sum of vectors, affine space, 2}
и \EqRef{sum of vectors, affine space, 3}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{vectors of affine space, opposite vector}
Пусть
\ShowEq{a = AB}.
Тогда
\ShowEq{vectors of affine space, opposite vector}
и это равенство
не зависит от выбора точки $A$.
\end{\TheoremStyle}
\begin{proof}
Из равенства
\EqRef{sum of vectors, affine space, 1} следует
\ShowEq{sum of vectors, affine space, 4}
Равенство \EqRef{vectors of affine space, opposite vector}
следует из равенства \EqRef{sum of vectors, affine space, 4}.
Применяя аксиому
\ref{axiom: 4, drc affine space}
к равенству
\ShowEq{sum of vectors, affine space, 9}
получим
\ShowEq{sum of vectors, affine space, 10}
или, что то же,
\ShowEq{sum of vectors, affine space, 11}
В силу аксиомы
\ref{axiom: 4, drc affine space}
снова
следует
\ShowEq{sum of vectors, affine space, 12}.
Следовательно, равенство \EqRef{vectors of affine space, opposite vector}
не зависит от выбора точки $A$.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{vectors of affine space, independence of sum on point}
Сумма векторов $\Vector a$ и $\Vector b$ не зависит от выбора точки $A$.
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{sum of vectors, affine space, 14}
Пусть
\ShowEq{sum of vectors, affine space, 15}
Пусть
\ShowEq{sum of vectors, affine space, 16}
Согласно аксиоме
\ref{axiom: 4, drc affine space}
\ShowEq{sum of vectors, affine space, 5}
Применяя аксиому
\ref{axiom: 4, drc affine space}
к крайним членам равенства \EqRef{sum of vectors, affine space, 5},
получаем
\ShowEq{sum of vectors, affine space, 6}
Из равенства \EqRef{sum of vectors, affine space, 6}
следует утверждение теоремы.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{vectors of affine space, sum associative}
Сложение векторов ассоциативно.
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{a = AB},
\ShowEq{b = BC},
\ShowEq{c = CD}.
Из равенства
\ShowEq{vectors of affine space, sum associative, 3}
следует
\ShowEq{vectors of affine space, sum associative, 1}
Из равенства
\ShowEq{vectors of affine space, sum associative, 4}
следует
\ShowEq{vectors of affine space, sum associative, 2}
Из сравнения равенств
\EqRef{vectors of affine space, sum associative, 1} и
\EqRef{vectors of affine space, sum associative, 2}
следует ассоциативность сложения.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{vectors of affine space, Abelian group}
На множестве $\Vector V$ определена структура абелевой группы.
\end{\TheoremStyle}
\begin{proof}
Из теорем \RefTheorem{vectors of affine space, zero vector},
\RefTheorem{vectors of affine space, opposite vector},
\RefTheorem{vectors of affine space, independence of sum on point},
\RefTheorem{vectors of affine space, sum associative}
следует, что операция сложение векторов определяет группу.

Пусть
\ShowEq{a = AB},
\ShowEq{b = BC}.
\ShowEq{sum of vectors, affine space, 7}
Согласно аксиоме
\ref{axiom: 3, drc affine space}
существует точка $D$ такая, что
\ShowEq{sum of vectors, affine space, 17}
Согласно аксиоме
\ref{axiom: 4, drc affine space}
\ShowEq{sum of vectors, affine space, 18}
Согласно определению суммы векторов
\ShowEq{sum of vectors, affine space, 8}
Из сравнения равенств
\EqRef{sum of vectors, affine space, 7} и
\EqRef{sum of vectors, affine space, 8}
следует коммутативность сложения.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{vectors of affine space, Abelian group representation}
Отображение
\ShowEq{drc affine space, map to A circle}
определённое равенством
\FrameEqRef{axiom: 3, drc affine space}1
является однотранзитивным представлением абелевой группы $\Vector V$.
\end{\TheoremStyle}
\begin{proof}
Аксиома
\ref{axiom: 3, drc affine space}
определяет отображение
\EqRef{drc affine space, map to A circle}.
Из теоремы
\RefTheorem{vectors of affine space, independence of sum on point}
следует, что отображение \EqRef{drc affine space, map to A circle}
является представлением.
Эффективность представления следует
из теоремы \RefTheorem{vectors of affine space, zero vector}
и аксиомы
\ref{axiom: 2, drc affine space}.
Из аксиомы
\ref{axiom: 2, drc affine space},
следует также, что представление транзитивно.
Эффективное и однотранзитивное представление однотранзитивно.
\end{proof}

\section{Аффинная структура на множестве}

\begin{\DefinitionStyle}
\labelDefinition{affine structure on set}
Ковариантное однотранзитивное правостороннее представление абелевой группы $G$
в множестве $M$ называется
\AddIndex{аффинной структурой на множестве}{affine structure on set} $M$.
Элементы множества $M$ называются точками.
Образ точки $A\in M$ при преобразовании, порождённом $a\in G$,
мы обозначим $A+a$.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
\labelTheorem{affine structure on set}
Аффинная структура на множестве $M$
удовлетворяет аксиомам определения
\RefDefinition{drc affine space, 1}.
\end{\TheoremStyle}
\begin{proof}
Мы полагаем, что множество $M$ не пусто, поэтому аксиома
\eqref{axiom: 1, drc affine space} выполнена.
Поскольку $a\in G$ порождает преобразование множества,
то для любого $A\in M$ однозначно определён $B\in M$ такое, что
$B=A+a$.
Это утверждение доказывает аксиому \eqref{axiom: 3, drc affine space}.
Поскольку представление однотранзитивно, то для любых
$A$, $B\in M$ существует единственное $a\in G$ такое, что
$B=A+a$.
Это утверждение позволяет ввести обозначение
\ShowEq{affine structure on set, 1},
а также доказывает аксиому \eqref{axiom: 2, drc affine space}.
Чтобы доказать теорему, нам осталось доказать, что из утверждения теоремы
следует аксиома \eqref{axiom: 4, drc affine space}.

Пусть
\ShowEq{axiom: 4, drc affine space, 21}
Из равенства
\EqRef{axiom: 4, drc affine space, 21}
следует
\ShowEq{axiom: 4, drc affine space, 22}
Пусть
\ShowEq{axiom: 4, drc affine space, 23}
Из равенств
\EqRef{axiom: 4, drc affine space, 23 1},
\EqRef{axiom: 4, drc affine space, 22 2}
следует, что
\ShowEq{axiom: 4, drc affine space, 24}
Из равенств
\EqRef{axiom: 4, drc affine space, 22 1},
\EqRef{axiom: 4, drc affine space, 23 2}
следует, что
\ShowEq{axiom: 4, drc affine space, 25}
Поскольку группа $G$ коммутативна, то из равенства
\EqRef{axiom: 4, drc affine space, 24}
следует
\ShowEq{axiom: 4, drc affine space, 26}
Из равенств
\EqRef{axiom: 4, drc affine space, 25},
\EqRef{axiom: 4, drc affine space, 26}
следует, что
\ShowEq{axiom: 4, drc affine space, 27}
Поскольку представление группы $G$ однотранзитивно,
то из равенства
\EqRef{axiom: 4, drc affine space, 27}
следует
\ShowEq{axiom: 4, drc affine space, 28}
Из равенств
\EqRef{axiom: 4, drc affine space, 22 1},
\EqRef{axiom: 4, drc affine space, 22 2},
\EqRef{axiom: 4, drc affine space, 28}
следует, что
\ShowEq{axiom: 4, drc affine space, 29}
Следовательно, мы доказали аксиому
\eqref{axiom: 4, drc affine space}.
\end{proof}

Несмотря на то, что теорема
\RefTheorem{affine structure on set}
утверждает, что аффинная структура на множестве $M$ удовлетворяет
аксиомам определения \RefDefinition{drc affine space, 1},
определение \RefDefinition{affine structure on set}
не эквивалентно определению \RefDefinition{drc affine space, 1}.
В определении \RefDefinition{drc affine space, 1}
предполагается, что на множестве $G$ определена структура векторного пространства.
Поэтому, если мы хотим изучать аффинное пространство,
мы должны рассмотреть диаграмму представлений: представление поля $F$
в абелевой группе $G$ и представление абелевой группы $G$ в множестве $M$.
Очевидно, что мы можем рассмотреть алгебру с делением $D$ вместо поля $F$.
Таким образом, мы приходим к следующему определению аффинного пространства.

\begin{\DefinitionStyle}
\labelDefinition{Dstar affine space}
Пусть $D$ - тело характеристики $0$,  $\Vector V$ - абелева группа
и $\Vcirc$ - множество.
\AddIndex{Левое $D$\Hyph аффинное пространство}{affine space}
- это диаграмма представлений
\ShowEq{drc affine space, tower of representations}
где $f_{1,2}$ - эффективное левостороннее представление тела $D$ в абелевой группе $\Vector V$
и $f_{2,3}$ - однотранзитивное правостороннее представление абелевой группы $\Vector V$
в множестве $\Vcirc$.
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
Пусть $D$ - тело характеристики $0$,  $\Vector V$ - абелева группа
и $\Vcirc$ - множество.
\AddIndex{Правое $D$\Hyph аффинное пространство}{affine space}
- это диаграмма представлений
\ShowEq{rcd affine space, tower of representations}
где $f_{1,2}$ - эффективное правостороннее представление тела $D$ в абелевой группе $\Vector V$
и $f_{2,3}$ - однотранзитивное правостороннее представление абелевой группы $\Vector V$
в множестве $\Vcirc$.
\end{\DefinitionStyle}

\section{Однотранзитивное представление}

Рассмотрим однотранзитивное представление $f$ $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$.
Мы можем отождествить $a\in A$ с соответствующим преобразованием $f(a)$.
В этой разделе мы будем обозначать действие $a\in A$ на $m\in M$
посредством выражения
\[m+a\]

\begin{\TheoremStyle}
\labelTheorem{single transitive representation A M}
Если представление $f$ $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$
однотранзитивно,
то базисом представления $f$ является произвольная точка $v_0\in M$.
Мощность множества $M$ равна мощности множества $A$.
\end{\TheoremStyle}
\begin{proof}
Выберем произвольный \(v_0\in M\).
Для любого $v\in M$ существует единственный
\ShowEq{single transitive representation A M 1}
такой, что
\ShowEq{single transitive representation A M 2}
Выражение
\EqRef{single transitive representation A M 2}
является $\Omega_2$\Hyph словом.
Следовательно, $v_0$ является базисом представления $f$.
Равенство
\EqRef{single transitive representation A M 2}
устанавливает взаимно однозначное соответствие между множествами
$A$ и $M$. Следовательно,
мощности множеств $A$ и $M$ равны.
\end{proof}

Для отображения $g$
мы будем пользоваться обозначением
\ShowEq{single transitive representation A M 3}
и запишем равенство
\EqRef{single transitive representation A M 2}
в следующем виде
\ShowEq{single transitive representation A M 4}

\begin{\TheoremStyle}
\labelTheorem{single transitive representation Omega1}
Пусть представление $f$ $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$
однотранзитивно.
Если мы выбрали базис $v_0$ представления $f$,
то соответствие
\ShowEq{single transitive representation A M 5}
позволяет нам перенести структуру $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебру $M$.\,\footnotemark
\end{\TheoremStyle}

\footnotetext{\,
Важно иметь в виду,
что структура $\Omega_1$\Hyph алгебры на множестве $M$
зависит от выбора точки $v_0$.
Это замечание также справедливо для всех последующих теорем,
которые мы рассмотрим ниже в этом разделе.
Чтобы подчеркнуть, что рассматриваемая $\Omega_1$ алгебра зависит
от выбора точки $O$, мы будем пользоваться обозначением
\ShowEq{Omega algebra induced by representation}.
}

\begin{proof}
Рассмотрим операцию $\omega\in\Omega_1(n)$.
Для произвольных
\ShowEq{single transitive representation A M 6}
мы положим
\ShowEq{single transitive representation A M 7}
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{single transitive endomorphism}
Пусть представление $f$ $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$
однотранзитивно.
Если мы выбрали базис $v_0$ представления $f$,
то произвольному эндоморфизму $f$ $\Omega_1$\Hyph алгебры $A$
соответствует эндомофизм
\ShowEq{single transitive endomorphism A M}
$\Omega_1$\Hyph алгебры $(M,v_0)$.
\end{\TheoremStyle}
\begin{proof}
Из определения отображения $f'$
\EqRef{single transitive endomorphism A M}
и равенства
\EqRef{single transitive representation A M 4}
непосредственно следует
\ShowEq{single transitive endomorphism A M 0}
Из равенства
\EqRef{single transitive endomorphism A M 02}
следует
\ShowEq{single transitive endomorphism A M 03}

Пусть $\omega\in\Omega_1(n)$.
Из равенства
\EqRef{single transitive representation A M 7}
следует
\ShowEq{single transitive endomorphism A M 1}
Из равенств
\EqRef{single transitive endomorphism A M 1},
\EqRef{single transitive endomorphism A M 01}
следует
\ShowEq{single transitive endomorphism A M 2}
Так как отображение $f$ является эндоморфизмом,
то из равенства
\EqRef{single transitive endomorphism A M 2}
следует
\ShowEq{single transitive endomorphism A M 3}
Из равенств
\EqRef{single transitive endomorphism A M 3},
\EqRef{single transitive endomorphism A M 03}
следует
\ShowEq{single transitive endomorphism A M 4}
Из равенств
\EqRef{single transitive endomorphism A M 4},
\EqRef{single transitive representation A M 7}
следует
\ShowEq{single transitive endomorphism A M 5}
Из равенства
\EqRef{single transitive endomorphism A M 5}
следует, что отображение $f'$ является эндоморфизмом
$\Omega_1$\Hyph алгебры $(M,v_0)$.
\end{proof}

\begin{\TheoremStyle}
Пусть представление $f$ $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $M$
однотранзитивно.
Если мы выбрали базис $v_0$ представления $f$,
то соответствие
\ShowEq{single transitive representation A M 5}
позволяет нам перенести структуру $\Omega_2$\Hyph алгебры
в $\Omega_1$\Hyph алгебру $A$.
\end{\TheoremStyle}
\begin{proof}
Рассмотрим операцию $\omega\in\Omega_2(n)$.
Для произвольных
\ShowEq{single transitive representation A M 8}
существуют
\ShowEq{single transitive representation A M 6}
такие, что
\ShowEq{single transitive representation A M 9}
Мы положим
\ShowEq{single transitive representation A M 10}
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{extend single transitive representation}
Рассмотрим диаграмму $(\Vector V,\Vector f)$ представлений
$\Vector{\Omega}$\Hyph алгебр.
Пусть представление $f_{i+1,i+2}$
однотранзитивно,
и $a_{i+2\cdot 0}$ - базис представления $f_{i+1,i+2}$.
Тогда представлению
$f_{i,i+1}$
$\Omega_i$\hyph алгебры $A_i$
в $\Omega_{i+1}$\hyph алгебре $A_{i+1}$ соответствует представление
\ShowEq{extend single transitive representation}
$\Omega_i$\hyph алгебры $A_i$
в $\Omega_{i+2}$\hyph алгебре $A_{i+2}$.
\end{\TheoremStyle}
\begin{proof}
Поскольку отображение $f_{i,i+1}(a_i)$ является эндоморфизмом
$\Omega_{i+1}$\Hyph алгебры $A_{i+1}$, то, согласно теореме
\RefTheorem{single transitive endomorphism},
отображение $f'_{i,i+2}(a_i)$ является эндоморфизмом
$\Omega_{i+1}$\Hyph алгебры $(A_{i+2},a_{i+2\cdot 0})$.
\end{proof}

Из равенства
\EqRef{extend single transitive representation}
следует
\ShowEq{extend single transitive representation 11}
\ShowEq{extend single transitive representation 12}
Из равенства
\EqRef{extend single transitive representation 12}
следует
\ShowEq{extend single transitive representation 2}

\begin{\TheoremStyle}
\labelTheorem{extend single transitive endomorphism}
Рассмотрим диаграмму $(\Vector V,\Vector f)$ представлений
$\Vector{\Omega}$\Hyph алгебр.
Пусть представление $f_{i+1,i+2}$
однотранзитивно,
и $a_{i+2\cdot 0}$ - базис представления $f_{i+1,i+2}$.
Эндоморфизм $r_{i+1}$ представления $f_{i,i+1}$
порождает эндоморфизм $r'_{i+2}$ представления $f'_{i,i+2}$
\ShowEq{extend single transitive endomorphism}
\end{\TheoremStyle}
\begin{remark}
Из равенства
\EqRef{extend single transitive endomorphism}
следует
\ShowEq{extend single transitive endomorphism 0}
\end{remark}
\begin{proof}
Поскольку отображение $r_{i+1}$ является эндоморфизмом
$\Omega_{i+1}$\Hyph алгебры $A_{i+1}$, то, согласно теореме
\RefTheorem{single transitive endomorphism},
отображение $r'_{i+2}$ является эндоморфизмом
$\Omega_{i+1}$\Hyph алгебры $(A_{i+2},a_{i+2\cdot 0})$.

Для доказательства теоремы достаточно показать, что верно следующее равенство
\ShowEq{extend single transitive endomorphism 1}
Равенство
\EqRef{extend single transitive endomorphism 1}
можно записать в виде
\ShowEq{extend single transitive endomorphism 2}
Из равенств
\EqRef{extend single transitive endomorphism 2},
\EqRef{extend single transitive representation},
\EqRef{extend single transitive endomorphism}
следует
\ShowEq{extend single transitive endomorphism 3}
Из равенств
\EqRef{extend single transitive endomorphism 3},
\EqRef{extend single transitive representation 2},
\EqRef{extend single transitive endomorphism 0}
следует
\ShowEq{extend single transitive endomorphism 4}
Равенство
\EqRef{extend single transitive endomorphism 4}
верно, так как отображение $(r_i,r_{i+1})$
является эндоморфизмом представления $f_{i,i+1}$.
Следовательно, отображение $(r_i,r'_{i+2})$
является эндоморфизмом представления $f'_{i,i+2}$.
\end{proof}

\section{Базис в правом \texorpdfstring{$D$}{D}-аффинном пространстве}
\labelSection{rcd Affine Space}

Рассмотрим правое $D$\Hyph аффинное пространство $\Vrow$.

Абелевая группа $\Vector V$ действует однотранзитивно на множестве $\Vcirc$.
Согласно теореме \RefTheorem{single transitive representation A M},
базис множества $\Vcirc$ относительно представления
абелевой группы $\Vector V$ состоит из одной точки. Эту точку обычно обозначают
буквой $O$ и называют
\AddIndex{началом системы координат правого $D$\Hyph аффинного пространства}
{origin of coordinate system of affine space}.
Следовательно, произвольную точку $A\in\Vcirc$
можно представить с помощью вектора
\ShowEq{affine space coordinates 1}
\ShowEq{affine space coordinates 2}
Согласно теореме \RefTheorem{single transitive representation A M},
мощности множеств $\Vcirc$ и $\Vector V$ равны.

Тип аффинного пространства определяется типом векторного пространства
в диаграмме представлений (раздел
\xRef[0701.238]{section: vector space type}).

Пусть $\Vector V$ - правое $D$\Hyph векторное пространство столбцов.
Правое $D$\Hyph аффинное пространство $\Vrow$
называется
\AddIndex{правым $D$\Hyph аффинным пространством столбцов}{affine space of columns}.
Пусть $\Basis e$ - базис \rcd векторного пространства $\Vector V$.
Тогда разложение вектора $\overset{\longrightarrow}{OA}$
относительно \rcd базиса $\Basis e$ имеет вид
\ShowEq{affine space coordinates 3}

Из равенств
\EqRef{affine space coordinates 2},
\EqRef{affine space coordinates 3}
следует
\ShowEq{affine space coordinates 5}

\begin{\DefinitionStyle}
\labelDefinition{rcd affine basis, division ring}
\AddIndex{Аффинный базис}{Affine Basis}
\ShowEq{Affine Basis}
- это максимальное множество
линейно независимых векторов
\ShowEq{rcd affine basis, vector, division ring}
с общей начальной точкой $O$.
Множество координат
\ShowEq{point A, rcd affine space}
вектора $\Vect OA$
называется
\AddIndex{координатами точки $A$
правого $D$\Hyph аффинного пространства столбцов $\Vrow$
относительно базиса $(\Basis e,O)$}
{coordinates in affine space}.
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
\AddIndex{Многообразие базисов
\ShowEq{Basis Manifold, Affine Space}
правого $D$\Hyph аффинного пространства столбцов}
{Basis Manifold, Affine Space}
- это множество базисов этого пространства.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
\labelTheorem{endomorphism rcd affine space}
Пусть
\ShowEq{rcd affine space, tower of representations}
правое $D$\Hyph аффинное пространство столбцов.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{endomorphism rcd affine space, f23}
Эндоморфизм представления $f_{2,3}$ имеет вид
\ShowEq{parallel shift, rcd affine space}
\item
\labelItem{endomorphism rcd affine space, f12}
Эндоморфизм представления $f_{1,2}$ имеет вид
\ShowEq{linear transformation, rcd affine space}
\end{enumerate}
\end{\TheoremStyle}
\begin{proof}
Пусть $h$ - эндоморфизм представления $f_{2,3}$.
Из определения
\xRef[8443-0072]{definition: morphism of representations of F algebra}
следует, что
\ShowEq{parallel shift 1, rcd affine space}
Пусть
\ShowEq{parallel shift 2, rcd affine space}
Из равенств
\EqRef{parallel shift 1, rcd affine space},
\EqRef{parallel shift 2, rcd affine space}
следует
\ShowEq{parallel shift 3, rcd affine space}
Из равенств
\EqRef{parallel shift 2, rcd affine space},
\EqRef{parallel shift 3, rcd affine space}
следует
\ShowEq{parallel shift 4, rcd affine space}
Из аксиомы
\ref{axiom: 4, drc affine space}
и равенства
\EqRef{parallel shift 4, rcd affine space}
следует
\ShowEq{parallel shift 5, rcd affine space}
Поскольку $\Vector a$ - произвольный вектор, то из равенств
\EqRef{parallel shift 5, rcd affine space},
\EqRef{parallel shift 2, rcd affine space}
следует
\ShowEq{parallel shift 6, rcd affine space}
для любой точки
\ShowEq{parallel shift 7, rcd affine space}
Следовательно, любой эндоморфизм представления $f_{2,3}$ имеет вид
\EqRef{parallel shift, rcd affine space}.

Утверждение
\RefItem{endomorphism rcd affine space, f12}
подробно рассмотрено в разделе
\xRef[0701.238]{section: Linear Map of Vector Spaces}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{parallel shift, rcd affine space}
Преобразование
\EqRef{parallel shift, rcd affine space}
называется
\AddIndex{параллельным сдвигом правого $D$\Hyph аффинного пространства столбцов}
{parallel shift, rcd affine space}.
Координаты параллельного сдвига
\EqRef{parallel shift, rcd affine space}
правого $D$\Hyph аффинного пространства столбцов имеют вид
\ShowEq{parallel shift, coordinates, rcd affine space}
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{point A, rcd affine space}
- координаты точки $A$ относительно базиса $(\Basis e,O)$.
Из равенства
\EqRef{affine space coordinates 5}
следует
\ShowEq{point A 1, rcd affine space}
Пусть
\ShowEq{point A', rcd affine space}
- координаты точки $A'$ относительно базиса $(\Basis e,O)$.
Из равенства
\EqRef{affine space coordinates 5}
следует
\ShowEq{point A' 1, rcd affine space}
Пусть
\ShowEq{vector a, rcd affine space}
разложение вектора $\Vector a$ относительно базиса $\Basis e$.
Подставив равенства
\EqRef{point A 1, rcd affine space},
\EqRef{point A' 1, rcd affine space},
\EqRef{vector a, rcd affine space}
into the equation
\EqRef{parallel shift, rcd affine space},
мы получим
\ShowEq{parallel shift, coordinates 1, rcd affine space}
Поскольку представление $f_{2,3}$ однотранзитивно,
то из равенства
\EqRef{parallel shift, coordinates 1, rcd affine space}
следует
\ShowEq{parallel shift, coordinates 2, rcd affine space}
Поскольку векторы $\Vector e_i$ линейно независимы,
то равенство
\EqRef{parallel shift, coordinates, rcd affine space}
следует из равенства
\EqRef{parallel shift, coordinates 2, rcd affine space}.
\end{proof}

\begin{\TheoremStyle}
Пусть $(\Basis e,O)$ - базис
правым $D$\Hyph аффинного пространства столбцов
\ShowEq{rcd affine space, tower of representations}
\StartLabelItem
\begin{enumerate}
\item
\labelItem{rcd affine space, generates sum}
Представление $f_{2,3}$ порождает
операцию сложения на множестве $\Vcirc$
\ShowEq{f23 generates, rcd affine space}
\item
\labelItem{rcd affine space, generates representation}
Представление $f_{1,2}$ порождает представление
\ShowEq{f12 generates, rcd affine space}
\item
\labelItem{rcd affine space, generates endomorphism}
Эндоморфизм $\Vector g$ представления $f_{1,2}$ порождает эндоморфизм
$\Vector g'$ представления $f'_{1,2}$
\ShowEq{g generates, rcd affine space}
\end{enumerate}
\end{\TheoremStyle}
\begin{proof}
Так как представление $f_{2,3}$ однотранзитивно, то
\begin{itemize}
\item
утверждение
\RefItem{rcd affine space, generates sum}
является следствием теоремы
\RefTheorem{single transitive representation Omega1}.
\item
утверждение
\RefItem{rcd affine space, generates representation}
является следствием теоремы
\RefTheorem{extend single transitive representation}.
\item
утверждение
\RefItem{rcd affine space, generates endomorphism}
является следствием теоремы
\RefTheorem{extend single transitive endomorphism}.
\end{itemize}
\end{proof}

\begin{\TheoremStyle}
Преобразование
\EqRef{g generates, rcd affine space}
называется
\AddIndex{линейным преобразованием правого $D$\Hyph аффинного пространства столбцов}
{linear transformation, affine space}.
Координаты линейного преобразования
\EqRef{g generates, rcd affine space}
правого $D$\Hyph аффинного пространства столбцов имеют вид
\ShowEq{linear transformation, coordinates, rcd affine space}
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{point A, rcd affine space}
- координаты точки $A$ относительно базиса $(\Basis e,O)$.
Из равенства
\EqRef{affine space coordinates 3}
следует
\ShowEq{point A 3, rcd affine space}
Пусть
\ShowEq{point A', rcd affine space}
- координаты точки $A'$ относительно базиса $(\Basis e,O)$.
Из равенства
\EqRef{affine space coordinates 5}
следует
\ShowEq{point A' 2, rcd affine space}
Из равенства
\EqRef{g generates, rcd affine space}
следует
\ShowEq{g generates 1, rcd affine space}
Из равенств
\EqRef{point A 3, rcd affine space},
\EqRef{point A' 2, rcd affine space},
\EqRef{g generates 1, rcd affine space}
следует
\ShowEq{g generates 2, rcd affine space}
Равенство
\EqRef{linear transformation, coordinates, rcd affine space}
следует из равенства
\EqRef{g generates 2, rcd affine space},
так как $(\Vector e,O)$ - базис правого $D$\Hyph аффинного пространства столбцов.
\end{proof}

Последовательное выполнение параллельного сдвига
и линейного преобразования
правого $D$\Hyph аффинного пространства столбцов, порождает
\AddIndex{\rcd аффинное преобразование}{affine transformation}
\ShowEq{rcd affine transformation}
Это преобразование правого $D$\Hyph аффинного пространства столбцов можно представить
как отображение базиса $(\Basis e,O)$ в базис $(\Basis e',O')$.
Отображение базиса $(\Basis e,O)$ в базис $(\Basis e',O')$
можно представить как композицию отображения базиса $(\Basis e,O)$ в
базис $(\Basis e,O')$ и \drc линейного отображения базиса
$(\Basis e,O')$ в базис $(\Basis e',O')$.
Следовательно, \drc преобразование имеет вид
\ShowEq{drc quasi affine transformation of basis, division ring}

Вводя координаты $A^1,...,A^n$ точки $A\in\mathcal{A}_n$
как координаты вектора $\Vect OA$ относительно базиса $\Basis e$,
мы можем записать
линейное преобразование как
\ShowEq{Drc Affine Transformation}
%Производная этого преобразования определена матрицей $\|P^i_j\|$
%и не зависит от точки $A$.
Вектор
$(\aU R1,...,\aU Rn)$ выражает смещение в аффинном пространстве.

\begin{\TheoremStyle}
\labelTheorem{Drc Affine Transformation}
Множество преобразований
\EqRef{Drc Affine Transformation}
- это группа Ли, которую мы обозначим
\symb{GL(\mathcal{A}_n)}{affine transformation group}1
и будем называть
\AddIndex{группой аффинных преобразований}{affine transformation group}.
\end{\TheoremStyle}
\begin{proof}
Рассмотрим преобразования $(P,R)$ и $(Q,S)$.
Последовательное выполнение этих преобразований имеет вид
\ShowEq{Drc Affine Transformation, product (P,R) (Q,S)}
Следовательно, мы можем записать произведение преобразований
$(P,R)$ и $(Q,S)$ в виде
\ShowEq{Drc Affine Transformation, product (P,R) (Q,S), definition}
\end{proof}

Мы будем называть активное преобразование
\AddIndex{аффинным преобразованием}{affine drc transformation}.% no index
Мы будем называть пассивное преобразование
\AddIndex{квазиаффинным преобразованием}{quasi affine drc transformation}.

Если мы не заботимся о начальной точке вектора, мы получим несколько отличный
тип пространства, которое мы будем называть центро-аффинным пространством
\symb{CA_n}{central affine space}1.
%В центро-аффинном пространстве мы можем идентифицировать все
%касательные пространства и обозначить их $T\mathcal{CA}_n$.
Если мы предположим, что начальная точка
вектора - это начало $O$ координатной системы в пространстве,
то мы можем отождествить любую
точку $A\in CA_n$ с вектором $a=\Vect OA$.
%Это ведёт
%к идентификации $\mathcal{CA}_n$ и $T\mathcal{CA}_n$.
Теперь преобразование - это просто отображение
\ShowEq{affine transformation a map}
и такие преобразования порождают группу Ли $GL_n$.

\begin{\DefinitionStyle}
\AddIndex{Центро-аффинный базис}{Central Affine Basis}
\ShowEq{Central Affine Basis}
- это множество
линейно независимых векторов $\aD ei$.
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
\AddIndex{Многообразие базисов
\ShowEq{Basis Manifold, Central Affine Space}
центро\hyph аффинного пространства}{Basis Manifold, Central Affine Space}
- это множество базисов этого пространства.
\end{\DefinitionStyle}

\section{Плоскость в \texorpdfstring{$D$}{D}-аффинном пространстве}

Рассмотрим правое $D$\Hyph аффинное пространство столбцов
\ShowEq{rcd affine space, tower of representations}
Пусть $\Vector V_1\subset\Vector V$ - векторное подпространство
векторного пространства $\Vector V$.
Следовательно, $\Vector V_1$
является подгруппой абелевой группы $\Vector V$.
В диаграмме подпредставлений
\ShowEq{rcd affine space 1, tower of representations}
представление $f_{2,3}$ не является однотранзитивным.
Согласно теореме
\ShowEq{proper definition of orbit}
множество $\Vcirc$ может быть представленно
как пересечение не пересекающихся орбит представления $f_{2,3}$.
Однако, так как представление $f_{2,3}$ эффективно,
то представление $f_{2,3}$
однотранзитивно на орбите представления.
Следовательно,
если мы выберем произвольную точку $A\in\Vcirc$ и орбиту представления
\ShowEq{rcd affine space 2, tower of representations}
то мы получим диаграмму представлений
\ShowEq{rcd affine space 3, tower of representations}
описывающую правОЕ $D$\Hyph аффиннОЕ пространство столбцов, называемое
\AddIndex{аффинной плоскостью}{affine plane}, проходящей через точку $A$.

Пусть
\ShowEq{rcd affine space, basis}
базис правого векторного пространства $\Vector V$.
Пусть базис правого векторного пространства $\Vector V_1$
\ShowEq{rcd affine plane, basis}
имеет следующее разложение относительно базиса $\Basis e$
\ShowEq{rcd affine plane, basis, 1}
Пусть $\Vector v\in\Vector V_1$
имеет следующее разложение относительно базиса $\Basis e$
\ShowEq{rcd affine plane, basis, 2}
Согласно теореме
\xRef[0701.238]{theorem: rc rank of matrix, sups-rows}
\ShowEq{rcd affine plane, basis, 3}
Если мы предположим, что первые $k$ строк составляют
невырожденную матрицу, то мы получим $n-k$ \rcd линейных уравнений
\ShowEq{rcd affine plane, basis, 4}
которым удовлетворяют координаты вектора $\Vector v$.

Пусть точка $A$ имеет представление
\ShowEq{rcd affine plane, A}
относительно базиса $(\Basis e,O)$.
Пусть
\ShowEq{rcd affine plane, B}
произвольная точка аффинной плоскости $\Vrow_1$.
Тогда
\ShowEq{rcd affine plane, v}
Из равенства
\ShowEq{rcd affine plane, B=A+v}
и равенств
\EqRef{rcd affine plane, A},
\EqRef{rcd affine plane, B},
\EqRef{rcd affine plane, v}
следует
\ShowEq{rcd affine plane, B=A+v 1}
Из равенств
\EqRef{rcd affine plane, basis, 4},
\EqRef{rcd affine plane, B=A+v 1}
следует, что координаты точки $B$ удовлетворяют
системе линейных уравнений
\ShowEq{rcd affine plane, basis, 5}

Пусть задано семейство векторов
\ShowEq{n-1 vectors affine space}
Мы говорим, что вектор $\overline a=\overset{\longrightarrow}{A_0A}$
лежит в плоскости, натянутой на векторы
\ShowEq{n-1 vectors affine space, 1},
если вектор
\ShowEq{vector an affine space}
является линейной комбинацией векторов
\ShowEq{n-1 vectors affine space, 1}.


==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

%22. A.G. Kurosh, Lectures on General Algebra, Chelsea, New York, 1963

\BiblioItem{Doctor Ouch}
{
Корней Чуковский. Айболит.
\\
Детский мир, ISBN 978-5-91315-875-8, 2012
}%

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462.
%
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
%
%
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 94, М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Richardson 1928}
{
A. R. Richardson. Simultaneous Linear Equations over a Division Algebra.
Proceedings of the London Mathematical Society.
Volume s2-28, Issue 1, 1928, Pages 395-420.
}%

\BiblioItem{Jacobson. Lie algebras}
{
Джекобсон. Алгебры Ли.
Перевод с английского А. Б. Жижченко
под редакцией А. И. Кострикина.
М., Мир, 1964
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3).
Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{https://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{2110.04354}
{
Dimitri Gurevich, Varvara Petrova, Pavel Saponov,
q-Casimir and q-cut-and-join operators related to Reflection Equation Algebras,
eprint \href{https://arxiv.org/abs/2110.04354}{arXiv:gr-qc/2110.04354} (2021)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{Lang Manifold}
{
Serge Lang,
Differential Manifold, Springer, 1985
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem{8176-4374}
{
Mariano Giaquinta, Giuseppe Modica,
Mathematical Analysis: Linear and Metric Structures and Continuity.
\\
Springer, 2007, ISBN-13: 978-0-8176-4374-4
}%

\BiblioItem{319-09203}
{
Ralf Schiffler,
Quiver Representations.
\\
Springer, 2014, ISBN-13: 978-3-319-09203-4
}%

\BiblioItem{511-34545}
{
Ibrahim Assem, Daniel Simson, Andrzej Skowro\'nski,\\
Elements of the Representation Theory
of Associative Algebras.
\\
Volume 1: Techniques of Representation Theory.
\\
Cambridge University Press, 2006, ISBN-13: 978-0-511-34545-6
}%

\DefBiblioItem{Rashevsky}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{978-0-8176-8384-9}
{
Garret Sobczyk, New Foundations in Mathematics: The Geometric Concept of Number,
\\
Springer, 2013, ISBN: 978-0-8176-8384-9
}%

\BiblioItem{978-0538497817}
{
James Stewart, Calculus,
\\
Cengage Learning, 2012, ISBN: 978-0-538-49781-7
}%

\BiblioItem{470-38334}
{
William E. Boyce, Richard C. DiPrima,
Elementary Differential Equations and Boundary Value Problems,
\\
John Wiley \& Sons, Inc., 2009, ISBN 978-0-470-38334-6
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\DefBiblioItem{Korn}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{1708.01190}
{
Nathan BeDell,
Doing Algebra over an Associative Algebra,
\\
eprint \href{https://arxiv.org/abs/1708.01190}{arXiv:1708.01190} (2017)
}%

\BiblioItem{Karthika Viji 2021}
{
S. Karthika, M. Viji,
Unit elements in the path algebra of an acyclic quiver,
Indian J Pure Appl Math\\
Published online: 10 June 2021
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\DefBiblioItem{math.QA-0208146}%

\DefBiblioItem{q-alg-9705026}

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{0911.4454}
{
Vladimir Retakh,
From factorizations of noncommutative polynomials to combinatorial topology,\\
eprint \href{http://arxiv.org/abs/0911.4454}{arXiv:0911.4454} (2009)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{McCrimmon: Jordan Algebras}
{
Kevin McCrimmon;
A Taste of Jordan Algebras;\\
Springer, 2004
}%

\BiblioItem{Zharinov: foundation of mathematical physics}
{
В. В. Жаринов, 
Алгебро-геометрические основы математической физики,\\
Лекционные курсы научно-образовательного центра, 9, МИАН,\\
М., 2008
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники). ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer rule over quaternion skew field,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная универсальная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts{T}представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\DefBiblioItem{0812.4763}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1102.1776}
{
Александр Клейн, Иван Кирчей,
Соответствие между строчно\Hyph столбцовыми определителями
и квазидетерминантами матриц над кватернионной алгеброй,\\
eprint \href{http://arxiv.org/abs/1102.1776}{arXiv:1102.1776} (2011)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1111.6035}
{
Александр Клейн,
Базис представления универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/1111.6035}{arXiv:1111.6035} (2011)
}%

\BiblioItem{1201.4158}
{
Александр Клейн, Александер Ложье,
Ортонормированный базис в пространстве Минковского,\\
eprint \href{http://arxiv.org/abs/1201.4158}{arXiv:1201.4158} (2012)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1206.0200}
{
Александр Клейн,
Алгебра частных алгебры с сопряжением,\\
eprint \href{http://arxiv.org/abs/1206.0200}{arXiv:1206.0200} (2012)
}

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\DefBiblioItem{1302.7204}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{1412.5425}
{
Александр Клейн,
Деление в ассоциативной $D$-алгебре,\\
eprint \href{http://arxiv.org/abs/1412.5425}{arXiv:1412.5425} (2014)
}%

\DefBiblioItem{1502.04063}%

\BiblioItem{1505.03625}
{
Александр Клейн,
Производная отображения банаховой алгебры,\\
eprint \href{http://arxiv.org/abs/1505.03625}{arXiv:1505.03625} (2015)
}%

\BiblioItem{1506.00061}
{
Александр Клейн,
Квадратное уравнение над ассоциативной $D$\Hyph алгеброй,\\
eprint \href{http://arxiv.org/abs/1506.00061}{arXiv:1506.00061} (2015)
}%

\DefBiblioItem{1601.03259}%

\DefBiblioItem{1801.01628}

\DefBiblioItem{1908.04418}

\BiblioItem{2020.06.01}
{
Александр Клейн,
Система дифференциальных уравнений над банаховой алгеброй,\\
Geometry of differential equations seminar 2020\\
eprint \href{https://gdeq.org/files/Aleks_Kleyn-2020.06.01.Russian.pdf)}{talk:2020.06.01} (2020)
}%

\BiblioItem{2021.01.06}
{
Александр Клейн,
Математический анализ над алгеброй кватернионов,\\
Joint Mathematics Meetings January 2020\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}%

\BiblioItem{2112.00613}
{
Александр Клейн,
Многочлен в некомутативной алгебре,\\
eprint \href{http://arxiv.org/abs/2112.00613}{arXiv:2112.00613} (2021)
}%

\BiblioItem{322019412}
{
Александр Клейн,
Дневник поиска, 2017\\
eprint \href{https://www.researchgate.net/publication/322019412}{RG:322019412} (2017)
}%

\BiblioItem{323966352}
{
Александр Клейн,
Дневник поиска, 2018\\
eprint \href{https://www.researchgate.net/publication/323966403}{RG:323966403} (2018)
}%

\BiblioItem{348311191}
{
Александр Клейн,
Дневник поиска, 2021\\
eprint \href{https://www.researchgate.net/publication/348311191}{RG:348311191} (2021)
}%

\BiblioItem{323236904}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
eprint \href{https://www.researchgate.net/publication/323238274}{RG:323238274} (2018)
}%

\DefBiblioItem{2207.06506}

\BiblioItem{2307.09982}
{
Александр Клейн,
Введение в некоммутативную алгебру,
Том 2, Модуль над алгеброй\\
eprint \href{http://arxiv.org/abs/2307.09982}{arXiv:2307.09982} (2019)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Александр Клейн.\\
Линейная алгебра над телом: Система линейных уравнений.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-5029-8247-6
}%

\BiblioItem{4975-6381}
{
Александр Клейн.\\
Математический анализ отображений одной переменной: Некоммутативная банахова алгебра.\\
CreateSpace Independent Publishing Platform, 2017;\\
ISBN-13: 978-1-4975-6368-1
}%

\BiblioItem{4993-2400}
{
Александр Клейн.\\
Линейная алгебра над телом: Векторное пространство.\\
CreateSpace Independent Publishing Platform, 2014;\\
ISBN-13: 978-1-4993-2394-8
}%

\BiblioItem{5059-9176}
{
Александр Клейн.\\
Нормированная \(\Omega\)-группа.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5059-9235-9
}%

\BiblioItem{5114-6019}
{
Александр Клейн.\\
Представление универсальной алгебры: Полиморфизм.\\
CreateSpace Independent Publishing Platform, 2015;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5148-4632}
{
Александр Клейн.\\
Некоммутативная алгебра: Введение.\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-5114-6494-9
}%

\BiblioItem{5410-9916}
{
Александр Клейн.\\
Интеграл Лебега в абелевой $\Omega$-группе.\\
CreateSpace Independent Publishing Platform, 2016;\\
ISBN-13: 978-1-5410-9984-5
}%

\BiblioItem{9856-6693}
{
Александр Клейн,
Краткий курс математического анализа над банаховой алгеброй\\
CreateSpace Independent Publishing Platform, 2018;\\
ISBN-13: 978-1-9856-6808-9
}%

\BiblioItem{7287-9339}
{
Aleks Kleyn,
Quadratic Equation over Associative $D$\Hyph Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-7287-9339-9
}%

\BiblioItem{9835-2163}
{
Aleks Kleyn,
Differential Equation over Banach Algebra\\
Kindle Direct Publishing, 2018;\\
ISBN-13: 978-1-9835-2163-8
}%

\BiblioItem{6860-2955}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{0767-8264}
{
Александр Клейн,
Система дифференциальных уравнений над банаховой алгеброй: Экспонента,\\
Kindle Direct Publishing, 2019;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{5284-0163}
{
Александр Клейн,
Введение в дифференциальные уранения, банаховая алгебра,\\
Kindle Direct Publishing, 2021;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{8428-0408}
{
Александр Клейн,
Введение в некоммутативную алгебру, Том 1: Алгебра с делением,\\
Kindle Direct Publishing, 2022;\\
ISBN-13: %978-1511464949
}%

\BiblioItem{CACAA.01.109}
{
Aleks Kleyn,
Mappings of Conjugation of Quaternion Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 1, pages 109 - 121, 2012
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{CACAA.02.097}
{
Aleks Kleyn,
Polynomial over Associative $D$-Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 2, Issue 2, pages 97 - 115, 2013
}%

\BiblioItem{CACAA.04.001}
{
Aleks Kleyn,
Integral of Map into Abelian $\Omega$-group.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 4, Issue 1, pages 1 - 68, 2013
}%

\BiblioItem{CACAA.05.001}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 5, issue 1, pages 1 - 68, 2016 
}%

\BiblioItem{CACAA.06.121}
{
Aleks Kleyn,
Differential Forms in Banach Algebra.\\
Clifford Analysis, Clifford Algebras and their applications,
volume 6, issue 2, pages 121 - 214, 2017 
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{1807.05583}
{
V. Sokolov, T. Wolf,
Non\Hyph commutative generalization of integrable quadratic ODE systems,\\
eprint \href{http://arxiv.org/abs/1807.05583}{arXiv:1807.05583} (2019)
}%

\BiblioItem{1506.05848}
{
Rida T. Farouki, Graziano Gentili, Carlotta Giannelli, Alessandra Sestini,
Caterina Stoppato,\\
Solution of a quadratic quaternion equation with mixed coefficients,\\
eprint \href{http://arxiv.org/abs/1506.05848}{arXiv:1506.05848} (2015)
}%

\BiblioItem{2003.05263}
{
Florian-Horia Vasilescu,
Spectrum and Analytic Functional Calculus in Real and Quaternionic Frameworks,\\
eprint \href{http://arxiv.org/abs/2003.05263}{arXiv:2003.05263} (2003)
}%

\BiblioItem{1702.04935}
{
M. Irene Falc\~{a}o, Fernando Miranda, Ricardo Severino, M. Joana Soares,
Weierstrass method for quaternionic polynomial root-finding,\\
eprint \href{http://arxiv.org/abs/1702.04935}{arXiv:1702.04935} (2017)
}%

\DefBiblioItem{1812.03397}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010).
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008).
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\DefBiblioItem{1510.02224}%

\BiblioItem{1902.09800}
{
Dong Cheng, Kit Ian Kou, Yong Hui Xia.
Floquet Theory for Quaternion-valued Differential Equations.\\
eprint \href{http://arxiv.org/abs/1902.09800}{arXiv:1902.09800} (2019)
}%

\BiblioItem{Zharinov Kursy NOC, 9}
{
V. V. Zharinov,
Algebraic and geometric foundation of mathematical physics.
\\
Lekts. Kursy NOC, 9, Steklov Math. Institute of RAS, Moscow, 2008, 3–209 
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 1}
{
Paul M. Cohn,
Algebra, Volume 1,
John Wiley \& Sons, 1982
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\DefBiblioItem{Cohn: Skew Fields}%

\BiblioItem
{Lam: Noncommutative Rings}
{
T. Y. Lam,
A First Course in
Noncommutative Rings,
Springer-Verlag, 1991
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 1 - 3,
перевод с французского Ю. А. Бахтурина И Г. И. Ольшанского
под редакцией А. А. Кириллова И А. И. Кострикина,
М. Мир, 1976
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{Basic Concepts of Differential Geometry}
{
Алексеевский Д. В., Виноградов А. М., Лычагин В. В.,
Основные понятия дифференциальной геометрии
\\
Итоги ВИНИТИ 28
\\
М. ВИНИТИ, 1988
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\DefBiblioItem{Sudbery Quaternionic Analysis}%

\BiblioItem{Sudbery 2657821}
{
A. Sudbery,
Quaternionic Analysis,\\
eprint \href{https://www.researchgate.net/publication/2657821}{ResearchGate:2657821} (1977)
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{R. Serodio 2001}
{
R. Ser\^odio, E. Pereira, J. Vit\'oria,
Computing the zeros of quaternion polynomials,
Computers \& Mathematics with Applications 42(s 8–9), Pages 1229-1237
}

\BiblioItem{Bulletin AMS 1944 246-248}
{
Samuel Eilenberg, Ivan Niven,
The “fundamental theorem of algebra” for quaternions,
Bulletin of the American Mathematical Society, {\bf 50} (1944), 246-248
}

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Bilinear.Map.Russian.tex <==
%auto-ignore

\input{Bilinear.Map.Eq}

\chapter{Квадратичное отображение тела}

\section{Билинейное отображение тела}

\begin{\TheoremStyle}
\labelTheorem{standard representation of bilinear map, division ring}
Пусть $D$ - тело характеристики $0$.
Пусть $F$ - поле, которое является подкольцом центра
тела $D$.
Допустим \eV
- базис тела $D$ над полем $F$.
\AddIndex{Стандартное представление над полем $F$ билинейного отображения тела}
{bilinear map, standard representation, division ring}
имеет вид
\ShowEq{def standard component of bilinear map}
\ShowEq{bilinear map, division ring, standard representation}
Выражение
$\ShowSymbol{standard component of bilinear map, division ring}{}$
в равенстве \EqRef{bilinear map, division ring, standard representation}
называется
\AddIndex{стандартной компонентой над полем $F$ билинейного отображения $f$}
{standard component of bilinear map, division ring}.
\end{\TheoremStyle}
\begin{proof}
Следствие теоремы
\xRef[0701.238]{theorem: standard representation of polylinear map, division ring}.
Здесь даны перестановки
\ShowEq{bilinear map, division ring, standard representation, 1}
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{bilinear map over field, division ring}
Пусть поле $F$ является подкольцом центра $Z(D)$ тела $D$.
Пусть \eV - базис тела $D$ над полем $F$.
Билинейное отображение
\ShowEq{bilinear map g, division ring}
можно представить в виде $D$-значной билинейной формы
над полем $F$
\ShowEq{bilinear map over field, division ring}
где
\ShowEq{biadditive map over field, coordinates, division ring}
и величины $\aD g{ij}$ являются координатами $D$-значного ковариантного
тензора над полем $F$.
\end{\TheoremStyle}
\begin{proof}
Следствие теоремы
\xRef[0701.238]{theorem: polylinear map over field, division ring}.
\end{proof}

Матрица $G=|\aD g{ij}|$ называется
\AddIndex{матрицей билинейной функции}{matrix of bilinear function}.
Если матрица $G$ невырождена, то билинейная функция $g$ называется
\AddIndex{невырожденной}{nonsingular bilinear function}.

\begin{\TheoremStyle}
\labelTheorem{bilinear map symmetric, division ring}
Билинейное отображение
\ShowEq{bilinear map g, division ring}
симметрично тогда и только тогда, когда
матрица $G$ симметрична
\ShowEq{biadditive map symmetric, division ring}
\end{\TheoremStyle}
\begin{proof}
Следствие теоремы
\xRef[0701.238]{theorem: polylinear map symmetric, division ring}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{bilinear map skew symmetric, division ring}
Билинейное отображение
\ShowEq{bilinear map g, division ring}
косо симметрично тогда и только тогда, когда
матрица $G$ косо симметрична
\ShowEq{biadditive map skew symmetric, division ring}
\end{\TheoremStyle}
\begin{proof}
Следствие теоремы
\xRef[0701.238]{theorem: polylinear map skew symmetric, division ring}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{coordinates of bilinear map, division ring over field}
Компоненты билинейного отображения
\ShowEq{bilinear map g, division ring}
и его матрица над полем $F$
связаны равенством
\ShowEq{coordinates of biadditive map, division ring over field}
\ShowEq{coordinates of biadditive map, division ring over field, 1}
\end{\TheoremStyle}
\begin{proof}
Следствие теоремы
\xRef[0701.238]{theorem: coordinates of polylinear map, division ring over field}.
Для доказательства утверждения достаточно подставить
\EqRef{bilinear map, division ring, standard representation, 1}
в равенства
\EqRef[0701.238]{coordinates of polylinear map, division ring over field},
\EqRef[0701.238]{coordinates of polylinear map, division ring over field, 1}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{two bilinear maps, division ring}
Если билинейное отображение
\ShowEq{bilinear map g, division ring}
имеет матрицу $G=\|\aD g{ij}\|$, то существует
билинейное отображение
\ShowEq{bilinear map g prim, division ring}
которое имеет матрицу
\ShowEq{bilinear map g prim matrix, division ring}
\end{\TheoremStyle}
\begin{proof}
Положим
\ShowEq{two bilinear maps, assumption, division ring}
Из равенств
\EqRef{coordinates of biadditive map, division ring over field, 1},
\EqRef{two bilinear maps, assumption, division ring}
следует
\ShowEq{two bilinear maps, division ring}
\end{proof}

%Для кватернионов равенство
%\EqRef{coordinates of biadditive map, division ring over field, 1}
%имеет вид
%\ShowEq{coordinates of biadditive map, division ring over field, 2}

\section{Квадратичное отображение тела}

\begin{\DefinitionStyle}
Пусть $D$ - тело.
Отображение
\[
h:D\rightarrow R
\]
называется \AddIndex{квадратичным}
{Quadratic Map of Division Ring}, если существует
билинейное отображение
\ShowEq{bilinear map g, division ring}
такое, что
\[
h(a)=g(a,a)
\]
Билинейное отображение $g$ называется отображением,
ассоциированным отображению $h$.
\end{\DefinitionStyle}

Отображение $g$ определено неоднозначно для заданного отображения $h$.
Однако согласно теореме
\RefTheorem{two bilinear maps, division ring},
мы всегда можем положить, что билинейное отображение $g$
симметрично
\[
g(a,b)=g(b,a)
\]
Действительно, если билинейное отображение $g_1$, ассоциированное
отображению $h$, не симметрично, то мы положим
\[
g(a,b)=(g_1(a,b)+g_1(b,a))/2
\]

Так как билинейное отображение однородно степени $1$ над полем $R$
по каждой переменной,
квадратичное отображение однородно степени $2$ над полем $R$.

\begin{\TheoremStyle}
\labelTheorem{standard representation of quadratic map, division ring}
Пусть $D$ - тело характеристики $0$.
Пусть $F$ - поле, которое является подкольцом центра
тела $D$.
Допустим $\Basis p$
- базис тела $D$ над полем $F$.
\AddIndex{Стандартное представление квадратичного отображения тела над полем $F$}
{quadratic map, standard representation, division ring}
имеет вид
\ShowEq{def quadratic map, division ring, standard representation}
\ShowEq{quadratic map, division ring, standard representation}
Выражение
$\ShowSymbol{standard component of quadratic map, division ring}{}$
в равенстве
\EqRef{quadratic map, division ring, standard representation}
называется
\AddIndex{стандартной компонентой квадратичного отображения $f$ над полем $F$}
{standard component of quadratic map, division ring}.
\end{\TheoremStyle}
\begin{proof}
Следствие теоремы
\RefTheorem{standard representation of bilinear map, division ring}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{quadratic map over field, division ring}
Пусть поле $F$ является подкольцом центра $Z(D)$ тела $D$.
Пусть $\Basis e$ - базис тела $D$ над полем $F$.
Квадратичного отображение $f$
можно представить в виде $D$-значной квадратичной формы
над полем $F$
\ShowEq{quadratic map over field, division ring}
где
\ShowEq{quadratic map over field, coordinates, division ring}
и $g$ - ассоциированное билинейное отображение.
Величины $\aD f{ij}$ являются координатами $D$-значного ковариантного
тензора над полем $F$.
\end{\TheoremStyle}
\begin{proof}
Для выбранного билинейного отображения $g$, ассоциированного отображению $f$,
утверждение теоремы является следствием теоремы
\RefTheorem{bilinear map over field, division ring}.
Нам надо доказать независимость координат квадратичного отображения от
выбора ассоциированного отображения $g$.

Допустим, $g_1$, $g_2$ - билинейные отображения, ассоциированные отображению $f$.
Тогда
\ShowEq{associative biadditive map, 1, division ring}
Для произвольного $a\in D$
\ShowEq{associative biadditive map, 2, division ring}
Если для данных $i$, $j$ мы рассмотрим $a\in D$,
для которого $a_i=a_j=1$, то мы получим
\ShowEq{associative biadditive map, 3, division ring}
Из равенств
\EqRef{associative biadditive map, 1, division ring},
\EqRef{associative biadditive map, 3, division ring}
следует
\ShowEq{associative biadditive map, 4, division ring}
Следовательно, если ассоциированное билинейное отображение симметрично,
то оно определенно однозначно.
\end{proof}

Матрица $F=|\aD f{ij}|$ называется
\AddIndex{матрицей квадратичного отображения}
{matrix of quadratic map, division ring}.
Если матрица $F$ невырождена, то квадратичное отображение $f$
называется \AddIndex{невырожденным}{}.
Ранг матрицы $F$ называется
\AddIndex{рангом квадратичного отображения}
{rank of quadratic map, division ring} $f$.

\begin{\TheoremStyle}
\labelTheorem{coordinates of quadratic map, division ring over field}
Отображение
\[
f:D\rightarrow D
\]
квадратичное над полем $F$,
определено как отображение над телом тогда и только тогда, когда
\ShowEq{coordinates of quadratic map, division ring over field}
\ShowEq{coordinates of quadratic map, division ring over field, 1}
\end{\TheoremStyle}
\begin{proof}
Подставим
\ShowEq{coordinates of quadratic map, division ring over field, 1a}
в равенство
\EqRef{quadratic map, division ring, standard representation}.
Тогда равенство \EqRef{quadratic map, division ring, standard representation}
примет вид
\ShowEq{coordinates of quadratic map, division ring over field, 1b}
Равенство
\EqRef{coordinates of quadratic map, division ring over field}
следует из сравнения равенств
\EqRef{coordinates of quadratic map, division ring over field, 1b}
и
\EqRef{quadratic map over field, division ring}.
\end{proof}

Из теоремы \RefTheorem{quadratic map over field, division ring}
следует, что координаты $\aD f{pq}$ образуют тензор.
В теореме
\xRef[0701.238]{theorem: linear map over field, division ring}
описана структура допустимых преобразований.

\begin{\TheoremStyle}
\labelTheorem{additive equation ax+xa=b, division ring}
Пусть поле $F$ является подкольцом центра $Z(D)$ тела $D$.
Пусть $\Basis p$ - базис тела $D$ над полем $F$.
Пусть $C^{\gik}_{\gi{ij}}$ - структурные константы тела $D$ над полем $F$.
Если
\ShowEq{additive equation ax+xa=b, division ring, 0}
то уравнение
\ShowEq{additive equation ax+xa=b, division ring}
имеет единственного решение.

Если определитель равен $0$,
то условием существования
решения является $F$\Hyph линейная зависимость вектора $b$ от векторов
\ShowEq{additive equation ax+xa=b, division ring, 1}.
В этом случае, уравнение
\EqRef{additive equation ax+xa=b, division ring}
имеет бесконечно много решений. В противном случае уравнение не
имеет решений.
\end{\TheoremStyle}
\begin{proof}
Из равенств
\EqRef{product, division ring over field},
\EqRef{additive equation ax+xa=b, division ring}
следует
\ShowEq{additive equation ax+xa=b, division ring, 2}
Так как векторы $\aD pk$ линейно независимы,
то из равенства
\EqRef{additive equation ax+xa=b, division ring, 2}
следует, что координаты $x^{\gi j}$ удовлетворяют
системе линейных уравнений
\ShowEq{additive equation ax+xa=b, division ring, 3}
Следовательно, если определитель системы
\EqRef{additive equation ax+xa=b, division ring, 3}
не равен $0$, то система имеет единственное решение.

Аналогично, если определитель равен $0$,
то условием существования
решения является равенство ранга расширенной матрицы и ранга
матрицы системы линейных уравнений.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{quadratic map over field, division ring, reduce}
Пусть поле $F$ является подкольцом центра $Z(D)$ тела $D$.
Существует квадратичное отображение $f$ такое, что можно найти
базис $\Basis p$ над полем $F$, в котором отображение $f$ представлено как
сумма квадратов.
\end{\TheoremStyle}
\begin{proof}
Приведение квадратичной формы к диагональному виду выполнено
аналогично тому как это сделано в \citeBib{Kurosh: High Algebra},
с. 169 - 172.
%Как мы увидим в процессе доказательства,
%существуют ограничения на выбор формы, допускающей приведение
%к диагональному виду. Однако мы не будем задерживаться
%на формулировке этих ограничений и укажем как необходимо
%выполнить требуемое построение.
Рассматриваемые преобразования переменных
связаны с соответствующими преобразованиями базиса.
Нас не интересует,
является ли эти преобразования базиса допустимыми.
Причина состоит в том, что базис, выбранный вначале может быть не связан
с каноническим базисом допустимым преобразованием.
Однако для нас важно,
чтобы окончательное представление отображения $f$ было допустимым.

%Пусть $h$ - биаддитивная форма, ассоциированная с отображением $f$.
%Все преобразования, выполняемые над отображением $f$, мы будем выполнять также
%с формой $h$.

Мы докажем утверждение индукцией
по числу переменных в представлении
квадратичного отображения.
Для этого мы будем записывать квадратичное отображение $f$
в виде отображения от $n$ переменных $a^{\giA}$, ..., $a^{\gin}$
\ShowEq{quadratic map over field, division ring, reduce 1}
Представление квадратичного отображения в виде
\EqRef{quadratic map over field, division ring, reduce 1}
называется \AddIndex{квадратичной формой}
{quadratic form, division ring}.

Утверждение очевидно, если квадратичная форма зависит от одной переменной $a^1$,
так как в этом случае квадратичная форма имеет вид
\ShowEq{quadratic map over field, division ring, reduce 1, 1}

Допустим утверждение теоремы справедливо
для квадратичной формы от $n-1$ переменной.

\begin{enumerate}
\item
\labelItem{quadratic map over field, division ring, reduce, case 1}
Пусть квадратичная форма содержит квадраты переменных.
Не нарушая общности, положим $\aD f{11}\ne 0$.
Рассмотрим отображение
\ShowEq{quadratic map over field, division ring, reduce 1, 2}
Мы выбираем значения ${}_{\gi j}h$ таким образом, чтобы удовлетворить равенство
\ShowEq{quadratic map over field, division ring, reduce 1, 3}
Когда $\gi j=\giA$, из равенства
\EqRef{quadratic map over field, division ring, reduce 1, 3}
следует
\ShowEq{quadratic map over field, division ring, reduce 1, 4}
Когда $\gi j>\giA$, из равенств
\EqRef{quadratic map over field, division ring, reduce 1, 2},
\EqRef{quadratic map over field, division ring, reduce 1, 4}
следует
\ShowEq{quadratic map over field, division ring, reduce 1, 5}
Из теоремы
\RefTheorem{additive equation ax+xa=b, division ring}
следует, что если
\ShowEq{quadratic map over field, division ring, reduce 1, 6}
то уравнение
\EqRef{quadratic map over field, division ring, reduce 1, 5}
имеет единственное решение.
Мы предположим, что условие
\EqRef{quadratic map over field, division ring, reduce 1, 6}
выполнено, и рассмотрим замену переменных
\ShowEq{quadratic map over field, division ring, reduce 1, 7}
Следовательно, отображение $f_1(a^{\giA},...,a^{\gin})$ не зависит от $b^{\giA}$.
Согласно определению
\EqRef{quadratic map over field, division ring, reduce 1, 2},
мы представили отображение $f(a^{\giA},...,a^{\gin})$ в виде суммы квадрата переменной
$b^{\giA}$ и квадратичного отображения от $b^{\giA}$ не зависящего.
\ShowEq{quadratic map over field, division ring, reduce 1, 8}
Так как форма $f_1$ зависит от $n-1$ переменной, то мы можем
найти преобразование переменных, приводящее эту форму к сумме
квадратов переменных.

\item
Если
\ShowEq{quadratic map over field, division ring, reduce 2, 1}
то нам нужно дополнительное
линейное преобразование, приводящее к появлению квадратов переменных.
Положим
\ShowEq{quadratic map over field, division ring, reduce 2, 2}
Совершим линейное преобразование
\ShowEq{quadratic map over field, division ring, reduce 2, 3}
В результате этого преобразования слагаемое
\ShowEq{quadratic map over field, division ring, reduce 2, 4}
примет вид
\ShowEq{quadratic map over field, division ring, reduce 2, 5}
Мы получили квадратичную форму, рассмотренную в случае
\RefItem{quadratic map over field, division ring, reduce, case 1}.
\end{enumerate}
\end{proof}

Если все коэффициенты квадратичной формы в каноническом представлении действительны, то
$f(a)\in R$ для любого $a\in D$.
%Мы должны доказать, что число положительных и отрицательных слагаемых
%не зависит от выбора функции.

Допустим, мы выбрали квадратичную форму $f$, принимающую
действительные значения.

\begin{\DefinitionStyle}
Пусть $D$ - тело.
Квадратичное отображение
\[
f:D\times D\rightarrow D
\]
называется
\AddIndex{положительно определённым}
{positive definite biadditive map, division rin},
если
\[
f(a)\in R
\]
для любого $a\in D$ и при этом выполнены условия
\begin{align*}
f(a)&\ge 0
\\
f(a)&=0=> a=0
\end{align*}
Положительно определённое квадратичное отображение
называется \AddIndex{эвклидовой метрикой на теле}
{Euclidean metric on division ring} $D$.
Симметричное ассоциированное билинейное отображение $g$
называется \AddIndex{эвклидовым скалярным произведением на теле}
{Euclidean scalar product on division ring} $D$.
\end{\DefinitionStyle}

Если квадратичное отображение $f$ не является положительно
определённым, то это отображение называется
\AddIndex{псевдоэвклидовой метрикой на теле}
{pseudo-Euclidean metric on division ring} $D$.
Симметричное ассоциированное билинейное отображение $g$ называется
\AddIndex{псевдоэвклидовым скалярным произведением на теле}
{pseudo-Euclidean scalar product on division ring} $D$.
Пусть $\Basis e$ - базис, относительно которого
форма $f$ представлена в виде суммы квадратов.
Существуют вектора базиса $\aD ei$,
для которых $f(\aD ei)<0$.
Для произвольного $a=\aU ai\aD ei$
определим операцию сопряжения равенством
\ShowEq{hermitian conjugation, division ring, 1}
Выражение
$\ShowSymbol{hermitian conjugation, division ring}{}$
называется
\AddIndex{эрмитовым сопряжением}{hermitian conjugation, division ring}.

Рассмотрим биаддитивное отображение
\ShowEq{hermitian conjugation, division ring, 2}
Отображение $f^{\star}(a)$ положительно определено
и называется \AddIndex{эрмитовой метрикой на теле}
{hermitian metric on division ring} $D$.
Симметричное ассоциированное отображение $g^{\star}$
называется \AddIndex{эрмитовым скалярным произведением на теле}
{hermitian scalar product on division ring} $D$.

Если отображение
\ShowEq{hermitian conjugation, division ring, 3}
линейно, то эрмитово скалярное произведение совпадает
с эвклидовым скалярнып произведением.
Аналогичное утверждение верно для метрики.

\ifx\texFuture\Defined
\section{Эвклидова норма на теле}

Рассмотрим положительно определённое квадратичное отображение
\[
f(a)=f^{\gi{ijk}}\ \aD ei\ a\ \aD ej\ a\ \aD ek
\]
на теле $D$. Мы можем рассматривать отображение $f$ как отображение
\[
f:D\rightarrow R
\]
тела $D$ в поле действительных чисел $R$.
Следовательно, мы можем определить отображение $F$ сограсно правилу
\[
F(a)=\sqrt{f(a)}
\]
Производная этого отображения имеет вид
\[
\partial F(a)(h)=\frac{\partial f(a)(h)}{2\sqrt{f(a)}}
=\frac{f^{\gi{ijk}}}
{2\sqrt{f(a)}}
(\aD ei\ h\ \aD ej\ a\ \aD ek
+\aD ei\ a\ \aD ej\ h\ \aD ek)
\]
\fi


==> Center.Ring.Russian.tex <==
%auto-ignore
\input{Center.Ring.Eq}

\begin{definition}
\labelDefinition{center of ring}
Пусть $D$ - кольцо.\,\footnote{\citeBib{Serge Lang},
стр. 84.} Множество \symb{Z(D)}{center of ring}1
элементов $a\in D$ таких, что
\ShowEq{center of ring}
для всех $x\in D$,
называется
\AddIndex{центром кольца $D$}{center of ring}.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{center of ring}
Центр $Z(D)$ кольца $D$ является подкольцом кольца $D$.
\end{theorem}
\begin{proof}
Непосредственно следует из определения \RefDefinition{center of ring}.
\end{proof}

\begin{definition}
Пусть $D$ - кольцо с единицей $e$.\,\footnote{Определение
дано согласно
определению из \citeBib{Serge Lang},
стр. 84, 85.} Отображение
\[
l:Z\rightarrow D
\]
для которого $l(n)=ne$ будет гомоморфизмом колец, и его ядро является
идеалом $(n)$, порождённым целым числом $n\ge 0$.
Канонический инъективный гомоморфизм
\[
Z/nZ\rightarrow D
\]
является изоморфизмом между $Z/nZ$ и подкольцом в $D$.
Если $nZ$ - простой идеал, то у нас возникает два случая.
\begin{itemize}
\item $n=0$. $D$ содержит в качестве подкольца
кольцо, изоморфное $Z$ и часто отождествляемое
с $Z$. В этом случае мы говорим, что $D$ имеет
\AddIndex{характеристику $0$}{ring has characteristic 0}.
\item $n=p$ для некоторого простого числа $p$. $D$ имеет
\AddIndex{характеристику $p$}{ring has characteristic p}, и $D$
содержит изоморфный образ $F_p=Z/pZ$.
\end{itemize}
\qed
\end{definition}

\begin{theorem}
\labelTheorem{integer subring of ring}
Пусть $D$ - кольцо характеристики $0$ и пусть $d\in D$.
Тогда любое целое число $n\in Z$ коммутирует с $d$.
\end{theorem}
\begin{proof}
Утверждение теоремы доказывается по индукции.
При $n=0$ и $n=1$ утверждение очевидно.
Допустим утверждение справедливо при $n=k$.
Из цепочки равенств
\[
(k+1)d=kd+d=dk+d=d(k+1)
\]
следует очевидность утверждения при $n=k+1$.
\end{proof}

\begin{theorem}
\labelTheorem{integer subring of center}
Пусть $D$ - кольцо характеристики $0$.
Тогда кольцо целых чисел $Z$ является подкольцом центра $Z(D)$ кольца $D$.
\end{theorem}
\begin{proof}
Следствие теоремы \RefTheorem{integer subring of ring}.
\end{proof}


==> Division.Ring.Russian.tex <==
%auto-ignore
\input{Division.Ring.Eq}
\chapter{Геометрия тела}
\labelChapter{Geometry of Division Ring}

\section{Центр тела}

\Input{Center.Ring}

Пусть $D$ - тело. Если $D$ имеет характеристику $0$,
$D$ содержит в качестве подполя изоморфный образ поля $Q$
рациональных чисел. Если $D$ имеет характеристику $p$,
$D$ содержит в качестве подполя изоморфный образ $F_p$.
В обоих случаях это подполе будет называться простым полем.
Так как простое поле является наименьшим подполем в $D$,
содержащим $1$ и не имеющим автоморфизмов, кроме тождественного,
его обычно отождествляют с $Q$ или $F_p$,
в зависимости от того, какой случай имеет место.

\begin{theorem}
\labelTheorem{center of division ring}
Центр $Z(D)$ тела $D$ является подполем тела $D$.
\end{theorem}
\begin{proof}
\begin{sloppypar}
Согласно теореме \RefTheorem{center of ring}
достаточно проверить, что $a^{-1}\in Z(D)$,
если $a\in Z(D)$.
Пусть $a\in Z(D)$.
Многократно применяя равенство \EqRef{center of ring},
мы получим цепочку равенств
\begin{equation}
\EqLabel{center of ring,1}
aa^{-1}x=x=xaa^{-1}=axa^{-1}
\end{equation}
Из \EqRef{center of ring,1} следует
\[
a^{-1}x=xa^{-1}
\]
Следовательно, $a^{-1}\in Z(D)$.
\end{sloppypar}
\end{proof}

\begin{theorem}
Пусть $D$ - тело характеристики $0$ и пусть $d\in D$.
Тогда для любого целого числа $n\in Z$
\ShowEq{inverse integer in division ring}
\end{theorem}
\begin{proof}
Согласно теореме \RefTheorem{integer subring of ring}
справедлива цепочка равенств
\ShowEq{inverse integer in division ring, 1}
Умножив правую и левую части равенства
\EqRef{inverse integer in division ring, 1} на $n^{-1}$,
получим
\ShowEq{inverse integer in division ring, 2}
Из \EqRef{inverse integer in division ring, 2} следует
\EqRef{inverse integer in division ring}.
\end{proof}

\begin{theorem}
\labelTheorem{division ring, rational number}
Пусть $D$ - тело характеристики $0$ и пусть $d\in D$.
Тогда любое рациональное число $p\in Q$ коммутирует с $d$.
\end{theorem}
\begin{proof}
Мы можем представить рациональное число $p\in Q$ в
виде $p=mn^{-1}$, $m$, $n\in Z$.
Утверждение теоремы следует из цепочки равенств
\[
pd=mn^{-1}d=n^{-1}dm=dmn^{-1}=dp
\]
основанной на утверждении теоремы \RefTheorem{integer subring of ring}
и равенстве \EqRef{inverse integer in division ring}.
\end{proof}

\begin{theorem}
\labelTheorem{rational subring of center}
Пусть $D$ - тело характеристики $0$.
Тогда поле рациональных чисел $Q$ является подполем центра $Z(D)$ тела $D$.
\end{theorem}
\begin{proof}
Следствие теоремы \RefTheorem{division ring, rational number}.
\end{proof}

\section{Геометрия тела над полем}
\labelSection{Geometry of Division Ring over Field}

\ShowConvention{we use separate color for index of element}

%\begin{remark}
%\labelRemark{Geometry of Division Ring over Field}
Мы можем рассматривать тело $D$ как векторное пространство над полем
\ShowEq{division ring over field}
Так как $F$ - поле, то мы можем писать все индексы справа от
корневой буквы.
При этом мы будем пользоваться следующими соглашением
\RefConvention{we use separate color for index of element}.
%\qed
%\end{remark}

\begin{remark}
\labelRemark{dimension of division ring}
Пусть $\Basis e$ - базис тела $D$ над полем $F$. Тогда произвольный
элемент $a\in D$ можно представить в виде
\ShowEq{expansion relative to basis, division ring}
Если размерность тела $D$ над полем $F$ бесконечна,
то базис может быть либо счётным, либо его мощность
может быть не меньше, чем мощность континуума.
Если базис счётный, то на коэффициенты $a^{\gi i}$
разложения \EqRef{expansion relative to basis, division ring} накладываются
определённые ограничения. Если мощность множества $I$ континуум,
то предполагается, что на множестве $I$ определена мера и
сумма в разложении \EqRef{expansion relative to basis, division ring}
является интегралом по этой мере.
\qed
\end{remark}

\begin{remark}
\labelRemark{Geometry of Division Ring over Field}
Поскольку в теле $D$ определена операция произведения, то мы можем рассматривать
тело как алгебру над полем
\ShowEq{division ring over field}
Для элементов базиса мы положим
\ShowEq{structural constants}
\ShowEq{product, division ring over field, basis}
Коэффициенты $\ShowSymbol{structural constants}{ring}$
разложения \EqRef{product, division ring over field, basis}
называются \AddIndex{структурными константами}{structural constants}
тела $D$ над полем $F$.
\end{remark}

Из равенств \EqRef{expansion relative to basis, division ring},
\EqRef{product, division ring over field, basis} следует
\ShowEq{product, division ring over field}
Из равенства \EqRef{product, division ring over field} следует
\ShowEq{product, division ring over field, associativity, proof}
Из ассоциативности произведения
\[
(ab)c=a(bc)
\]
и равенств \EqRef{product, division ring over field, associativity, proof, 1}
и \EqRef{product, division ring over field, associativity, proof, 2}
следует
\ShowEq{product, division ring over field, associativity, proof, 3}
Так как векторы $a$, $b$, $c$ произвольны, а
векторы $e_{\gik}$ линейно независимы, то из равенства
\EqRef{product, division ring over field, associativity, proof, 3}
следует
\ShowEq{product, division ring over field, associativity}

\begin{theorem}
\labelTheorem{division ring over field, change basis}
Координаты $a^{\gi j}$ вектора $a$ являются тензором
\ShowEq{division ring over field, change basis, 3}
\end{theorem}
\begin{proof}
Пусть $\Basis e'$ - другой базис. Пусть
\ShowEq{division ring over field, change basis}
преобразование, отображающее базис $\Basis e$ в
базис $\Basis e'$.
Так как вектор $a$ не меняется, то
\ShowEq{division ring over field, change basis, 1}
Из равенств \EqRef{division ring over field, change basis}
и \EqRef{division ring over field, change basis, 1}
следует
\ShowEq{division ring over field, change basis, 2}
Так как векторы $e_{\gi j}$ линейно независимы, то равенство
\EqRef{division ring over field, change basis, 3}
следует
из равенства
\EqRef{division ring over field, change basis, 2}.
Следовательно, компоненты вектора являются тензором.
\end{proof}

\begin{theorem}
Структурные константы тела $D$ над полем $F$ являются тензором
\ShowEq{product, division ring over field, structural constant prim}
\end{theorem}
\begin{proof}
Рассмотрим аналогичным образом преобразование произведения.
Равенство \EqRef{product, division ring over field}
в базисе $\Basis e'$ имеет вид
\ShowEq{product, division ring over field, prim}
Подставив \EqRef{division ring over field, change basis, 3}
и \EqRef{division ring over field, change basis}
в \EqRef{product, division ring over field, prim},
получим
\ShowEq{product, division ring over field, prim, 1}
Из \EqRef{product, division ring over field} и
\EqRef{product, division ring over field, prim, 1}
следует
\ShowEq{product, division ring over field, prim, 2}
Так как векторы $a$ и $b$ произвольны, а
векторы $e_{\gil}$ линейно независимы, то равенство
\EqRef{product, division ring over field, structural constant prim}
следует
из равенства
\EqRef{product, division ring over field, prim, 2}.
Следовательно, структурные константы являются тензором.
\end{proof}

%\section{Сопряжение в теле}

%Пусть ${}_ie$ - базис тела $D$ над полем $F$.
%Положим ${}_ie^*={}_ie$. Будем рассматривать базис,
%для которого ${}_0e=1$. Для произвольного элемента
%$a\in D$, $a=a^0\ {}_0e+a^i\ {}_ie$


==> Euclidean.Space.Russian.tex <==
%auto-ignore
\input{Euclidean.Space.Eq}
\chapter{Евклидово пространство}
\labelChapter{Euclidean Space}

\section{Евклидово пространство}

Пусть $V$ - $D$\Hyph векторное пространство.
Билинейное отображение
\ShowEq{Bilinear map, V times V to D}
можно представить в виде
\ShowEq{Bilinear map, vector space}
где $\GIJ$ - билинейное отображение
\ShowEq{Bilinear map, maps}

\begin{\DefinitionStyle}
Билинейное отображение
\ShowEq{Bilinear map, V times V to D}
называется \AddIndex{симметричным}{symmetric bilinear map}, если
\[
g(w,v)=g(v,w)
\]
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
Билинейное отображение
\ShowEq{Bilinear map, V times V to D}
называется
\AddIndex{эвклидовым скалярным произведением}
{Euclidean scalar product, vector space}
в $D$\Hyph векторном пространстве $V$,
если
$\GII$ - эвклидово скалярное произведение в теле $D$
и $\GIJ=0$ для $\gii\ne \gij$.
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
Билинейное отображение
\ShowEq{Bilinear map, V times V to D}
называется
\AddIndex{псевдоэвклидовым скалярным произведением}
{pseudo-Euclidean scalar product, vector space}
в $D$\Hyph векторном пространстве $V$,
если
$\GII$ - псевдоэвклидово скалярное произведение в теле $D$
и $\GIJ=0$ для $\gii\ne \gij$.
\end{\DefinitionStyle}

Если в теле $D$ определена операция эрмитова сопряжения,
то мы можем эту операцию распространить на
$D$\Hyph векторное пространство $V$,
а именно для данного вектора
\ShowEq{vector v}
мы определим
\AddIndex{эрмитово сопряжённый вектор}{hermitian conjugated vector}
\ShowEq{hermitian conjugated vector}

%Если все отображения $g_{ij}$ - эрмитовы, то
%\[
%g(v,w)=g_{ij}(v^i,w^j)=g_{ij}((w^j)^*,(v^i)^*)=
%g(v^*,w^*)
%\]

\begin{\DefinitionStyle}
Билинейное отображение
\ShowEq{Bilinear map, V times V to D}
называется
\AddIndex{эрмитовым скалярным произведением}
{hermitian scalar product, vector space}
в $D$\Hyph векторном пространстве $V$,
если
$\GII$ - эрмитово скалярное произведение в теле $D$
и $\GIJ=0$ для $\gii\ne \gij$.
\end{\DefinitionStyle}

%Существуют тела, в которых биаддитивная симметричная форма не может
%быть положительна определена.
%В этом случае мы будем рассматривать эрмитову форму.

\section{Базис в евклидовом пространстве}
\labelSection{Basis in Euclidean Space}

Когда мы определяем метрику в центро-аффинном пространстве, мы
получаем новую геометрию потому, что
мы можем измерять расстояние и длину вектора. Если метрика
положительно определена, мы будем называть пространство евклидовым
\ShowEq{Euclid space, division ring}
в противном случае мы будем называть пространство псевдоевклидовым
\ShowEq{pseudo Euclid space, division ring}

Преобразования, которые сохраняют длину,
образуют группу Ли $SO(n)$ для евклидова пространства и группу Ли $SO(n,m)$ для
псевдоэвклидова пространства, где $n$ и $m$ числа положительных
и отрицательных слагаемых в метрике.

\begin{\DefinitionStyle}
\AddIndex{Ортонормированный базис}{Orthonormal Basis, division ring}
\ShowEq{Orthonormal Basis, division ring}
- это множество
линейно независимых векторов $\Vector{e}_i$ таких, что длина
каждого вектора равна $1$ и различные векторы ортогональны.
\end{\DefinitionStyle}

%Существование ортогонального базиса доказывается с помощью
%процесса ортогонализации Грама--Шмидта.

\begin{\DefinitionStyle}
\AddIndex{Многообразие базисов
\ShowEq{FEn}
евклидова пространства}{Basis Manifold, Euclid Space, division ring}
- это множество ортонормированных базисов этого пространства.
\end{\DefinitionStyle}

Мы будем называть активное преобразование
\AddIndex{движением}{movement transformation}.
Мы будем называть пассивное преобразование
\AddIndex{квазидвижением}{quasi movement, division ring}.


==> Group.Representation.English.tex <==
%auto-ignore
\input{Group.Representation.Eq}
\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\chapter{Representation of Group}
\labelChapter{Representation of Group}
\fi

\section{Representation of Group}
\labelSection{Representation of Group}

Group is among few algebras that allow somebody to consider the
product of transformations of the $\Omega$\Hyph algebra $M$ in such a way that, if
transformations belong to the representation, then their product also
belongs to the representation.
We should remember that order of maps in product
depends on order of maps on diagram and how these
maps act over elements of the set (from left or from right).

\begin{definition}
\labelDefinition{left-side representation of group}
Let ${}^*M$ be a group with product
\ShowEq{fg *M Tstar}
and $\delta$ be unit of group ${}^\star M$.
Let $G$ be group.
We call a homomorphism of group
\ShowEq{left-side representation of group, map}
\AddIndex{left-side representation}{left-side representation} of group $G$
or
\AddIndex{\Ts{G}representation}{A* representation of algebra}
in $\Omega$\Hyph algebra $M$ if the map $f$ holds
\ShowEq{left-side representation of group}
\qed
\end{definition}

\begin{remark}
Since the map \EqRef{left-side representation of group, map}
is homomorhism, then
\ShowEq{left-side representation of group, map product}
We use here convention
\[
f(a)f(b)=f(a)\circ f(b)
\]
Thus, the idea of representation of group is
that we multiply elements of group in the same order
as we multiply transformations of representation.
From equations \EqRef{left-side representation of group}
and \EqRef{left-side representation of group, map product}
it follows
\ShowEq{left-side representation of group, associativity}
Equation
\EqRef{left-side representation of group, associativity}
together with associativity of product of transformations expresses
\AddIndex{associative law}{associative law}
for \Ts{G}representation.
This allows writing of equation
\EqRef{left-side representation of group, associativity}
without using of brackets
\[
f(ab)u=f(a)f(b)u
\]
\qed
\end{remark}

\begin{definition}
\labelDefinition{right-side representation of group} 
Let $M^\star$ be a group with product
\ShowEq{fg *M starT}
and $\delta$ be unit of group $M^\star$.
Let $G$ be group.
We call a homomorphism of group
\ShowEq{right-side representation of group, map}
\AddIndex{right-side representation}{right-side representation} of group $G$
or
\AddIndex{\sT{G}representation}{*A representation of algebra}
in $\Omega$\Hyph algebra $M$ if the map $f$ holds
\ShowEq{right-side representation of group}
\qed
\end{definition}

\begin{remark}
Since the map \EqRef{right-side representation of group, map}
is homomorhism, then
\ShowEq{right-side representation of group, map product}
From equations \EqRef{right-side representation of group}
and \EqRef{right-side representation of group, map product}
it follows
\ShowEq{right-side representation of group, associativity}
Equation
\EqRef{right-side representation of group, associativity}
together with associativity of product of transformations expresses
\AddIndex{associative law}{associative law}
for \sT{G}representation.
This allows writing of equation
\EqRef{right-side representation of group, associativity}
without using of brackets
\[
uf(ab)=uf(a)f(b)
\]
\qed
\end{remark}

\begin{definition}
\labelDefinition{nonsingular transformation} 
We call the transformation
\[
t:M\rightarrow M
\]
\AddIndex{nonsingular transformation}{nonsingular transformation},
if there exists inverse map.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{inverse transformation}
For any $g\in G$ transformation is
nonsingular and satisfies equation
\begin{equation}
\EqLabel{inverse transformation}
f(g^{-1})=f(g)^{-1}
\end{equation}
\end{theorem}
\begin{proof}
Since \EqRef{left-side representation of group} and
\ShowEq{f(e)=}
we have
\[
u=\delta (u)=f(gg^{-1})(u)=f(g)(f(g^{-1})(u))
\]
This completes the proof.
\end{proof}

\begin{theorem}
The group operation determines two different representations on the group:
\begin{itemize}
\item
The \AddIndex{left shift}{left shift}
\ShowEq{left shift =}
\ShowEq{left shift}
is \Ts{G}representation on the set\,\footnote{Left shift
is not a representation of group in a group,
because the transformation $t_\star$ is not a homomorphism of
group.
Similar remark is true for right shift.
} $G$
\ShowEq{left shift, product}
\item
The \AddIndex{right shift}{right shift}
\ShowEq{right shift =}
\ShowEq{right shift}
is \sT{G}representation on the set $G$
\ShowEq{right shift, product}
\end{itemize}
\end{theorem}
\begin{proof}
Equation \EqRef{left shift, product}
follows from associativity of product
\[
t_\star(ab)c=(ab)c=a(bc)=t_\star(a)(t_\star(b)c)
=(t_\star(a)\circ t_\star(b))c
\]
In a similar manner we prove the equation \EqRef{right shift, product}.
\end{proof}

\begin{definition}
\labelDefinition{orbit of left-side representation of group}
Let $G$ be group.
Let $f$ be \Ts{G}representation in $\Omega$\Hyph algebra $M$.
For any $v\in M$ we define \AddIndex{orbit of representation of the group $G$}
{orbit of representation of group} as set
\ShowEq{orbit of representation of group}
\qed
\end{definition}

Since $f(e)=\delta$ we have
$v\in f(G)v$.

\begin{theorem}
\labelTheorem{proper definition of orbit}
Suppose
\begin{equation}
\EqLabel{orbit, proposition}
v\in f(G)u
\end{equation}
Then
\[
f(G)u=f(G)v
\]
\end{theorem}
\begin{proof}
From \EqRef{orbit, proposition} it follows
that there exists $a\in G$ such that
\begin{equation}
v=f(a)u
\EqLabel{orbit, 1}
\end{equation}
Suppose $w\in f(G)v$. Then
there exists $b\in G$ such that
\begin{equation}
w=f(b)v
\EqLabel{orbit, 2}
\end{equation}
If we substitute \EqRef{orbit, 1}
into \EqRef{orbit, 2} we get
\begin{equation}
w=f(b)(f(a)u)
\EqLabel{orbit, 3}
\end{equation}
Since \EqRef{left-side representation of group},
we see that
from \EqRef{orbit, 3} it follows
that $w\in f(G)u$.
Thus
\[
f(G)v\subseteq f(G)u
\]

Since \EqRef{inverse transformation},
we see that
from \EqRef{orbit, 1} it follows
that
\begin{equation}
u=f(a)^{-1}v=f(a^{-1})v
\EqLabel{orbit, 4}
\end{equation}
From \EqRef{orbit, 4} it follows that
$u\in f(G)v$ and therefore
\[
f(G)u\subseteq f(G)v
\]
This completes the proof.
\end{proof}

Thus, \Ts{G}representation $f$ in $\Omega$\Hyph algebra $M$
forms equivalence $S$ and
the orbit $f(G)u$ is equivalence class.
We will use notation
\symb{M/f(G)}{space of orbits of G* representation}1
for quotient set $M/S$ and
this set is called
\AddIndex{space of orbits of \Ts{G}representation}
{space of orbits of G* representation} $f$.

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{direct product of representations}
Suppose $f_1$ is \Ts{G}representation in $\Omega$\Hyph algebra $M_1$ and
$f_2$ is \Ts{G}representation in $\Omega$\Hyph algebra $M_2$.
Then we introduce
\AddIndex{direct product of \Ts{G}representations}
{direct product of G* representations}
$f_1$ and $f_2$
\begin{align*}
f&=f_1\times f_2:G\rightarrow M_1\otimes M_2\\
f(g)&=(f_1(g),f_2(g))
\end{align*}
\end{theorem}
\begin{proof}
To show that $f$ is a representation,
it is enough to prove that $f$ satisfies the definition
\RefDefinition{left-side representation of group}.
\[f(e)=(f_1(e),f_2(e))=(\delta_1,\delta_2)=\delta\]
\begin{align*}
f(ab)u&=(f_1(ab)u_1,f_2(ab)u_2)\\
&=(f_1(a)(f_1(b)u_1),f_2(a)(f_2(b)u_2))\\
&=f(a)(f_1(b)u_1,f_2(b)u_2)\\
&=f(a)(f(b)u)
\end{align*}
\end{proof}
\fi

\section{Single Transitive Right-Side Representation of Group}
\labelSection{Single Transitive Representation of Group}

\begin{definition}
\labelDefinition{kernel of inefficiency of representation of group}
We call
\AddIndex{kernel of inefficiency of \Ts{G}representation}
{kernel of inefficiency of G* representation}
a set \[K_f=\{g\in G:f(g)=\delta\}\]
\qed
\end{definition}

\begin{theorem}
\labelTheorem{kernel of inefficiency, representation of group}
A kernel of inefficiency of \Ts{G}representation is a subgroup of the group $G$.
\end{theorem}
\begin{proof}
Assume
$f(a_1)=\delta$ and $f(a_2)=\delta$. Then
\[f(a_1a_2)u=f(a_1)(f(a_2)u)=u\]
\[f(a^{-1})=f^{-1}(a)=\delta\]
\end{proof}

\begin{theorem}
\Ts{G}representation is
\AddIndex{effective}{effective G* representation}
iff kernel of inefficiency $K_f=\{e\}$.
\end{theorem}
\begin{proof}
Statement is corollary of definitions
\RefDefinition{effective representation of algebra} and
\RefDefinition{kernel of inefficiency of representation of group} and
of the theorem \RefTheorem{kernel of inefficiency, representation of group}.
\end{proof}

If an action is not effective we can switch to an effective one
by changing group $G_1=G|K_f$
using factorization by the kernel of inefficiency.
This means that we can study only an effective action.

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{definition}
\labelDefinition{free representation of group}
Consider \Ts{G}representation $f$ in $\Omega$\Hyph algebra $M$.
A \AddIndex{little group}{little group} or
\AddIndex{stability group}{stability group} of $x\in M$ is the set
\ShowEq{little group}

\Ts{G}representation $f$ is said to be
\AddIndex{free}{free representation of group},
if for any $x\in M$ stability group $G_x=\{e\}$.
\qed
\end{definition}

\begin{theorem}%
\labelTheorem{free representation of group}
Given free \Ts{G}representation $f$ in the $\Omega$\Hyph algebra $A$,
there exist $1-1$ correspondence between orbits of representation,
as well between orbit of representation and group $G$.
\end{theorem}
\begin{proof}
Given $a\in A$
there exist $g_1$, $g_2\in G$
\begin{equation}
\EqLabel{free representation of group, 1}
f(g_1)a=f(g_2)a
\end{equation}
We multiply both parts of equation \EqRef{free representation of group, 1}
by $f(g_1^{-1})$
\[
a=f(g_1^{-1})f(g_2)a
\]
Since the representation is free, $g_1=g_2$.
Since we established $1-1$ correspondence between
orbit and group $G$, we proved the statement of the theorem.
\end{proof}
\else

\begin{definition}
\labelDefinition{transitive representation of group}
We call a representation of group
\AddIndex{transitive}{transitive representation of group}
if for any $a, b \in V$ exists such $g$ that
\[a=f(g)(b)\]
We call a representation of group
\AddIndex{single transitive}{single transitive representation of group}
if it is transitive and effective.
\qed
\end{definition}

\begin{theorem}%single transitive
\Ts{G}representation is single transitive if and only if for any $a, b \in M$
exists one and only one $g\in G$ such that $a=f(g)(b)$
\end{theorem}
\begin{proof}
Corollary of definitions \RefDefinition{effective representation of algebra}
and \RefDefinition{transitive representation of group}.
\end{proof}
\fi

\begin{definition}
We call a space $V$
\AddIndex{homogeneous space}{homogeneous space} of group $G$
if we have single transitive \Ts{G}representation on $V$.
\qed
\end{definition}

\begin{theorem}%
\labelTheorem{single transitive representation of group}
If we define a single transitive
representation $f$ of the group $G$ on the $\Omega$\Hyph algebra $A$
then we can uniquely define coordinates on $A$ using coordinates on the group $G$.

If $f$ is left-side representation
then $f(a)$ is equivalent to the left shift $t_\star(a)$ on the group $G$.
If $f$ is right-side representation
then $f(a)$ is equivalent to the right shift ${}_\star t(a)$ on the group $G$.
\end{theorem}
\begin{proof}
We select a point $v\in A$
and define coordinates of a point $w\in A$
as coordinates of $a\in G$ such that $w=f(a) v$.
Coordinates defined this way are unique
up to choice of an initial point $v\in A$
because the action is effective.

If $f$ is left-side representation,
we will use the notation
\[f(a)v=av\]
Because the notation
\[f(a)(f(b)v)=a(bv)=(ab)v=f(ab)v\]
is compatible with the group structure we see that
left-side representation $f$ is equivalent to the left shift.

If $f$ is right-side representation,
we will use the notation
\[vf(a)=va\]
Because the notation
\[(vf(b))f(a)=(vb)a=v(ba)=vf(ba)\]
is compatible with the group structure we see that
right-side representation $f$ is equivalent to the right shift.
\end{proof}

\begin{remark}
We will write effective
\Ts{G}representation as
\[v'=t_\star(a) v=av\]
Orbit of this representation is
\ShowEq{orbit of effective G* representation}
We will use notation
\ShowEq{space of orbits of effective G* representation}
for the space of orbits of effective \Ts{G}representation.
\qed
\end{remark}

\begin{remark}
We will write effective
\sT{G}representation as
\[v'=v\ {}_\star t(a)=va\]
Orbit of this representation is
\ShowEq{orbit of effective *G representation}
We will use notation
\ShowEq{space of orbits of effective *G representation}
for the space of orbits of effective \sT{G}representation.
\qed
\end{remark}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{Free representation is single transitive}
Free \Ts{G*}representation is effective.
Free \Ts{G*}representation $f$ in $\Omega$\Hyph algebra $M$ is
single transitive representation on orbit.
\end{theorem}
\begin{proof}
The statement of theorem is
the corollary of definition \RefDefinition{free representation of group}.
\end{proof}
\fi

\begin{theorem}%
\labelTheorem{shifts on group commuting}
Left and right shifts on group $G$ are commuting.
\end{theorem}
\begin{proof}
This is the consequence of the associativity on the group $G$
\[(t_\star(a)\circ\ {}_\star t(b))c = a(cb)=(ac)b
=({}_\star t(b)\circ t_\star(a))c\]
\end{proof}

Theorem \RefTheorem{shifts on group commuting} can
be phrased n the following way.

\begin{theorem}%
\labelTheorem{shift is automorphism of representation}
Let $G$ be group. For any $a\in G$, the map
$t_\star(a)$ is automorphism of representation ${}_\star t$.
\end{theorem}
\begin{proof}
According to theorem
\RefTheorem{shifts on group commuting}
\begin{equation}
t_\star(a)\circ {}_\star t(b)={}_\star t(b)\circ t_\star(a)
\EqLabel{shifts on group commuting}
\end{equation}
Equation \EqRef{shifts on group commuting}
coincides with equation
\EqRef{morphism of representations of F algebra, definition, 2}
from definition
\RefDefinition{morphism of representations of universal algebra}
when $r=id$, $R=t_\star(a)$.
\end{proof}

\begin{theorem}%
\labelTheorem{two representations of group}
Let \Ts{G}representation $f$
on $\Omega$\Hyph algebra $M$ be single transitive.
Then we can uniquely define a single transitive \sT{G}representation $h$
on $\Omega$\Hyph algebra $M$
such that diagram
\[
\xymatrix{
M\ar[rr]^{h(a)}\ar[d]^{f(b)} & & M\ar[d]^{f(b)}\\
M\ar[rr]_{h(a)}& &M
}
\]
is commutative for any $a$, $b\in G$.\,\footnote{You
can see this statement in \citeBib{Rashevsky}.}
\end{theorem}
\begin{proof}
We use group coordinates for points $v\in M$.
Then according to theorem \RefTheorem{single transitive representation of group}
we can write the left shift $t_\star(a)$ instead of the transformation $f(a)$.

Let $v_0, v\in M$. Then we can find
one and only one $a\in G$ such that
\[v=v_0 a=v_0\ {}_\star t(a) \]
We assume
\[h(a)=\ {}_\star t(a)\]
For some $b\in G$ we have
\[w_0=f(b)v_0=t_\star (b)v_0\ \ \ \ w=f(b)v=t_\star(b) v\]
According to the theorem \RefTheorem{shifts on group commuting}, the diagram
\begin{equation}
\xymatrix{
v_0\ar[rr]^{h(a)=\ {}_\star t(a)}\ar[d]^{f(b)=t_\star(b)}
& & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)=\ {}_\star t(a)}& &w
}
\label{Diagram: two representations of group}
\end{equation}
is commutative.

Changing $b$ we get that $w_0$ is an arbitrary point of $M$.

We see from the diagram that if $v_0=v$ then $w_0=w$ and therefore $h(e)=\delta$.
On other hand if $v_0\neq v$ then $w_0\neq w$ because
the \Ts{G}representation $f$ is single transitive.
Therefore the \sT{G}representation $h$ is effective.

In the same way we can show that for given $w_0$ we can find $a$
such that $w=h(a)w_0$. Therefore the \sT{G}representation $h$ is single transitive.

In general the product of transformations of
the \Ts{G}representation $f$ is not commutative and therefore
the \sT{G}representation $h$ is different from the \Ts{G}representation $f$.
In the same way we can create a \Ts{G}representation $f$ using the \sT{G}representation $h$.
\end{proof}

Representations $f$ and $h$ are called
\AddIndex{twin representations of the group}{twin representations of group} $G$.

\begin{remark}
\labelRemark{one representation of group}
It is clear that transformations $t_\star(a)$ and ${}_\star t(a)$
are different until the group $G$ is nonabelian.
However they both are maps onto.
Theorem \RefTheorem{two representations of group} states that if both
right and left shift presentations exist on the set $M$,
then we can define two commuting representations on the set $M$.
The right shift or the left shift only cannot represent both types of representation.
To understand why it is so let us change diagram \eqref{Diagram: two representations of group}
and assume $h(a)v_0=t_\star(a) v_0=v$
instead of $h(a)v_0=v_0{}_\star t(a)=v$ and let
us see what expression $h(a)$ has at
the point $w_0$. The diagram
\[\xymatrix{
v_0\ar[rr]^{h(a)=t_\star(a) }\ar[d]^{f(b)=t_\star(b)}
& & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)}& &w
}\]
is equivalent to the diagram
\[\xymatrix{
v_0\ar[rr]^{h(a)=t_\star(a)} & & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)}\ar[u]_{f^{-1}(b)=t_\star(b^{-1})}& &w
}\]
and we have $w=bv=bav_0=bab^{-1}w_0$. Therefore
\[h(a)w_0=(bab^{-1})w_0\] We see that the representation of $h$
depends on its argument.\qed  
%There is interesting question. If I have transformation $a\star$ in point $b$
%what is $c$ such that $a\star  b = R_c b$. We can find it from equation
%$ab=bc$, so $c=b^{-1}ab$, therefore
%\[a\star b = R_{b^{-1}ab} b\]?????
\end{remark}

\begin{theorem}%
\labelTheorem{twin representations of group, automorphism}
Let $f$ and $h$ be twin representations of the group $G$. For any $a\in G$ the map
$h(a)$ is automorphism of representation $f$.
\end{theorem}
\begin{proof}
The statement of theorem is corollary of theorems
\RefTheorem{shift is automorphism of representation} and
\RefTheorem{two representations of group}.
\end{proof}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{remark}
Is there a morphism of representations
from $t_\star$ to $t_\star$ different from automorphism $(\id,{}_\star t(a))$?
If we assume
\[
r(g)=cgc^{-1}
\]
\[
R(a)(m)=cmac^{-1}
\]
then it is easy to see that the map $(r,R(a))$ is
morphism of the representations from $t_\star$ to $t_\star$.
However this map is not
automorphism of the representation $t_\star$,
because $r\ne\id$.
\qed
\end{remark}
\fi


==> Group.Representation.Eq.tex <==
%auto-ignore

\DefEq
{
\symb{{}_\star t}{right shift}1
}
{right shift =}

\DefEquation
{
\begin{split}
b'&=b\ \ShowSymbol{right shift}1(a)=ba
\\
b'&=\ShowSymbol{right shift}1(a)(b)=ba
\end{split}
}
{right shift}

\DefEq
{
\[f(e)=\delta\]
}
{f(e)=}

\DefEquation
{
uf(ab)=(uf(a))f(b)
}
{right-side representation of group}

\DefEquation
{
f(ab)u=(f(a)f(b))u
}
{left-side representation of group, map product}

\DefEquation
{
f(ab)u=f(a)(f(b)u)
}
{left-side representation of group}

\DefEquation
{
uf(ab)=u(f(a)f(b))
}
{right-side representation of group, map product}

\DefEquation
{
u(f(a)f(b))=(uf(a))f(b)
}
{right-side representation of group, associativity}

\DefEquation
{
f:G\rightarrow {}^\star M
}
{left-side representation of group, map}

\DefEquation
{
f:G\rightarrow M^*
}
{right-side representation of group, map}

\DefEq
{
\[(f\circ g)x=f(gx)\]
}
{fg *M Tstar}

\DefEq
{
\[x(f\circ g)=(xf)g\]
}
{fg *M starT}

\DefEq
{
\symb[G-0]{G_x}0{little group}{}
\symb[G-0]{G_x}0{stability group}{}
\[
\ShowSymbol{little group}{}=\{g\in G:f(g)x=x\}
\]
}
{little group}

\DefEq
{
\symb{vG}{orbit of effective *G representation}{}
\[
\ShowSymbol{orbit of effective *G representation}{}
=v\ {}_\star t(G)
\]
}
{orbit of effective *G representation}

\DefEq
{
\symb{f(G)v}{orbit of representation}{}
\[
\ShowSymbol{orbit of representation}{}=\{w=f(g)v:g\in G\}
\]
}
{orbit of representation of group}

\DefEq
{
\symb{M/t_\star(G)}{space of orbits of effective G* representation}1
}
{space of orbits of effective G* representation}

\DefEq
{
\symb{M/{}_\star t(G)}{space of orbits of effective *G representation}1
}
{space of orbits of effective *G representation}

\DefEquation
{
(f(a)f(b))u=f(a)(f(b)u)
}
{left-side representation of group, associativity}

\DefEq
{
\symb{Gv}{orbit of effective G* representation}{}
\[
\ShowSymbol{orbit of effective G* representation}{}
=t_\star(G) v
\]
}
{orbit of effective G* representation}

\DefEq
{
\symb{t_\star}{left shift}1
}
{left shift =}

\DefEquation
{
\begin{split}
b'&=\ShowSymbol{left shift}1(a)b=ab
\\
b'&=\ShowSymbol{left shift}1(a)(b)=ab
\end{split}
}
{left shift}

\DefEquation
{
{}_\star t(ab)={}_\star t(a)\circ\ {}_\star t(b)
}
{right shift, product}

\DefEquation
{
t_\star(ab)=t_\star(a)\circ t_\star(b)
}
{left shift, product}



==> Group.Representation.Russian.tex <==
%auto-ignore
\input{Group.Representation.Eq}
\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\chapter{Представление группы}
\labelChapter{Representation of Group}
\fi

\section{Представление группы}
\labelSection{Representation of Group}

Группа - одна из немногих алгебр, которая позволяет рассматривать
произведение преобразований $\Omega$\Hyph алгебры $M$ таким образом, что если
преобразования принадлежат представлению, то их произведение также
принадлежит представлению.
При этом следует помнить, что порядок отображений при суперпозиции
зависит от порядка отображений на диаграмме и с какой стороны
отображения действуют на элементы множества.

\begin{definition}
\labelDefinition{left-side representation of group} 
Пусть ${}^*M$ - группа с произведением
\ShowEq{fg *M Tstar}
и $\delta$ - единица группы ${}^\star M$.
Пусть $G$ - группа.
Мы будем называть гомоморфизм групп
\ShowEq{left-side representation of group, map}
\AddIndex{левосторонним представлением}{left-side representation} группы $G$
или
\AddIndex{\Ts{G}представлением группы}{A* representation of algebra}
в $\Omega$\Hyph алгебре $M$, если отображение $f$ удовлетворяет условиям
\ShowEq{left-side representation of group}
\qed
\end{definition}

\begin{remark}
Поскольку отображение \EqRef{left-side representation of group, map}
- гомоморфизм, то
\ShowEq{left-side representation of group, map product}
Мы здесь пользуемся соглашением
\[
f(a)f(b)=f(a)\circ f(b)
\]
Таким образом, концепция представления групп состоит в том,
что в каком порядке мы перемножаем элементы группы,
в том же порядке перемножаются соответствующие преобразования представления.
Из равенств \EqRef{left-side representation of group}
и \EqRef{left-side representation of group, map product}
следует
\ShowEq{left-side representation of group, associativity}
Равенство
\EqRef{left-side representation of group, associativity}
совместно с ассоциативностью произведения преобразований
представляет собой
\AddIndex{закон ассоциативности}{associative law}
для \Ts{G}представления.
Это позволяет записывать равенство
\EqRef{left-side representation of group, associativity}
без использования скобок
\[
f(ab)u=f(a)f(b)u
\]
\qed
\end{remark}

\begin{definition}
\labelDefinition{right-side representation of group} 
Пусть $M^\star$ - группа с произведением
\ShowEq{fg *M starT}
и $\delta$ - единица группы $M^\star$.
Пусть $G$ - группа.
Мы будем называть гомоморфизм групп
\ShowEq{right-side representation of group, map}
\AddIndex{правосторонним представлением}{right-side representation} группы $G$
или
\AddIndex{\sT{G}представлением}{*A representation of algebra}
в $\Omega$\Hyph алгебре $M$, если отображение $f$ удовлетворяет условиям
\ShowEq{right-side representation of group}
\qed
\end{definition}

\begin{remark}
Поскольку отображение \EqRef{right-side representation of group, map}
- гомоморфизм, то
\ShowEq{right-side representation of group, map product}
Из равенств \EqRef{right-side representation of group}
и \EqRef{right-side representation of group, map product}
следует
\ShowEq{right-side representation of group, associativity}
Равенство
\EqRef{right-side representation of group, associativity}
совместно с ассоциативностью произведения преобразований
представляет собой
\AddIndex{закон ассоциативности}{associative law}
для \sT{G}представления.
Это позволяет записывать равенство
\EqRef{right-side representation of group, associativity}
без использования скобок
\[
uf(ab)=uf(a)f(b)
\]
\qed
\end{remark}

\begin{definition}
\labelDefinition{nonsingular transformation} 
Мы будем называть преобразование
\[
t:M\rightarrow M
\]
\AddIndex{невырожденным преобразованием}{nonsingular transformation},
если существует обратное отображение.
\qed
\end{definition}

\begin{theorem}
\labelTheorem{inverse transformation}
Для любого $g\in G$ преобразование $f(g)$ является
невырожденным и удовлетворяет равенству
\begin{equation}
\EqLabel{inverse transformation}
f(g^{-1})=f(g)^{-1}
\end{equation}
\end{theorem}
\begin{proof}
На основании \EqRef{left-side representation of group} и
\ShowEq{f(e)=}
мы можем записать
\[
u=\delta (u)=f(gg^{-1})(u)=f(g)(f(g^{-1})(u))
\]
Это завершает доказательство.
\end{proof}

\begin{theorem}
Групповая операция определяет два различных представления на группе:
\begin{itemize}
\item
\AddIndex{Левый сдвиг}{left shift}
\ShowEq{left shift =}
\ShowEq{left shift}
является \Ts{G}представлением на множестве\,\footnote{Левый сдвиг
не является представлением группы в группе,
так как преобразование $t_\star$ не является гомоморфизмом
группы.
Аналогичное замечание верно для правого сдвига.
} $G$
\ShowEq{left shift, product}
\item
\AddIndex{Правый сдвиг}{right shift}
\ShowEq{right shift =}
\ShowEq{right shift}
является \sT{G}представлением на множестве $G$
\ShowEq{right shift, product}
\end{itemize}
\end{theorem}
\begin{proof}
Равенство \EqRef{left shift, product}
следует из ассоциативности произведения
\[
t_\star(ab)c=(ab)c=a(bc)=t_\star(a)(t_\star(b)c)
=(t_\star(a)\circ t_\star(b))c
\]
Аналогично доказывается равенство \EqRef{right shift, product}.
\end{proof}

\begin{definition}
\labelDefinition{orbit of left-side representation of group}
Пусть $G$ - группа.
Пусть $f$ - \Ts{G}представление в $\Omega$\Hyph алгебре $M$.
Для любого $v\in M$ мы определим
\AddIndex{орбиту представления группы $G$}
{orbit of representation of group} как множество
\ShowEq{orbit of representation of group}
\qed
\end{definition}

Так как $f(e)=\delta$, то $v\in f(G)v$.

\begin{theorem}
\labelTheorem{proper definition of orbit}
Если
\begin{equation}
\EqLabel{orbit, proposition}
v\in f(G)u
\end{equation}
то
\[
f(G)u=f(G)v
\]
\end{theorem}
\begin{proof}
Из \EqRef{orbit, proposition} следует
существование $a\in G$ такого, что
\begin{equation}
v=f(a)u
\EqLabel{orbit, 1}
\end{equation}
Если $w\in f(G)v$, то
существует $b\in G$ такой, что
\begin{equation}
w=f(b)v
\EqLabel{orbit, 2}
\end{equation}
Подставив \EqRef{orbit, 1} в \EqRef{orbit, 2}, мы получим
\begin{equation}
w=f(b)(f(a)u)
\EqLabel{orbit, 3}
\end{equation}
На основании \EqRef{left-side representation of group}
из \EqRef{orbit, 3} следует,
что $w\in f(G)u$.
Таким образом,
\[
f(G)v\subseteq f(G)u
\]

На основании \EqRef{inverse transformation}
из \EqRef{orbit, 1} следует,
что
\begin{equation}
u=f(a)^{-1}v=f(a^{-1})v
\EqLabel{orbit, 4}
\end{equation}
Равенство \EqRef{orbit, 4} означает, что
$u\in f(G)v$ и, следовательно,
\[
f(G)u\subseteq f(G)v
\]
Это завершает доказательство.
\end{proof}

Таким образом, \Ts{G}представление $f$ в $\Omega$\Hyph алгебре $M$
порождает отношение эквивалентности $S$ и
орбита $f(G)u$ является классом эквивалентности.
Мы будем пользоваться обозначением
\symb{M/f(G)}{space of orbits of G* representation}1
для фактор множества $M/S$ и мы будем называть
это множество
\AddIndex{пространством орбит \Ts{G}представления}
{space of orbits of G* representation} $f$.

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{direct product of representations}
Если определены \Ts{G}представление $f_1$ в $\Omega$\Hyph алгебре $M_1$
и \Ts{G}представление $f_2$ в $\Omega$\Hyph алгебре $M_2$,
то мы можем определить
\AddIndex{прямое произведение \Ts{G}представлений}
{direct product of G* representations}
$f_1$ и $f_2$ группы
\begin{align*}
f&=f_1\times f_2:G\rightarrow M_1\otimes M_2\\
f(g)&=(f_1(g),f_2(g))
\end{align*}
\end{theorem}
\begin{proof}
Чтобы показать, что $f$ является представлением,
достаточно показать, что $f$ удовлетворяет определению
\RefDefinition{left-side representation of group}.
\[f(e)=(f_1(e),f_2(e))=(\delta_1,\delta_2)=\delta\]
\begin{align*}
f(ab)u&=(f_1(ab)u_1,f_2(ab)u_2)\\
&=(f_1(a)(f_1(b)u_1),f_2(a)(f_2(b)u_2))\\
&=f(a)(f_1(b)u_1,f_2(b)u_2)\\
&=f(a)(f(b)u)
\end{align*}
\end{proof}
\fi

\section{Однотранзитивное правостороннее представление группы}
\labelSection{Single Transitive Representation of Group}

\begin{definition}
\labelDefinition{kernel of inefficiency of representation of group}
Мы будем называть
\AddIndex{ядром неэффективности \Ts{G}представления}
{kernel of inefficiency of G* representation}
множество \[K_f=\{g\in G:f(g)=\delta\}\]
\qed
\end{definition}

\begin{theorem}
\labelTheorem{kernel of inefficiency, representation of group}
Ядро неэффективности \Ts{G}представления - это подгруппа группы $G$.
\end{theorem}
\begin{proof}
Допустим
$f(a_1)=\delta$ и $f(a_2)=\delta$. Тогда
\[f(a_1a_2)u=f(a_1)(f(a_2)u)=u\]
\[f(a^{-1})=f^{-1}(a)=\delta\]
\end{proof}

\begin{theorem}
\Ts{G}представление
\AddIndex{эффективно}{effective G* representation}
тогда и только тогда, когда ядро неэффективности $K_f=\{e\}$.
\end{theorem}
\begin{proof}
Утверждение является следствием определений
\RefDefinition{effective representation of algebra} и
\RefDefinition{kernel of inefficiency of representation of group} и
теоремы \RefTheorem{kernel of inefficiency, representation of group}.
\end{proof}

Если действие не эффективно, мы можем перейти к эффективному
заменив группой $G_1=G|K_f$,
пользуясь факторизацией по ядру неэффективности.
Это означает, что мы можем изучать только эффективное действие.

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{definition}
\labelDefinition{free representation of group}
Рассмотрим \Ts{G}представление $f$ в $\Omega$\Hyph алгебре $M$.
\AddIndex{Малая группа}{little group} или
\AddIndex{группа стабилизации}{stability group} элемента $x\in M$ -
это множество
\ShowEq{little group}

Мы будем называть \Ts{G}представление $f$
\AddIndex{свободным}{free representation of group},
если для любого $x\in M$ группа стабилизации $G_x=\{e\}$.
\qed
\end{definition}

\begin{theorem}%
\labelTheorem{free representation of group}
Если определено свободное \Ts{G}представление $f$ группы $G$ на $\Omega$\Hyph алгебре $A$,
то определено взаимно однозначное соответствие между орбитами представления,
а также между орбитой представления и группой $G$.
\end{theorem}
\begin{proof}
Допустим для точки $a\in A$
существуют $g_1$, $g_2\in G$
\begin{equation}
\EqLabel{free representation of group, 1}
f(g_1)a=f(g_2)a
\end{equation}
Умножим обе части равенства \EqRef{free representation of group, 1}
на $f(g_1^{-1})$
\[
a=f(g_1^{-1})f(g_2)a
\]
Поскольку представление свободное, $g_1=g_2$. Теорема доказана,
так как мы установили взаимно однозначное соответствие между
орбитой и группой $G$.
\end{proof}
\else

\begin{definition}
\labelDefinition{transitive representation of group}
Мы будем называть представление группы
\AddIndex{транзитивным}{transitive representation of group},
если для любых $a, b \in V$ существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление группы
\AddIndex{однотранзитивным}{single transitive representation of group},
если оно транзитивно и эффективно.
\qed
\end{definition}

\begin{theorem}%однотранзитивное
\Ts{G}представление однотранзитивно тогда и только тогда, когда для любых $a, b \in M$
существует одно и только одно $g\in G$ такое, что $a=f(g)(b)$
\end{theorem}
\begin{proof}
Следствие определений \RefDefinition{effective representation of algebra}
и \RefDefinition{transitive representation of group}.
\end{proof}
\fi

\begin{definition}
Мы будем называть пространство $V$
\AddIndex{однородным пространством}{homogeneous space} группы $G$,
если мы имеем однотранзитивное \Ts{G}представление на $V$.
\qed
\end{definition}

\begin{theorem}%
\labelTheorem{single transitive representation of group}
Если мы определим однотранзитивное
представление $f$ группы $G$ на $\Omega$\Hyph алгебре $A$,
то мы можем однозначно определить координаты на $A$, пользуясь координатами на группе $G$.

Если $f$ - левостороннее представление,
то $f(a)$ эквивалентно левому сдвигу $t_\star(a)$ на группе $G$.
Если $f$ - правостороннее представление, то $f(a)$ эквивалентно
правому сдвигу ${}_\star t(a)$ на группе $G$.
\end{theorem}
\begin{proof}
Мы выберем точку $v\in A$
и определим координаты точки $w\in A$
как координаты $a\in G$ такого, что $w=f(a) v$.
Координаты, определённые таким образом, однозначны
с точностью до выбора начальной точки $v\in A$,
так как действие эффективно.

Если $f$ - левостороннее представление,
мы будем пользоваться записью
\[f(a)v=av\]
Так как запись
\[f(a)(f(b)v)=a(bv)=(ab)v=f(ab)v\]
совместима с групповой структурой, мы видим, что
левостороннее представление $f$ эквивалентно левому сдвигу.

Если $f$ - правостороннее представление,
мы будем пользоваться записью
\[vf(a)=va\]
Так как запись
\[(vf(b))f(a)=(vb)a=v(ba)=vf(ba)\]
совместима с групповой структурой, мы видим, что
правостороннее представление $f$ эквивалентно правому сдвигу.
\end{proof}

\begin{remark}
Мы будем записывать эффективное
\Ts{G}представление в форме
\[v'=t_\star(a) v=av\]
Орбита этого представления имеет вид
\ShowEq{orbit of effective G* representation}
Мы будем пользоваться обозначением
\ShowEq{space of orbits of effective G* representation}
для пространства орбит эффективного \Ts{G}представления.
\qed
\end{remark}

\begin{remark}
Мы будем записывать эффективное
\sT{G}представление в форме
\[v'=v\ {}_\star t(a)=va\]
Орбита этого представления имеет вид
\ShowEq{orbit of effective *G representation}
Мы будем пользоваться обозначением
\ShowEq{space of orbits of effective *G representation}
для пространства орбит эффективного \sT{G}представления.
\qed
\end{remark}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{theorem}
\labelTheorem{Free representation is single transitive}
Свободное \Ts{G}представление эффективно.
Свободное \Ts{G}представление $f$ в $\Omega$\Hyph алгебре $M$
однотранзитивно на орбите.
\end{theorem}
\begin{proof}
Следствие определения
\RefDefinition{free representation of group}.
\end{proof}
\fi

\begin{theorem}%
\labelTheorem{shifts on group commuting}
Правый и левый сдвиги на группе $G$ перестановочны.
\end{theorem}
\begin{proof}
Это следствие ассоциативности группы $G$
\[(t_\star(a)\circ\ {}_\star t(b))c = a(cb)=(ac)b
=({}_\star t(b)\circ t_\star(a))c\]
\end{proof}

Теорема \RefTheorem{shifts on group commuting} может
быть сформулирована следующим образом.

\begin{theorem}%
\labelTheorem{shift is automorphism of representation}
Пусть $G$ - группа. Для любого $a\in G$ отображение
$t_\star(a)$ является автоморфизмом представления ${}_\star t$.
\end{theorem}
\begin{proof}
Согласно теореме
\RefTheorem{shifts on group commuting}
\begin{equation}
t_\star(a)\circ {}_\star t(b)={}_\star t(b)\circ t_\star(a)
\EqLabel{shifts on group commuting}
\end{equation}
Равенство \EqRef{shifts on group commuting}
совпадает с равенством
\EqRef{morphism of representations of F algebra, definition, 2}
из определения
\RefDefinition{morphism of representations of universal algebra}
при условии $r=id$, $R=t_\star(a)$.
\end{proof}

\begin{theorem}%
\labelTheorem{two representations of group}
Пусть \Ts{G}представление $f$
на $\Omega$\Hyph алгебре $M$ однотранзитивно.
Тогда мы можем однозначно определить однотранзитивное \sT{G}представление $h$
на $\Omega$\Hyph алгебре $M$
такое, что диаграмма
\[
\xymatrix{
M\ar[rr]^{h(a)}\ar[d]^{f(b)} & & M\ar[d]^{f(b)}\\
M\ar[rr]_{h(a)}& &M
}
\]
коммутативна для любых $a$, $b\in G$.\,\footnote{Это
утверждение можно также найти в \citeBib{Rashevsky}.}
\end{theorem}
\begin{proof}
Мы будем пользоваться групповыми координатами для точек $v\in M$.
Тогда согласно теореме \RefTheorem{single transitive representation of group}
мы можем записать левый сдвиг $t_\star(a)$ вместо преобразования $f(a)$.

Пусть $v_0, v\in M$. Тогда мы можем найти
одно и только одно $a\in G$ такое, что
\[v=v_0 a=v_0\ {}_\star t(a)\]
Мы предположим
\[h(a)=\ {}_\star t(a)\]
Существует $b\in G$ такое, что
\[w_0=f(b)v_0=t_\star (b)v_0\ \ \ \ w=f(b)v=t_\star(b) v\]
Согласно теореме \RefTheorem{shifts on group commuting} диаграмма
\begin{equation}
\xymatrix{
v_0\ar[rr]^{h(a)=\ {}_\star t(a)}\ar[d]^{f(b)=t_\star(b)}
& & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)=\ {}_\star t(a)}& &w
}
\label{Diagram: two representations of group}
\end{equation}
коммутативна.

Изменяя $b$ мы получим, что $w_0$ - это произвольная точка, принадлежащая $M$.

Мы видим из диаграммы, что, если $v_0=v$, то $w_0=w$ и следовательно $h(e)=\delta$.
С другой стороны, если $v_0\neq v$, то $w_0\neq w$ потому, что
\Ts{G}представление $f$ однотранзитивно.
Следовательно \sT{G}представление $h$ эффективно.

Таким же образам мы можем показать, что для данного $w_0$ мы можем найти $a$
такое, что $w=h(a)w_0$. Следовательно \sT{G}представление $h$ однотранзитивно.

В общем случае, произведение преобразований \Ts{G}представления $f$
не коммутативно и следовательно
\sT{G}представление $h$ отлично от \Ts{G}представления $f$.
Таким же образом мы можем создать \Ts{G}представление $f$, пользуясь \sT{G}представлением $h$.
\end{proof}

Мы будем называть представления $f$ и $h$
\AddIndex{парными представлениями группы}{twin representations of group} $G$.

\begin{remark}
\labelRemark{one representation of group}
Очевидно, что преобразования $t_\star(a)$ и ${}_\star t(a)$
отличаются, если группа $G$ неабелева.
Тем не менее, они являются отображениями на.
Теорема \RefTheorem{two representations of group} утверждает, что, если оба
представления правого и левого сдвига существуют на множестве $M$,
то мы можем определить два перестановочных представления на множестве $M$.
Только правый или левый сдвиг не может представлять оба типа представления.
Чтобы понять почему это так, мы можем изменить диаграмму \eqref{Diagram: two representations of group}
и предположить $h(a)v_0=t_\star(a) v_0=v$
вместо $h(a)v_0=v_0{}_\star t(a)=v$ и
проанализировать, какое выражение $h(a)$ имеет в
точке $w_0$. Диаграмма
\[\xymatrix{
v_0\ar[rr]^{h(a)=t_\star(a)}\ar[d]^{f(b)=t_\star(b)}
& & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)}& &w
}\]
эквивалентна диаграмме
\[\xymatrix{
v_0\ar[rr]^{h(a)=t_\star(a)} & & v\ar[d]^{f(b)=t_\star(b)}\\
w_0\ar[rr]_{h(a)}\ar[u]_{f^{-1}(b)=t_\star(b^{-1})}& &w
}\]
и мы имеем $w=bv=bav_0=bab^{-1}w_0$. Следовательно
\[h(a)w_0=(bab^{-1})w_0\] Мы видим, что представление $h$
зависит от его аргумента.\qed  
%There is interesting question. Если I имею преобразование $a\star$ in точке $b$
%what is $c$ такое, что $a\star b = R_c b$. Мы можем find it из равенства
%$ab=bc$, so $c=b^{-1}ab$, следовательно
%\[a\star b = R_{b^{-1}ab} b\]?????
\end{remark}

\begin{theorem}%
\labelTheorem{twin representations of group, automorphism}
Пусть $f$ и $h$ - парные преставления группы $G$. Для любого $a\in G$ отображение
$h(a)$ является автоморфизмом представления $f$.
\end{theorem}
\begin{proof}
Следствие теорем
\RefTheorem{shift is automorphism of representation} и
\RefTheorem{two representations of group}.
\end{proof}

\ePrints{4776-3181}
\ifx\Semafor\ValueOff
\begin{remark}
Существует ли морфизм представлений
из $t_\star$ в $t_\star$, отличный от автоморфизма $(\id,{}_\star t(a))$?
Если мы положим
\[
r(g)=cgc^{-1}
\]
\[
R(a)(m)=cmac^{-1}
\]
то нетрудно убедиться, что отображение $(r,R(a))$ является
морфизмом представлений из $t_\star$ в $t_\star$.
Но это отображение не является
автоморфизмом представления $t_\star$,
так как $r\ne\id$.
\qed
\end{remark}
\fi


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%202%*%*D вектор строка
   {$*D$\Hyph вектор строка}%
   {row *D vector}%
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) map}%
\Index%660%A%A*- модуль
   {$A*$\Hyph модуль}%
   {A*-module}%
\Index%575%A%A*-векторное пространство
   {$A*$\Hyph векторное пространство}%
   {A*-vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%15%A%A-векторное пространство
   {$A$\hyph векторное пространство}%
   {A vector space}%
\Index%864%A%A-представление в Omega алгебре
   {$A$\Hyph представление в $\Omega$\Hyph алгебре}%
   {A representation of algebra}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%705%C%cr вырожденная матрица
   {\CR вырожденная матрица}%
   {cr singular matrix}%
\Index%954%C%cr квазидетерминант
   {\CR квазидетерминант}%
   {cr-quasideterminant}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%956%C%cr невырожденная матрица
   {\CR невырожденная матрица}%
   {cr nonsingular matrix}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение
   {\CR произведение (произведение столбца на строку)}%
   {cr-product}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%949%C%CR экспонента
   {\CR экспонента}%
   {CR exponent}%
\Index%304%C%crd вектор
   {\crd вектор}%
   {crd vector}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%134%C%cr-обратная матрица
   {\CR обратная матрица}%
   {cr-inverse matrix}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%92%D%D* вектор столбец
   {$D*$\Hyph вектор столбец}%
   {column D* vector}%
\Index%93%D%D* вектор строка
   {$D*$\Hyph вектор строка}%
   {row D* vector}%
\Index%87%D%D*- векторное пространство матриц
   {$D*$\hyph векторное пространство матриц}%
   {matrices vector space}%
\Index%40%D%D*-векторное пространство
   {$D*$\hyph векторное пространство}%
   {D* vector space}%
\Index%156%D%D*-модуль
   {$D*$\Hyph модуль}%
   {D*-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%200%D%drc вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\Index%845%N%n-арная операция на множестве
   {$n$\Hyph арная операция на множестве}%
   {n-ary operation on set}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(\aUD{}ji)$\hyph \RC квазидетерминант}%
   {j i rc-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%rc вырожденная матрица
   {\RC вырожденная матрица}%
   {rc singular matrix}%
\Index%62%R%rc квазидетерминант
   {\RC квазидетерминант}%
   {rc-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%rc невырожденная матрица
   {\RC невырожденная матрица}%
   {r? nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение
   {\RC произведение (произведение строки на столбец)}%
   {rc-product}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%948%R%RC экспонента
   {\RC экспонента}%
   {RC exponent}%
\Index%600%R%RCcirc вырожденная матрица
   {$\RCcirc$\Hyph вырожденная матрица}%
   {RCcirc singular matrix}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица
   {$\RCcirc$\Hyph невырожденная матрица}%
   {RCcirc nonsingular matrix}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%218%R%rc-обратная матрица
   {\RC обратная матрица}%
   {rc-inverse matrix}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%185%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%187%T%Tstar- представление расслоенной группы
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%830%А%абелевая мультипликативная Omega группа
   {абелевая мультипликативная $\Omega$\Hyph группа}%
   {Abelian multiplicative Omega group}%
\Index%869%А%абелевая полугруппа
   {абелевая полугруппа}%
   {Abelian semigroup}%
\Index%284%А%абсолютная величина
   {абсолютная величина}%
   {absolute value}%
\Index%859%А%автоморфизм
   {автоморфизм}%
   {automorphism}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%22%А%автоморфизм векторного пространства
   {автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%939%А%автоморфизм диаграммы представлений
   {автоморфизм диаграммы представлений}%
   {automorphism of diagram of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное *G представление
   {активное \sT{G}представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%569%А%активное представление в многообразии базисов
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов
   {активное преобразование многообразия базисов}%
   {active transformation of basis}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%741%А%алгебра кватернионов
   {алгебра кватернионов}%
   {quaternion algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%167%А%алгебра с делением
   {алгебра с делением}%
   {division algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%907%А%альтернация полилинейного отображения
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
\Index%779%А%антилинейное отображение
   {антилинейное отображение}%
   {antilinear map}%
\Index%929%А%антилинейный гомоморфизм
   {антилинейный гомоморфизм}%
   {antilinear homomorphism}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%849%А%арность
   {арность}%
   {arity}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%89%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%943%А%ассоциативная мультипликативная Omega группа
   {ассоциативная мультипликативная $\Omega$\Hyph группа}%
   {associative multiplicative Omega group}%
\Index%866%А%ассоциативная операция
   {ассоциативная операция}%
   {associative operation}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%759%А%аффинная плоскость
   {аффинная плоскость}%
   {affine plane}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%736%А%аффинное пространство столбцов
   {аффинное пространство столбцов}%
   {affine space of columns}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%579%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%115%Б%базис
   {базис}%
   {Basis}%
\Index%203%Б%базис crd векторного пространства
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
\Index%106%Б%базис dcr векторного пространства
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
\Index%16%Б%базис drc векторного пространства
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
\Index%24%Б%базис rcd векторного пространства
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%26%Б%базис в векторном расслоении
   {базис в векторном расслоении}%
   {basis, vector bundle}%
\Index%197%Б%базис векторного пространства
   {базис векторного пространства}%
   {basis, vector space}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%699%Б%базис диаграммы представлений
   {базис диаграммы представлений}%
   {basis of diagram of representations}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Omega$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%901%В%вектор
   {вектор}%
   {vector}%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%192%В%векторное *A-пространство
   {векторное $*A$\Hyph пространство}%
   {*A-vector space}%
\Index%976%В%векторное подпространство
   {векторное подпространство}%
   {subspace}%
\Index%727%В%векторное пространство
   {векторное пространство}%
   {vector space}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\Hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%398%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%687%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%33%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%481%В%взаимно простые  A числа
   {взаимно простые  $A$\Hyph числа}%
   {relatively prime A numbers}%
\Index%908%В%внешнее произведение
   {внешнее произведение}%
   {exterior product}%
\Index%508%В%внешний дифференциал
   {внешний дифференциал}%
   {exterior differential}%
\Index%163%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%231%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%70%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%781%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\Index%675%В%вырожденный тензор
   {вырожденный тензор}%
   {singular tensor}%
\Index%723%В%вырожденный эндоморфизм
   {вырожденный эндоморфизм}%
   {singular endomorphism}%
\SetIndexSpace%
\Index%871%Г%геодезический эффект
   {геодезический эффект}%
   {geodetic effect}%
\Index%700%Г%геометрический объект
   {геометрический объект}%
   {geometric object}%
\Index%838%Г%гиперболический косинус
   {гиперболический косинус}%
   {hyperbolic cosine}%
\Index%837%Г%гиперболический синус
   {гиперболический синус}%
   {hyperbolic sine}%
\Index%61%Г%главная подматрица
   {главная подматрица}%
   {major submatrix}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%885%Г%голоморфное отображение
   {голоморфное отображение}%
   {holomorphic map}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%854%Г%гомоморфизм
   {гомоморфизм}%
   {homomorphism}%
\Index%959%Г%гомоморфизм векторного пространства
   {гомоморфизм векторного пространства}%
   {homomorphism of vector space}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%861%Г%гомоморфный образ
   {гомоморфный образ}%
   {homomorphic image}%
\Index%73%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%686%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%765%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%613%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%865%Д%декартова степень
   {декартова степень}%
   {Cartesian power}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%655%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%390%Д%декартово произведение групп
   {декартово произведение групп}%
   {Cartesian product of groups}%
\Index%199%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%625%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%825%Д%декартово произведением Omega алгебр
   {декартово произведением \(\Omega\)\Hyph алгебр}%
   {Cartesian product of Omega algebras}%
\Index%598%Д%деление без остатка
   {деление без остатка}%
   {division without remainder}%
\Index%573%Д%деление с остатком
   {деление с остатком}%
   {division with remainder}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%935%Д%диаграмма представлений универсальных алгебр
   {диаграмма представлений универсальных алгебр}%
   {diagram of representations of algebras}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%983%Д%диффеоморфизм
   {диффеоморфизм}%
   {diffeomorphism}%
\Index%661%Д%дифференциал независимой переменной
   {дифференциал независимой переменной}%
   {differential of independent variable}%
\Index%157%Д%дифференциал отображения
   {дифференциал отображения}%
   {differential of map}%
\Index%902%Д%дифференциальная p форма
   {дифференциальная $p$\Hyph форма}%
   {differential p form}%
\Index%737%Д%дифференциальная форма степени p
   {дифференциальная форма степени $p$}%
   {differential form of degree p}%
\Index%550%Д%дифференциальное многообразие
   {дифференциальное $B$\Hyph многообразие}%
   {differential manifold}%
\Index%919%Д%дифференциальное уравнение с разделёнными переменными
   {дифференциальное уравнение с разделёнными переменными}%
   {differential equation with separated variables}%
\Index%922%Д%дифференциальное уравнение с разделяющимися переменными
   {дифференциальное уравнение с разделяющимися переменными}%
   {differential separable equation}%
\Index%877%Д%дифференцируемое отображение
   {дифференцируемое отображение}%
   {differentiable map}%
\Index%78%Д%долгота
   {долгота}%
   {longitude}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%44%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\Index%875%Е%естественный гомоморфизм
   {естественный гомоморфизм}%
   {natural homomorphism}%
\SetIndexSpace%
\Index%662%З%закон ассоциативности
   {закон ассоциативности}%
   {associative law}%
\Index%672%З%закон дистрибутивности
   {закон дистрибутивности}%
   {distributive law}%
\Index%964%З%закон коммутативности
   {закон коммутативности}%
   {commutative law}%
\Index%701%З%закон сокращения
   {закон сокращения}%
   {cancellation law}%
\Index%673%З%закон унитарности
   {закон унитарности}%
   {unitarity law}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%80%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\Index%261%З%звёздное множество
   {звёздное множество}%
   {starlike set}%
\SetIndexSpace%
\Index%971%И%идеал
   {идеал}%
   {ideal}%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%164%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%855%И%изоморфизм
   {изоморфизм}%
   {isomorphism}%
\Index%31%И%изоморфизм векторных пространств
   {изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%385%И%индукция по диаграмме представлений
   {индукция по диаграмме представлений}%
   {induction over diagram of representations}%
\Index%257%И%интеграл дифференциальной 1 формы вдоль пути
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
\Index%680%И%интеграл Лебега
   {интеграл Лебега}%
   {Lebesgue integral}%
\Index%438%И%интегрируемая дифференциальная форма
   {интегрируемая дифференциальная форма}%
   {integrable differential form}%
\Index%111%И%интегрируемая форма
   {интегрируемая форма}%
   {integrable form}%
\Index%918%И%интегрируемое дифференциальное уравнение
   {интегрируемое дифференциальное уравнение}%
   {integrable differential equation}%
\Index%693%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%368%К%каноническое отображение
   {каноническое отображение}%
   {canonical map}%
\Index%913%К%каноническое отображение
   {каноническое отображение}%
   {canonical map}%
\Index%599%К%каноническое представление деления с остатком
   {каноническое представление деления с остатком}%
   {canonical representation of division with remainder}%
\Index%726%К%каноническое частное от деления
   {каноническое частное от деления}%
   {canonical remainder of the division}%
\Index%981%К%карта
   {карта}%
   {chart}%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%177%К%категория левосторонних представлений
   {категория левосторонних представлений}%
   {category of left-side representations}%
\Index%176%К%категория левосторонних представлений Omega1 алгебры A
   {категория левосторонних представлений $\Omega$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
\Index%887%К%категория представлений
   {категория представлений}%
   {category of representations}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%842%К%квадратное уравнение
   {квадратное уравнение}%
   {quadratic equation}%
\Index%841%К%квадратный корень
   {квадратный корень}%
   {square root}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%535%К%квазибазис
   {квазибазис}%
   {quasibasis}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of maps}%
\Index%962%К%квазиэкспонента
   {квазиэкспонента}%
   {quasiexponent}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%969%К%ковариантное представление
   {ковариантное представление}%
   {covariant representation}%
\Index%258%К%колинеарные векторы
   {колинеарные векторы}%
   {colinear vectors}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%577%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%936%К%коммутативная диаграмма представлений универсальных алгебр
   {коммутативная диаграмма представлений универсальных алгебр}%
   {commutative diagram of representations}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%867%К%коммутативная операция
   {коммутативная операция}%
   {commutative operation}%
\Index%832%К%коммутативность представлений
   {коммутативность представлений}%
   {commutativity of representations}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%879%К%компонента производной
   {компонента производной}%
   {component of derivative}%
\Index%883%К%компонента производной второго порядка
   {компонента производной второго порядка}%
   {component of derivative of Second Order}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%873%К%конгруенция
   {конгруенция}%
   {congruence}%
\Index%170%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%968%К%контравариантное представление
   {контравариантное представление}%
   {contravariant representation}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%210%К%координатное векторное расслоение
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
\Index%697%К%координатное представление
   {координатное представление}%
   {coordinate representation}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%664%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%738%К%координаты
   {координаты}%
   {coordinates}%
\Index%558%К%координаты A числа относительно множества
   {координаты $A_2$\Hyph числа $m$ относительно множества $X$}%
   {coordinates relative to set}%
\Index%927%К%координаты ассоциатора
   {координаты ассоциатора}%
   {coordinates of associator}%
\Index%25%К%координаты базиса
   {координаты базиса}%
   {coordinates of basis}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%221%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
\Index%974%К%координаты гомоморфизма
   {координаты гомоморфизма}%
   {coordinates of homomorphism}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%967%К%координаты морфизма диаграммы представлений
   {координаты морфизма диаграммы представлений}%
   {coordinates of morphism, diagram of representations}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%945%К%координаты приведенного морфизма представления
   {координаты приведенного морфизма представления}%
   {coordinates of reduced morphism of representation}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%910%К%копроизведение в категории
   {копроизведение в категории}%
   {coproduct in category}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%941%К%кортеж Omega слов
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%533%К%кортеж стабильных множеств диаграммы представлений
   {кортеж стабильных множеств диаграммы представлений}%
   {tuple of stable sets of diagram of representations}%
\Index%840%К%косинус
   {косинус}%
   {cosine}%
\Index%904%К%косо симметричное полилинейное отображение
   {косо симметричное полилинейное отображение}%
   {skew symmetric polylinear map}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в аффинном пространстве}%
   {connection coefficients, affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%166%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%950%Л%левая линейная комбинация
   {левая линейная комбинация}%
   {left linear combination}%
\Index%896%Л%левое A векторное пространство
   {левое $A$\Hyph векторное пространство}%
   {left A vector space}%
\Index%585%Л%левое D векторное пространство столбцов
   {левое $D$\hyph векторное пространство столбцов}%
   {left vector space of columns}%
\Index%576%Л%левое D векторное пространство строк
   {левое $D$\hyph векторное пространство строк}%
   {left vector space of rows}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%952%Л%левое пространство A-столбцов
   {левое пространство $A$\Hyph столбцов}%
   {left A-column space}%
\Index%955%Л%левое пространство A-строк
   {левое пространство $A$\Hyph строк}%
   {left A-row space}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%899%Л%левостороннее A представление
   {левостороннее $A_1$\Hyph представление}%
   {left-side A representation}%
\Index%184%Л%левостороннее представление
   {левостороннее представление}%
   {left-side representation}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%892%Л%левостороннее произведение
   {левостороннее произведение}%
   {left-side product}%
\Index%665%Л%левостороннее произведение вектора на скаляр
   {левостороннее произведение вектора на скаляр}%
   {left-side product of vector over scalar}%
\Index%271%Л%левостороннее произведение отображения на скаляр
   {левостороннее произведение отображения на скаляр}%
   {left-side product of map over scalar}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%895%Л%левый A модуль
   {левый $A$\Hyph модуль}%
   {left A module}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%975%Л%левый идеал
   {левый идеал}%
   {left ideal}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%731%Л%левый сдвиг модуля
   {левый сдвиг модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {left shift, fibered group}%
\Index%973%Л%левый смежный класс
   {левый смежный класс}%
   {left coset}%
\Index%88%Л%линейная комбинация
   {линейная комбинация}%
   {linear combination}%
\Index%32%Л%линейная оболочка
   {линейная оболочка}%
   {linear span, vector space}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%21%Л%линейно зависимое множество
   {линейно зависимое множество}%
   {linearly dependent set}%
\Index%136%Л%линейно зависимы слева
   {линейно зависимы слева}%
   {left linear dependent}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%833%Л%линейно зависимый
   {линейно зависимый}%
   {linearly dependent}%
\Index%34%Л%линейно независимое множество
   {линейно независимое множество}%
   {linearly independent set}%
\Index%37%Л%линейное G* представление
   {линейное \Ts{G}представление}%
   {linear G* representation}%
\Index%921%Л%линейное однородное уравнение
   {линейное однородное уравнение}%
   {linear homogeneous equation}%
\Index%35%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%735%Л%линейное преобразование аффинного пространства
   {линейное преобразование аффинного пространства}%
   {linear transformation, affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%769%Л%линейный гомоморфизм
   {линейный гомоморфизм}%
   {linear homomorphism}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%894%М%матрица
   {матрица}%
   {matrix}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%255%М%матрица Вронского
   {матрица Вронского}%
   {Wronskian matrix}%
\Index%958%М%матрица гомоморфизма
   {матрица гомоморфизма}%
   {matrix of homomorphism}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear maps}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of maps}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%890%М%матрица Якоби отображения
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
\Index%161%М%мера
   {мера}%
   {measure}%
\Index%165%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%835%М%метод последовательного дифференцирования
   {метод последовательного дифференцирования}%
   {method of successive differentiation}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%536%М%многообразие базисов
   {многообразие базисов}%
   {basis manifold}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%847%М%множество допускает операцию
   {множество допускает операцию}%
   {set admits operation}%
\Index%846%М%множество замкнуто относительно операции
   {множество замкнуто относительно операции}%
   {set is closed with respect to operation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%942%М%множество кортежей Omega слов
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%715%М%множество кортежей координат диаграммы представлений
   {множество кортежей координат диаграммы представлений}%
   {coordinate set of diagram of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%332%М%множество образующих
   {множество образующих}%
   {generating set}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%356%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%860%М%может быть вложена
   {может быть вложена}%
   {can be embeded}%
\Index%856%М%мономорфизм
   {мономорфизм}%
   {monomorphism}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни представлений в башню представлений
   {морфизм из башни представлений в башню представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%698%М%морфизм из диаграммы представлений в диаграмму представлений
   {морфизм из диаграммы представлений в диаграмму представлений}%
   {morphism from diagram of representations into diagram of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%828%М%мультипликативная Omega группа
   {мультипликативная $\Omega$\Hyph группа}%
   {multiplicative Omega group}%
\Index%829%М%мультипликативное отображение
   {мультипликативное отображение}%
   {multiplicative map}%
\Index%85%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%207%Н%наибольший общий делитель
   {наибольший общий делитель}%
   {highest common factor}%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система линейных уравнений
   {невырожденная система линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%219%Н%невырожденная система правых AU* линейных уравнений
   {невырожденная система правых $A^*$\Hyph линейных уравнений}%
   {nonsingular system of right AU* linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм
   {невырожденный эндоморфизм}%
   {regular endomorphism}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%29%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%870%Н%нейтральный элемент операции
   {нейтральный элемент операции}%
   {neutral element of operation}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%834%Н%неопределённый интеграл
   {неопределённый интеграл}%
   {indefinite integral}%
\Index%460%Н%непрерывная матрица
   {непрерывная матрица}%
   {continuous matrix}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%960%Н%непрерывный базис Шаудера
   {непрерывный базис Шаудера}%
   {continuous Schauder basis}%
\Index%978%Н%непрерывный квазибазис Шаудера
   {непрерывный квазибазис Шаудера}%
   {continuous Schauder quasi-basis}%
\Index%641%Н%норма
   {норма}%
   {norm}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%928%Н%норма октониона
   {норма октониона}%
   {norm of octonion}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%702%Н%нормальная подгруппа
   {нормальная подгруппа}%
   {normal subgroup}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%977%Н%нормированная группа
   {нормированная группа}%
   {normed group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%979%Н%нормированное Omega кольцо
   {нормированное $\Omega$\Hyph кольцо}%
   {normed Omega ring}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\Index%364%Н%нормированный модуль
   {нормированный модуль}%
   {normed module}%
\Index%852%Н%носитель Omega-алгебры
   {носитель $\Omega$\Hyph алгебры}%
   {carrier of Omega-algebra}%
\SetIndexSpace%
\Index%848%О%область операторов
   {область операторов}%
   {operator domain}%
\Index%970%О%образ отображения
   {образ отображения}%
   {image of map}%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%482%О%общий делитель
   {общий делитель}%
   {common factor}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство
   {однородное пространство}%
   {homogeneous space}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен
   {однородный многочлен}%
   {homogeneous polynomial}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%844%О%операция на множестве
   {операция на множестве}%
   {operation on set}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%740%О%определённый интеграл
   {определённый интеграл}%
   {definite integral}%
\Index%212%О%определитель Вронского
   {определитель Вронского}%
   {Wronskian determinant}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear map}%
\Index%893%О%орбита представления
   {орбита представления}%
   {orbit of representation}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%484%О%остаток от деления
   {остаток от деления}%
   {remainder of the division}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%931%О%отношение эквивалентности
   {отношение эквивалентности}%
   {equivalence}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%886%О%отображение согласовано с операцией
   {отображение согласовано с операцией}%
   {map is compatible with operation}%
\Index%876%О%отображение сопряжения
   {отображение сопряжения}%
   {map of conjugation}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг аффинного пространства
   {параллельный сдвиг аффинного пространства}%
   {parallel shift, affine space}%
\Index%587%П%парные представления
   {парные представления}%
   {twin representations}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное G-представление
   {пассивное $G$\Hyph представление}%
   {passive G representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%695%П%пассивное представление в многообразии базисов
   {пассивное представление в многообразии базисов}%
   {passive representation in basis manifold}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%336%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation, vector space}%
\Index%570%П%пассивное преобразование многообразия базисов
   {пассивное преобразование многообразия базисов}%
   {passive transformation of basis}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%963%П%первый интеграл
   {первый интеграл}%
   {first integral}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%863%П%перестановка
   {перестановка}%
   {permutation}%
\Index%853%П%подалгебра Omega-алгебры
   {подалгебра $\Omega$\Hyph алгебры}%
   {subalgebra of Omega-algebra}%
\Index%230%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%909%П%подмодуль
   {подмодуль}%
   {submodule}%
\Index%940%П%подпредставление
   {подпредставление}%
   {subrepresentation}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%345%П%полилинейное косо симметричное отображение
   {полилинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%764%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%980%П%полное Omega кольцо
   {полное $\Omega$\Hyph кольцо}%
   {complete Omega ring}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%868%П%полугруппа
   {полугруппа}%
   {semigroup}%
\Index%169%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%186%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%19%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%578%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%953%П%правая линейная комбинация
   {правая линейная комбинация}%
   {right linear combination}%
\Index%961%П%правое A subs векторное пространство
   {правое $A_*$\Hyph векторное пространство}%
   {right A subs vector space}%
\Index%898%П%правое A векторное пространство
   {правое $A$\Hyph векторное пространство}%
   {right A vector space}%
\Index%671%П%правое D векторное пространство столбцов
   {правое $D$\hyph векторное пространство столбцов}%
   {right vector space of columns}%
\Index%654%П%правое D векторное пространство строк
   {правое $D$\hyph векторное пространство строк}%
   {right vector space of rows}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%951%П%правое пространство A-столбцов
   {правое пространство $A$\Hyph столбцов}%
   {right A-column space}%
\Index%957%П%правое пространство A-строк
   {правое пространство $A$\Hyph строк}%
   {right A-row space}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%900%П%правостороннее A представление
   {правостороннее $A_1$\Hyph представление}%
   {right-side A representation}%
\Index%355%П%правостороннее представление
   {правостороннее представление}%
   {right-side representation}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%891%П%правостороннее произведение
   {правостороннее произведение}%
   {right-side product}%
\Index%674%П%правостороннее произведение вектора на скаляр
   {правостороннее произведение вектора на скаляр}%
   {right-side product of vector over scalar}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%897%П%правый D модуль
   {правый $D$\Hyph модуль}%
   {right D module}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%912%П%правый идеал
   {правый идеал}%
   {right ideal}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%704%П%правый смежный класс
   {правый смежный класс}%
   {right coset}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%703%П%представитель геометрического объекта
   {представитель геометрического объекта}%
   {representative of geometric object}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%82%П%представление Omega1 алгебры A в Omega2 алгебре *A
   {\sT{A}представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре}%
   {*A representation of algebra}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%90%П%представление в Omega2- алгебре A*
   {\Ts{A}представление в $\Omega_2$\Hyph алгебре}%
   {A* representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%719%П%преобразование подобия
   {преобразование подобия}%
   {similarity transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%23%П%преобразование сопряжения
   {преобразование сопряжения}%
   {conjugation transformation}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%843%П%приведенное квадратное уравнение
   {приведенное квадратное уравнение}%
   {reduced quadratic equation}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%831%П%приведенный морфизм представлений
   {приведенный морфизм представлений}%
   {reduced morphism of representations}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%384%П%принцип ковариантности
   {принцип ковариантности}%
   {principle of covariance}%
\Index%162%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%395%П%произведение в категории
   {произведение в категории}%
   {product in category}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%133%П%произведение гомоморфизмов
   {произведение гомоморфизмов}%
   {product of homomorphisms}%
\Index%663%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%172%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%937%П%произведение морфизмов диаграммы представлений
   {произведение морфизмов диаграммы представлений}%
   {product of morphisms of diagram of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%882%П%производная Гато второго порядка
   {производная второго порядка}%
   {derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%878%П%производная отображения
   {производная отображения}%
   {derivative of map}%
\Index%884%П%производная порядка n
   {производная порядка $n$}%
   {derivative of Order n}%
\Index%483%П%простое A число
   {простое $A$\Hyph число}%
   {prime A number}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит G* представления
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
\Index%684%П%пространство орбит левостороннего представления
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%911%П%прямая сумма
   {прямая сумма}%
   {direct sum}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%412%П%прямое произведение G* представлений
   {прямое произведение \Ts{G}представлений}%
   {direct product of G* representations}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%826%П%прямое произведением Omega алгебр
   {прямое произведением \(\Omega\)\Hyph алгебр}%
   {direct product of Omega algebras}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%67%Р%ранг матрицы
   {ранг матрицы}%
   {rank of matrix}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный изоморфизм}%
   {fibered coordinate isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица
   {расширенная матрица}%
   {augmented matrix}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%932%Р%рефлексивное соответствие
   {рефлексивное соответствие}%
   {reflexive correspondence}%
\Index%782%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%331%С%свободная абелевая группа
   {свободная абелевая группа}%
   {free Abelian group}%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%862%С%свободное представление
   {свободное представление}%
   {free representation}%
\Index%441%С%свободное представление группы
   {свободное представление группы}%
   {free representation of group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль
   {свободный модуль}%
   {free module}%
\Index%517%С%связное множество
   {связное множество}%
   {connected set}%
\Index%549%С%связность
   {связность}%
   {connection}%
\Index%583%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%906%С%симметрирование полилинейного отображения
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение
   {симметричное билинейное отображение}%
   {symmetric bilinear map}%
\Index%903%С%симметричное полилинейное отображение
   {симметричное полилинейное отображение}%
   {symmetric polylinear map}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%933%С%симметричное соответствие
   {симметричное соответствие}%
   {symmetric correspondence}%
\Index%214%С%симплекс
   {симплекс}%
   {simplex}%
\Index%839%С%синус
   {синус}%
   {sine}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%220%С%система левых AD* линейных уравнений
   {система левых $A_*$\Hyph линейных уравнений}%
   {system of left AD* linear equations}%
\Index%201%С%система линейных уравнений
   {система линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%721%С%система правых AU* линейных уравнений
   {система правых $A^*$\Hyph линейных уравнений}%
   {system of right AU* linear equations}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%965%С%собственная строка
   {собственная строка}%
   {eigenrow}%
\Index%946%С%собственное значение
   {собственное значение}%
   {eigenvalue}%
\Index%966%С%собственный вектор
   {собственный вектор}%
   {eigenvector}%
\Index%947%С%собственный столбец
   {собственный столбец}%
   {eigencolumn}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%683%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%789%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%881%С%стандартная компонента производной
   {стандартная компонента производной}%
   {standard component of derivative}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%880%С%стандартное представление производной
   {стандартное представление производной}%
   {derivative, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%171%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%283%С%столбец непрерывной матрицы
   {столбец непрерывной матрицы}%
   {column of continuous matrix}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%346%С%строка непрерывной матрицы
   {строка непрерывной матрицы}%
   {row of continuous matrix}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%351%С%сумма отображений
   {сумма отображений}%
   {sum of maps}%
\Index%323%С%суперпозиция координат
   {суперпозиция координат}%
   {superposition of coordinates,}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\Index%168%С%сферические координаты
   {сферические координаты}%
   {spherical coordinates}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение
   {тензорное произведение}%
   {tensor product}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%135%Т%тип геометрического объекта
   {тип геометрического объекта}%
   {type of geometric object}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%724%Т%точная последовательность
   {точная последовательность}%
   {exact sequence}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\Index%934%Т%транзитивное соответствие
   {транзитивное соответствие}%
   {transitive correspondence}%
\Index%972%Т%тривиальное ядро гомоморфизма
   {тривиальное ядро гомоморфизма}%
   {trivial kernel}%
\SetIndexSpace%
\Index%851%У%универсальная алгебра
   {универсальная алгебра}%
   {universal algebra}%
\Index%688%У%универсально отталкивающий  объект категории
   {универсально отталкивающий  объект категории}%
   {universally repelling}%
\Index%914%У%универсально притягивающий объект категории
   {универсально притягивающий объект категории}%
   {universally attracting}%
\Index%132%У%унитальная алгебра
   {унитальная алгебра}%
   {unital algebra}%
\Index%915%У%унитальное кольцо
   {унитальное кольцо}%
   {unital ring}%
\Index%916%У%унитальное расширение
   {унитальное расширение}%
   {unital extension}%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%920%У%уравнение в полных дифференциалах
   {уравнение в полных дифференциалах}%
   {exact differential equation}%
\Index%925%У%уравнение Картана
   {уравнение Картана}%
   {Cartan equation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%926%У%уравнение Максвела
   {уравнение Максвела}%
   {Maxwell equation}%
\Index%923%У%уравнение поля
   {уравнение поля}%
   {field equation}%
\Index%924%У%уравнение Эйнштейна
   {уравнение Эйнштейна}%
   {Einstein equation}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%369%Ф%факторгруппа
   {факторгруппа}%
   {factor group}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%722%Ц%центр A числа
   {центр $A$\Hyph числа}%
   {center of A number}%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%888%Ч%частная производная
   {частная производная}%
   {partial derivative}%
\Index%889%Ч%частная производная второго порядка
   {частная производная второго порядка}%
   {partial derivative of second order}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\Index%827%Ч%частное от деления
   {частное от деления}%
   {quotient divided by}%
\Index%905%Ч%чётность перестановки
   {чётность перестановки}%
   {parity of permutation}%
\SetIndexSpace%
\Index%501%Ш%широта
   {широта}%
   {latitude}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%917%Э%эквивалентные нормы
   {эквивалентные нормы}%
   {equivalent norms}%
\Index%836%Э%экспонента
   {экспонента}%
   {exponent}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%982%Э%элементарное многообразие
   {элементарное $B$\Hyph многообразие}%
   {simple manifold}%
\Index%858%Э%эндоморфизм
   {эндоморфизм}%
   {endomorphism}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%938%Э%эндоморфизм диаграммы представлений
   {эндоморфизм диаграммы представлений}%
   {endomorphism of diagram of representations}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%857%Э%эпиморфизм
   {эпиморфизм}%
   {epimorphism}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%872%Э%эффект увлечения системы отсчёта
   {эффект увлечения системы отсчёта}%
   {frame dragging effect}%
\Index%516%Э%эффективное G* представление
   {эффективное \Ts{G}представление}%
   {effective G* representation}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%500%Э%эффективное представление
   {эффективное представление}%
   {effective representation}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%874%Я%ядро гомоморфизма
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности G* представления
   {ядро неэффективности \Ts{G}представления}%
   {kernel of inefficiency of G* representation}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%930%Я%ядро отображения
   {ядро отображения}%
   {kernel of map}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%850%O%Omega алгебра
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%944%O%Omega группоид
   {$\Omega$\Hyph группоид}%
   {Omega groupoid}%
\Index%656%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Preface.0906.0135.English.tex <==
%auto-ignore

\chapter{Preface}

\section{Tower of Representations}

The main goal of this book is considering of simple
geometry over division ring.

However I decided not to bind this book by description of affine and Euclidean geometry.
During description of affine geometry I discovered interesting structure.
At first I define \drc vector space $\Vector V$. This is left\Hyph side representation
of the division ring $D$ in
additive group. Then I consider a set of points where the representation of
\drc vector space $\Vector V$ is defined.
This many-tier structure stimulate my interest and I returned to exploration
of left\Hyph side representations of universal algebra.

Thus the concept of tower of left\Hyph side representations emerged.
As soon as I began draw diagrams related to the tower of left\Hyph side representations,
I discovered pattern similar to diagrams in paper
\citeBib{9705.009}.
Although I did not succeed to
carry this analogy to its logical conclusion,
I hope that this analogy can bring to interesting results.

\ifx\texFuture\Defined

Я считаю диаграммы важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я расказывал своим коллегам
какие преимущества иммет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.

Эту аналогию я вижу в разных вариантах.

Например, в section \RefSection{Tower of Representations of Algebras}
мы можем рассмотреть $2$\Hyph категорию, единственным объектом которой является
множество $A_3$. Множество морфизмов имеет вид $f_{2,3}(a_2)$, $a_2\in A_2$.
Множество $2$\Hyph морфизмов имеет вид $f_{1,3}(a_1)$, $a_1\in A_1$.
Однако в такой модели может возникнуть проблема с произведением морфизмов.
Наибольший интерес для меня представляет $n$\Hyph категория башни of left\Hyph side представлений в разделе
\RefSection{Morphism of Tower of Representations},
которую я рассматриваю по аналогии с определением
\RefDefinition{category of left-side representations of Omega1 algebra}
категории of left\Hyph side представлений.

Consideration of different structures related to left\Hyph side representation of
$\mathfrak{F}$\Hyph algebra stimulated consideration of
left\Hyph side representation of $\mathfrak{F}$\Hyph algebra in category.
\fi

\section{Morphism and Basis of Representation}

Exploring of the theory of representations of $\mathfrak{F}$\Hyph algebra
shows that this theory has a lot of common with theory of
$\mathfrak{F}$\Hyph algebra.
In \citeBib{0701.238,0707.2246,0803.2620},
I explored morphisms of representation.
They are maps that preserve the structure of representation
of $\mathfrak{F}$\Hyph algebra (or of tower of
representations).

Linear maps of vector spaces are examples of
morphism of representations. The definition of basis is important
structure
in the theory of linear spaces. Concept of basis
is directly linked to statement that
the group of morphisms of linear space
has two single transitive representations.
The main function of basis is to form linear space.

The natural question arises. Can we generalize this structure
to arbitrary representation?
The basis is not the only set that forms
the vector space.
This statement is initial point where I started
exploring of generating set of representation.
Generating set of representation is one more interesting
parallel between theory of representations and
theory of universal algebra.

For some representations, the possibility to find generating
set is not equivalent to the possibility to build basis. The problem to find
the set of representations that allow to construct basis is
interesting and important problem.
I wonder is it possible to find effective algorithm of construction of
basis of quantum geometry.

\ifx\texFuture\Defined
Let us define an additional structure on vector space $\mathcal{V}$
(for instance, a scalar product or a norm of a vector).
Then not every \drc linear map keeps properties of the selected structure.
In this case we need subgroup
$G$ of the group $\RCGL nD$
\drc linear maps from which hold properties of the selected structure.
We usually call group $G$
symmetry group.
Without loss of generality we identify element $g$ of group $G$
with corresponding transformation of representation
and write its action on vector $\Vector V\in\mathcal{V}$ as $v\RCstar g$.

Not every two bases can be mapped by a transformation
from the symmetry group
because not every nonsingular linear transformation belongs to
the representation of group $G$. Therefore, we can represent
the set of bases
as a union of orbits of group $G$.

Properties of basis depend on the symmetry group.
We can select basis $\Basis{e}$ vectors of which are
in a relationship which is invariant relative to symmetry group.
In this case all bases from orbit $\Basis{e}G$
have vectors which satisfy the same relationship. Such a basis we call
\AddIndex{$G$\Hyph basis}{G-basis}.
In each particular case we need to prove the existence of a basis
with certain properties. If such a basis does not exist
we can choose an arbitrary basis.

Basis $\Basis{e}$ creates coordinates in $\mathcal{V}$.
In different types of space it may be done in different ways.
In affine space if node of basis is point $A$ then
point $B$ has the same coordinates as vector $\overset{\longrightarrow}{AB}$
relative basis $\Basis{e}$.
In a general case we introduce coordinates of a vector as coordinates
relative to the selected basis.
Using only bases of type $G$ means using of specific coordinates on $\mathcal{A}_n$.
To distinguish them we call this \AddIndex{$G$\Hyph coordinates}{G-coordinates}.
We also call the space $\mathcal{V}$ with such coordinates
\AddIndex{$G$\Hyph space}{GSpace}.
\fi

\section{\texorpdfstring{$D$}{D}-Affine space}

Like in the case of $D$\Hyph vector space,
I can start from considering of \drc affine space
and then move to exploring of $D$\Hyph affine space.
However I do not expect something new on this way. Because I
explore operations related to differentiation, I start immediately
from exploring of $D$\Hyph affine space.

From the moment when I realized that affine space is
tower of representations and linear maps of affine space
are morphisms of tower of representations, I realized what
form the connection has in manifold with $D$\Hyph affine connection.
However, I decided to explore curvilinear coordinates
in the affine space
before I explore the manifold with affine connections.

Although it was clear in my mind
what happens when I change coordinates,
the picture that I saw  appears more
interesting then I expected. I have met two very important ideas.

I started from construction of affine space as tower of representations.
it turned out, that there exists one more model where we represent vector
fields as sets of maps.\,\footnote{At this time it is
not clear whether this model leads me to geometry that
Alain Connes explores in \citeBib{Alain Connes 1994}.
Answer on this question requires further research.}
However these two models do not contradict one to another,
but rather are complementary.

Second observation did not come as a surprise for me.
When I started to explore $D$\Hyph vector space, I was ready
to consider linear combination of vectors as polylinear form;
however I got the conclusion that this does not change
dimension of space, and for this reason I did not go beyond exploration
of \drc basis.

It is interesting to observe
how new concept appears during writing of book.
Construction that I made in chapter
\RefChapter{Calculus in Affine Space}
again returned me to a linear combination as sum of linear
forms. However at this time I have linear dependence of
$1$\Hyph forms. And coefficients of linear dependence
are not outside of $1$\Hyph form, but inside. If we consider
$1$\Hyph forms over field, then $1$\Hyph form is transparent for scalars
of the field, and there is no difference for us whether coefficients are
outside or inside the form.

Linear dependence is not subject of this book. I will explore this
question in following papers. In this book I use this
definition assuming that its properties are clear from written equations.

Exploring of curvilinear coordinates also gave opportunity to see
transformation rule of
coordinates of $D$\Hyph affine connection when we change
coordinates. However,
I think it was luck
that I was able to write the explicit transformation law,
and this luck was
associated with the fact that the connection has only one 
contravariant index. I have reason to believe 
that such an operation, like raising or lowering the index of the tensor 
in Riemannian space can have only an implicit form of record.

For years affine geometry was symbol for me of the simplest
geometry. I am glad to see that I was wrong. At the right moment
affine geometry turned out to be a source of inspiration.
Affine geometry is the gate of differential geometry.
Although, in order to plunge deeply into the differential
geometry, I need good knowledge about differential equations,
I conclude the book with very brief excursion into the manifold 
with affine connections.
It can give to reader the taste of the new geometry.


==> Preface.0906.0135.Russian.tex <==
%auto-ignore

\chapter{Предисловие}

\section{Башня представлений}

Основная задача предлагаемой книги - это рассмотрение простейших
геометрических конструкций над телом.

Однако я решил не ограничивать эту книгу описанием аффинной и эвклидовой геометрии.
В процессе построения аффинной геометрии я обнаруживаю интересную конструкцию.
Я сперва определяю \drc векторное пространство $\Vector V$. Это левостороннее представление тела $D$ в
аддитивной группе. Затем я рассматриваю множество точек, в котором определено
представление \drc векторного пространства $\Vector V$.
Эта многоярусная конструкция пробудила мой интерес и вернула меня к изучению
левосторонних представлений универсальной алгебры.

Таким образом возникла концепция башни левосторонних представлений.
Как только я начал рисовать диаграммы, связанные с башней левосторонних представлений,
я увидел узор, похожий на диаграммы, построенные в статье
\citeBib{9705.009}.
Хотя мне не удалось довести эту аналогию до конца,
я надеюсь, что эта аналогия может привести к интересным результатам.

\ifx\texFuture\Defined

Я считаю диаграммы важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я расказывал своим коллегам
какие преимущества иммет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.

Эту аналогию я вижу в разных вариантах.

Например, в разделе \RefSection{Tower of Representations of Algebras}
мы можем рассмотреть $2$\Hyph категорию, единственным объектом которой является
множество $A_3$. Множество морфизмов имеет вид $f_{2,3}(a_2)$, $a_2\in A_2$.
Множество $2$\Hyph морфизмов имеет вид $f_{1,3}(a_1)$, $a_1\in A_1$.
Однако в такой модели может возникнуть проблема с произведением морфизмов.
Наибольший интерес для меня представляет $n$\Hyph категория башни левосторонних представлений в разделе
\RefSection{Morphism of Tower of Representations},
которую я рассматриваю по аналогии с определением
\RefDefinition{category of left-side representations of Omega1 algebra}
категории левосторонних представлений.

Рассмотрение различных конструкций, связанных с левосторонним представлением
$\mathfrak{F}$\Hyph алгебры, послужило толчком к рассмотрению
левостороннего представления $\mathfrak{F}$\Hyph алгебры в категории.
\fi

\section{Морфизм и базис представления}

Изучение теории представлений $\mathfrak{F}$\Hyph алгебры
показывает, что эта теория имеет много общего с теорией
$\mathfrak{F}$\Hyph алгебры.
В \citeBib{0701.238,0707.2246,0803.2620}
я изучал морфизмы представления.
Это отображения, которые сохраняют структуру представления
$\mathfrak{F}$\Hyph алгебры (или башни
представлений).

Линейные отображения векторных пространств являются примерами
морфизма представлений. Понятие базиса является важной конструкцией
в теории линейных пространств. Понятие базиса
непосредственно связано с тем, что группа морфизмов линейного пространства
имеет два однотранзитивных представления.
Основная функция базиса - это порождать линейное пространство.

Возникает естественный вопрос. Можно ли обобщить эту конструкцию
на произвольное представление?
Базис - это не единственное множество, которое порождает
векторное пространство.
Это утверждение является исходной точкой, от которой я начал
изучение множества образующих представления.
Множество образующих представления - это ещё одна интересная
параллель теории представлений с теорией универсальной алгебры.

Не для всякого представления возможность найти множество образующих
равносильна возможности построения базиса. Задача найти
класс представлений, где возможно построение базиса является
интересной и важной задачей.
Мне интересно, можно ли найти эффективный алгоритм построения
базиса квантовой геометрии.

\ifx\texFuture\Defined
Если на векторном пространстве $\mathcal{V}$ определена дополнительная структура
(например, скалярное произведение или норма вектора),
не всякий \drc линейное отображение сохраняет свойства заданной структуры.
В этом случае нас интересует подгруппа
$G$ группы $\RCGL nD$,
\drc линейное отображения которой сохраняют свойства заданной структуры.
Мы обычно будем называть группу $G$
группой симметрии.
Не нарушая общности, мы будем отождествлять элемент $g$ группы $G$
с соответствующим преобразованием представления
и записывать его действие на вектор $\Vector V\in\mathcal{V}$
в виде $v\RCstar g$.

Не всякие два базиса могут быть связаны
преобразованием группы симметрии
потому, что не всякое невырожденное линейное преобразование принадлежит
представлению группы $G$. Таким образом, множество базисов
можно представить как объединение орбит группы $G$.

Свойства базиса зависят от группы симметрии.
Мы можем выбрать базисы $\Basis{e}$, векторы которых находятся
в отношении, которое инвариантно относительно группы симметрии.
В этом случае все базисы из орбиты $\Basis{e}G$
имеют векторы, которые удовлетворяют одному и тому же отношению.
Такой базис мы будем называть
\AddIndex{$G$\Hyph базисом}{G-basis}.
В каждом конкретном случае мы должны доказать существование
базиса с искомыми свойствами. Если подобного типа базиса
не существует, мы можем выбрать произвольный базис.

Базис $\Basis{e}$ порождает координаты на $\mathcal{V}$.
В различных типах пространства это может быть сделано различным образом.
В аффинном пространстве, если вершина базиса является точкой $A$, то
точка $B$ имеет те же координаты, что и вектор $\overset{\longrightarrow}{AB}$
относительно базиса $\Basis{e}$.
В общем случае мы вводим координаты вектора как координаты
относительно выбранного базиса.
Использование только $G$\Hyph пространства означает использование специальных координат на $\mathcal{A}_n$.
Для того, чтобы отличать их, мы будем называть их
\AddIndex{$G$\Hyph координатами}{G-coordinates}.
Мы также будем называть пространство $\mathcal{V}$ с такими координатами
\AddIndex{$G$\Hyph пространством}{GSpace}.
\fi

\section{\texorpdfstring{$D$}{D}-аффинное пространство}

Так же как и в случае $D$\Hyph векторных пространств,
я могу начать с рассмотрения \drc аффинного пространства
и затем перейти к рассмотрению $D$\Hyph аффинных пространств.
Однако на этом пути я не ожидаю новых явлений. Так как меня
интересуют операции, связаные с дифференцированием, я сразу начинаю
с рассмотрения $D$\Hyph аффинного пространства.

С того момента, как я понял, что аффинное пространство является
башней представлений, а линейные отображения аффинных пространств
являются морфизмами башни представлений, я понял как будет
выглядеть связность в многообразии $D$\Hyph аффинной связности.
Тем не менее, прежде чем изучать многообразие аффинной связности,
я решил исследовать криволинейные координаты в аффинном пространстве.

Хотя я хорошо представлял, что должно происходить при замене координат,
увиденное превзошло мои ожидания. Я встретил две очень важные концепции.

Я начал с построения аффинного пространства как башни представлений.
Оказалось, что существует ещё одна модель, в которой векторные поля
представлены в виде множества отображений.\,\footnote{Пока неясно,
приведёт ли меня эта модель к геометрии, которую изучает
Ален Конн в \citeBib{Alain Connes 1994}.
Ответ на этот вопрос требует дальнейшего исследования.}
Тем не менее эти две модели не противоречат друг другу,
а скорее дополняют друг друга.

Второе наблюдение для меня не оказалось неожиданностью.
Когда я начал изучать $D$\Hyph векторные пространства, я был готов
рассмотреть линейную комбинацию векторов как полилинейную форму,
однако я очень быстро пришёл к выводу, что это не изменит
размерности пространства, и потому ограничился рассмотрением
\drc базиса.

Интересно наблюдать,
как в процессе создания книги появляется новая конценция.
Построения, выполненные в главе
\RefChapter{Calculus in Affine Space}
снова вернули меня к линейной комбинации как сумме линейных
форм. Однако на этот раз речь идёт о линейной зависимости
$1$\Hyph форм. При этом коэффициенты линейной зависимости
находятся не вне $1$\Hyph формы, а внутри. Если мы рассматриваем
$1$\Hyph формы над полем, то $1$\Hyph форма прозрачна для скаляров
поля и для нас не имеет значение находятся ли коэффициенты
вне формы или внутри.

Линейная зависимость не является темой этой книги. Я рассмотрю этот
вопрос в последующих работах. В этой книге я буду пользоваться этим
понятием, полагая, что его свойства понятны из приводимых равенств.

Изучение криволинейных координат также позволило увидеть как
преобразуются координаты $D$\Hyph аффинной связности при замене
координат. Однако, то что мне удалось записать явный закон преобразования,
на мой взгляд удача, связанная с тем, что связность имеет только один
контравариантный индекс. У меня есть все основания полагать,
что такая операция, как поднятие или опускание индекса тензора
в римановом пространстве может иметь только неявную форму записи.

Многие годы для меня аффинная геометрия была символом самой простой
геометрии. Я рад увидеть, что я ошибался. В нужную минуту
аффинная геометрия оказалась источником вдохновения.
Аффинная геометрия - это врата дифференциальной геометрии.
И хотя, для того, чтобы погрузиться в дифференциальную
геометрию, я должен хорошо освоиться с дифференциальными уравнениями,
я завершаю книгу очень коротким экскурсом в многообразия
аффинной связности, для того, чтобы почуствовать вкус новой геометрии.


==> Preliminary.Representation.Russian.tex <==
%auto-ignore
\input{Preliminary.Representation.Eq}

\ePrints{4975-6381,6860-2955}%
\Items{5410-9916,9835-2163,7287-9339}
\ifx\Semafor\ValueOff
\Chapter{Представление универсальной алгебры}

\ShowText{Preliminary Definitions}
\fi

\ePrints{4975-6381,1506.00061,8428-0408,8525-2526,2207.06506,5148-4632,1908.04418,6860-2955}
\Items{1601.03259,5410-9916,9835-2163,7287-9339,5284-0163}
\Items{1801.01628,2307.09982,MAlgebra4}
\ifx\Semafor\ValueOn

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Отношение эквивалентности}

\begin{\DefinitionStyle}
\labelDefinition{equivalence}
Соответствие
\ShowEq{Phi in AxA}
называется
\AddIndex{отношением эквивалентности}{equivalence},
если\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
соответствие $\Phi$
\AddIndex{рефлексивно}{reflexive correspondence}
\ShowEq{reflexive correspondence}
\item
соответствие $\Phi$
\AddIndex{симметрично}{symmetric correspondence}
\ShowEq{symmetric correspondence}
\item
соответствие $\Phi$
\AddIndex{транзитивно}{transitive correspondence}
\ShowEq{transitive correspondence}
\end{enumerate}
\end{\DefinitionStyle}
\footnotetext{\,
Смотри также определение на странице
\citeBib{Cohn: Universal Algebra}\Hyph 27.
}

\begin{\TheoremStyle}
Для отображения
\ShowEq{f:A->B}fAB
множество
\ShowEq{kernel of map}
\ShowEq{def kernel of map}
является отношением эквивалентности и
называется
\AddIndex{ядром отображения}{kernel of map}.\,\footnotemark
\end{\TheoremStyle}
\footnotetext{\,
Смотри также определение на странице
\citeBib{Cohn: Universal Algebra}\Hyph 28.
}
\begin{proof}
\begin{ShadedLemma}
\labelLemma{ker - reflexive correspondence}
{\it
Соответствие
\ShowEq{ker f}
рефлексивно.
}
\end{ShadedLemma}

{\sc Доказательство.}
Из равенства
\ShowEq{fa=fa}
и определения
\EqRef{def kernel of map}
следует, что
\DrawEq[aa]{ab in ker}{aa}
Лемма является следствием утверждения
\eqRef{ab in ker}{aa}
и определения
\RefItem{reflexive correspondence}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{ker - symmetric correspondence}
{\it
Соответствие
\ShowEq{ker f}
симметрично.
}
\end{ShadedLemma}

{\sc Доказательство.}
Равенство
\DrawEq[ab]{fa=fb}{ab symmetric}
является следствием утверждения
\DrawEq[ab]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[ba]{fa=fb}{ba}
является следствием равенства
\eqRef{fa=fb}{ab symmetric}.
Утверждение
\DrawEq[ba]{ab in ker}{}
является следствием равенства
\eqRef{fa=fb}{ba}
и определения
\EqRef{def kernel of map}.
Следовательно, мы доказали утверждение
\ShowEq{ab in ker -> ba in ker}
Лемма является следствием утверждения
\EqRef{ab in ker -> ba in ker}
и определения
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{ker - transitive correspondence}
{\it
Соответствие
\ShowEq{ker f}
транзитивно.
}
\end{ShadedLemma}

{\sc Доказательство.}
Равенство
\DrawEq[ab]{fa=fb}{ab transitive}
является следствием утверждения
\DrawEq[ab]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[bc]{fa=fb}{bc}
является следствием утверждения
\DrawEq[bc]{ab in ker}{}
и определения
\EqRef{def kernel of map}.
Равенство
\DrawEq[ac]{fa=fb}{ac}
является следствием равенств
\eqRef{fa=fb}{ab transitive},
\eqRef{fa=fb}{bc}.
Утверждение
\DrawEq[ac]{ab in ker}{}
является следствием равенства
\eqRef{fa=fb}{ac}
и определения
\EqRef{def kernel of map}.
Следовательно, мы доказали утверждение
\ShowEq{ab,ac in ker -> ac in ker}
Лемма является следствием утверждения
\EqRef{ab,ac in ker -> ac in ker}
и определения
\RefItem{symmetric correspondence}.
\hfill\(\odot\)

Утверждение теоремы является следствием лемм
\ShowEq{lemmas for ker}
и определения
\RefDefinition{equivalence}.
\end{proof}
\else
\Section{Универсальная алгебра}
\fi

\ePrints{8428-0408,8525-2526,2207.06506,2307.09982,MAlgebra4}
\ifx\Semafor\ValueOn
\begin{\DefinitionStyle}
Для отображения
\ShowEq{f:A->B}fAB
множество
\ShowEq{image of map}
\ShowEq{show image of map}
называется
\AddIndex{образом отображения}{image of map}
$f$.
\end{\DefinitionStyle}
\fi

\ePrints{5410-9916,9835-2163,5284-0163,1801.01628}
\ePrints{8428-0408,8525-2526,2207.06506,2307.09982,MAlgebra4,0906.0135}
\ifx\Semafor\ValueOff
\begin{\TheoremStyle}
\labelTheorem{maps and kernel equivalence}
Пусть $N$ - отношение эквивалентности
на множестве $A$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
отображения\,\,\footnotemark
\ShowEq{maps category}
Мы определим морфизм $f_1\rightarrow f_2$
как отображение $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{maps category, diagram}
Отображение
\ShowEq{maps category, universal}
является универсально отталкивающим в категории $\mathcal A$.\,\footnotemark
\end{\TheoremStyle}
\ShowPrevFootnote{
Утверждение теоремы
\RefTheorem{maps and kernel equivalence}
аналогично утверждению на с. \citeBib{Serge Lang}-94.
}
\ShowNextFootnote{
Определение универсального объекта смотри в определении
на с. \citeBib{Serge Lang}-47.
}
\begin{proof}
Рассмотрим диаграмму
\ShowEq{maps category, universal, diagram}
\ShowEq{maps category, universal, ker}
Из утверждения
\EqRef{maps category, universal, ker}
и равенства
\ShowEq{maps category 1}
следует
\ShowEq{maps category 2}
Следовательно, мы можем однозначно определить отображение $h$
с помощью равенства
\ShowEq{maps category, h}
\end{proof}
\fi

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Универсальная алгебра}
\fi

\begin{\DefinitionStyle}
\labelDefinition{Cartesian power}
Для любых множеств\,\footnotemark
$A$, $B$,
\AddIndex{декартова степень}{Cartesian power}
\ShowEq{Cartesian power}
- это множество отображений
\ShowEq{f:A->B}fAB
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению из примера (iV),
\citeBib{Cohn: Universal Algebra}, страницы 17, 18.
}

\begin{\DefinitionStyle}
\labelDefinition{operation on set}
Пусть дано множество $A$ и целое число $n\ge 0$. Отображение\,\footnotemark
\ShowEq{o:An->A}
называется
\AddIndex{$n$\Hyph арной операцией на множестве}{n-ary operation on set}
$A$ или просто
\AddIndex{операцией на множестве}{operation on set}
$A$.
Для любых
\ShowEq{b1n in B}aA,
мы пользуемся любой из форм записи
\ShowEq{a1no=oa1n}
для обозначения образа отображения $\omega$.
\end{\DefinitionStyle}
\footnotetext{\,
\ePrints{2307.09982,5148-4632,1908.04418,6860-2955,MAlgebra4}
\ifx\Semafor\ValueOn
Определения
\RefDefinition{operation on set},
\RefDefinition{set is closed with respect to operation}
опираются
\else
Определение
\RefDefinition{operation on set}
опирается
\fi
на определение в примере (vi),
страница \citeBib{Cohn: Universal Algebra}\Hyph 26.
}

\ePrints{9835-2163,5284-0163,1801.01628,0906.0135}
\ifx\Semafor\ValueOff
\begin{remark}
\labelRemark{o in AAn}
Согласно определениям
\RefDefinition{Cartesian power},
\RefDefinition{operation on set},
$n$\Hyph арная операция
\ShowEq{o in AAn}
\qed
\end{remark}
\fi

\begin{\DefinitionStyle}
\AddIndex{Область операторов}{operator domain}
- это множество операторов\,\footnotemark
\ShowEq{operator domain}
вместе с отображением
\ShowEq{f:A->B}a{\Omega}N
Если
\ShowEq{omega in Omega}{},
то $a(\omega)$ называется
\AddIndex{арностью}{arity}
оператора $\omega$. Если
\ShowEq{a(o)=n}
то оператор $\omega$ называется $n$\Hyph арным.
\ShowEq{set of n-ary operators}
Мы пользуемся обозначением
\ShowEq{set of n-ary operators =}
для множества $n$\Hyph арных операторов.
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению 1,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}

\begin{\DefinitionStyle}
\labelDefinition{Omega-algebra}
Пусть $A$ - множество, а $\Omega$ - область операторов.\,\footnotemark
Семейство отображений
\ShowEq{O(n)->AAn}
называется структурой $\Omega$\Hyph алгебры на $A$.
Множество $A$ со структурой $\Omega$\Hyph алгебры называется
\AddIndex{$\Omega$\Hyph алгеброй}{Omega-algebra}
\ShowEq{Omega-algebra}
или
\AddIndex{универсальной алгеброй}{universal algebra}.
\ePrints{9835-2163,0767-8264,5284-0163,1801.01628,0906.0135}
\ifx\Semafor\ValueOff
Множество $A$ называется
\AddIndex{носителем $\Omega$\Hyph алгебры}{carrier of Omega-algebra}.
\fi
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению 2,
страница \citeBib{Cohn: Universal Algebra}\Hyph 62.
}

\ePrints{9835-2163,0767-8264,5284-0163,1801.01628,0906.0135}
\ifx\Semafor\ValueOff
Область операторов $\Omega$ описывает множество $\Omega$\Hyph алгебр.
Элемент множества $\Omega$ называется оператором,
так как операция предполагает некоторое множество.
Согласно замечанию
\ref{remark: o in AAn}
и определению
\RefDefinition{Omega-algebra},
каждому оператору
\ShowEq{omega n ari}{}{}n{}
сопоставляется $n$\Hyph арная операция $\omega$ на $A$.
\fi

\ePrints{2307.09982,5148-4632,1908.04418,6860-2955,MAlgebra4}
\ifx\Semafor\ValueOn

\begin{\TheoremStyle}
\labelTheorem{Cartesian power is universal algebra}
Пусть множество $B$ является $\Omega$\Hyph алгеброй.
Тогда множество $B^A$ отображений
\ShowEq{f:A->B}fAB
также является $\Omega$\Hyph алгеброй.
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{omega n ari}{}{}n.
Для отображений
\ShowEq{f1n in B**A}
мы определим операцию $\omega$ равенством
\DrawEq{f1n omega=}{}
\end{proof}
\fi

\ePrints{2307.09982,5148-4632,1908.04418,6860-2955,MAlgebra4}
\ifx\Semafor\ValueOn
\begin{\DefinitionStyle}
\labelDefinition{set is closed with respect to operation}
{\it
Пусть
\ShowEq{B subset A}.
Если для любых
\ShowEq{b1n in B}bB,
\ShowEq{b1no in B}
то мы говорим, что $B$
\AddIndex{замкнуто относительно}{set is closed with respect to operation}
$\omega$ или что $B$
\AddIndex{допускает операцию}{set admits operation}
$\omega$.
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
$\Omega$\Hyph алгебра $B_{\Omega}$ является
\AddIndex{подалгеброй}{subalgebra of Omega-algebra}
$\Omega$\Hyph алгебры $A_{\Omega}$,
если верны следующие утверждения\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{B subset A}.
\item
Если оператор
\ShowEq{omega in Omega}{}{}
определяет операции $\omega_A$ на $A$ и $\omega_B$ на $B$, то
\ShowEq{oAB=oB}
\end{enumerate}
\qed
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 62.
}
\fi

\ShowFootnote{iso end aut morphism}1

\begin{\DefinitionStyle}
\labelDefinition{homomorphism}
Пусть $A$, $B$ - $\Omega$\Hyph алгебры и
\ShowEq{omega n ari}{}{}n.
Отображение\,\refFootnote{iso end aut morphism}1
\ShowEq{f:A->B}fAB
\AddIndex{согласовано с операцией}{map is compatible with operation}
$\omega$, если, для любых
\ShowEq{b1n in B}aA,
\DrawEq[fa]{afo=aof}{}
Отображение $f$ называется
\AddIndex{гомоморфизмом}{homomorphism}
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$,
если $f$ согласовано с каждым
\ShowEq{omega in Omega}{}.
\ePrints{1908.04418,6860-2955}%
\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of homomorphisms}
множество гомоморфизмов
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$.
\fi
\end{\DefinitionStyle}

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\begin{\TheoremStyle}
\labelTheorem{Hom empty A B=B**A}
Если область операторов пуста,
то гомоморфизм
$\Omega$\Hyph алгебры $A$ в $\Omega$\Hyph алгебру $B$
- это отображение
\ShowEq{f:A->B}fAB
Следовательно,
\ShowEq{Hom empty A B=B**A}
\end{\TheoremStyle}
\begin{proof}
Теорема является следствием определений
\RefDefinition{Cartesian power},
\RefDefinition{homomorphism}.
\end{proof}
\fi

\ePrints{2307.09982,5148-4632,1908.04418,6860-2955,8428-0408,8525-2526,2207.06506,MAlgebra4}
\ifx\Semafor\ValueOn
\ShowFootnote{iso end aut morphism}2

\begin{\DefinitionStyle}
\labelDefinition{isomorphism}
Гомоморфизм
\ShowEq{f:A->B}fAB
назывется\,\refFootnote{iso end aut morphism}2
\AddIndex{изоморфизмом}{isomorphism}
между $A$ и $B$, если соответствие $f^{-1}$ является гомоморфизмом.
Если существует изоморфизм между $A$ и $B$, то говорят,
что $A$ и $B$ изоморфны, и пишут
\ShowEq{isomorphic}
Инъективный гомоморфизм называется
\AddIndex{мономорфизмом}{monomorphism}.
Суръективный гомоморфизм называется
\AddIndex{эпиморфизмом}{epimorphism}.
\end{\DefinitionStyle}
\fi

\begin{\DefinitionStyle}
\labelDefinition{endomorphism}
Гомоморфизм
\ShowEq{f:A->B}fAA
источником и целью которого является одна и таже алгебра, называется
\AddIndex{эндоморфизмом}{endomorphism}.
%\ePrints{1908.04418,6860-2955}%
%\ifx\Semafor\ValueOn%
Мы обозначим
\ShowEq{set of endomorphisms}
множество эндоморфизмов
$\Omega$\Hyph алгебры $A$.
%\fi
\ePrints{4975-6381,1506.00061,7287-9339,0906.0135}%
\Items{1601.03259,2307.09982,5148-4632,9835-2163,0767-8264,5284-0163,1801.01628}%
\ifx\Semafor\ValueOff%
Изоморфизм
\ShowEq{f:A->B}fAA
называется
\AddIndex{автоморфизмом}{automorphism}.
\fi
\end{\DefinitionStyle}

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn

\begin{\TheoremStyle}
\labelTheorem{End A=Hom AA}
\ShowEq{End A=Hom AA}
\end{\TheoremStyle}
\begin{proof}
Теорема является следствием определений
\RefDefinition{homomorphism},
\RefDefinition{endomorphism}.
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{End empty A=A**A}
Если область операторов пуста,
то эндоморфизм множества $A$
- это отображение
\ShowEq{t:A->A}
Следовательно,
\ShowEq{End empty A=A**A}
\end{\TheoremStyle}
\begin{proof}
Теорема является следствием теорем
\RefTheorem{Hom empty A B=B**A},
\RefTheorem{End A=Hom AA}.
\end{proof}
\fi

\ePrints{1908.04418,6860-2955,2207.06506,8525-2526,2307.09982,MAlgebra4}%
\ifx\Semafor\ValueOn
\begin{\TheoremStyle}
\labelTheorem{product of homomorphisms}
Пусть отображение
\DrawEq[fAB{}]{f: A->B}{}
является гомоморфизмом $\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебры $B$.
Пусть отображение
\DrawEq[gBC{}]{f: A->B}{}
является гомоморфизмом $\Omega$\Hyph алгебры $B$
в $\Omega$\Hyph алгебры $C$.
Тогда отображение\,\footnotemark
\DrawEq[{h=g\circ f}AC{}]{f: A->B}{}
является гомоморфизмом $\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебры $C$.
\end{\TheoremStyle}
\footnotetext{\,
Я следую предложению
\citeBib{Cohn: Universal Algebra}\Hyph 3.2
на странице
\citeBib{Cohn: Universal Algebra}\Hyph 71.
}
\begin{proof}
Пусть
\ShowEq{omega in Omega}n{}
- n\Hyph арная операция.
Тогда
\DrawEq[fa]{afo=aof}{fa}
для любых
\ShowEq{b1n in B}aA,
и
\DrawEq[gb]{afo=aof}{gb}
для любых
\ShowEq{b1n in B}bB.
Равенство
\ShowEq{agfo=aogf}
является следствием равенств
\eqRef{afo=aof}{fa},
\eqRef{afo=aof}{gb}.
Теорема является следствием равенства
\EqRef{agfo=aogf}
для любой операции $\omega$.
\end{proof}
\fi

\ePrints{4975-6381,1506.00061,7287-9339,5148-4632,5410-9916,0906.0135}%
\Items{8428-0408,1601.03259,2307.09982,MAlgebra4,9835-2163,0767-8264,5284-0163,1801.01628}%
\ifx\Semafor\ValueOff%
\begin{\DefinitionStyle}
Если существует мономорфизм $\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебру $B$, то говорят, что
\AddIndex{$A$ может быть вложена в $B$}{can be embeded}.
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
Если существует эпиморфизм из $A$ в $B$, то $B$ называется
\AddIndex{гомоморфным образом}{homomorphic image} алгебры $A$.
\end{\DefinitionStyle}
\fi
\fi

\ePrints{2307.09982,MAlgebra4,5148-4632,4975-6381}
\ePrints{5410-9916,9835-2163,0767-8264,5284-0163,1801.01628,0906.0135}
\ifx\Semafor\ValueOn
\ShowConvention{A number}{\Omega}{алгебры}
\fi

\ePrints{1908.04418,6860-2955,8428-0408,8525-2526,2207.06506,,MAlgebra4,5284-0163,1801.01628}
\ifx\Semafor\ValueOn

\Section{Декартово произведение универсальных алгебр}

\ePrints{8428-0408,8525-2526,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\begin{\DefinitionStyle}
\labelDefinition{universally attracting object of category}
Пусть $\mathcal C$ - некоторая категория.
Объект $P$ категории $\mathcal C$ называется
\AddIndex{универсально притягивающим}{universally attracting},\,\footnotemark
если для любого объекта $R$ категории $\mathcal C$
существует единственный морфизм
\ShowEq{f:A->B}fRP
\end{\DefinitionStyle}
\footnotetext{\,
Смотри также определение в \citeBib{Serge Lang}, страница 47.
}

\begin{\DefinitionStyle}
\labelDefinition{universally repelling object of category}
Пусть $\mathcal C$ - некоторая категория.
Объект $P$ категории $\mathcal C$ называется
\AddIndex{универсально отталкивающим}{universally repelling},\,\footnotemark
если для любого объекта $R$ категории $\mathcal C$
существует единственный морфизм
\ShowEq{f:A->B}fPR
\end{\DefinitionStyle}
\footnotetext{\,
Смотри также определение в \citeBib{Serge Lang}, страница 47.
}

\begin{\DefinitionStyle}
\labelDefinition{product in category, 2020}
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Пусть
\ShowEq{category A(Bi)}
- категория,
объектами которой являются кортежи $(P,f)$,
где $P$ - объект категории $\mathcal A$
и $f$ - множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
Универсально притягивающий объект категории
\ShowEq{category A(Bi)}
\ShowEq{product in category}
называется
\AddIndex{произведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{product in category}.\,\footnotemark

Если $|I|=n$, то для произведения множества объектов
$\{B_i,\iI\}$ в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{product in category, 1 n}
\end{\DefinitionStyle}
\footnotetext{\,
Определение дано согласно определению на странице
\citeBib{Serge Lang}\Hyph 45.
}

\begin{\TheoremStyle}
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Произведение множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$
- это объект
\ShowEq{product in category}
и множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
такие, что
для любого объекта $R$ и множества морфизмов
\ShowEq{set f:A->B}gR{B_i}
существует единственный морфизм
\ShowEq{f:A->B}hRP
такой, что диаграмма
\ShowEq{product in category diagram}
коммутативна для всех $i\in I$.
\end{\TheoremStyle}

\begin{proof}
Теорема является следствием определений
\RefDefinition{universally attracting object of category},
\RefDefinition{product in category, 2020}.
\end{proof}
\else
\ShowDefinition{product in category}
\fi

\begin{example}
Пусть \(\mathcal S\) - категория множеств.\,\footnote{\,
Смотри также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\ShowEq{ref product in category}
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}A{}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
\qed
\end{example}

\begin{\TheoremStyle}
\labelTheorem{product exists in category of Omega algebras}
Произведение существует в категории \(\mathcal A\) \(\Omega\)\Hyph алгебр.
Пусть \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\).
%семейства \(\Omega\)\Hyph алгебр
Тогда
\StartLabelItem
\begin{enumerate}
\item
\labelItem{set A is Cartesian product}
Множество \(A\) является декартовым произведением
семейства множеств
\ShowEq{Ai iI}A{}
\item
\labelItem{homomorphism is projection on factor}
Гомоморфизм \(\Omega\)\Hyph алгебры
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
\item
Любое \(A\)\Hyph число $a$ может быть однозначно представлено
в виде кортежа
\ShowEq{tuple represent A number}
\(A_i\)\Hyph чисел.
\labelItem{tuple represent A number}
\item
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Тогда операция $\omega$ определена покомпонентно
\ShowEq{operation is defined componentwise}
где
\ShowEq{a=ai 1n}.
\labelItem{operation is defined componentwise}
\end{enumerate}
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{Cartesian product of sets}
декартово произведение
семейства множеств
\ShowEq{Ai iI}A{}
и, для каждого \iI, отображение 
\ShowEq{projection on i factor}
является проекцией на \(i\)\Hyph й множитель.
Рассмотрим диаграмму морфизмов в категории множеств $\mathcal S$
\ShowEq{operation is defined componentwise, diagram}
где отображение $g_i$ определено равенством
\ShowEq{gi()=}
Согласно определению
\ShowEq{ref product in category}
отображение $\omega$ определено однозначно из множества диаграмм
\EqRef{operation is defined componentwise, diagram}
\ShowEq{omega(ai)=(omega ai)}
Равенство
\EqRef{operation is defined componentwise}
является следствием равенства
\EqRef{omega(ai)=(omega ai)}.
\end{proof}

\begin{\DefinitionStyle}
Если \(\Omega\)\Hyph алгебра \(A\)
и семейство морфизмов
\ShowEq{p:A->Ai i in I}
является произведением в категории \(\mathcal A\),
то \(\Omega\)\Hyph алгебра \(A\) называется
\AddIndex{прямым}{direct product of Omega algebras}
или
\AddIndex{декартовым произведением \(\Omega\)\Hyph алгебр}
{Cartesian product of Omega algebras}
\ShowEq{Ai iI}A.
\end{\DefinitionStyle}

\begin{\TheoremStyle}
\labelTheorem{map from product into product}
Пусть множество \(A\) является
декартовым произведением множеств
\ShowEq{Ai iI}A{}
и множество \(B\) является
декартовым произведением множеств
\ShowEq{Ai iI}B.
Для каждого \iI, пусть
\ShowEq{f:A->B i}
является отображением множества $A_i$ в множество $B_i$.
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras diagram}
где отображения
\ShowEq{pi p'i}
являются проекцией на \(i\)\Hyph й множитель.
Множество коммутативных диаграмм
\EqRef{homomorphism of Cartesian product of Omega algebras diagram}
однозначно определяет отображение
\ShowEq{f:A->B}fAB
\DrawEq{f:A->B=}{}
\end{\TheoremStyle}
\begin{proof}
Для каждого \iI, рассмотрим коммутативную диаграмму
\ShowEq{homomorphism of Cartesian product of Omega algebras}
Пусть \(a\in A\).
Согласно утверждению
\RefItem{tuple represent A number},
\(A\)\Hyph число \(a\)
может быть представлено в виде кортежа \(A_i\)\Hyph чисел
\ShowEq{a=p(a)i}
Пусть
\ShowEq{b=f(a)}
Согласно утверждению
\RefItem{tuple represent A number},
\(B\)\Hyph число \(b\)
может быть представлено в виде кортежа \(B_i\)\Hyph чисел
\ShowEq{b=p(b)i}
Из коммутативности диаграммы $(1)$
и из равенств
\EqRef{b=f(a)},
\EqRef{b=p(b)i}
следует, что
\ShowEq{b=g(a)i}
Из коммутативности диаграммы $(2)$
и из равенства
\EqRef{a=p(a)i}
следует, что
\ShowEq{b=f(a)i}
\end{proof}

\begin{\TheoremStyle}
\labelTheorem{homomorphism of Cartesian product of Omega algebras}
Пусть \(\Omega\)\Hyph алгебра \(A\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Ai iI}A{}
и \(\Omega\)\Hyph алгебра \(B\) является
декартовым произведением \(\Omega\)\Hyph алгебр
\ShowEq{Ai iI}B.
Для каждого \iI,
пусть отображение
\ShowEq{f:A->B i}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
Тогда отображение
\ShowEq{f:A->B}fAB
определённое равенством
\DrawEq{f:A->B=}{homomorphism}
является гомоморфизмом \(\Omega\)\Hyph алгебры.
\end{\TheoremStyle}
\begin{proof}
Пусть
\ShowEq{omega in Omega}{}{}
- n\Hyph арная операция.
Пусть
\ShowEq{a=ai 1n} и
\ShowEq{b=bi 1n}.
Из равенств
\EqRef{operation is defined componentwise},
\eqRef{f:A->B=}{homomorphism}
следует, что
\ShowEq{f:A->B omega}
\end{proof}

\begin{\DefinitionStyle}
Эквивалентность на $\Omega$\Hyph алгебре $A$,
которая является подалгеброй $\Omega$\Hyph алгебры $A^2$,
называется
\AddIndex{конгруенцией}{}\,\footnotemark
на $A$.
\end{\DefinitionStyle}
\footnotetext{\,
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 71.
}

\begin{\TheoremStyle}[первая теорема об изоморфизмах]
\labelTheorem{first isomorphism theorem}
Пусть
\ShowEq{f:A->B}fAB
гомоморфизм $\Omega$\Hyph алгебр с ядром $s$.
Тогда отображение $f$ имеет разложение
\ShowEq{decomposition of map f}
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{Ядро гомоморфизма}{kernel of homomorphism}
\ShowEq{kernel of homomorphism}
является конгруэнцией на $\Omega$\Hyph алгебре $A$.
\labelItem{kernel of homomorphism}
\item
Множество
\ShowEq{A/ker f}
является $\Omega$\Hyph алгеброй.
\labelItem{A/ker f is Omega-algebra}
\item
Отображение
\ShowEq{p:A->/ker}
является эпиморфизмом и называется
\AddIndex{естественным гомоморфизмом}{natural homomorphism}.
\labelItem{natural homomorphism}
\item
Отображение
\ShowEq{q:A/ker->f(A)}
является изоморфизмом.
\labelItem{q:A/ker->f(A) isomorphism}
\item
Отображение
\ShowEq{r:f(A)->B}
является мономорфизмом.
\labelItem{r:f(A)->B monomorphism}
\end{enumerate}
\end{\TheoremStyle}
\begin{proof}
Утверждение
\RefItem{kernel of homomorphism}
является следствием предложения II.3.4
(\citeBib{Cohn: Universal Algebra}, страница 72).
Утверждения
\RefItem{A/ker f is Omega-algebra},
\RefItem{natural homomorphism}
являются следствием теоремы II.3.5
(\citeBib{Cohn: Universal Algebra}, страница 72)
и последующего определения.
Утверждения
\RefItem{q:A/ker->f(A) isomorphism},
\RefItem{r:f(A)->B monomorphism}
являются следствием теоремы II.3.7
(\citeBib{Cohn: Universal Algebra}, страница 74).
\end{proof}

\ePrints{8428-0408,8525-2526,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowDefinition{coproduct in category}

\ShowTheorem{coproduct in category}
\ShowProof{coproduct in category}
\fi
\fi

\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
\Section{Полугруппа}

Обычно операция
\ShowEq{omega n ari}{}{}2{}
называется произведением
\ShowEq{abo=ab}
либо суммой
\ShowEq{abo=a+b}

\begin{\DefinitionStyle}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй и
\ShowEq{omega n ari}{}{}2.
$A$\Hyph число $e$ называется
\AddIndex{нейтральным элементом операции}{neutral element of operation}
$\omega$, если для любого $A$\Hyph числа $a$ верны равенства
\ShowEq{left neutral element}
\ShowEq{right neutral element}
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega n ari}{}{}2{}
называется
\AddIndex{ассоциативной}{associative operation},
если верно равенство
\ShowEq{associative operation}
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
{\it
Пусть $A$ является $\Omega$\Hyph алгеброй.
Операция
\ShowEq{omega n ari}{}{}2{}
называется
\AddIndex{коммутативной}{commutative operation},
если верно равенство
\ShowEq{commutative operation}
}
\qed
\end{\DefinitionStyle}

\begin{\DefinitionStyle}
\labelDefinition{semigroup}
{\it
Пусть
\ShowEq{Omega=omega}
Если операция
\ShowEq{omega n ari}{}{}2{}
ассоциативна, то $\Omega$\Hyph алгебра называется
\AddIndex{полугруппой}{semigroup}.
Если операция в полугруппе коммутативна,
то полугруппа называется
\AddIndex{абелевой полугруппой}{Abelian semigroup}.
}
\qed
\end{\DefinitionStyle}
\fi

\ePrints{4975-6381,1506.00061,7287-9339,8428-0408,8525-2526,2207.06506,1601.03259,5148-4632}%
\Items{2307.09982,5410-9916,9835-2163,0767-8264,5284-0163,1801.01628,MAlgebra4}%
\Items{0906.0135}%
\ifx\Semafor\ValueOn%
\Section{Представление универсальной алгебры}
\labelSection{Representation of Universal Algebra}

\ShowDefinition{representation of algebra}

Мы будем также пользоваться записью
\ShowEq{f:A->*B}f{A_1}{A_2}
для обозначения представления $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.

\begin{\DefinitionStyle}
\labelDefinition{effective representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{эффективным}{effective representation},\,\footnotemark
если отображение
\ShowEq{representation of algebra}
является изоморфизмом $\Omega_1$\Hyph алгебры $A_1$ в
\ShowEq{End O2}{A_2}.
\end{\DefinitionStyle}
\footnotetext{\,
Аналогичное определение эффективного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16,
\citeBib{Basic Concepts of Differential Geometry}, страница 111,
\citeBib{Cohn: Algebra 1}, страница 51
(Кон называет такое представление точным).
}

\ePrints{2307.09982,5148-4632}
\ifx\Semafor\ValueOn

\begin{\TheoremStyle}
\labelTheorem{representation is effective}
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только, когда из утверждения
\ShowEq{a1 ne b1}
следует существование
\ShowEq{a in A}2{}
такого, что\,\footnotemark
\ShowEq{fam ne fbm}
\end{\TheoremStyle}
\footnotetext{\,
Для группы теорема
\RefTheorem{representation is effective}
имеет следующий вид.
{\it
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
эффективно тогда и только тогда, когда для любого $A_1$\Hyph числа $a\ne e$
существует
\ShowEq{a in A}2{}
такое, что
\ShowEq{fam ne m}
}
}
\ProofTheorem{\RefRepresentation}{representation is effective}
\fi

\ePrints{1506.00061,7287-9339,5284-0163,1801.01628,8525-2526,2207.06506,8428-0408,0906.0135}%
\ifx\Semafor\ValueOn%
\begin{\DefinitionStyle}
\labelDefinition{free representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},\,\footnotemark
если из утверждения
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2{}
следует, что $a=b$.
\end{\DefinitionStyle}
\footnotetext{\,
Аналогичное определение свободного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16.
}

\ePrints{1506.00061,7287-9339}%
\ifx\Semafor\ValueOff%
\begin{\TheoremStyle}
\labelTheorem{Free representation is effective}
Свободное представление эффективно.
\end{\TheoremStyle}
\ProofTheorem{\RefRepresentation}{Free representation is effective}

\begin{remark}
Представление группы вращений в аффинном пространстве эффективно,
но не свободно, так как начало координат
является неподвижной точкой любого преобразования.
\qed
\end{remark}

\begin{\DefinitionStyle}
\labelDefinition{transitive representation of algebra}
Мы будем называть представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph алгебры
\AddIndex{транзитивным}{transitive representation of algebra},\,\footnotemark
если для любых
\ShowEq{ab in A}2{}
существует такое $g$, что
\[a=f(g)(b)\]
Мы будем называть представление $\Omega_1$\Hyph алгебры
\AddIndex{однотранзитивным}{single transitive representation of algebra},
если оно транзитивно и свободно.
\end{\DefinitionStyle}
\footnotetext{\,
Аналогичное определение транзитивного представления группы смотри в
\citeBib{Basic Concepts of Differential Geometry}, страница 110,
\citeBib{Cohn: Algebra 1}, страница 51.
}

\ShowTheorem{Representation is single transitive iff}
\ShowProof{Representation is single transitive iff}

\ShowTheorem{single transitive representation generates algebra}
\ProofTheorem{\RefRepresentation}{single transitive representation generates algebra}
\fi
\fi

\ShowDefinition{morphism of representations of universal algebra}

\ShowRemark{morphism of representations of universal algebra as map}

\ePrints{5148-4632,2307.09982,8428-0408,8525-2526,2207.06506,5284-0163,1801.01628,0906.0135}
\ifx\Semafor\ValueOn

\ShowRemark{notation for morphism of representations}

\ShowTheorem{Tuple of maps is morphism of representations iff}
\ProofTheorem{\RefRepresentation}{Tuple of maps is morphism of representations iff}

\ShowRemark{morphism of representations of universal algebra}
\fi

\ShowDefinition{morphism of representation f}

\ePrints{aa}%2307.09982,5148-4632}
\ifx\Semafor\ValueOn

\ShowTheorem{unique morphism of representations of universal algebra}
\ProofTheorem{\RefRepresentation}{unique morphism of representations of universal algebra}

\ShowDefinition{transformation coordinated with equivalence}

\ShowTheorem{transformation correlated with equivalence}
\ProofTheorem{\RefRepresentation}{transformation correlated with equivalence}

\ShowTheorem{decompositions of morphism of representations}
\ProofTheorem{\RefRepresentation}{decompositions of morphism of representations}
\fi

\ShowDefinition{reduced morphism of representations}

\ShowTheorem{map is reduced morphism of representations iff}
\ProofTheorem{\RefRepresentation}{map is reduced morphism of representations iff}
\fi

\ePrints{8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOn

\ShowDefinition{category of representations A1(mA2)}

\ShowTheorem{product of effective representations}
\ProofTheorem{\RefRepresentation}{product of effective representations}
\fi

\ePrints{5148-4632,2307.09982,5410-9916,8428-0408,8525-2526,2207.06506,5284-0163,1801.01628,MAlgebra4}
\ifx\Semafor\ValueOn
\Input{Preliminary.Omega}
\fi

\ePrints{2307.09982,5148-4632,8428-0408,8525-2526,2207.06506,5284-0163,1801.01628,MAlgebra4,0906.0135}
\ifx\Semafor\ValueOn

\Section{Базис представления универсальной алгебры}

\ShowDefinition{stable set of representation}

\ShowTheorem{subrepresentation of representation}
\ProofTheorem{\RefRepresentation}{subrepresentation of representation}

\ShowTheorem{lattice of subrepresentations}
\ProofTheorem{\RefRepresentation}{lattice of subrepresentations}

\ShowRemark{closure operator, representation}

\ShowDefinition{generating set of representation}

\ShowTheorem{structure of subrepresentations}
\ProofTheorem{\RefRepresentation}{structure of subrepresentations}

\ePrints{2307.09982,5148-4632,8428-0408,8525-2526,2207.06506,5284-0163,1801.01628}
\ifx\Semafor\ValueOn
\ShowDefinition{word of element relative to set, representation}

\ShowTheorem{map of words of representation}
\ProofTheorem{\RefRepresentation}{map of words of representation}

\ShowDefinition{quasibasis of representation}

\ShowTheorem{X is quasibasis of representation}
\ProofTheorem{\RefRepresentation}{X is quasibasis of representation}

\ShowRemark{X is quasibasis of representation}

\ShowRemark{representation in form of Omega2-word is ambiguous}

\ShowRemark{three reasons of ambiguity in Omega2-word}

\ShowDefinition{equivalence on the set of Omega2-words}

\ShowTheorem{equivalence generated by basis}
\ProofTheorem{\RefRepresentation}{equivalence generated by basis}

\ShowDefinition{basis of representation}
\else
\begin{\DefinitionStyle}
\labelDefinition{basis of representation}
Если множество $X\subset A_2$ является множеством образующих
представления $f$, то любое множество $Y$, $X\subset Y\subset A_2$
также является множеством образующих представления $f$.
Если существует минимальное множество $X$, порождающее
представление $f$, то такое множество $X$ называется
\AddIndex{базисом представления}{basis of representation} $f$.
\qed
\end{\DefinitionStyle}

\begin{\TheoremStyle}
\labelTheorem{X is basis of representation}
Множество образующих $X$ представления $f$ является базисом
тогда и только тогда, когда для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
\end{\TheoremStyle}
\ProofTheorem{\RefRepresentation}{X is basis of representation}

\begin{remark}
\labelRemark{X is basis of representation}
Доказательство теоремы
\RefTheorem{X is basis of representation}
даёт нам эффективный метод построения базиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить базис этого представления.

Как отметил Кон в 
\citeBib{Cohn: Universal Algebra}, cтр. 96, 97,
представление может иметь неэквивалентные базисы.
Например, циклическая группа шестого порядка имеет
базисы $\{a\}$ и $\{a^2,a^3\}$, которые нельзя отобразить
один в другой эндоморфизмом представления.
\qed
\end{remark}
\fi

\ePrints{0906.0135}
\ifx\Semafor\ValueOff
\ShowTheorem{automorphism uniquely defined by image of basis}
\ProofTheorem{\RefRepresentation}{automorphism uniquely defined by image of basis}
\fi
\fi

\ePrints{2307.09982,5148-4632,8428-0408,8525-2526,2207.06506,0906.0135}
\ifx\Semafor\ValueOn

\Section{Диаграмма представлений универсальных алгебр}

\ShowDefinition{diagram of representations}

\ShowRemark{diagram of representations}

\ShowDefinition{commutative diagram of representations}

Мы можем проиллюстрировать определение
\RefDefinition{diagram of representations}
с помощью теоремы
\RefTheorem{diagram of representations, define map fik}.

\ShowTheorem{diagram of representations, define map fik}
\ProofTheorem{\RefRepresentation}{diagram of representations, define map fik}

\ShowDefinition{Morphism of Diagram of Representations}

\ShowRemark{Morphism of Diagram of Representations}
\fi

\ePrints{2307.09982,5148-4632,4975-6381,1601.03259,309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
\Section{Перестановка}

\begin{\DefinitionStyle}
{\it
Инъективное отображение конечного множества в себя называется
\AddIndex{перестановкой}{permutation}.\,\footnotemark
}
\qed
\end{\DefinitionStyle}
\footnotetext{\,
Смотри определение и свойства перестановки в
\citeBib{Kurosh: High Algebra}, страницы 28 - 32,
\citeBib{Cohn: Algebra 1}, страницы 58, 59.
}

Обычно перестановку $\sigma$ мы записываем в виде матрицы
\ShowEq{permutation as matrix}
Запись
\EqRef{permutation as matrix}
перестановки эквивалентна утверждению
\ShowEq{a->sigma a}
Поэтому порядок столбцов в записи
\EqRef{permutation as matrix}
несущественен.

Если на множестве
\ShowEq{set a1n}{}
задан некоторый порядок
(например, мы предполагаем, что $a_i$ предшествует $a_j$,
если $i<j$),
то мы можем подразумевать, что элементы первой строки
записаны согласно предполагаемому порядку
и будем отождествлять перестановку со второй строкой
\ShowEq{permutation as matrix 2}

\ShowDefinition{parity of permutation}
\fi

\ShowEq{PreliminaryRefOff}


==> Prolog.Cite.Russian.tex <==
%auto-ignore

\DefCiteBib{1302.7204}
{
Александр Клейн,
Многочлен над ассоциативной $D$-алгеброй,\\
eprint \href{http://arxiv.org/abs/1302.7204}{arXiv:1302.7204} (2013)
}

\DefCiteBib{1801.01628}
{
Александр Клейн,
Дифференциальное уравнение над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1801.01628}{arXiv:1801.01628} (2018)
}

\DefCiteBib{1908.04418}
{
Александр Клейн,
Диаграмма представлений универсальных алгебр,\\
eprint \href{http://arxiv.org/abs/1908.04418}{arXiv:1908.04418} (2019)
}

\DefCiteBib{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М.,
Наука, 1974
}

\DefCiteBib{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}

\DefCiteBib{1502.04063}
{
Александр Клейн,
Линейное отображение $D$\Hyph алгебры,\\
eprint \href{http://arxiv.org/abs/1502.04063}{arXiv:1502.04063} (2015)
}

\DefCiteBib{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}

\DefCiteBib{1601.03259}
{
Александр Клейн,
Введение в математический анализ над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1601.03259}{arXiv:1601.03259} (2016)
}

\DefCiteBib{2207.06506}
{
Александр Клейн,
Введение в некоммутативную алгебру,
Том 1, Алгебра с делением\\
eprint \href{http://arxiv.org/abs/2207.06506}{arXiv:2207.06506} (2022)
}


==> Prolog.Russian.tex <==
%auto-ignore
\ifx\setCACAA\Defined
\maketitle
\input{Prolog.Eq}
\Input{Abstract.\BookNumber}
%\tableofcontents
\Input{Preface.\BookNumber}
\else
\Prolog
\fi

\DefText{converse theorem is also true}
{
Обратная теорема также верна.
}

\DefText{Preliminary Definitions}
{
\ifx\PrintBook\undefined
В этом разделе
\else
В этой главе
\fi
собраны определения и теоремы,
которые необходимы для понимания текста предлагаемой
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi
Поэтому читатель может обращаться к утвердениям из
\ifx\PrintBook\undefined
этого раздела
\else
этой главы
\fi
по мере чтения основного текста
\ifx\PrintBook\undefined
статьи.
\else
книги.
\fi
}

\ePrints{4975-6381,6860-2955}%
\Items{5410-9916,9835-2163,7287-9339,309618526,CACAA.06.121,0767-8264}
\ifx\Semafor\ValueOn%
\Chapter{Предварительные определения}

\ShowText{Preliminary Definitions}
\fi

\ShowText{Preliminary.Representation}


==> Statement.Russian.tex <==
%auto-ignore

\def\OneTheorem{теоремы }
\def\ManyTheorems{теорем }

\newenvironment{ProofRef}[2]{%
\def\TheoremList{theorem}
\def\TheoremRef{}

{\sc Доказательство теоремы}
\def\Temp{}%
\edef\Tempa{#2}%
\ifx\Tempa\Temp%
\RefTheorem{#1}.
\else
\refTheorem{#1}{#2}.
\fi
}%
{\qed}

\author{Александр Клейн}
\ifx\setCACAA\undefined
\newtheorem{theorem}{Теорема}[section]
\newtheorem{corollary}[theorem]{Следствие}
\newtheorem{example}[theorem]{Пример}
\newtheorem{definition}[theorem]{Определение}
\newtheorem{remark}[theorem]{Замечание}
\newtheorem{question}[theorem]{Вопрос}
\newtheorem{summary}[theorem]{Сводка результатов}
%\theoremstyle{lemma}
\newtheorem{lemma}[theorem]{Лемма}
\else
\theoremstyle{definition}
\theoremstyle{remark}
\fi
\newtheorem{Statement}[theorem]{Утверждение}
\newtheorem{convention}[theorem]{Соглашение}
\newtheorem{xca}[theorem]{Exercise}
\ifx\PrintBook\undefined
\newcommand{\BibTitle}{%
\section{Список литературы}%
}
\else
\newcommand{\BibTitle}{%
\chapter{Список литературы}%
}
\fi


==> Stmt.2023.01.07.Russian.tex <==
%auto-ignore
\input{Stmt.2023.01.07.Eq}
 
\DefText{Vector space as direct sum of basis}
{
Пусть $V$ - \SideRu вое $A$\Hyph векторное пространство столбцов
размерности $\gin$.
Пусть
\ShowEq{basis e of V}
- базис $A$\Hyph векторного пространства $V$.
Для любого $\gii$ множество
\ShowEq{Aei \SideNS}
является подпространством $A$\Hyph векторного пространства $V$.
$A$\Hyph векторное пространство $V$
является прямой суммой $A$\Hyph векторных пространств
\ShowEq{Aei \SideNS}
\ShowEq{V=V1o+...o+Vn \SideNS}
}

\DefText{homomorphisms, non-associative algebra}
{
Если $U$, $V$, $W$ - \SideRu вые модули \ColsA над
неассоциативной алгеброй $A$,
то равенство
\ShowEq{product of homomorphisms, non-associative \SideNS-\Cols}
является следствием теоремы
\refTheorem{product of homomorphisms is homomorphism, A vector space}{\SideNS}.
Однако равенство
\EqRef{product of homomorphisms, non-associative \SideNS-\Cols}
является теоремой существования,
так как у нас нет механизма определить матрицу $f$.
}

\DefText{product of linear maps has form}
{
Пусть линейное отображение
\ShowEq{f:A->B}aAA
имеет представление
\DrawEq[as]{a o x=...}a
и линейное отображение
\ShowEq{f:A->B}bAA
имеет представление
\DrawEq[bt]{a o x=...}b
Тогда произведение отображений $a$ и $b$ имеет вид
\ShowEq{a o b o x=...}
}

\DefTheorem{We can identify linear map}
{
Мы можем отождествить линейное отображение
\ShowEq{f:A->B}aAA
$D$\Hyph алгебруы $A$
и тензор
\ShowEq{a0 ox a1}
посредством равенства
\ShowEq{a0 ox a1 o x}
}


==> Stmt.Fiber.Russian.tex <==
%auto-ignore
\input{Stmt.Fiber.Eq}

\DefDefinition{Bundle}
{
Расслоение
\ShowSymb{bundle}
- это проекция
топологического пространства $E$
на топологическое пространство $M$.
Множество $M$ называется базой расслоения.
Прообраз точки множества $M$ называется слоем,
и разные слои гомеоморфны.
Мы будем отождествлять непрерывное отображение $\bundle{}pE{}$
и расслоение \EqRef{def symb bundle}.
}

\DefDefinition{fibered module}
{
Расслоенный $A$\Hyph модуль - это расслоение $\bundle{}pV{}$,
слоем которого является нормированный $A$\Hyph модуль $V$
и операция в модуле непрерывно зависит от слоя.
}

\DefDefinition{product range matrices}
{
Пусть $A$ - коммутативная алгебра.
Пусть множество значений индекса столбцов матрицы $a$
совпадает с множество значений индекса строк матрицы $b$.
Произведение матриц $a$ и $b$ имеет вид
\ShowEq{product range matrices}
}

\DefDefinition{row over column range product}
{
Пусть $A$ - некоммутативная алгебра.
Пусть множество значений индекса столбцов матрицы $a$
совпадает с множество значений индекса строк матрицы $b$.
\AddIndex{\RC произведение}{rc-product}
матриц $a$ и $b$ имеет вид
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
\ShowEq{entry rc-product of matrices}
\ShowEq{rc-product, matrices}
\RC произведение может быть выражено как произведение строк матрицы $a$
и столбцов матрицы $b$.
}

\DefDefinition{column over row range product}
{
Пусть $A$ - некоммутативная алгебра.
Пусть множество значений индекса строк матрицы $a$
совпадает с множество значений индекса столбцов матрицы $b$.
\AddIndex{\CR произведение}{cr-product}
матриц $a$ и $b$ имеет вид
\ShowEq{cr-product}
\ShowEq{cr-product of matrices}
\ShowEq{entry cr-product of matrices}
\ShowEq{cr-product, matrices}
\CR произведение может быть выражено как произведение столбцов матрицы $a$
и строк матрицы $b$.
}

\DefLabeledDefinition{continuous Schauder quasi-basis}{\Base-\SideNS}
{
Пусть $V$ -
\SideRuTo $\Base$\Hyph модуль,
представленный как
прямая сумма
\DrawEq{Continuous module as direct sum}{\Base-\SideNS}
копий \algebrae $\Base$.
Рассмотрим непрерывное отображение
\ShowEq{continuous Schauder quasi-basis}
такое, что
\DrawEq{Schauder quasibasis of left module}{\Base-\SideNS}
где почти всюду множество
\DrawEq[\Base]{eA= iI}{\Base-\SideNS}
является
\def\tempa{A}%
\ifx\tempa\Base%
\SideRu вым
\fi%
квазибазисом \algebrae $\Base$.
Тогда отображение \eV
является квазибазисом
\def\tempa{A}%
\ifx\tempa\Base%
\SideRu вого
\fi%
$\Base$\Hyph модуля $V$.

Если \SideRuTo квазибазис \algebrae $\Base$
является базисом, то отображение \eV также является базисом.
}

\DefLabeledFootnote[6]{homomorphism of A module MCB}{\SideNS-\Cols(#1#2#3)}
{
В теоремах
\refTheorem{homomorphism A module MCB}{\SideNS-\Cols(#1#2#3)},
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)},
мы опираемся на следующее соглашение.
\ShowEq{prolog homomorphism of vector space MCB(#1#2#3)}{#1}{#2}{#3}{#4}{#5}{#6}
}

\DefText[6]{Let be quasibasis of module MCB}
{
Пусть множество векторов
\DrawEq[{#1_i}{#2}{#3}]{basis ei of MCB module #5}{#6}
является квазибазисом \SideRu вого $#4$\Hyph \VectorSetRuB $#1_i$.%
}

\DefLabeledTheorem[6]{homomorphism A module MCB}{\SideNS-\Cols(#1#2#3)}
{
Гомоморфизм\refFootnote{homomorphism of A module MCB}{\SideNS-\Cols(#1#2#3)}
%\ShowRef{homomorphism A module}{#1}{#2}{#3}{\Vector g}{\Vector f}
\DrawEq[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{\SideNS-\Cols}
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB \ColsA $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA \ColsA $V_{#6}$
имеет представление
\ShowText{g:A1->A2, D module(#1#2#3)}{}
\ShowText{f o (ae)=a o f e MCB(#2#3)}{#1}{#2}{#3}
относительно выбранных базисов.
Здесь
\begin{itemize}
\ShowText{homomorphism of vector space, algebra(#2)}{#1}{#2}{#3}{#4}{#5}{#6}{}
\ShowText{homomorphism of vector space, algebra 1 MCB}{#1}{#2}{#3}{#4}{#5}{#6}
\end{itemize}
\ShowText{matrix of homomorphism relative bases MCB #2#3}{#1}{#2}{#3}{#5}
}

\DefText[4]{matrix of homomorphism relative bases MCB 1}
{
Для заданного гомоморфизма $\Vector f$
матрица $f$ почти всюду определена однозначно и называется
{\bf матрицей гомоморфизма}
$\Vector f$
относительно базисов \eV[1][,] \eV[2][.]
}

\DefLabeledTheorem[6]{matrix generates A module homomorphism MCB}{\SideNS-\Cols(#1#2#3)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrices of numbers MCB(#2#3)}{#4}{#5}{#1}{#2}%
\ShowText{matrix generates A module homomorphism MCB}{#1}{#2}{#3}{#4}{#5}{#6}
{\refFootnote{homomorphism of A module MCB}{\SideNS-\Cols(#1#2#3)}}
Гомоморфизм
\ShowRef{homomorphism A module}{#1}{#2}{#3}{\Vector g}{\Vector f}
который имеет%
\ShowText{define homomorphism by given matrix(#2)}%
определён однозначно.
}

\DefText[7]{matrix generates A module homomorphism MCB}
{
Отображение#7
\ShowRef{homomorphism A module}{#1}{#2}{#3}{\Vector g}{\Vector f}
\ShowText{equality #2#3}
\ShowText{define homomorphism A module by matrix MCB(#1#2#3)}
является гомоморфизмом
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB \ColsA $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA \ColsA $V_{#6}$.
}

\DefText[7]{matrix of numbers MCB}
{
Пусть
\ShowEq{matrix fIJ MCB}{#3}{#4}{#5}{#6}{#7}
матрица $#1_{#2}$\Hyph чисел.
}

\DefText[6]{coordinates of the linear map 4 MCB}
{
\item $#1$ - координатная матрица множества $#2_2$\Hyph чисел
\ShowEq{Vector f(e1) module MCB}#1{#3}#5#6
относительно базиса \eV[#4][.]
}

\DefLabeledDefinition{Continuous Schauder Basis}{\Base-\SideNS}
{
Пусть $V$ -
\SideRuTo $\Base$\Hyph модуль.
Пусть $\giI$ - конечное множество.
Отображение
\ShowEq{Continuous Schauder Basis}
называется
{\bf непрерывным базисом Шаудера}
\SideRu\From $\Base$\Hyph модуля $V$,
если из равенства
\DrawEq{aiei=0 CSB}{\Base-\SideNS}
следует, что
\[\aU a{ki}=0\]
почти всюду.
}

\DefRemark{Continuous Schauder Basis}
{
Я напомню, что согласно соглашению Эйнштейна о сумме,
равенство
\eqRef{aiei=0 CSB}{\Base-\SideNS}
имеет вид
\ShowEq{int aiei=0 CSB}
Здесь мы видим существенное отличие от модуля конечной размерности.
Мы требуем, чтобы координаты вектора относительно базиса
модуля конечной размерности были определены однозначно.
Однако мы не можем потребовать этого для вектора
модуля с непрерывным базисом Шаудера.
}

\DefTheorem{Continuous module as direct sum}
{
$A$\Hyph модуль с
непрерывным базисом Шаудера
может быть представлен как прямая сумма
\DrawEq{Continuous module as direct sum}{}
копий алгебры $A$.
}

\DefText{Continuous module as direct sum}
{
Теорема
\RefTheorem{Continuous module as direct sum}
даёт возможность обобщить определение
\refDefinition{Continuous Schauder Basis}{\Base-\SideNS}.
Если $A$\Hyph модуль $V$ имеет конечную размерность,
то мы можем отождествить $V$\Hyph число и
матрицу $A$\Hyph чисел.
Мы можем рассмотреть эту модель
для $A$\Hyph модуля с
непрерывным базисом Шаудера.
}

\DefLabeledTheorem{Continuous Schauder Basis}{\Base-\SideNS}
{
Пусть $V$ -
\SideRu вый $\Base$\Hyph модуль с
непрерывным базисом Шаудера.
Координаты вектора $v\in V$
относительно базиса \eV
\DrawEq{v=viei CSB}{\Base-\SideNS}
определены однозначно почти всюду.
}

\DefText{Matrix with Continuous Indices}
{
Элемент матрицы $a$ имеет вид $\aUD aij$,
где $\gi i$ - индекс, нумерующий строки,
и $\gi j$ - индекс, нумерующий столбцы.
Множество значений индекса может быть конечным,
счётным или может иметь мощность континуума.

Если аргумент $x$ отображения $f$
принадлежит множеству мощности континуума,
мы обычно пишем значение отображения $f$ в точке $x$
в виде $f(x)$.
Поэтому мы не можем представить матрицу как таблицу элементов.
Тем не менее, мы можем по-прежнему рассматривать
элементы матрицы с заданным индексом
как строку или столбец матрицы.
Поэтому мы сохраним структуру записи для элементов матрицы
и запишем
значение отображения $f$ в точке $x$
в виде $\aU fx$ либо $\aD fx$.

Мы будем пользоваться соглашением Эйнштейна о сумме,
в котором повторяющийся индекс (один вверху и один внизу)
подразумевает сумму по повторяющемуся индексу
\ShowEq{sum aibi}
\begin{itemize}
\item
Если множество значений индекса счётно,
то мы будем полагать, что множество слагаемых,
отличных от нуля, конечно.
Если $A$ - банаховая алгебра,
то мы ослабим требование к слагаемым
и будем требовать, чтобы сумма сходилась.
\item
Если множество значений индекса - непрерывное множество,
то мы полагаем, что дифференцируемое многообразие
является множество значений индекса,
и вместо суммы мы пишем интеграл
по области значения индекса.
Мы распространим соглашение Эйнштейна о сумме
и будем подразумевать интеграл по повторяющемуся индексу
\ShowEq{int aibi}
\end{itemize}

Это соглашение позволит записывать выражения,
которые не зависят от области значений индекса.
Смотри, например, равенства
\EqRef{sum aibi},
\EqRef{int aibi}.
Если выражение содержит индексы с разными областями определения,
то выражение может иметь вид
\ShowEq{int sum aibi}

Произведение матриц зависит от того
коммутативна алгебра $A$ или нет.
}

\DefText{M is topological space}
{
Пусть $A$, $B$ - банаховые алгебры такие,
что существует гомоморфизм
\DrawEq[fBA{}]{f: A->B}{}
Пусть $M$ является дифференциальным $B$\Hyph многообразием класса $C^1$.
Тогда геометрический объект над банаховой алгеброй $A$
является геометрическим объектом над
дифференциальным $B$\Hyph многообразием $M$.
На дифференциальном $B$\Hyph многообразии $M$ определена мера $\mu$.
}

\DefDefinition{chart}
{
Пусть $B$ - банаховая алгебра
и $M$ - топологическое пространство.
Если существует гомеоморфизм
\DrawEq[fMN{}]{f: A->B}{}
где $N$ - выпуклое множество пространства \aU Bn,
то гомеоморфизм $f$ называется
\AddIndex{картой}{chart}
множества $M$.
}

\DefRemark{chart}
{
Если отображение
\ShowEq{local map}{}
является картой множества $M$,
то каждой точке $m\in M$
можно сопоставить кортеж
\ShowEq{tuple aU1n}m{}
$B$\Hyph чисел,
который однозначно определяет точку $m$.
}

\DefTheorem{chart coordinate basis}
{
Пусть отображение
\ShowEq{local map}{}
является картой множества $M$.
Множество производных
\ShowEq{chart coordinate basis}
}

\DefProof{chart coordinate basis}
{
}

\DefRemark{2 charts}
{
Если существует две карты
\ShowEq{local map}1
\ShowEq{local map}2
то отображение $f$ на коммутативной диаграмме
\DrawEq{simple manifold}1
является гомеоморфизмом.
Гомеоморфизм $f$ может быть представлен
в виде системы равенств
\ShowEq{simple manifold f}
где
\ShowEq{simple manifold x}x1,
\ShowEq{simple manifold x}y2.
Если отображения
\ShowEq{aU A1n}fn{}
имеют производные порядка $k$,
то отображение $f$ называется
\AddIndex{диффеоморфизмом}{diffeomorphism}
класса $C^k$.
}

\DefDefinition{simple manifold}
{
Пусть $B$ - банаховая алгебра.
Множество $M$ называется
\AddIndex{элементарным $B$\Hyph многообразием}{simple manifold}
класса $C^k$,
если для любых двух карт $f_1$, $f_2$
отображение $f$ на коммутативной диаграмме
\newline
\FrameEqRef{simple manifold}1
\newline
является диффеоморфизмом класса $C^k$.
}

\DefDefinition{differential manifold}
{
Топологическое пространство $M$ называется
\AddIndex{дифференциальным $B$\Hyph многообразием}{differential manifold}
класса $C^k$
если топологическое пространство $M$
является объединением элементарных $B$\Hyph многообразий
\ShowEq{set Ai}M
и пересечение
$M_i\cap M_j$
элементарных $B$\Hyph многообразий
$M_i$, $M_j$
так же является элементарным $B$\Hyph многообразием.
}

\DefTheorem{fibered module}
{
Расслоенный модуль является прямой суммой слоёв.
}


==> Stmt.Module.Russian.tex <==
%auto-ignore
\input{Stmt.Module.Eq}

\DefExample{Abelian Group is Z module}
{
Из теорем
\refTheorem{action of ring of rational integers in Abelian group}{+},
\refTheorem{Abelian group is free}{+}
и определения
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
следует, что свободная абелевая группа $G$ является модулем над кольцом целых чисел $Z$.
}

\DefText[2]{ix-xi-1 roots}
{
многочлен
\DrawEq[1]{ix-xi-1}{#1}
не имеет корней
и многочлен
\DrawEq[k]{ix-xi-1}{#2}
имеет множество корней
\DrawEq{x=c12+j}{#2}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{module over ring}
Пусть коммутативное кольцо $D$ имеет единицу $1$.
Эффективное представление
\DrawEq{D->*V}{def}
кольца $D$
в абелевой группе $V$
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
Эффективное представление
\eqRef{D->*V}{def}
поля $D$ в абелевой группе $V$
называется
\AddIndex{векторным пространством над полем}{vector space over field} $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\end{ShadedDefinition}
}
{... definition: module over ring}
%\DefEq

\DefTheorem{tensor product of D-algebras is D-algebra}
{
Пусть
\ShowEq{A1...n}
- $D$\Hyph алгебры.
Тензорное произведение
$\Tensor A$
$D$\Hyph модулей
\ShowEq{A1...n}
является $D$\Hyph алгеброй,
если мы определим произведение согласно правилу
\ShowEq{xA1n*xA1n->oxA1n=}
}

\DefTheorem{representation of algebra H2 in LH}
{
Пусть произведение в алгебре
\AoxA H
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{RH}
Представление
\DrawEq[RH]{h:AoxA->L(A)}H
$R$\Hyph алгебры
\AoxA H
в абелевой группе
\ShowEq{L(A->B)}RHH,
определённое равенством
\DrawEq[RH]{representation AA in LA}{RH}
является левым \BoxB{H}модулем.
Если мы положим $g=E$,
где
\ShowEq{product in algebra AA 3}RHE
- тождественное отображение,
то мы можем отождествить линейное отображение
\DrawEq[fHH{}]{f: A->B}-
алгебры кватернионов и тензор
\DrawEq{linear map f, basis E}1
опираясь на равенство
\ShowEq{value of linear map f, basis E}
}

\DefProof{representation of algebra H2 in LH}
{
Теорема является следствием утверждения
что отображение
\ShowEq{Eox=x}
порождает любое линейное отображение алгебры кватернионов
}

\DefDefinition{square root}
{
Решение
\ShowEq{square root}
уравнения
\DrawEq{x2=a}{root}
в $D$\Hyph алгебре $A$
называется
\AddIndex{квадратным корнем}{square root}
$A$\Hyph числа $a$.
}

\DefDefinition{polynomial*polynomial}
{
Билинейное отображение
\ShowEq{polynomial*polynomial}
определено равенством
\ShowEq{polynomial*polynomial, 1}
}

\DefTheorem{(a*b)x=(ax)(bx)}
{
Для любых тензоров
\ShowEq{a in Aoxn}a{n+1},
\ShowEq{a in Aoxn}b{m+1}{},
произведение однородных многочленов
\ShowEq{polynomials a o x,b o x}
определено равенством
\ShowEq{(a*b)x=(ax)(bx)}
}

\DefTheorem{x2=a quaternion root}
{
Пусть $H$ - алгебра кватернионов и $a$ - $H$\Hyph число.
\StartLabelItem
\begin{enumerate}
\item
Если
\ShowEq{Re sqrt a ne 0}
то уравнение
\DrawEq{x2=a}{}
имеет корни
\ShowEq{x=x12}
такие, что
\ShowEq{x2=-x1}
\labelItem{Re sqrt a ne 0}
\item
Если $a=0$, то уравнение
\DrawEq{x2=a}{}
имеет корень $x=0$ кратности $2$.
\labelItem{a=0}
\item
Если условия
\RefItem{Re sqrt a ne 0},
\RefItem{a=0}
не верны,
то уравнение
\DrawEq{x2=a}{}
имеет бесконечно много корней таких, что
\ShowEq{|x|=sqrt a}
\labelItem{Re sqrt a=0}
\end{enumerate}
}

\DefDefinition{polylinear map of algebras, property}
{
Полилинейное отображение $D$\Hyph алгебры $A$
\ShowEq{f:A->B}f{A^n}A
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{1}
\DrawEq[f]{f(pai)=pfai}{1}
\ShowEq{polylinear map of algebras, 1}AD
Обозначим
\ShowEq{set polylinear maps An}DAA
множество $n$\hyph линейных отображений
$D$\Hyph алгебры $A$.
}

\DefRemark{monomial of power k}
{
В теореме
\RefTheorem{monomial of power k}
я рассмотрел рекурсивное представление одночлена в ассоциативной $D$\Hyph алгебре.
Так как скобки в произведении
я могу расставить произвольно,
то в ассоциативной $D$\Hyph алгебре
рекурсивное представление одночлена неоднозначно.
Например, одночлен $ax^2bxcx^3d$
может быть записан в любой из следующих форм
\ShowEq{ax^2bxcx^3d}
Я выбрал равенство
\EqRef{monomial of power k, F=1}
как самое простое для алгоритма деления многочленов.
}

\DefTheorem{monomial of power k}
{
Пусть $p_k(x)$ -
\AddIndex{одночлен степени}{monomial of power} $k$
над ассоциативной $D$\Hyph алгеброй $A$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Одночлен степени $0$ имеет вид
\ShowEq{p0(x)=a0}
\item
Если $k>0$, то
\labelItem{monomial of power k}
\ShowEq{monomial of power k, F=1}
где $a_k\in A$.
\end{enumerate}
}

\DefProof{monomial of power k}
{
Мы докажем утверждение теоремы индукцией по степени
$n$ одночлена.

Пусть $n=0$.
Так как одночлен $p_0(x)$ является константой,
то мы получаем утверждение
\RefItem{monomial of power 0}.

Пусть $n=k$. Последний множитель одночлена $p_k(x)$ является либо $a_k\in A$,
либо имеет вид $x^l$, $l\ge 1$.
В последнем случае мы положим $a_k=1$.
Множитель, предшествующий $a_k$, имеет вид $x^l$, $l\ge 1$.
Мы можем представить этот множитель в виде $x^{l-1}x$.
Следовательно, утверждение доказано.
}

\DefTheorem{r=+q circ p}
{
Пусть
\ShowEq{p=p circ x}
- многочлен степени $1$ и $p_1$ - невырожденный тензор.
Пусть
\ShowEq{r power k}
многочлен степени $k$.
Тогда
\ShowEq{r=+q circ p}
где
\ShowEq{qij i j}
- однородный многочлен степени $i$.
}

\DefText{linear map of A vector space V1->V2}
{
Из определения
\RefDefinition{linear map A module}
следует, что
линейное отображение
$A_1$\Hyph \VectorSetRuB $V_1$
в $A_2$\Hyph \VectorSetRuA $V_2$
- это линейное отображение
$D_1$\Hyph \VectorSetRuB $V_1$
в $D_2$\Hyph \VectorSetRuA $V_2$.
}

\DefLabeledDefinition{linear map of A vector space}{\SideNS}
{
\ShowText{algebra over ring ()}
Пусть $V$, $W$ - \SideRu вые векторные пространства над $D$\Hyph алгеброй $A$.
Линейное отображение
\ShowEq{f:A->B}fVW
$D$\Hyph векторного пространства $V$
в $D$\Hyph векторное пространство $W$
называется
\AddIndex{линейным отображением}{linear map}
\SideRu вого $A$\Hyph векторного пространства $V$
в \SideRu вое $A$\Hyph векторное пространство $W$.
Обозначим
\ShowEq{set linear maps, VW module}
множество линейных отображений
\SideRu вого $A$\Hyph векторного пространства $V$
в \SideRu вое $A$\Hyph векторное пространство $W$.
}

\DefDefinition{component of linear map, basis E}
{
Выражение
\ShowEq{component of linear map, basis E}
в равенстве
\eqRef{linear map f, basis E}1
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
}

\DefTheorem{representation of algebra A2 in LA}
{
Пусть $A$ является $D$\Hyph алгеброй.
Пусть произведение в $D$\Hyph модуле
\AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{}
Представление
\DrawEq[DA]{h:AoxA->L(A)}{}
$D$\Hyph алгебры
\AoxA A
в модуле
\ShowEq{L(A->B)}DAA,
определённое равенством
\DrawEq[DA]{representation AA in LA}{}
позволяет отождествить тензор
\ShowEq{d in AxoA}A
с линейным отображением
\ShowEq{product in algebra AA 2}DA{\delta},
где
\ShowEq{product in algebra AA 3}DA{\delta}
- тождественное отображение.
Линейное отображение
\ShowEq{a ox b}{\delta}
имеет вид
\DrawEq{a ox b c=}1
}

\AddEq[1]{theorem: matrices fUD I}
{
\begin{ShadedTheorem}
\labelTheorem{#1, matrices fUD I}
Отображения сопряжения
имеют
стандартное представление
\ShowEq{#1. standard representation I}
\end{ShadedTheorem}
}

\AddEq[2]{proof: matrices fUD I}
{
Согласно равенству
\EqRef{#2x= #1},
отображение сопряжения
\ShowEq{Map of Conjugation}{#2}
имеет матрицу
\ShowEq{#1. matrix I#2}
Равенство
\DrawEq[{#2}{}]{#1.fUD->fUU I}{#1#2}
является следствием равенств
\EqRef{#1.fUD->fUU},
\EqRef{#1. matrix I#2}.
}

\DefTheorem{unit of ring and Z}
{
Пусть $D$ - кольцо с единицей \(1_D\).
\StartLabelItem
\begin{enumerate}
\item
Отображение
\DrawEq[fnZ{n1_D}D]{f:a in A->b in B}{}
является гомоморфизмом кольца $Z$ в кольцо $D$
и позволяет отождествить \(Z\)\Hyph число \(n\)
и \(D\)\Hyph число \(n\,1_D\).
\labelItem{homomorphism n->n1}
\item
Кольцо \(Z/\ker f\) является подкольцом кольца $D$.
\labelItem{Z is subring of D}
\end{enumerate}
}

\DefProof{unit of ring and Z}
{
Пусть
\ShowEq{d12 in D}nZ
Равенство
\DrawEq[nD]{d1+d2 in A}{nD}
является следствием равенства
\EqRef{(m+n)a=ma+na (+)}.
Равенство
\DrawEq[nD]{d1 d2 in A}{nD}
является следствием равенств
\EqRef{product Z bilinear 1 (+)},
\EqRef{product Z bilinear 2 (+)}.
Утверждение
\RefItem{homomorphism n->n1}
является следствием равенств
\eqRef{d1+d2 in A}{nD},
\eqRef{d1 d2 in A}{nD}.
Утверждение
\RefItem{Z is subring of D}
является следствием утверждения
\RefItem{homomorphism n->n1}.
}

\DefTheorem{ring product Z bilinear}
{
Произведение в кольце $D$ билинейно над
кольцом $Z$
\ShowEq{product Z bilinear 1 (+)}
\ShowEq{product Z bilinear 2 (+)}
}

\DefTheorem{unit of algebra and ring}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с единицей \(1_A\).
\StartLabelItem
\begin{enumerate}
\item
Отображение
\DrawEq[fdD{d1_A}A]{f:a in A->b in B}{}
является гомоморфизмом кольца $D$ в центр алгебры $A$
и позволяет отождествить \(D\)\Hyph число \(d\)
и \(A\)\Hyph число \(d\,1_A\).
\labelItem{isomorphism d->d1}
\item
Кольцо \(D\) является подалгеброй алгебры $A$.
\labelItem{D is subalgebra of A}
\item
\ShowEq{D in Z(A)}
\end{enumerate}
}

\DefProof{unit of algebra and ring}
{
Пусть
\ShowEq{d12 in D}dD
Согласно утверждению
\RefItem{distributive law, module},
\DrawEq[dA]{d1+d2 in A}{dA}
Согласно определению
\RefDefinition{algebra over ring},
\DrawEq[dA]{d1 d2 in A}{dA}
Утверждение
\RefItem{isomorphism d->d1}
является следствием равенств
\eqRef{d1+d2 in A}{dA},
\eqRef{d1 d2 in A}{dA}.
Утверждение
\RefItem{D is subalgebra of A}
является следствием утверждения
\RefItem{isomorphism d->d1}.

Согласно определению
\RefDefinition{algebra over ring},
\ShowEq{ad=da in A}
Утверждение
\RefItem{D in Z(A)}
следует из равенства
\EqRef{ad=da in A}.
}

\DefTheorem{multiplication in algebra is distributive over addition}
{
Произведение в алгебре $A$ дистрибутивно по отношению к сложению
\ShowEq{(a+b)c=.}
\ShowEq{a(b+c)=.}
}

\DefProof{multiplication in algebra is distributive over addition}
{
Утверждение теоремы следует из цепочки равенств
\ShowEq{product distributive in algebra}
}

\DefText{multiplication in algebra}
{
Произведение в алгебре может быть ни коммутативным,
ни ассоциативным. Следующие определения основаны на
определениях, данным в \citeBib{Richard D. Schafer}, с. 13.
}

\DefTheoremNote{associator of algebra}
{
Пусть $A$ - алгебра над коммутативным кольцом $D$.\,\footnotemark
\ShowEq{associator of algebra, 1}
для любых $a$, $b$, $c$, $d\in A$.
}
{
Утверждение
теоремы опирается на равенство
\citeBib{Richard D. Schafer}-(2.4).
}

\DefProof{associator of algebra}
{
Равенство \EqRef{associator of algebra, 1}
следует из цепочки равенств
\ShowEq{associator of algebra, 2}
}

\DefLabeledFootnote{LR ideal}{\VectorSetNS}
{
Смотри также определение на странице
\citeBib{Serge Lang}\Hyph 75.
}

\DefLabeledDefinition{LR ideal}{\SideWS \VectorSetNS}
{
\AddIndex{\SideRuC вый идеал}{\SideWS ideal}\,\refFootnote{LR ideal}{\VectorSetNS}
$\Set_1$ \AlgebraSetRuB $\Set$
- это подгруппа аддитивной группы $\Set$
такая, что
\ShowEq{D1 D in D1}
}

\DefLabeledDefinition{ideal}{\VectorSetNS}
{
\AddIndex{Идеал}{ideal}\,\refFootnote{LR ideal}{\VectorSetNS}
- это подгруппа аддитивной группы $\Set$,
которая одновременно является левым и правым идеалами.
}

\DefText{trivial ideal}
{
Если $\Set$ - \AlgebraSetRuNS,
то множество $\{0\}$ и само $\Set$
являются идеалами,
которые мы называем тривиальными идеалами.
}

\DefLabeledTheorem{LR ideal}{\SideWS \AlgebraLabel}
{
Если $\Set_1$ является \SideRu вым идеалом
унитальн\EndB \AlgebraSetRuB $\Set$, то
\ShowEq{D1 D=D1}
}

\DefProof{LR ideal}
{
Теорема является следствием определения
\refDefinition{LR ideal}{\SideWS \VectorSetNS}
и равенства
\ShowEq{D1 1=D1}
}

\DefDefinition{module over commutative ring}
{
Эффективное представление коммутативного кольца $D$
в абелевой группе $V$
\DrawEq{D->*V}{module}
называется
\AddIndex{модулем над кольцом}{module over ring} $D$
или
\AddIndex{$D$\Hyph модулем}{D module}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
\ePrints{309618526,CACAA.06.121}
\ifx\Semafor\ValueOn
Если $D$ - поле, то абелевая группа $V$
называется
\AddIndex{векторным пространством}{vector space} над полем $D$
или
\AddIndex{$D$\Hyph векторным пространством}{D vector space}.
\fi
}

\DefDefinition{linear map of algebra}
{
\ShowEq{def DModule}
\ShowEq{=DD}
Линейное отображение
%\ShowEq{f:A->B}fHH
%алгебры кватернионов $H$
\ShowEq{f:A->B}fAA
$D$\Hyph алгебры $A$
удовлетворяет равенствам
\DrawEq[fab]{f(a+b)=...}{D }
\DrawEq[{}fa]{f(da)=h... module}{module}
\ShowEq{D ab in A, d in D}DA
Обозначим
%\ShowEq{set linear maps, module}RHH
\ShowEq{set linear maps, module}DAA
множество линейных отображений
%алгебры кватернионов $H$.
$D$\Hyph алгебры $A$.
}

\DefLabeledDefinitionNote{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}
{
Копроизведение в категории
\scSide $\Base$\Hyph \CatModule
называется
\AddIndex{прямой суммой}{direct sum}.\,\footnotemark
Мы будем пользоваться записью
\ShowEq{direct sum of modules}{\Module}{\ModuleA}
для прямой суммы \SideRu\TO $\Base$\Hyph \VectorsSetRuB $\Module$ и $\ModuleA$.
}{
Смотри так же определение
прямой суммы модулей в
\citeBib{Serge Lang},
страница 98.
Согласно теореме 1 на той же странице, прямая сумма модулей существует.
}

\DefText{category of modules}
{
Пусть
\scSide $\Base$\Hyph \CatModule
- категория \SideRu\TO $\Base$\Hyph \VectorsSetRuB,
морфизмы которой - это гомоморфизмы $\Base$\Hyph модуля.
}

\DefLabeledTheoremNote{direct sum of D modules 2024}{\SideWS \Base-\VectorsSetNS}
{
В категории
\scSide $\Base$\Hyph \CatModule
существует прямая сумма
\SideRu\TO $\Base$\Hyph \VectorsSetRuBNS.\,\footnotemark
Пусть
\ShowEq{set Bi}{\Module}
- семейство \SideRu\TO $\Base$\Hyph \VectorsSetRuBNS.
Тогда представление
\ShowEq{\SideWS D->*o+A}{\Base}{\Module}{\ANumber}{\VNumber}
\ShortAlgebraRuBWS $\Base$
в прямой сумме абелевых групп
\ShowEq{o+Ai}{\Module}
является прямой суммой \SideRu\TO $\Base$\Hyph \VectorsSetRuB
\ShowEq{o+Ai}{\Module}
}
{
Смотри также предложение
\citeBib{Serge Lang}\Hyph 1
на странице 98.
}

\DefProof{direct sum of D modules 2024}
{
Пусть
\ShowEq{set Ai}V
- множество \SideRu\TO $\Base$\Hyph \VectorsSetRuBNS.
Пусть
\ShowEq{A=o+Ai}V
прямая сумма абелевых групп.
Пусть
\ShowEq{a=ai in A}
Мы определим действие $\Base$\Hyph числа $a$
на $V$\Hyph число $v$ согласно равенству
\DrawEq{a(vi)=(avi)}{\SideWS \Base-\VectorsSetNS}
\ShowEq{def additive}%

Согласно теореме
\refTheorem{definition of A module, property}{\SideNS},
\ShowEq{direct sum of modules i}
для любых
\ShowEq{p,q in D, v,w in V, i}
Равенства
\ShowEq{direct sum of modules ...}
являются следствием равенств
\ShowEq{module, ..., i}
для любых
\ShowEq{p,q in D, v,w in V, direct sum}

Из равенства
\eqRef{distributive law, direct sum of modules, 1}{\SideWS \Base-\VectorsSetNS}
следует, что отображение
\ShowEq{f:A->B}av{\Multiply av}
определённое равенством
\eqRef{a(vi)=(avi)}{\SideWS \Base-\VectorsSetNS},
является эндоморфизмом абелевой группы $V$.
Из равенств
\eqRef{direct sum of modules, associative law}{\SideWS \Base-\VectorsSetNS},
\eqRef{distributive law, direct sum of modules, 2}{\SideWS \Base-\VectorsSetNS}
следует, что отображение
\eqRef{a(vi)=(avi)}{\SideWS \Base-\VectorsSetNS}
является гомоморфизмом \ShortAlgebraRuBWS $\Base$ в
множество эндоморфизмов абелевой группы $V$.
Следовательно, отображение
\eqRef{a(vi)=(avi)}{\SideWS \Base-\VectorsSetNS}
является представлением \ShortAlgebraRuBWS $\Base$ в абелевой группе $V$.

Пусть $a_1$, $a_2$ - такие $\Base$\Hyph числа, что
\DrawEq{a1(vi)=a2(vi)}{\SideWS \Base-\VectorsSetNS}
для произвольного $V$\Hyph числа
\ShowEq{A=Ai iI}v.
Равенство
\DrawEq{(a1vi)=(a2vi)}{\SideWS \Base-\VectorsSetNS}
является следствием равенства
\eqRef{a1(vi)=a2(vi)}{\SideWS \Base-\VectorsSetNS}.
Из равенства
\eqRef{(a1vi)=(a2vi)}{\SideWS \Base-\VectorsSetNS}
следует, что
\DrawEq{Ai a1vi=a2vi}{\SideWS \Base-\VectorsSetNS}
Поскольку для любого \iI, $V_i$ - $\Base$\Hyph \VectorSetRuANS,
то соответствующее представление эффективно
согласно определению
\ShowRef{module over algebra \Base-\VectorSetNS}
Следовательно, равенство $a_1=a_2$ является следствием утверждения
\eqRef{Ai a1vi=a2vi}{\SideWS \Base-\VectorsSetNS}
и отображение
\eqRef{a(vi)=(avi)}{\SideWS \Base-\VectorsSetNS}
является эффективным представлением \ShortAlgebraRuBWS $\Base$ в абелевой группе $V$.
Следовательно, абелевая группе $V$ является \SideRu\What $\Base$\Hyph \VectorSetRuENS.

Пусть
\ShowEq{set f:A->B}f{\Module_i}{\ModuleA}
семейство линейных отображений в \SideRuTo $\Base$\Hyph \VectorSetRuA $W$.
Мы определим отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
пользуясь равенством
\DrawEq{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
Сумма в правой части равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
конечна, так как все слагаемые, кроме конечного числа, равны $0$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(x+y)i=}
Из равенства
\ShowEq{fi(dx)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(dx)i=}
Следовательно, отображение $f$ является линейным отображением.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\eqRef{lj(x)=0x0}{\GroupLbl},
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\refDefinition{direct sum of Abelian groups}{+}.
}

\DefLabeledTheorem{direct sum of D modules}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{set Bi}{\Module}
- семейство \SideRu\TO $\Base$\Hyph \VectorsSetRuBNS.
Тогда представление
\ShowEq{\SideWS D->*o+A}{\Base}{\Module}{\ANumber}{\VNumber}
\ShortAlgebraRuBWS $\Base$
в прямой сумме абелевых групп
\ShowEq{o+Ai}{\Module}
является прямой суммой \SideRu\TO $\Base$\Hyph модулей
\ShowEq{o+Ai}{\Module}
}

\DefProof{direct sum of D modules}
{
Пусть
\ShowEq{set f:A->B}f{\Module_i}{\ModuleA}
семейство линейных отображений в \SideRuTo $\Base$\Hyph модуль $V$.
Мы определим отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
пользуясь равенством
\DrawEq{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
Сумма в правой части равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
конечна, так как все слагаемые, кроме конечного числа, равна $0$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(x+y)i=}
Из равенства
\ShowEq{fi(dx)=}
и равенства
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}
следует, что
\ShowEq{f(dx)i=}
Следовательно, отображение $f$ является линейным отображением.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\eqRef{lj(x)=0x0}{\GroupLbl},
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\refDefinition{direct sum of Abelian groups}{+}.
}

\DefProof{cr-power, 1}
{
Равенство
\ShowEq{cr-power, 1 1}
является следствием равенств
\eqRef{cr power, 0}1,
\eqRef{cr-power, n}1.
Равенство
\EqRef{cr-power, 1}
является следствием равенства
\EqRef{cr-power, 1 1}.
}

\DefProof{rc-power, 1}
{
Равенство
\ShowEq{rc-power, 1 1}
является следствием равенств
\eqRef{rc power, 0}1,
\eqRef{rc-power, n}1.
Равенство
\EqRef{rc-power, 1}
является следствием равенства
\EqRef{rc-power, 1 1}.
}

\DefLabeledTheorem[3]{Kernel of Linear Map}{(#1)}
{
Пусть отображение
\newline
\FrameEqRef[fV]{homomorphism D algebra #11}{Vector module, coordinates \Cols}
\newline
является линейным отображением
$D_{#1}$\Hyph модуля $V_1$
в $D_{#2}$\Hyph модуль $V_2$.
Множество
\ShowEq{kernel of linear map}{#3}
\DrawEq[{#3}{}]{ker linear map}{D#3}
называется
\AddIndex{ядром линейного отображения}{kernel of linear map}
$#3$.
Ядро линейного отображения $#3$
является подмодулем модуля $V_1$.
}

\DefProof[4]{Kernel of Linear Map}
{
Пусть
\ShowEq{vw in V1}
Тогда
\DrawEq{fvw=0 V2}{(#1)}
Равенство
\ShowEq{f v+w=0}
является следствием равенств
\eqRef{homomorphism, f v+w=}{f D module #11},
\eqRef{fvw=0 V2}{(#1)}.
Следовательно, множество
$\ker#3$
является подгруппой аддитивной группы $V_1$.
Равенство
\ShowEq{fpv=0 V2h}{#4}
является следствием равенств
\eqRef{left homomorphism, f av=}{f D module 11},
\eqRef{fvw=0 V2}{(#1)}.
Следовательно, определено представление кольца $D_{#1}$
на множестве
$\ker#3$.
Согласно определению
\refDefinition{submodule}{\SideWS module},
множество
$\ker#3$
является подмодулем $D_{#1}$\Hyph модуля $V_1$.
}

\DefTheorem{a in ZAb=>b in ZAa}
{
Если
\ShowEq{c in ZAa}ab,
то
\ShowEq{c in ZAa}ba.
}

\DefProof{a in ZAb=>b in ZAa}
{
Пусть
\ShowEq{c in ZAa}ab.
Равенство
\DrawEq{ab=ba}Z
является следствием утверждения
\eqRef{c in S=>bc=cb}{Z(A,b)}.
Теорема является следстием равенства
\eqRef{ab=ba}Z.
}

\DefTheorem{a in ZAb, c in ZA=>a in ZAbc}
{
Если
\ShowEq{c in ZAa}ab{}
и
\ShowEq{c in ZA}c
то
\ShowEq{c in ZAa}a{bc}.
}

\DefProof{a in ZAb, c in ZA=>a in ZAbc}
{
Равенство
\ShowEq{a(bc)=...=(bc)a}
является следствием определений
\RefDefinition{nucleus of algebra},
\RefDefinition{center of algebra}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
Теоремя является следствием равенства
\EqRef{a(bc)=...=(bc)a}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
}

\DefLemma{pk ck in Za}
{
Пусть $A$ - некоммутативная $D$\Hyph алгебра.
Для любого $a\in A$, если
\ShowEq{c in ZAa}{p,\ c}a,
то
\DrawEq[n]{pcn in Za}n
}

\DefProof{pk ck in Za}
{
Согласно теореме
\RefTheorem{c in S=>bc=cb submodule of A},
\ShowEq{p0 in Za}
Пусть утверждение
\eqRef{pcn in Za}n
верно для $n=k-1$, $k>0$,
\DrawEq[{k-1}{}]{pcn in Za}{k-1}
Тогда утверждение
\ShowEq{pck in Za}
является следсвием утверждения
\eqRef{pcn in Za}{k-1}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
Согласно принципу математической индукции,
утверждение
\eqRef{pcn in Za}n
верно для любого $n\ge 0$.
}

\DefTheorem{c in Za=> p(c) in Za}
{
Пусть $A$ - некоммутативная $D$\Hyph алгебра.
Для любого $a\in A$, если
\ShowEq{c in ZAa}ca,
то
\DrawEq[{p(c)}a{}{}]{c in ZAa}1
для любого многочлена
\DrawEq{p(c) p in D}1
}

\DefProof{c in Za=> p(c) in Za}
{
Теорема является следствием леммы
\RefLemma{pk ck in Za}
и теоремы
\RefTheorem{c in S=>bc=cb submodule of A}.
}

\DefTheorem{c in S=>bc=cb submodule of A}
{
Пусть $A$ - некоммутативная $D$\Hyph алгебра.
Для любого $b\in A$ существует подалгебра
\ShowEq{center of A number}
$D$\Hyph алгебры $A$ такая, что
\DrawEq[{Z(A,b)}{}]{c in S=>bc=cb}{Z(A,b)}
$D$\Hyph алгебра
\ShowEq{center Ac}{}
называется
\AddIndex{центром $A$\Hyph числа}{center of A number}
$b$.
}

\DefProof{c in S=>bc=cb submodule of A}
{
Подмножество
\ShowEq{center Ac}{}
не пусто так как
\ShowEq{c in ZAa}0b,
\ShowEq{c in ZAa}bb.
Пусть
\ShowEq{d in D c in S 12}
Тогда
\ShowEq{dcb=bdc}
Откуда следует
\ShowEq{dc in S}
Следовательно, множество
\ShowEq{center Ac}{}
является $D$\Hyph модулем.

Пусть
\ShowEq{c in ZAb}
Тогда
\ShowEq{c1c2 in ZAb}
Из равенства
\EqRef{c1c2 in ZAb}
следует, что
\ShowEq{c1 c2 in ZAb}
Следовательно, $D$\Hyph модуль
\ShowEq{center Ac}{}
является $D$\Hyph алгеброй.
}

\DefTheorem{set of maps B->A is Abelian group}
{
Пусть $A$ - алгебра над коммутативным кольцом $D$.
Для любого множества $B$
множество отображений $A^B$ является абелевой группой относительно операции
\ShowEq{(f+g)x=}x
}

\DefProof{set of maps B->A is Abelian group}
{
Теорема является следствием определений
\ShowRef{set of maps B->A is Abelian group}
}

\DefTheorem{set of endomorphisms - D module}
{
Множество
\ShowEq{End DV}{}
эндоморфизмов $D$\Hyph модуля $V$
является $D$\Hyph модулем.
}

\DefProof{set of endomorphisms - D module}
{
Теорема является следсвием определения
\RefDefinition{D module, endomorphism}
и следсвия
\RefCorollary{product of linear map over scalar, D module}.
}

\DefDefinition{D module, endomorphism}
{
Линейное отображение
\DrawEq[fVV]{f: A->B}{}
$D$\Hyph модуля $V$
называется
\AddIndex{эндоморфизмом}{endomorphism}
$D$\Hyph модуля $V$.
Обозначим
\ShowEq{set of endomorphisms D module}
множество эндоморфизмов
$D$\Hyph модуля $V$.
}

\DefLabeledDefinition{module over algebra}{\SideWS \VectorSetNS}
{
Пусть $\Base$ - \AlgebraRu \DivisionRuNS.
Эффективное \SideRu \SidePresentationRuWS представление
\DrawEq{\SideWS \Base->*V}{\SideWS \VectorSetNS}
\ShortAlgebraRuBWS $\Base$
в \SetRepresentationRu $V$
называется
\AddIndex{\SideRu \SideModuleC \VectorSetRuE}{\SideWS \VectorSetNS}
над \ShortAlgebraRuCWS $\Base$.
Мы также будем говорить, что \SetRepresentationRuA $V$ является
\AddIndex{\SideRu \SideModuleC $\Base$\Hyph \VectorSetRuENS}{\SideWS A \VectorSetNS}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
Билинейное отображение
\DrawEq{\SideWS \Base*V->V}{\VectorSet}
порождённое \SideRu \SidePresentationRuBWS представлением
\DrawEq{\Base*V->V to \SideWS product}{\VectorSetNS}
называется
%\AddIndex{\SideRu \SidePresentationRuBWS произведением}{\SideNS\SidePresentation product}
\SideRu \SidePresentationRuBWS произведением
вектора на скаляр.
}

\DefTheorem{quasibasis of so(3) module}
{
Пусть
\ShowEq{V=so3+so3}
- левый $so(3)$\Hyph модуль столбцов.
Множество векторов
\ShowEq{quasibasis of so(3) module}
является квазибазисом левого $so(3)$\Hyph модуля $V$.
}

\DefProof{quasibasis of so(3) module}
{
Согласно теоремам
\ShowRef{so3 quasibasis e}
$V$\Hyph число
\ShowEq{so3 V number}
имеет разложение
\ShowEq{so3 V number expansion}
относительно множества векторов \eV[V][.]
Следовательно, множества векторов \eV[V]
является квазибазисом левого $so(3)$\Hyph модуля $V$.
Из равенства
\ShowEq{so3 V basis dependence}
следует, что квазибазис \eV[V] не является базисом.
}

\DefLabeledTheorem[1]{so3 quasibasis e}{#1}
{
Матрица
\DrawEq[#1]{so3 quasibasis e=}{#1}
является левым квазибазисом
алгебры $so(3)$.
Координаты матрицы
\newline
\FrameEqRef{so3 matrix c}{#1}
\newline
относительно матрицы
\eqRef{so3 quasibasis e=}{#1}
имееют следующий вид
\DrawEq{so3 matrix c coordinates e#1}1
}

\DefProof[1]{so3 quasibasis e}
{
Мы можем представить матрицу
\DrawEq{so3 matrix c}{#1}
в виде
\DrawEq[{#1}]{Jacobson Coordinates of matrix 1}{#1}
Равенство
\DrawEq[{#1}]{Jacobson Coordinates of matrix}{#1}
является следствием равенств
\eqRef{so3 quasibasis e=}{#1},
\eqRef{Jacobson Coordinates of matrix 1}{#1}
Равенство
\ShowEq{Jacobson Coordinates of matrix (#1)}
является следствием равенств
\EqRef{so3 matrix product 2},
\eqRef{Jacobson Coordinates of matrix}{#1}.
Из равенства
\EqRef{Jacobson Coordinates of matrix (#1)}
следует, что координаты матрицы
\newline
\FrameEqRef{so3 matrix c}{#1}
\newline
относительно матрицы
\newline
\FrameEqRef[{#1}]{so3 quasibasis e=}{#1}
\newline
имееют следующий вид
\newline
\FrameEqRef{so3 matrix c coordinates e#1}1
\newline
Из равенства
\eqRef{so3 matrix c coordinates e#1}1
следует, что
матрица $\aD e{#1}$ является не базисом, а левым квазибазисом,
так как значение $q$ произвольно.
}

\DefDefinition{algebra so(3)}
{
Алгебра Ли $so(3)$ - это множество матриц
действительных чисел
\DrawEq[c]{so3 matrix}1
и произведение на множестве $so(3)$ определено равенством
\ShowEq{so3 matrix product 2a}
}

\DefTheorem{algebra so(3)}
{
Произведение в алгебре Ли $so(3)$ определено равенством
\ShowEq{so3 matrix product 2}
}

\DefProof{algebra so(3)}
{
Равенство
\ShowEq{so3 matrix product}
является следствием равенств
\eqRef{so3 matrix}1,
\EqRef{so3 matrix product 2a}.
Равенство
\ShowEq{so3 matrix product 1}
является следствием равенства
\EqRef{so3 matrix product}
Равенство
\EqRef{so3 matrix product 2}
является следствием равенства
\EqRef{so3 matrix product 1}.
}

\DefLabeledDefinition{module over associative algebra}{\SideWS \VectorSetNS}
{
Пусть $\Base$ - \AlgebraRu \DivisionRuNS.
Пусть $V$ - $\CBase$\Hyph \VectorSetRuANS.
Пусть в $\CBase$\Hyph \VectorSetRuD
\ShowEq{End DV}{}
определено произведение эндоморфизмов как композиция отображений.
Пусть определён гомоморфизм
\DrawEq[{g_{34}}A{\End(D,V)}{}]{f: A->B}{\SideWS g34}
$\CBase$\Hyph алгебры $A$
в $\CBase$\Hyph алгебру
\ShowEq{End DV}.

Эффективное \SideRu \SidePresentationRuWS представление
\DrawEq{\SideWS \Base->*V}{\SideWS \VectorSetNS}
\ShortAlgebraRuBWS $\Base$
в \SetRepresentationRu $V$
называется
\AddIndex{\SideRu \SideModuleC \VectorSetRuE}{\SideWS \VectorSetNS}
над \ShortAlgebraRuCWS $\Base$.
Мы также будем говорить, что \SetRepresentationRuA $V$ является
\AddIndex{\SideRu \SideModuleC $\Base$\Hyph \VectorSetRuENS}{\SideWS A \VectorSetNS}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
Билинейное отображение
\DrawEq{\SideWS \Base*V->V}{\VectorSet}
порождённое \SideRu \SidePresentationRuBWS представлением
\DrawEq{\Base*V->V to \SideWS product}{\VectorSetNS}
называется
%\AddIndex{\SideRu \SidePresentationRuBWS произведением}{\SideNS\SidePresentation product}
\SideRu \SidePresentationRuBWS произведением
вектора на скаляр.
}

\DefText{module over associative algebra}
{
Если $D$\Hyph алгебра $A$ ассоциативна, то мы можем уточнить определение
\refDefinition{module over non-commutative algebra}{\SideWS \VectorSetNS}.
}

\DefLabeledDefinition{module over non-commutative algebra}{\SideWS \VectorSetNS}
{
Пусть $\Base$ - некоммутативная $D$\Hyph алгебра.
Пусть $V$ - $\CBase$\Hyph \VectorSetRuANS.
Пусть в $\CBase$\Hyph \VectorSetRuD
\ShowEq{End DV}{}
определено произведение эндоморфизмов
таким образом, что
существует гомоморфизм
\DrawEq[{g_{34}}A{\End(D,V)}{}]{f: A->B}{}
$\CBase$\Hyph алгебры $A$
в $\CBase$\Hyph алгебру
\ShowEq{End DV}.

Эффективное \SideRu \SidePresentationRuWS представление
\DrawEq{\SideWS \Base->*V}{\SideWS nonA \VectorSetNS}
\ShortAlgebraRuBWS $\Base$
в \SetRepresentationRu $V$
называется
\AddIndex{\SideRu \SideModuleC \VectorSetRuE}{\SideWS \VectorSetNS}
над \ShortAlgebraRuCWS $\Base$.
Мы также будем говорить, что \SetRepresentationRuA $V$ является
\AddIndex{\SideRu \SideModuleC $\Base$\Hyph \VectorSetRuENS}{\SideWS A \VectorSetNS}.
$V$\Hyph число называется
\AddIndex{вектором}{vector}.
Билинейное отображение
\DrawEq{\SideWS \Base*V->V}{nonA \VectorSet}
порождённое \SideRu \SidePresentationRuBWS представлением
\DrawEq{\Base*V->V to \SideWS product}{nonA \VectorSetNS}
называется
%\AddIndex{\SideRu \SidePresentationRuBWS произведением}{\SideNS\SidePresentation product}
\SideRu \SidePresentationRuBWS произведением
вектора на скаляр.
}

\DefLabeledTheorem{module over algebra}{\SideNS}
{
Следующая диаграмма представлений описывает \SideRuTo $\Base$\Hyph модуль $V$
\DrawEq[{}{}{}{}]{diagram of representations, \SideWS module}1
В диаграмме представлений
\eqRef{diagram of representations, \SideWS module}1
верна
\AddIndex{коммутативность представлений}{commutativity of representations}
\BaseRings
в абелевой группе $V$
\DrawEq{\SideWS module, a d v}1
}

\DefProof{module over algebra}
{
Диаграмма представлений
\eqRef{diagram of representations, \SideWS module}1
является следствием определения
\ShowRef{\SideWS module over algebra}
и теоремы
\def\Temp{}
\ifx\SideNS\Temp
\refTheorem{action of ring of rational integers in Abelian group}{+}.
\else
\RefTheorem{Free Algebra over Ring}.
\fi
Равенство
\eqRef{\SideWS module, a d v}1
является следствием утверждения, что
\SideRu\HSide преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph модуля $V$.
}

\DefProof{module over non-associative algebra}
{
Диаграмма представлений
\eqRef{diagram of representations, \SideWS module}1
является следствием определения
\refDefinition{module over non-commutative algebra}{\SideWS \VectorSetNS}
и теоремы
\RefTheorem{Free Algebra over Ring}.
Равенство
\eqRef{\SideWS module, a d v}1
является следствием утверждения, что
\SideRu\HSide преобразование $\ATransf(a)$
является эндоморфизмом $\CBase$\Hyph модуля $V$.
}

\DefProof{Free Algebra over Ring}
{
Структура $D$\Hyph модуля $A$ порождена эффективным представлением
\ShowEq{f:A->*B}{g_{12}}DA
кольца $D$ в абелевой группе $A$.

\begin{ShadedLemma}
\labelLemma{structure of D algebra is generated by product}
Пусть в $D$\Hyph модуле $A$
определена структура $D$\Hyph алгебры $A$,
порождённая произведением
\DrawEq{product in D algebra}{}
\AddIndex{Левый сдвиг $D$\Hyph модуля $A$}{left shift of module},
определённый равенством
\ShowEq{l(v):w->vw}
порождает представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$
в $D$\Hyph модуле $A$
\end{ShadedLemma}

{\sc Доказательство.}
Согласно определениям
\RefDefinition{algebra over ring}
и
\RefDefinition{polylinear map of modules},
левый сдвиг $D$\Hyph модуля $A$
является линейным отображением.
Согласно определению
\refDefinition{linear map of D module}1,
отображение \(l\circ v\)
является эндоморфизмом $D$\Hyph модуля $A$.
Равенство
\ShowEq{l(v1+v2)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{def sum of linear maps}
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(v1+v2)}
является следствием равенства
\EqRef{l(v1+v2)w}.
Равенство
\ShowEq{l(dv)w}
является следствием определения
\RefDefinition{polylinear map of modules}
и равенства
\EqRef{l(v):w->vw}.
\ShowEq{ref sum of linear maps}
равенство
\ShowEq{l(dv)}
является следствием равенства
\EqRef{l(dv)w}.
Лемма является следствием равенств
\EqRef{l(v1+v2)},
\EqRef{l(dv)}.
\hfill\(\odot\)

\begin{ShadedLemma}
\labelLemma{representation of D module in D module determines the product}
Представление
\ShowEq{endomorphism of module from product, 1}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
\end{ShadedLemma}

{\sc Доказательство.}
Поскольку отображение $g_{23}\circ v$ является эндоморфизмом $D$\Hyph модуля $A$, то
\ShowEq{endomorphism of module from product, 3}
Поскольку отображение $g_{23}$
является линейным отображением
\ShowEq{g23:A->L}
то,
\ShowEq{ref sum and product over scalar, linear map}
\ShowEq{endomorphism of module from product, 4}
\ShowEq{endomorphism of module from product, 7}
Из равенств
\EqRef{endomorphism of module from product, 3},
\EqRef{endomorphism of module from product, 4},
\EqRef{endomorphism of module from product, 7}
и определения
\RefDefinition{polylinear map of modules},
следует, что отображение $g_{23}$ является билинейным отображением.
Следовательно, отображение $g_{23}$ определяет произведение в
$D$\Hyph модуле $A$ согласно правилу
\ShowEq{endomorphism of module from product, 8}
\hfill\(\odot\)

Теорема является следствием лемм
\RefLemma{structure of D algebra is generated by product},
\RefLemma{representation of D module in D module determines the product}.
}

\DefLabeledTheorem{A module -> algebra is associative}{\SideNS}
{
Пусть $g$ - эффективное левостороннее представление $D$\Hyph алгебры $A$
в $D$\Hyph модуле $V$.
Тогда $D$\Hyph алгебра $A$ ассоциативна.
}

\DefProof{A module -> algebra is associative}
{
Пусть
\ShowEq{abc in A, v in v}
Равенство
\DrawEq{\SideWS module, associative law}0
является следствием утверждения, что \SideRu востороннее представление
$g$ является
\SideRu восторонним представлением
мультипликативной группы $D$\Hyph алгебры $A$.
Равенство
\ShowEq{a(b(cv))=(a(bc))v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Так как
\ShowEq{cv \SideNS}
равенство
\ShowEq{a(b(cv))=((ab)c)v \SideNS}
является следствием равенства
\eqRef{\SideWS module, associative law}0.
Равенство
\ShowEq{(a(bc))v=((ab)c)v \SideNS}
является следствием равенств
\EqRef{a(b(cv))=(a(bc))v \SideNS},
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Поскольку $v$ - произвольный вектор $A$\Hyph модуля $V$,
равенство
\ShowEq{a(bc)=(ab)c \SideNS}
является следствием равенства
\EqRef{(a(bc))v=((ab)c)v \SideNS}.
Следовательно, $D$\Hyph алгебра $A$ ассоциативна.
}

\DefLabeledTheorem[1]{action of unital ring}{\SideWS \VectorSetNS}
{
Пусть $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS.
Для любого $\Base_{\BaseExt}$\Hyph числа
определён эндоморфизм
абелевой группы $V$
\DrawEq[{#1}vV{}]{module, a+d:V->V}{\SideNS,\VectorSetNS}
\DrawEq[{#1}{\Base}]{module, (a+n)v=av+nv}{\SideNS}
Множество преобразований
\eqRef{module, a+d:V->V}{\SideNS-\VectorSetNS}
порождает \SideRu\HSide представление \ShortAlgebraRuBWS $\Base_{(1)}$ в абелевой группе $V$.
Мы будем пользоваться обозначением
\ShowEq{set of vectors generated by vector \Base}
для множества векторов, порождённых вектором $v$.
}

\DefProof{action of unital ring}
{
Согласно теореме
\refTheorem{module over algebra}{\SideNS},
выражения $av$, $\DArg v$ являются $V$\Hyph числами.
Поскольку $V$ является абелевой группой, выражение
\eqRef{module, (a+n)v=av+nv}{\SideNS}
также является $V$\Hyph числом.
}

\DefLabeledTheoremNote{set of vectors generated by set of vectors}{\SideWS \VectorSetNS}
{
Пусть $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS.
Для любого множества $V$\Hyph чисел
\DrawEq[vV]{v(i) V}{\SideWS \VectorSetNS}
вектор, порождённый диаграммой представлений
\eqRef{diagram of representations, \SideWS module}1,
имеет следующий вид\,\footnotemark
\DrawEq[{\Base}{\BaseExt}{}]{w=sum vi, module=Jv}{\SideWS \Base}
\def\Temp{module}
\ifx\Temp\VectorSetNS
где \algebraa $\Base_{(1)}$
является унитальным расширением
\ShortAlgebraRuBWS $\Base$.
\fi
}
{
Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.
}

\DefLabeledTheorem[3]{homomorphism non-associative module}{\SideNS-\Cols(#1#2#3)}
{
Пусть
\ShowEq{Ai, i=}V
- \SideRu вый модуль столбцов
над неассоциативной $D$\Hyph алгеброй $A$.
Пусть \eV[i] - квазибазис $A$\Hyph модуль $V_i$.
Гомоморфизм
\DrawEq[f{V_1}{V_2}{}]{f: A->B}{}
$A$\Hyph модуля $V_1$ в $A$\Hyph модуль $V_2$
имеет представление
\DrawEq{v=w(fe2) \SideNS-\Cols}{(#1#2#3)}
где $f$ - матрица $A$\Hyph чисел.
Если квазибазис \eV[2] является базисом,
то матрица $f$ определена однозначно.
}

\DefText[1]{quasibasis module}
{
Пусть \AlgebraSetRu $\Set$ \ColsA
имеет \SideRuBasis квазибазис
\DrawEq[{\Set}]{eA= iI}{#1}
Пусть \SideRuBasis $\Set$\Hyph модуль $V$
является прямой суммой
\DrawEq{V=+V jJ}{#1}
Тогда \SideWS $\Set$\Hyph модуль $V$ имеет квазибазис
\DrawEq{quasibasis of left module}{#1}
}

\DefLabeledTheorem{quasibasis module}{\SideNS-\Set.\Cols}
{
\ShowText{quasibasis module}{\SideNS-\Set.\Cols}
}

\DefLabeledTheorem{when quasibasis of module is basis}{\SideNS-\Set}
{
Если \SideRuBasis квазибазис \eV[\Set]
\AlgebraSetRuB $\Set$
является \SideRu\What базисом,
то соответствующий квазибазис \SideRu\Which $\Set$\Hyph модуля $V$
является базисом.
}

\DefLabeledExample{A module over Lie algebra L}{\SideNS}
{
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Пусть $V$ является \SideRu вым $A$\Hyph \VectorSetRuENS.
Пусть
\ShowEq{End DV}{}
- $D$\Hyph алгебра эндоморфизмов \SideRu вого $A$\Hyph \VectorSetRuB $V$,
где произведение эндоморфизмов определено как композиция отображений.
Рассмотрим \SideRu \SidePresentationRuWS представление
\ShowEq{f:A->*B}f{\End(D,V)}V
$D$\Hyph алгебры
\ShowEq{End DV}{}
в $A$\Hyph \VectorSetRuD $V$,
определённое равенством
\ShowEq{av=a o v}
Рассмотрим эффективное \SideRu \SidePresentationRuWS представление
\ShowEq{f:A->*B}gLV
алгебры Ли $L$
в $A$\Hyph \VectorSetRuD $V$,
определённое равенством
\ShowEq{ab=[ab]}
Вообще говоря
\DrawEq{a(bv) ne (ab)v}{Lie}
}

\DefLabeledExample{non-associative A module}{\SideNS}
{
Пусть $A$ - неассоциативная $D$\Hyph алгебра.
Рассмотрим $D$\Hyph модуль
\ShowEq{V=+A iI}
Множество отображений
\ShowEq{a in A, av=}
порождает \SideRu \SidePresentationRuWS представление
$D$\Hyph алгебры $A$ в $D$\Hyph модуле $V$
и, следовательно, порождает структуру
\SideRu \SideModuleC $\Base$\Hyph \VectorSetRuB $V$.
Вообще говоря
\DrawEq{a(bv) ne (ab)v}{nonA}
}

\DefLabeledTheorem{associative law of A module}{\SideNS}
{
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Тогда
\AddIndex{закон ассоциативности}{associative law}
в \SideRu вом $A$\Hyph \VectorSetRuD $V$
принимает вид
\DrawEq{associative law, \SideWS module}1
\ShowEq{p,q in D, v in V}
}

\DefText{unitarity law, module}
{
\DrawEq{unitarity law, module}{\SideWS \Base}
Если \algebrac имеет единицу, то равенство
\eqRef{unitarity law, module}{\SideWS \Base}
имеет вид
\DrawEq{unitarity law, vector space}{\SideWS \Base-\VectorSetNS}
}

\DefText{unitarity law, vector space}
{
\DrawEq{unitarity law, vector space}{\SideWS \Base}
}

\DefLabeledTheorem{definition of A module, property}{\SideNS}
{
Пусть $V$ является \SideRu\What $\Base$\Hyph \VectorSetRuENS.
$V$\Hyph числа удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закон коммутативности}{commutative law}
\DrawEq{commutative law}{\SideWS vector space}
\item
\AddIndex{закон ассоциативности}{associative law}
\labelItem{associative law, \SideWS module}
\DrawEq{associative law, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\labelItem{distributive law, \SideWS module}
\DrawEq{distributive law, \SideWS module, 1}1
\DrawEq{distributive law, \SideWS module, 2}1
\item
\AddIndex{закон унитарности}{unitarity law}
\labelItem{unitarity law, \SideWS \Base-module}
\ShowText{unitarity law, \VectorSetNS}
\end{enumerate}
для любых
\ShowEq{p,q in D, v,w in V}
}

\DefLabeledTheorem{definition of A module, property, 2023}{\SideNS}
{
Пусть $V$ является \SideRu вым $A$\Hyph \VectorSetRuENS.
$V$\Hyph числа удовлетворяют соотношениям
\StartLabelItem
\begin{enumerate}
\item
\AddIndex{закон коммутативности}{commutative law}
\DrawEq{commutative law}{\SideWS nonA vector space}
\item
\AddIndex{закон ассоциативности}{associative law}
\labelItem{associative law, nonA \SideWS module}
\DrawEq{associative law*, \SideWS module}1
\item
\AddIndex{закон дистрибутивности}{distributive law}
\labelItem{distributive law, nonA \SideWS module}
\DrawEq{distributive law, \SideWS module, 1}1
\DrawEq{distributive law, \SideWS module, 2}1
\item
\AddIndex{закон унитарности}{unitarity law}
\labelItem{unitarity law, nonA \SideWS \Base-module}
\ShowEq{unitarity law, \SideWS \Base-module}
\end{enumerate}
для любых
\ShowEq{m,n in D}
\ShowEq{p,q in D, v,w in V}
}

\DefProof{definition of A module, property}
{
Пусть $v\in V$.

Пусть $\Base_{(1)}$ - множество отображений
\eqRef{module, a+d:V->V}{\SideNS}.
Равенство
\eqRef{distributive law, \SideWS module, 1}1
и утверждение
\RefItem{\SideWS representation of D1 in Abelian group}
являются следствием леммы
\refLemma{action of D algebra}{\SideNS}.

Пусть
\ShowEq{p,q in D1}
Согласно утверждению
\RefItem{\SideWS representation of D1 in Abelian group},
мы определим сумму $\Base_{(1)}$\Hyph чисел $p$ и $q$ равенством
\eqRef{distributive law, \SideWS module, 2}1.
Равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=, 1}
является следствием равенства
\eqRef{distributive law, \SideWS module, 2}1.
Равенство
\DrawEq[nmv]{distributive law,, \SideWS module, 2}{\CBase}
является следствием утверждения, что представление
$\DTransf$ является гомоморфизмом аддитивной группы кольца $\CBase$.
Равенство
\DrawEq[abv]{distributive law,, \SideWS module, 2}{\Base}
является следствием утверждения, что \SideRu\HSide представление
$\ATransf$ является гомоморфизмом аддитивной группы \ShortAlgebraRuBWS $\Base$.
Так как $V$ является абелевой группой, то равенство
\ShowEq{\SideWS module, (a+n)+(b+m)=}
является следствием равенств
\ShowRef{module, (a+n)+(b+m)=}
Из равенства
\EqRef{\SideWS module, (a+n)+(b+m)=}
следует, что определение
\eqRef{(a+n)+(b+m)=}{db(\SideNS)}
суммы на множестве $\Base_{(1)}$ не зависит от вектора $v$.

Равенства
\eqRef{associative law, \SideWS module}1,
\EqRef{unitarity law, \SideWS \Base-module}
являются следствием утверждения
\RefItem{\SideWS representation of D1 in Abelian group}.
Пусть
\ShowEq{p,q in D1}
\def\Temp{}
\ifx\SideNS\Temp
Равенство
\DrawEq{associative law, \CBase, \SideWS module}1
является следствием утверждения, что представление $\DTransf$
является представлением мультипликативной группы кольца $\CBase$.
Равенство
\DrawEq{\SideWS module, associative law}1
является следствием утверждения, что представление $g_2$
является представлением мультипликативной группы кольца $D$.
Равенство
\DrawEq{associative law, \CBase\Base, \SideWS module}1
является следствием утверждения, что кольцо $D$
является абелевой группой.
Равенство
\ShowEq{module, (a+n)(b+m)=}
является следствием равенств
\ShowEq{ref module, (a+n)(b+m)=}%
Равенство
\eqRef{(a+n)(b+m)=}{db(\SideNS)}
является следствием равенства
\EqRef{module, (a+n)(b+m)=}.
\else%
Опираясь на определение
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS},
мы рассмотрим произведение
$\Base_{(1)}$\Hyph чисел $p$ и $q$
как билинейное отображение
\ShowEq{f:D1xD1->D1}
такое, что верны равенства
\DrawEq{fab=ab}{\SideWS module}
\DrawEq{f1p=p}{\SideWS module}
Равенство
\DrawEq{pq=fpq}{\SideWS module}
является следствием равенств
\eqRef{fab=ab}{\SideWS module},
\eqRef{f1p=p}{\SideWS module}.
Равенство
\eqRef{(a+n)(b+m)=}{db(\SideNS)}
является следствием равенства
\eqRef{pq=fpq}{\SideWS module}.
\fi%

Утверждение
\RefItem{Algebra is \SideWS ideal of algebra (1)}
является следствием равенства
\eqRef{(a+n)(b+m)=}{db(\SideNS)}.
}

\DefLabeledDefinition{submodule}{\SideWS module}
{
Подпредставление \SideRu\From $\Base$\Hyph \VectorSetRuB $V$ называется
\AddIndex{\VectorSubSetRuD}{\VectorSubSetNS}
\SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
}

\DefLabeledTheorem{submodule}{\SideWS module}
{
Пусть
\ShowEq{vi V}{}
- множество векторов \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
Если векторы
\ShowEq{set vi cols}v
принадлежат \VectorSubSetRuE $V'$ \SideRu\From $\Base$\Hyph \VectorSetRuB $V$,
то линейная комбинация векторов
\ShowEq{set vi cols}v
принадлежит \VectorSubSetRuE $V'$.
}

\DefProof{submodule}
{
Теорема является следствием
теоремы
\refTheorem{set of vectors generated by set of vectors}{\SideWS \VectorSetNS}
и определений
\refDefinition{linear combination of vectors}{\SideNS},
\refDefinition{submodule}{\SideWS module}.
}

\AddEq{ref in item cvk module}
{
теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{definition of A \VectorSetNS}{\SideNS}
}

\AddEq{ref in item cvk vector space}
{
теоремы
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
определения
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS}.
}

\DefLabeledTheorem{set of automorphisms}{\SideNS}
{
Множество $GL(V)$
автоморфизмов
\SideRu вого $A$\Hyph векторного пространства $V$
является группой.
}

\DefLabeledTheorem{active transformations in module}{\SideNS-\Cols}
{
\ShowEq{Let V be vector space of and basis}
Любой автоморфизм $\Vector f$ \SideRu вого $A$\Hyph векторного пространства
$V$ имеет вид
\DrawEq[{v'}{}v{}f{}]{v1=v2*a \SideNS-\Cols}{automorphism}
где $f$ - \ProductType невырожденная матрица.
Матрицы автоморфизмов \SideRu вого $A$\Hyph векторного пространства \ColsA порождают группу
%\Group nA.
$GL(V_*)$,
изоморфную группе $GL(V)$.
Автоморфизмы \SideRu вого $A$\Hyph векторного пространства \ColsA порождают
\OtherSideRu востороннее линейное
эффективное представление
\DrawEq[{GL(V_*)}{V_*}{}]{A->*B}{\SideNS-\Cols}
группы $GL(V_*)$
в \SideRu вом $A$\Hyph векторном пространстве $V_*$.
}

\DefLabeledTheoremNote{set of vectors generate set of vectors}{\SideWS \VectorSetNS}
{
Пусть $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS.
Существует
множество $V$\Hyph чисел
\DrawEq[vV]{v(i) V}{}
такое, что любое $V$\Hyph число
имеет вид\,\footnotemark
\DrawEq[{\Base}{\BaseExt}{}]{w=sum vi, module=Jv}{\SideWS \Base}
\ShowEq{linear combination()}%
Множество $v$ называется
\AddIndex{множеством образующих}{generating set}
\SideRu\From $\Base$\Hyph модуля $V$.
Выражение
\ShowEq{A linear combination() =}
называется
\AddIndex{линейной комбинацией}{linear combination} векторов
\ShowEq{v(i)}
Вектор
\ShowEq{w=c(i)v(i)}
называется
\AddIndex{линейно зависимым}{linearly dependent}
от векторов
\ShowEq{v(i)}
}
{Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.}

\DefText{Let be algebra D}
{
Пусть $D$ - кольцо.
}

\DefText{Let be algebra A}
{
Пусть $A$ - $D$\Hyph алгебра.
}

\DefLabeledLemma[4]{action n of D algebra}{#1#2-\SideNS-\VectorSetNS}
{
Пусть 
\ShowEq{module, d in D}{#1}{#2}.
Отображение
\DrawEq[{#1}{#3}{#4}{\Multiply{#1}{#3}}{#4}{}]{f:a in A->b in B}{#1#2-\SideNS-\VectorSetNS}
является эндоморфизмом абелевой группы $#4$.
}

\DefProof[4]{action n of D algebra}
{
Утверждение
\ShowEq{module, dv in V}{#1}{#3}{#4}%{}
является следствием
\ShowText{#1#3 \VectorSetNS}
Согласно
\ShowText{#1#3 \VectorSetNS,1}
отображение
\eqRef{f:a in A->b in B}{#1#2-\SideNS-\VectorSetNS}
является эндоморфизмом абелевой группы $#4$.
}

\DefLabeledLemma[4]{action of D algebra}{\SideNS-\VectorSetNS}
{
Пусть 
\ShowEq{module, d in D}{#1}{#2},
\ShowEq{module, d in D}a{#4}.
Отображение
\DrawEq[{#1}{#3}{#4}{}]{module, a+d:V->V}{\SideNS-\VectorSetNS}
определённое равенством
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS}
является эндоморфизмом абелевой группы $#4$.
}

\DefText{nd module}
{
определения
\ShowRef{nd module}
}

\DefText{nd module,1}
{
теореме
\refTheorem{action of ring of rational integers in Abelian group}{+}
и определению
\RefDefinition{representation of algebra},
}

\DefText{ad module}
{
определения
\ShowRef{ad module}
}

\DefText{ad module,1}
{
утверждению
\RefItem{Product is distributive over sum},
и теоремам
\RefTheorem{0a=0},
\refTheorem{monoid-homomorphism}{+},
}

\DefText{db algebra}
{
определений
\ShowRef{nd algebra}
}

\DefText{db algebra,1}
{
равенству
\eqRef{distributive law, module, 1}1
}

\DefText{ab algebra}
{
определения
\RefDefinition{algebra over ring}.
}

\DefText{ab algebra,1}
{
теореме
\RefTheorem{multiplication in algebra is distributive over addition}
}

\DefProof[4]{action of D algebra}
{
Так как $#4$ является абелевой группой, то утверждение
\ShowEq{module, dv+av in V}{#3}{#4}
является следствием лемм
\refLemma{action n of D algebra}{#1#2-\SideNS-\VectorSetNS},
\refLemma{action n of D algebra}{a#4-\SideNS-\VectorSetNS}.
Следовательно,
для любого $\CBase$\Hyph числа $\DArg$
и любого $\Base$\Hyph числа $a$,
мы определили отображение
\eqRef{module, a+d:V->V}{\SideNS-\VectorSetNS}.
Согласно леммам
\refLemma{action n of D algebra}{#1#2-\SideNS-\VectorSetNS},
\refLemma{action n of D algebra}{a#4-\SideNS-\VectorSetNS}
и теореме
\refTheorem{monoid-homomorphism, sum}{+},
отображение
\eqRef{module, a+d:V->V}{\SideNS-\VectorSetNS}
является эндоморфизмом абелевой группы $V$.
}

\DefExample{q equation ix-xi=k}
{
Рассмотрим уравнение
\DrawEq{ix-xi=k}1
Умножая уравнение
\eqRef{ix-xi=k}1
на
\ShowEq{ijk}
мы получим уравнения
\ShowEq{ix-xi-k=0 i}
\ShowEq{ix-xi-k=0 j}
\ShowEq{ix-xi-k=0 k}
Положим
\ShowEq{xijk}
Тогда мы получим систему линейных уравнений
\ShowEq{ix-xi-k=0 1ijk}
Решение системы линейных уравнений
\EqRef{ix-xi-k=0 1ijk}
имеет вид
\ShowEq{q equation 3 1ijk j-k x=}
Однако значение $x$ в равенстве
\EqRef{q equation 3 1ijk j-k x=}
не является корнем уравнения
\eqRef{ix-xi=k}1.
Здесь важно обратить внимание, что решение
\DrawEq{x=c12+j}1
уравнения
\eqRef{ix-xi=k}1
зависит от двух действительных произвольных постоянных,
а решение
\EqRef{q equation 3 1ijk j-k x=}
системы линейных уравнений
\EqRef{ix-xi-k=0 1ijk}
зависит от одной кватернион\Hyph значной произвольной постоянной.
}

\DefRef{associative module}
{
равенств
\EqRef{(nm)a=n(ma) (+)},
}

\DefRef{associative algebra}
{
определений
\RefDefinition{algebra over ring},
\RefDefinition{associator of algebra},
равенства
}

\DefRef{associative 1 module}
{
утверждений
\RefItem{() is associative},
\RefItem{A is multiplicative monoid},
теоремы
\refTheorem{homomorphism f(na)=nf(a)}{+},
}

\DefRef{associative 1 algebra}
{
}

\DefText{associative module}
{
}

\DefText{associative algebra}
{
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
}

\DefSummary{Unital Extension of Ring}
{
}

\DefLabeledTheoremNote[2]{unital extension of D algebra}{\AlgebraLabel}
{
\ShowText{associative \VectorSetNS}
Множество отображений
\ShowEq{a o+ b}{#1}
порождает\,\footnotemark
\AlgebraSetRuD $\Set_{(1)}$
где сложение определено равенством
\DrawEq[{#1}{}]{(a+n)+(b+m)=}{#1#2(\VectorSetNS)}
и произведение определено равенством
\DrawEq[{#1}{}]{(a+n)(b+m)=}{#1#2(\VectorSetNS)}
\StartLabelItem
\begin{enumerate}
\item
Если \AlgebraSetRu $\Set$ имеет единицу, то
\ShowEq{A1=A unital extension}
\item
Если \AlgebraSetRu $\Set$ является идеалом $\BaseSet$, то
\ShowEq{A1=D unital extension}
\item
В противном случае
\ShowEq{A1=A+D unital extension}
\item
\AlgebraSetRuC $\Set$ является идеалом \AlgebraSetRuB $\Set_{(1)}$.
\labelItem{Algebra is ideal of algebra (1) \AlgebraLabel}
\end{enumerate}
\AlgebraSetRuC $\Set_{(1)}$ называется
\AddIndex{унитальным расширением}{unital extension}
\AlgebraSetRuB $\Set$.
}
{
Смотри определение унитального расширения также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 52,
\citeBib{Zharinov: foundation of mathematical physics}\Hyph 64.
}

\DefProof[4]{unital extension of ring}
{
\ShowText{step of proof unital extension}{#1}{#2}{#3}{#4}

Утверждение
\RefItem{Algebra is ideal of algebra (1) \SideNS-\VectorSetNS}
является следствием леммы
\refLemma{action of D algebra}{\SideNS-\VectorSetNS}.
}

\DefProof[4]{unital extension of D algebra}
{
Выражение для операций на множестве $#4_{(1)}$
не зависит от того, действует ли эндоморфизм
\ShowEq{a o+ b}{#1}
на $#4$\Hyph числа слева или справа.
Однако текст доказательства слегка отличается.
Поэтому мы рассмотрим оба варианта доказательства.

\TwoColText
{
\ShowEq{def left}
\ShowText{step of proof unital extension}{#1}{#2}{#3}{#4}
}
{
\ShowEq{def right}
\ShowText{step of proof unital extension}{#1}{#2}{#3}{#4}
}

\ShowEq{def ab=ba}
Утверждение
\RefItem{Algebra is ideal of algebra (1) \SideNS-\VectorSetNS}
является следствием определения
\refDefinition{ideal}{\VectorSetNS}
и лемм
\refLemma{action of D algebra}{left-\VectorSetNS},
\refLemma{action of D algebra}{right-\VectorSetNS}.
}

\DefText[4]{step of proof unital extension}
{
Согласно теореме
\refTheorem{monoid-homomorphism, sum}{+},
равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv +i}{\SideNS-\VectorSetNS}
является следствием равенства
\eqRef{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS}.
Равенство
\eqRef{(a+n)+(b+m)=}{#1#3(\VectorSetNS)}
является следствием равенства
\eqRef{module, (a+d)v=av+dv +i}{\SideNS-\VectorSetNS}.

Согласно теореме
\RefTheorem{product of homomorphisms},
равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv *i}{#1#3 \SideNS-\VectorSetNS}
является следствием равенства
\eqRef{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS}.
Равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv *i1}{#1#3 \SideNS-\VectorSetNS}
является следствием
\ShowRef{associative \VectorSetNS}
\eqRef{module, (a+d)v=av+dv *i}{#1#3 \SideNS-\VectorSetNS},
\ShowRef{associative 1 \VectorSetNS}
леммы
\refLemma{action n of D algebra}{a#4-\SideNS-\VectorSetNS}.
Равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv *i2}{}%{#1#3 \SideNS-\VectorSetNS}
\begin{sloppypar}
\noindent
а следовательно и равенство
\eqRef{(a+n)(b+m)=}{#1#3(\VectorSetNS)},
является следствием равенств
\eqRef{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS},
\eqRef{module, (a+d)v=av+dv *i1}{#1#3 \SideNS-\VectorSetNS}
и лемм
\refLemma{action n of D algebra}{#1#2-\SideNS-\VectorSetNS},
\refLemma{action n of D algebra}{a#4-\SideNS-\VectorSetNS}.
\end{sloppypar}

Пусть \algebraa $#4$ имеет единицу $e$.
Тогда мы можем отождествить $#1\in #2$ и
$\Multiply{#1}e\in #4$.
Равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv Z in D}{\SideNS-\VectorSetNS}
является следствием равенства
\newline
\FrameEqRef[{#1}{#3}{}]{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS}
\newline
Утверждение
\RefItem{A1=A unital extension -\VectorSetNS}
является следствием равенства
\eqRef{module, (a+d)v=av+dv Z in D}{\SideNS-\VectorSetNS}.

Пусть \algebraa $#4$ является идеалом $\CBase$.
Тогда
$#4\subseteq\CBase$.
Равенство
\DrawEq[{#1}{#3}{}]{module, (a+d)v=av+dv D in Z}{\SideNS-\VectorSetNS}
является следствием равенства
\eqRef{module, (a+d)v=av+dv}{\SideNS-\VectorSetNS}.
Утверждение
\RefItem{A1=D unital extension -\VectorSetNS}
является следствием равенства
\eqRef{module, (a+d)v=av+dv D in Z}{\SideNS-\VectorSetNS}.
}

\DefText{quasibasis of algebra}
{
Если для любого $a\in A$,
\ShowEq{Aa ne A}
то в $D$\Hyph алгебре $A$ существует \SideRu вый квазибазис,
имеющий более чем одно $A$\Hyph число.
}

\DefLabeledTheorem{Quasi-basis of direct sum}{\Cols}
{
Пусть $A$ - $\Omega$\Hyph кольцо.
Пусть $V_1$, $V_2$ - $A$\Hyph модули \ColsNA.
Пусть \eV[i][,] $i=1$, $2$, - квазибазис $A$\Hyph модуля $V_i$.
Тогда множество векторов
\DrawEq{Quasi-basis of direct sum}{\Cols}
является квазибазисом прямой суммы
\ShowEq{V1o+V2}
$A$\Hyph модулей $V_1$, $V_2$.

Если квазибазисы \eV[i][,] $i=1$, $2$,
являются базисами, то квазибазис \eV является базисом.
}

\DefText{quasibasis and principal ideal}
{
Пусть \eV - \SideRuBasis квазибазис
\AlgebraSetRuB $\Set$.
Тогда \AlgebraSetRu $\Set$
является прямой суммой главных идеалов
\DrawEq{A=Aiei}{\SideNS-\Set.\Cols}
}

\DefLabeledDefinition{quasibasis of algebra}{\SideNS-\Set.\Cols}
{
Пусть \AlgebraSetRu $\Set$ является \SideRu\What $\Set$\Hyph модулем \ColsNA.
Если множество $\Set$\Hyph чисел
\DrawEq[a{\Set}]{v(i) V}{a\Set \SideNS.\Cols}
является минимальным множеством таким, что
любое $\Set$\Hyph число имеет представление
\DrawEq[{\Set}{(1)}ab]{w=sum vi, module}{\SideNS-\Set.\Cols}
то множество $a$
называется \SideRu\What квазибазисом \AlgebraSetRuB $\Set$.
}

\DefLabeledDefinition{quasibasis of algebra is basis}{\SideNS}
{
Пусть \eV - \SideRu вый квазибазис
$D$\Hyph алгебры $A$ \ColsNA.
Если
\ShowEq{w(i)=0}c
следует из уравнения
\DrawEq[ce]{wi vi=0}{algebra \SideNS}
то \SideRu вый квазибазис \eV называется \SideRu вым базисом
$D$\Hyph алгебры $A$.
}

\DefLemmaProof{w=w12 in Xk-1}
{\leftskip=25pt
Согласно равенству
\eqRef{w=sum vi, module=Jv*}{\SideWS \Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{g(i)12}w
такие, что
\DrawEq[w]{w()12=* \SideNS}{\VectorSetNS}
где множества
\DrawEq[w]{|c(i)12 ne 0|}{\SideWS \VectorSet nonA}
конечны.
Так как $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS,
то из равенств
\eqRef{distributive law, \SideWS module, 2}1,
\eqRef{w()12= \SideNS}{\VectorSetNS}
следует, что
\DrawEq[w]{w()1+w()2=* \SideNS}{\VectorSetNS}
Из равенства
\eqRef{|c(i)12 ne 0|}{\SideWS \VectorSet nonA}
следует, что
множество
\ShowEq{|gi() 1+2 ne 0|}w
конечно.
}

\DefLabeledSummary{Vector Space Type 10-28-2023}{\SideNS-\Cols}
{
Мы представили множество векторов
\ShowEq{\RowN() 1n}vm{}
в виде
\RowA матрицы
\newline
\FrameEqRef[vm]{a=(a1.n \RowN)}{vm \SideNS-\Cols}
\newline
и множество $\Base_{\BaseExt}$\Hyph чисел
\ShowEq{\ColNS() 1n}cm{}
в виде
\ColA матрицы
\newline
\FrameEqRef[cm]{a=(a1.n \ColNS)}{cm \SideNS-\Cols}
\newline
Соответствующее представление \SideRu\Which $\Base$\Hyph \VectorSetRuB $V$ мы будем называть
\AddIndex{\SideRu\What $\Base$\Hyph \VectorSetRuE \ColsNA}{\SideWS A-\ColNWS space},
а $V$\Hyph число мы будем называть
\AddIndex{вектор\Hyph \ColWS}{\ColNWS vector}.
Мы можем записать линейную комбинацию
векторов
\ShowEq{\RowNWS set 1n}vm{}
в виде \ProductType произведения матриц
\newline
\FrameEqRef[cvm]{w.e, \SideNS-\Cols}{cv}
\newline
В частности,
если мы запишем векторы базиса $\Basis e$
в виде \RowA матрицы
\newline
\FrameEqRef[en]{a=(a1.n \RowN)}{type \SideNS-\Cols}
\newline
и координаты вектора
\ShowEq{w=w*e \SideNS-\Cols}w{}
относительно базиса $\Basis e$ в виде
\ColA матрицы
\newline
\FrameEqRef[wn]{a=(a1.n \ColNS)}{type \SideNS-\Cols}
\newline
то мы можем представить вектор
$\Vector w$
в виде \ProductType произведения матриц
\newline
\FrameEqRef[w]{vector w=w*e \SideNS-\Cols}w
}

\DefLabeledSummary{basis of module 10-28-2023}{\SideNS}
{
$X$ является
множеством образующих
\SideRu\From $\Base$\Hyph модуля $V$,
если любое $V$\Hyph число
является линейной комбинацией $V$\Hyph чисел из $X$.
Если существует минимальное множество \eV[][,] порождающее
\SideRuTo $\Base$\Hyph \VectorSetRuA $V$, то такое множество \eV называется
квазибазисом \SideRu\From $D$\Hyph \VectorSetRuB $V$.
Пусть уравнение
\newline
\FrameEqRef[ce]{wi vi=0}{\SideNS}
\newline
имеет единственное решение
\ShowEq{w(i)=0}c
Тогда квазибазис \eV является
базисом \SideRu\From $\Base$\Hyph модуля $V$.

\SideRuC\To $\Base$\Hyph модуль $V$ -
\AddIndex{свободный \SideRuTo $\Base$\Hyph модуль}{free module},
если \SideRuTo $\Base$\Hyph модуль $V$ имеет базис.
Координаты вектора $v\in V$ относительно базиса $\Basis e$
\SideRu\Which $\Base$\Hyph \VectorSetRuB $V$
определены однозначно.
Из равенства
\newline
\FrameEqRef{e*v=e*w,\SideNS}{\Cols}
\newline
следует, что
\ShowEq{=> v=w}
}

\DefLabeledTheoremNote{set of vectors generated* by set of vectors}{\SideWS \VectorSetNS}
{
Пусть $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS.
Множество $V$\Hyph чисел, порождённое множеством $V$\Hyph чисел
\DrawEq[vV]{v(i) V}{\SideWS \VectorSetNS}
имеет вид\,\footnotemark
\DrawEq[{\Base}{\BaseExt}]{w=sum vi, module=Jv*}{\SideWS \Base}
}
{Для множества $A$,
мы обозначим $|A|$ мощность множества $A$.
Запись $|A|<\infty$ означает, что множество $A$ конечно.}

\DefRef{structure of subrepresentations, module}
{
и теоремам
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{action of unital ring}{\SideWS \VectorSetNS},
}

\DefRef{structure of subrepresentations, vector space}
{
и теореме
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
}

\DefLabeledLemma[1]{w=w12 in Xk-1}{\SideWS \VectorSet #1}
{\leftskip=25pt
Пусть
\ShowEq{w=w12 in Xk-1}.
Тогда $w\in J(v)$.
}

\DefLabeledLemma{w=aw in Xk-1}{\SideWS \VectorSetNS}
{\leftskip=25pt
Пусть
\ShowEq{w=aw in Xk-1,\SideNS}
Тогда $w\in J(v)$.
}

\DefLabeledLemma{w=a*w in Xk-1}{\SideWS \VectorSetNS}
{\leftskip=25pt
Пусть
\ShowEq{w=a*w in Xk-1,\SideNS}
Тогда $w\in J(v)$.
}

\DefLemmaProof{w=a*w in Xk-1}
{\leftskip=25pt
Согласно утверждению
\RefItem[\RefRepresentation]{ax in Xk+1},
для любого $\Base_{\BaseExt}$\Hyph числа $a$,
\ShowEq{aw1 in Xk \SideWS module}
Согласно равенству
\eqRef{w=sum vi, module=Jv*}{\SideWS \Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{set au v(i)}{w_1}
такие, что
\ShowEq{w()=* \SideWS module}
где
\DrawEq{|w(i) ne 0|}{\SideWS module}
Из равенства
\EqRef{w()=* \SideWS module}
следует, что
\ShowEq{aw()=* \SideWS module}
Из утверждения
\eqRef{|w(i) ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{\SideWS module, |aw(i) ne 0|}
конечно.
}

\DefText{set of vectors, step 1, module}
{
Для произвольного
\ShowEq{vk in Jv}{}
положим
\ShowEq{c(i)=0 o+ dik}
Тогда равенство
\DrawEq[{\Base_{\BaseExt}}{}]{v(k)=sum v(i)}{\SideWS \Base}
является следствием равенства
\eqRef{module, (a+n)v=av+nv}{\SideNS}.
Из равенств
\eqRef{w=sum vi, module=Jv}{\SideWS \Base},
\eqRef{v(k)=sum v(i)}{\SideWS \Base}.
следует, что
теорема верна на множестве
\ShowEq{X0=v in J}
}

\DefText{set of vectors, step 1, vector space}
{
Для произвольного
\ShowEq{vk in Jv}{}
положим
\ShowEq{c(i)=dik}
Тогда
\DrawEq[{\Base_{\BaseExt}}{}]{v(k)=sum v(i)}{\SideWS \Base}
Из равенств
\eqRef{w=sum vi, module=Jv}{\SideWS \Base},
\eqRef{v(k)=sum v(i)}{\SideWS \Base}.
следует, что
теорема верна на множестве
\ShowEq{X0=v in J}
}

\DefProof{set of vectors generated by set of vectors}
{
Мы докажем теорему по индукции, опираясь на теорему
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

\ShowText{set of vectors, step 1, \VectorSetNS}

Пусть
\ShowEq{Xk in Jv}{k-1}
Согласно определению
\ShowRef{\SideWS module over algebra}
\ShowRef{structure of subrepresentations, \VectorSetNS}
если $w\in X_k$, то либо
\ShowEq{w=w12 in Xk-1},
либо
\ShowEq{w=aw in Xk-1,\SideNS}

{\leftskip=25pt
\ShowLemma{w=w12 in Xk-1}A

{\sc Доказательство.}
Согласно равенству
\eqRef{w=sum vi, module=Jv}{\SideWS \Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{g(i)12}w
такие, что
\DrawEq[w]{w()12= \SideNS}{\VectorSetNS}
где множества
\DrawEq[w]{|c(i)12 ne 0|}{\SideWS \VectorSetNS}
конечны.
Так как $V$ - \SideRuTo $\Base$\Hyph \VectorSetRuANS,
то из равенств
\eqRef{distributive law, \SideWS module, 2}1,
\eqRef{w()12= \SideNS}{\VectorSetNS}
следует, что
\DrawEq[w]{w()1+w()2= \SideNS}{\VectorSetNS}
Из равенства
\eqRef{|c(i)12 ne 0|}{\SideWS \VectorSetNS}
следует, что
множество
\ShowEq{|gi() 1+2 ne 0|}w
конечно.
\hfill\(\odot\)

\ShowLemma{w=aw in Xk-1}

{\sc Доказательство.}
Согласно утверждению
\RefItem[\RefRepresentation]{ax in Xk+1},
для любого $\Base_{\BaseExt}$\Hyph числа $a$,
\ShowEq{aw1 in Xk \SideWS module}
Согласно равенству
\eqRef{w=sum vi, module=Jv}{\SideWS \Base},
существуют $\Base_{\BaseExt}$\Hyph числа
\ShowEq{set au v(i)}w
такие, что
\ShowEq{w()= \SideWS module}
где
\DrawEq{|w(i) ne 0|}{\SideWS module}
Из равенства
\EqRef{w()= \SideWS module}
следует, что
\ShowEq{aw()= \SideWS module}
Из утверждения
\eqRef{|w(i) ne 0|}{\SideWS module}
следует, что
множество
\ShowEq{\SideWS module, |aw(i) ne 0|}
конечно.
\hfill\(\odot\)

\,
}

Из лемм
\refLemma{w=w12 in Xk-1}{\SideWS \VectorSet A},
\refLemma{w=aw in Xk-1}{\SideWS \VectorSetNS}
следует, что
\ShowEq{Xk in Jv}k
}

\DefProof{set of vectors generated* by set of vectors}
{
Мы докажем теорему по индукции, опираясь на теорему
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

Для произвольного
\ShowEq{vk in Jv}{}
положим
\ShowEq{c(i)=dik}
Тогда
\DrawEq[{\Base_{\BaseExt}}{}]{v(k)=sum v(i), \SideWS module*}{\Base}
Из равенств
\eqRef{w=sum vi, module=Jv*}{\SideWS \Base},
\eqRef{v(k)=sum v(i), \SideWS module*}{\Base}.
следует, что
теорема верна на множестве
\ShowEq{X0=v in J}

Пусть
\ShowEq{Xk in Jv}{k-1}
Согласно определению
\refDefinition{module over non-commutative algebra}{left \VectorSetNS}
и теоремам
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
если $w\in X_k$, то либо
\ShowEq{w=w12 in Xk-1},
либо
\ShowEq{w=a*w in Xk-1,\SideNS}

{\leftskip=25pt
\ShowLemma{w=w12 in Xk-1}{nonA}
\ShowProof{w=w12 in Xk-1}

\ShowLemma{w=a*w in Xk-1}
\ShowProof{w=a*w in Xk-1}

\,
}

Из лемм
\refLemma{w=w12 in Xk-1}{\SideWS \VectorSet A},
\refLemma{w=a*w in Xk-1}{\SideWS \VectorSetNS}
следует, что
\ShowEq{Xk in Jv}k
}

\DefLabeledTheorem{da in DA->da in D1A}{\SideWS module}
{
Отображение
\ShowEq{da in DA->da in D1A}
является гомоморфизмом \SideRu\From $\Base$\Hyph модуля $V$
в \SideRuTo $\Base_{(1)}$\Hyph модуль $V$.
}

\DefProof{da in DA->da in D1A}
{
Равенство
\DrawEq[{\AArg}]{(d1+0)+(d2+0)}{\SideWS module}
является следствием равенства
\eqRef{(a+n)+(b+m)=}{nd(\VectorSetNS)}.
Равенство
\DrawEq[{\AArg}]{(d1+0)(d2+0)}{\SideWS module}
является следствием равенства
\eqRef{(a+n)(b+m)=}{nd(\VectorSetNS)}.
Из равенств
\eqRef{(d1+0)+(d2+0)}{\SideWS module},
\eqRef{(d1+0)(d2+0)}{\SideWS module}
следует, что отображение $I_{(1)}$
является гомоморфизмом \ShortAlgebraRuBWS $\Base$
в \ShortAlgebraRuEWS $\Base_{(1)}$.

Равенство
\ShowEq{da in DA->da in D1A 1, \SideWS module}
является следствием равенства
\ShowRef{da in DA->da in D1A}
Теорема является следствием равенства
\EqRef{da in DA->da in D1A 1, \SideWS module}
и определения
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra}.
}

\DefLabeledConvention{da in DA->da in D1A}{\SideNS}
{
Согласно теоремам
\refTheorem{set of vectors generated by set of vectors}{\SideWS module},
\refTheorem{da in DA->da in D1A}{\SideWS module},
множество слов, порождающих
\SideRuTo $\Base$\Hyph модуль $V$,
совпадает с множество слов, порождающих
\SideRuTo $\Base_{(1)}$\Hyph модуль $V$.
Поэтому, не нарушая общности,
мы будем предполагать, что \algebrac $\Base$
имеет единицу.
}

\DefLabeledConvention{linear combination of vectors}{\SideNS}
{
Если необходимо явно указать,
что мы умножаем вектор $v(\gii)$
на $\Base_{\BaseExt}$\Hyph число $c(i)$ с\SideRu ва,
то мы будем называть выражение
\ShowEq{the linear combination()}
\AddIndex{\SideRu вой линейной комбинацией}{\SideWS linear combination}.
Мы будем применять это соглашение к аналогичным терминам.
Например, мы будем говорить, что вектор
\ShowEq{w=c(i)v(i)}
линейно зависит
от векторов
\ShowEq{set vi *}v
с\SideRu ва.
}

\DefLabeledDefinition{linear combination of vectors}{\SideNS}
{
Пусть $\Module$ - \SideRu\HSide \VectorSetRuA.
Пусть
\DrawEq[vV]{v(i) V}{}
- множество векторов.
\ShowEq{linear combination()}%
Выражение
\ShowEq{A linear combination() =}
называется
\AddIndex{линейной комбинацией}{linear combination} векторов
\ShowEq{v(i)}
Вектор
\ShowEq{w=c(i)v(i)}
называется
\AddIndex{линейно зависимым}{linearly dependent}
от векторов
\ShowEq{v(i)}
}

\DefLabeledDefinition{generating set of module}{\SideNS}
{
$J(v)$ называется
\AddIndex{подмодулем}{submodule},
порождённым множеством $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
подмодуля $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu\From $\Base$\Hyph модуля $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
}

\DefLabeledDefinition{generating set of vector space}{\SideNS}
{
$J(v)$
называется
векторным подпространством, порождённым множеством $v$,
а $v$ -
\AddIndex{множеством образующих}{generating set}
векторного подпространства $J(v)$.
В частности,
\AddIndex{множеством образующих}{generating set}
\SideRu вого $\Base$\Hyph векторного пространства $V$
будет такое подмножество $X\subset V$, что
\ShowEq{generating set of module}
}

\DefText{generating set of module}
{
Следующее определение является следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{set of vectors generated by set of vectors}{\SideWS \VectorSetNS}
и определения
\RefDefinition[\RefRepresentation]{generating set of representation}.
}

\DefText{quasibasis of module}
{
Следующее определение является следствием теорем
\RefTheorem[\RefRepresentation]{structure of subrepresentations},
\refTheorem{set of vectors generated by set of vectors}{\SideWS \VectorSetNS}
и определения
\RefDefinition[\RefRepresentation]{basis of representation}.
}

\DefDefinition{RCo product of matrices of maps}
{
Пусть
\ShowEq{Let aij rco bij}.
Мы определим \RCo произведение матриц отображений
\ShowEq{aij rco bij}
пользуясь равенством
\DrawEq{a rco b ij}o
}

\DefText{product of maps can be extended}
{
Рассмотренное выше
произведение отображений
\ShowEq{a o b=...}
может быть распространено на произведение матриц отображений
\ShowEq{matrix of maps}a,
\ShowEq{matrix of maps}b.
}

\DefLabeledDefinition{basis of module}{\SideNS}
{
Если множество $X\subset V$ является множеством образующих
\SideRu\From $\Base$\Hyph \VectorSetRuB $V$, то любое множество $Y$, $X\subset Y\subset V$
также является множеством образующих \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
Если существует минимальное множество $X$, порождающее
\SideRuTo $\Base$\Hyph \VectorSetRuA $V$, то такое множество $X$ называется
\AddIndex{квазибазисом}{quasibasis} \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
}

\DefLabeledTheorem{linearly depends on rest of vectors}{\SideWS module}
{
Пусть $\Base$ - \DivAlgebraRu.
Если уравнение
\DrawEq[wv]{wi vi=0}{1 \SideWS \Cols}
предполагает существования индекса
\ShowEq{i=j}
такого, что
\ShowEq{wj ne 0}w,
то вектор
\ARow vj{}
линейно зависит от остальных векторов $v$.
}

\DefProof{linearly depends on rest of vectors}
{
Теорема является следствием равенства
\ShowEq{\SideWS vj=sum vi}vw
и определения
\refDefinition{linear combination of vectors}{\SideNS}.
}

\DefText{0=0vi}
{
Очевидно, что для любого множества векторов
\ARow vi{}
\ShowEq{\SideWS 0=0vi}
}

\DefLabeledDefinitionNote{linearly independent vectors}{\SideNS}
{
Множество векторов\,\footnotemark
\ShowEq{set vi *}v
\SideRu\From $\Base$\Hyph \VectorSetRuB $V$
\AddIndex{линейно независимо}{linearly independent set},
если
\ShowEq{w(i)=0}c
следует из уравнения
\DrawEq[cv]{wi vi=0}{\SideNS}
В противном случае, множество векторов
\ShowEq{set vi *}v
\AddIndex{линейно зависимо}{linearly dependent set}.
}
{Я следую определению на страница
\citeBib{Serge Lang}\Hyph  100.}

\DefLabeledTheorem{quasibasis of module}{\SideNS}
{
Множество векторов
\ShowEq{basis, module}
является квазибазисом \SideRu\From $\Base$\Hyph модуля
$V$, если верны следующие утверждения.
\StartLabelItem
\begin{enumerate}
\item
\labelItem{vector is linear combination of set, \SideWS module}
Произвольный вектор $v\in V$
является линейной комбинацией
векторов множества $\Basis e$.
\item
\labelItem{cannot be represented as a linear combination, \SideWS module}
Вектор $e(\gii)$
нельзя представить в виде линейной комбинации
остальных векторов множества $\Basis e$.
\end{enumerate}
}

\DefProof{quasibasis of module}
{
Согласно утверждению
\RefItem{vector is linear combination of set, \SideWS module},
теореме
\refTheorem{set of vectors generated by set of vectors}{\SideWS module}
и определению
\refDefinition{linear combination of vectors}{\SideNS},
множество $\Basis e$ порождает \SideRuTo $\Base$\Hyph модуль $V$
(определение
\refDefinition{generating set of module}{\SideNS}).
Согласно утверждению
\RefItem{cannot be represented as a linear combination, \SideWS module},
множество $\Basis e$ является минимальным множеством,
порождающим \SideRuTo $\Base$\Hyph модуль $V$.
Согласно определению
\refDefinition{generating set of module}{\SideNS},
множество $\Basis e$ является квазибазисом  \SideRu\From $\Base$\Hyph модуля $V$.
}

\DefLabeledTheorem{basis over division algebra}{\SideNS}
{
Пусть $\Base$ - \AlgebraRu\DivisionRuNS.
Множество векторов
\ShowEq{basis, module}
является
\AddIndex{базисом \SideRu\From $\Base$\Hyph векторного пространства}{basis, vector space}
$V$, если векторы
\ARow ei
линейно независимы и любой вектор $v\in V$
линейно зависит от векторов
\ARow ei.
}

\DefLabeledTheorem{vector space is free module}{\SideNS}
{
\SideRuCTo $\Base$\Hyph векторное пространство
является свободным $\Base$\Hyph модулем.
}

\DefProof{basis over division algebra}
{
Пусть множество векторов
\ShowEq{set vi \Cols}e
линейно зависимо. Тогда в равенстве
\DrawEq[we]{wi vi=0}{}
существует индекс $\gii=\gij$ такой, что
\ShowEq{wj ne 0}w.
Согласно теореме
\refTheorem{linearly depends on rest of vectors}{\SideWS module},
вектор
\ARow ej{}
линейно зависит от остальных векторов множества $\Basis e$.
Согласно определению
\refDefinition{basis of module}{\SideNS},
множество векторов
\ShowEq{set vi \Cols}e
не является базисом \SideRu\From $\Base$\Hyph векторного пространства $V$.

Следовательно, если множество векторов
\ShowEq{set vi \Cols}e
является базисом, то эти векторы
линейно независимы.
Так как произвольный вектор $v\in V$
является линейной комбинацией векторов
\ShowEq{set vi \Cols}e
то множество векторов $v$,
\ShowEq{set vi \Cols}e
не является линейно независимым.
}

\DefLabeledConvention{unit of algebra in basis}{\Cols}
{
Пусть \eV - базис $D$\Hyph алгебры \ColsA $A$.
Если $D$\Hyph алгебра $A$ имеет единицу,
положим \ARow e0 - единица $D$\Hyph алгебры $A$.
}

\DefTheoremNote{algebra A2 representation in LA}
{
Пусть $A_1$ и $A_2$ являются $D$\Hyph алгебрами.
Пусть произведение в алгебре \AoxA A
определено согласно правилу
\DrawEq[pq]{product in algebra AA}{A2}
Линейное отображение
\ShowEq{representation A2 in LA}
определённое равенством
\ShowEq{representation A2 in LA, 1}
является представлением\,\footnotemark
алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
}
{Определение представления
$\Omega$\Hyph алгебры дано в определении
\ShowEq{ref definition: representation of algebra}.}

\DefLabeledTheorem[4]{matrix generates D module homomorphism}{\Cols(#1#2)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrix of numbers}D{#3}fiIjJ
Отображение\refFootnote{homomorphism of D module}{\Cols(#1#2)}
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
%\newline
определённое равенством
\ShowText{define homomorphism D module by matrix(#1)}
является гомоморфизмом
$D_{#1}$\Hyph модуля \ColsA $V_{#2}$
в $D_{#3}$\Hyph модуль \ColsA $V_{#4}$.
Гомоморфизм
\eqRef{homomorphism D algebra #1#2}{Vector module, coordinates \Cols},
который имеет%
\ShowText{define homomorphism by given matrix()}%
определён однозначно.
}

\DefProof[5]{matrix generates D module homomorphism}
{
Равенство
\ShowEq{fo(v+w) \Cols(#1)}
\begin{sloppypar}
\noindent
является следствием равенств
\ShowRef{homomorphism of D module}{#1}{#2}{#5}
Из равенства
\EqRef{fo(v+w) \Cols(#1)}
следует, что отображение $\Vector f$ является гомоморфизмом
абелевой группы.
Равенство
\end{sloppypar}
\ShowEq{fo(va) \Cols(#1)}
является следствием равенства
\eqRef{left homomorphism, f av=}{f D module #1#2}.
Из равенства
\EqRef{fo(va) \Cols(#1)}
и определений
\RefDefinition{Morphism of Diagram of Representations},
\refDefinition{linear map of D module}{#1#2}
следует, что отображение
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
\newline
\begin{sloppypar}
\noindent
является гомоморфизмом
$D_{#1}$\Hyph модуля \ColsA $V_{#2}$
в $D_{#3}$\Hyph модуль \ColsA $V_{#4}$.
\end{sloppypar}

Пусть $f$ -
матрица гомоморфизмов $\Vector f$, $\Vector g$
относительно базисов
\ShowEq{Bases eVW}12{}.%
Равенство
\ShowEq{fov=gov \Cols(#1)}
является следствием теоремы
\refTheorem{linear map of D module}{#1#2}.
Следовательно, $\Vector f=\Vector g$.
}

\DefLabeledTheorem[4]{matrix generates D algebra homomorphism}{\Cols(#1#2)}
{
\ShowText{map be homomorphism of ring (#1)}
\ShowText{matrix of numbers and C}D{#3}fiIjJ{#1}{#2}
Отображение\refFootnote{homomorphism of d algebra}{#1#2\Cols}
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
%\newline
определённое равенством
\ShowText{define homomorphism D module by matrix(#1)}
является гомоморфизмом
$D_{#1}$\Hyph алгебры \ColsA $A_{#2}$
в $D_{#3}$\Hyph алгебру \ColsA $A_{#4}$.
Гомоморфизм
\eqRef{homomorphism D algebra #1#2}{Vector module, coordinates \Cols},
который имеет%
\ShowText{define homomorphism by given matrix()}%
определён однозначно.
}

\DefProof[5]{matrix generates D algebra homomorphism}
{
Согласно теореме
\refTheorem{matrix generates D module homomorphism}{\Cols(#1#2)},
отображение
\eqRef{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
является гомоморфизмом
$D_{#1}$\Hyph модуля $A_{#2}$
в $D_{#3}$\Hyph модуль $A_{#4}$
и гомоморфизм
\eqRef{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
определён однозначно.

Пусть
\ShowEq{a=ai ei}a1i,
\ShowEq{a=ai ei}b1i.
Равенство
\DrawEq{algebra, homomorphism and product abe #1#2}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product (#1#2)}{\Cols(\SideNS)}.
\ShowText{matrix generates D algebra homomorphism (#1)}
Равенство
\DrawEq{algebra, homomorphism and product abe 3(#1)}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product abe 2(#1)}{\Cols}
и равенства
\ShowRef{homomorphism of d algebra, coordinates 1}{#1}{#2}
Равенство
\DrawEq{algebra, homomorphism and product abe 4(#1)}{\Cols}
является следствием равенства
\ShowEq{algebra, homomorphism and product, 1}
Равенство
\DrawEq{algebra, homomorphism and product abe 5(#1)}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product abe 4(#1)}{\Cols}
и равенства
\ShowRef{homomorphism of d algebra, coordinates 1}{#1}{#2}
Равенство
\ShowRef{homomorphism, f vw=}{#1}{#2}
является следствием равенств
\ShowRef{algebra, homomorphism and product 1}{#1}{#2}
Согласно теореме
\refTheorem{homomorphism from A1 to A2, D algebra}{#1#2},
отображение
\eqRef{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
является гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
}

\DefText{matrix generates D algebra homomorphism (1)}
{
Так как отображение $h$ является гомоморфизмом
кольца $D_1$ в кольцо $D_2$, то
\DrawEq{algebra, homomorphism and product abe 2}{\Cols}
Равенство
\DrawEq{algebra, homomorphism and product abe 2(1)}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product abe 2}{\Cols}
и равенства
\ShowRef{product in algebra}
}

\DefText{matrix generates D algebra homomorphism ()}
{
Равенство
\DrawEq{algebra, homomorphism and product abe 2()}{\Cols}
является следствием равенства
\ShowRef{product in algebra}
}

\DefLabeledDefinition[1]{exact sequence, D module}{(#1)}
{
Пусть
\ShowEq{Ai, 1n}V
- $D_{#1}$\Hyph модули.
Последовательность гомоморфизмов
\ShowEq{V1->...->Vn (#1)}
называется
\AddIndex{точной}{exact sequence},
если
\ShowEq{Im f=ker hf (#1)}
}

\DefTheorem{submodule is kernel}
{
Пусть $D$\Hyph модуль $V_1$ является свободной аддитивной группой.
Пусть $U$ - подмодуль $D$\Hyph модуля $V_1$.
Существует гомоморфизм
\newline
\FrameEqRef[fV]{homomorphism D algebra 1}{Vector module, coordinates \Cols}
\newline
такой, что
\[\ker f=U\]
}

\DefProof{submodule is kernel}
{
Согласно теореме
\RefTheorem{direct sum of submodules},
существует подмодуль $W$ такой, что
\ShowEq{V=Uo+W}1
Отображение
\ShowEq{u o+ w->w}
является гомоморфизмом и
\[\ker f=U\]
}

\DefTheorem{direct sum of submodules}
{
Пусть $D$\Hyph модуль $V$ является свободной аддитивной группой.
Пусть $U$ - подмодуль $D$\Hyph модуля $V$.
Существует подмодуль $W$ такой, что
\ShowEq{V=Uo+W}{}
}

\DefProof{direct sum of submodules}
{
Согласно определениям
\refDefinition{module over algebra}{\SideWS \VectorSetNS},
\refDefinition{submodule}{\SideWS module},
$U$ является подгруппой аддитивной группы $V$.
Согласно теоремам
\RefTheorem{A=C o+ D free group},
\RefTheorem{B=Ao+B/A},
существует подгруппа $W$ аддитивной группы $V$ такая, что
группа $W$ изоморфна группе $V/U$ и
\ShowEq{V=Uo+W}{}

Согласно теореме
\refTheorem{direct sum of D modules 2024}{\SideWS \Base-\VectorsSetNS},
действие $D$\Hyph числа $a$ на произвольное $V$\Hyph число
\ShowEq{v=u0+0w}
имеет вид
\ShowEq{av=u0+0w}
Следовательно, $W$ является подмодулем $D$\Hyph модуля $V$.
}

\DefLabeledFootnote[4]{homomorphism of D module}{\Cols(#1#2)}
{
В теоремах
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
\refTheorem{matrix generates D module homomorphism}{\Cols(#1#2)},
мы опираемся на следующее соглашение.
\ShowEq{Let be basis of module}1{}iI{}D{#1}V{#2}
\ShowEq{Let be basis of module}2{}jJ{}D{#3}V{#4}
}

\DefLabeledFootnote[6]{homomorphism of A module}{\SideNS-\Cols(#1#2#3)}
{
В теоремах
\refTheorem{homomorphism A module}{\SideNS-\Cols(#1#2#3)},
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)},
мы опираемся на следующее соглашение.
\ShowEq{prolog homomorphism of vector space(#1#2#3)}{#1}{#2}{#3}{#4}{#5}{#6}
}

\DefLabeledFootnote[6]{Coordinates of Linear Map}{\SideNS-\Cols(#1#2#3)}
{
В теореме %ах
\refTheorem{linear map of A module, coordinates}{\SideNS-\Cols(#1#2#3)},
%\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)},
мы опираемся на следующее соглашение.
\ShowEq{prolog homomorphism of vector space 2020(#1#2#3)}{#1}{#2}{#3}{#4}{#5}{#6}
}

\DefLabeledFootnote[6]{homomorphism of A module 2020}{\SideNS-\Cols(#1#2#3)}
{
В теоремах
\refTheorem{homomorphism A module 2020}{\SideNS-\Cols(#1#2#3)},
\refTheorem{matrix generates A module homomorphism}{\SideNS-\Cols(#1#2#3)},
мы опираемся на следующее соглашение.
\ShowEq{prolog homomorphism of vector space 2020(#1#2#3)}{#1}{#2}{#3}{#4}{#5}{#6}
}

\DefLabeledDefinition[4]{homomorphism from A1 to A2, D algebra}{#1#2}
{
\ShowText{algebra over ring (#1#2)}
Пусть
\DrawEq[{#1}{1.}{#2}h]{diagram of representations of D algebra}{->1(#1#2)}
диаграмма представлений, описывающая $D_1$\Hyph алгебру $A_1$.
Пусть
\DrawEq[{#3}{2.}{#4}h]{diagram of representations of D algebra}{->2(#1#2)}
диаграмма представлений, описывающая $D_2$\Hyph алгебру $A_2$.
Морфизм
\DrawEq[fA]{homomorphism D algebra #1#2}1
диаграммы представлений
\eqRef{diagram of representations of D algebra}{->1(#1#2)}
в диаграмму представлений
\eqRef{diagram of representations of D algebra}{->2(#1#2)}
называется
\AddIndex{гомоморфизмом}{homomorphism}
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
Обозначим
\ShowEq{set homomorphisms, D algebra #1#2}
множество гомоморфизмов
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$.
}

\DefLabeledTheorem[5]{homomorphism from A1 to A2, D algebra}{#1#2}
{
Гомоморфизм
\newline
\FrameEqRef[fA]{homomorphism D algebra #1#2}1
\newline
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#3}$\Hyph алгебру $A_{#4}$
- это линейное отображение
\eqRef[fA]{homomorphism D algebra #1#2}1
$D_{#1}$\Hyph модуля $A_{#2}$
в $D_{#3}$\Hyph модуль $A_{#4}$
такое, что
\DrawEq[fab]{homomorphism, f vw=}{(#1#2)g}
и удовлетворяет следующим равенствам
\ShowEq{define homomorphism of D algebra #1#2}{#1}{#2}{#5}
}

\DefProof[4]{homomorphism from A1 to A2, D algebra}
{
Согласно определениям
\ShowRef{Morphism of Diagram of Representations}
отображение
\eqRef{homomorphism D algebra #1#2}1
явлется морфизмом представления $h_{1.12}$,
описывающего $D_{#1}$\Hyph модуль $A_{#2}$,
в представления $h_{2.12}$,
описывающего $D_{#3}$\Hyph модуль $A_{#4}$.
Следовательно, отображение $f$ является линейным отображением $D_{#1}$\Hyph модуля $A_{#2}$
в $D_{#3}$\Hyph модуль $A_{#4}$ и равенства
\ShowEq{ref homomorphism of D algebra(#1)}{#1}{#2}
являются следствием теоремы
\refTheorem{linear map of D module}{#1#2}.

Согласно определениям
\ShowRef{Morphism of Diagram of Representations}
отображение $f$
явлется морфизмом представления $h_{1.23}$
в представления $h_{2.23}$.
Равенство
\DrawEq{morphism of representation, algebra, 23}{#1#2}
следует из равенства
\eqRef{morphism of representations of universal algebra, 2m}{representation}.
Из равенств
\eqRef{diagram of representations of D algebra}{->1(#1#2)},
\eqRef{diagram of representations of D algebra}{->2(#1#2)},
\eqRef{morphism of representation, algebra, 23}{#1#2},
следует
\DrawEq{algebra, morphism of representation 23, 1}{#1#2}
Равенство
\eqRef{homomorphism, f vw=}{(#1#2)g}
следует из равенств
\eqRef{product in D algebra}{definition},
\eqRef{algebra, morphism of representation 23, 1}{#1#2}.
}

\AddEq{definition: unital algebra}
{
\begin{ShadedDefinition}
\labelDefinition{unital algebra}
Если произведение в $D$\Hyph алгебре $A$ имеет единичный элемент,
то $D$\Hyph алгебра $A$ называется
\AddIndex{унитальной алгеброй}{unital algebra}.\,\footnotemark
\end{ShadedDefinition}
\footnotetext{\,
Смотри определение унитальной алгебры также на страницах
\citeBib{McCrimmon: Jordan Algebras}\Hyph 137.
}
}

\DefDefinition{division algebra}
{
\(D\)\Hyph алгебра \(A\) называется
\AddIndex{алгеброй с делением}{division algebra},
если для любого \(A\)\Hyph числа \(a\ne 0\)
существует \(A\)\Hyph число \(a^{-1}\).
}

\DefTheorem{division algebra}
{
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Из утверждения
\ShowEq{ab=ac a ne 0}
следует, что $b=c$.
}

\DefProof{division algebra}
{
Равенство
\ShowEq{ab=ac a ne 0 1}
является следствием утверждения
\EqRef{ab=ac a ne 0 1}.
}

\DefLabeledDefinition[4]{linear map of D module}{#1#2}
{
Морфизм представлений
\DrawEq[fV]{homomorphism D algebra #1#2}{module}
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$
называется гомоморфизмом или
\AddIndex{линейным отображением}{linear map}
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$.
Обозначим
\ShowEq{set linear maps, module (#1#2)}DV
множество линейных отображений
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$.
}

\DefTheorem[3]{module of skew symmetric polylinear maps}
{
Множество
\ShowEq{module of skew symmetric polylinear maps}{#1}{#2}{#3}
косо симметричных полилинейных отображений
является $D$\Hyph модулем.
}

\AddEq[3]{remark: module of skew symmetric polylinear maps}
{
Не нарушая общности, мы положим
\ShowEq{L(A1,A0,B)=}{#1}{#2}{#3}
}

\DefTheorem{norm in D module A->B}
{
Пусть $A$ - нормированный $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - нормированный $D$\Hyph модуль с нормой $|y|_B$.
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
}

\DefTheorem{set of A->B is D module}
{
Пусть $A$ - банаховый $D$\Hyph модуль с нормой $|x|_A$.
Пусть $B$ - банаховый $D$\Hyph модуль с нормой $|y|_B$.
\StartLabelItem
\begin{enumerate}
\item
Множество
$B^A$
отображений
\ShowEq{f:A->B}fAB
является $D$\Hyph модулем.
\labelItem{set of A->B is D module}
\item
Отображение
\ShowEq{f in BA->|f|}
определённое равенством
\ShowEq{norm of map}
\ShowEq{norm of map, algebra}
является нормой в $D$\Hyph модуле $B^A$
и величина
\ShowEq{show|f|}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
\labelItem{norm of map}
\end{enumerate}
}

\DefTheorem{symmetrization of polylinear map}
{
Пусть
\ShowEq{f in L(A->B)}D{A^n}B{}
- полилинейное отображение.
Тогда отображение
\ShowEq{symmetrization of polylinear map}
\EqParm{<f>}{=c}
определённое равенством
\ShowEq{symmetrization of polylinear map =}
является симметричным полилинейным отображением
и называется
\AddIndex{симметрированием полилинейного отображения}{symmetrization of polylinear map}
$f$.
}

\DefTheorem{exterior product = skew symmetric}
{
Внешнее произведение удовлетворяет следующему равенству
\ShowEq{exterior product = skew symmetric}
}

\DefProof{exterior product = skew symmetric}
{
Равенство
\EqRef{exterior product = skew symmetric}
является следствием равенств
\EqRef{alternation of polylinear map =},
\EqRef{exterior product =}.
}

\DefDefinition{exterior product polylinear map}
{
Косо симметричное полилинейное отображение
\ShowEq{exterior product}
\ShowEq{exterior product =}
называется
\AddIndex{внешним произведением}{exterior product}.
}

\AddEq{remark: product of polylinear maps}
{
Если $B_1=B_2$, то в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем произведение $B_1$\Hyph чисел
\ShowEq{f()},
\ShowEq{g()}.
Согласно теореме
\RefTheorem{Free Algebra over Ring},
это определение совместимо с определением
\RefDefinition{product of polylinear maps}.
}

\AddEq{definition: product of polylinear maps}
{
\begin{ShadedDefinition}
\labelDefinition{product of polylinear maps}
Пусть $A$, $B_2$ - свободные алгебры над коммутативным кольцом $D$.\,\footnotemark
Пусть
\ShowEq{h:B1->*B2}
левостороннее представление
свободной ассоциативной $D$\Hyph алгебры $B_1$ в $D$\Hyph модуле $B_2$.
Отображение
\ShowEq{hpq:Lpq->Lp+q}
определено равенством
\ShowEq{hpq(fg)=}
где в правой части равенства
\EqRef{hpq(fg)=}
мы предполагаем левостороннее произведение
$B_2$\Hyph числа
\ShowEq{g()}{}
на $B_1$\Hyph число
\ShowEq{f()}.
\end{ShadedDefinition}
\footnotetext{\,
Я дал определение произведения косо симметричных полилинейных отображениий
согласно определению в разделе
\citeBib{Cartan differential form}-1.4 главы 3,
страницы 195 - 198.
}
}

\DefDefinition{symmetric polylinear map}
{
Пусть $A$, $B$ - алгебры над коммутативным кольцом $D$.
Полилинейное отображение
\ShowEq{f in L(A->B)}D{A^n}B{}
называется
\AddIndex{симметричным}{symmetric polylinear map},
если
\ShowEq{fa=fsa}
для любой перестановки $\sigma$ множества
\ShowEq{set a1n}.
}

\DefTheoremNote{fx1n=0, xi=xi1}
{
Полилинейное отображение
\ShowEq{f in L(A->B)}D{A^n}B{}
косо симметрично тогда и только тогда, когда
\ShowEq{fx1n=0}
при условии
$a_i=a_{i+1}$
хотя бы для одного\,\footnotemark
\ShowEq{1<=i<n}
}{
В книге
\citeBib{Cartan differential form},
страница 192,
Анри Картан рассматривает теорему
\RefTheorem{fx1n=0, xi=xi1}
как определение косо симметричного отображения.
}

\DefTheorem[3]{alternation of polylinear map}
{
Пусть
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
- полилинейное отображение.
Тогда отображение
\ShowEq{alternation of polylinear map}
\ShowEq{[f]},
определённое равенством
\ShowEq{alternation of polylinear map =}
является косо симметричным полилинейным отображением
и называется
\AddIndex{альтернацией полилинейного отображения}{alternation of polylinear map}
$f$.
}

\DefDefinition[3]{skew symmetric polylinear map}
{
Полилинейное отображение
\ShowEq{f in L(A->B)}{#1}{#2^n}{#3}{}
называется
\AddIndex{косо симметричным}{skew symmetric polylinear map},
если
\ShowEq{fa=sfsa}
для любой перестановки $\sigma$ множества
\ShowEq{set a1n}.
}

\DefText[4]{quasibasis of A-module}
{
Пусть
\DrawEq[{#2}{#3}{#4}]{basis e of module cols}-
- квазибазис $A$\Hyph модуля $#1$.
}

\DefLabeledTheorem{a quasibasis of A}{\SideNS}
{
$D$\Hyph алгебра $A$ имеет квазибазис
\ShowEq{e=a in A}
если
\ShowEq{Aa=A}
и $A$\Hyph число $a$ является \OtherSideRu вым делителем нуля.
}

\DefText[2]{quasibasis 1n of A-module}
{
Пусть
\ShowEq{basis e of module 1n}{#1}{#2}
квазибазис $A$\Hyph модуля $#1$.
}

\DefTheorem{there exist tensor g=1/f}
{
Пусть
$\aUD Ck{ij}$
- структурные константы $D$\Hyph алгебры $A$.
Пусть
\DrawEq[f]{f=...ei o ek}{f-}
стандартное представление тензора
\ShowEq{f in AoA}f.
Пусть существует тензор
\ShowEq{g=f-}{}{}
и
\DrawEq[g]{f=...ei o ek}{g-}
стандартное представление тензора $g$.
Тогда стандартные компоненты тензора $g$
удовлетворяют системе линейных уравнений
\ShowEq{fg=1 e o e}
}

\DefProof{there exist tensor g=1/f}
{
Теорема является следствием равенства
\ShowEq{g o h=1}
и теоремы
\RefTheorem{standard representation of product of tensors}.
}

\DefText{system of linear equations linear map}
{
Пусть
\ShowEq{f:A->B}fVW
линейное отображение $A$\Hyph векторного пространства $V$
в $A$\Hyph векторное пространство $W$.
Отображение координатной матрицы вектора $v\in V$
относительно базиса $\Basis e_V$
в координатную матрицу вектора $f\circ v\in W$
относительно базиса $\Basis e_W$
имеет вид
\DrawEq[vf{(f\circ v)}mn]{system of linear equations linear map}{}
и не зависит от того, рассматриваем мы левое $A$\Hyph векторное пространство
или правое $A$\Hyph векторное пространство.
Чтобы найти координатную матрицу вектора
\ShowEq{v in V, fv=w}
мы должны решить систему линейных уравнений
\DrawEq[vfwmn]{system of linear equations linear map}{preface}
}

\DefLabeledTheorem[2]{direct sum over quasibasis}{\Cols,\SideNS-\VectorSetNS}
{
\def\Temp{#2}%
\def\One{1}%
\ifx\Temp\One%
\ShowText{quasibasis of A-module}V{}iI
\else%
\ShowEq{Let be basis of module}1{}iI{\SideRu\Which}{#1}{}V{}
\fi%
Тогда мы можем представить $#1$\Hyph модуль $V$
как прямую сумму
\DrawEq[{#1}{}]{V=+eiA}{\SideWS \Cols}
}

\DefProof[1]{direct sum over quasibasis}
{
Отображение
\ShowEq{V->+eiA}{#1}
является изоморфизмом.
}

\DefLabeledTheorem{quasibasis and linear map}{\SideWS \Cols}
{
\ShowText{quasibasis of A-module}VViI
\ShowText{quasibasis of A-module}WWjJ
Тогда линейное отображение
\DrawEq[{\Vector f}VW{}]{f: A->B}{fVW \SideWS \Cols}
имеет представление
\DrawEq{quasibasis and linear map}{\SideWS \Cols}
где матрица
\DrawEq{quasibasis and matrix of linear map}{\SideWS \Cols}
называется матрицей линейного отображения $\Vector f$
относительно выбранных базисов.
}

\DefLabeledTheorem{finite quasibasis and product linear map}{}
{
\ShowText{quasibasis 1n of A-module}Uk
\ShowText{quasibasis 1n of A-module}Vn
\ShowText{quasibasis 1n of A-module}Wm
Пусть линейное отображение
\DrawEq[{\Vector f}UV{}]{f: A->B}{}
имеет представление
\DrawEq[funk]{quasibasis nm and linear map}{fu \SideWS \Cols}
относительно выбранных квазибазисов.
Пусть линейное отображение
\DrawEq[{\Vector g}VW{}]{f: A->B}{}
имеет представление
\DrawEq[gvmn]{quasibasis nm and linear map}{gv \SideWS \Cols}
относительно выбранных квазибазисов.
Тогда линейное отображение $f\circ g$
имеет матрицу
\ShowEq{matrix linear f o g}
\ShowEq{matrix linear (f o g)}
относительно выбранных квазибазисов.
}

\DefLabeledTheorem{finite quasibasis and linear map}{}
{
\ShowText{quasibasis 1n of A-module}Vn
\ShowText{quasibasis 1n of A-module}Wm
Тогда линейное отображение
\newline
\FrameEqRef[{\Vector f}VW{}]{f: A->B}{fVW \SideWS \Cols}
\newline
имеет представление
\DrawEq[fvnm]{quasibasis nm and linear map}{\SideWS \Cols}
относительно выбранных квазибазисов.
}

\DefText{linear dependence between vectors of basis}
{
Согласно теореме
\refTheorem{linear dependence between vectors of basis}{\SideWS module},
может существовать линейная зависимость между векторами квазибазиса.
}

\DefLabeledTheorem{linear dependence between vectors of basis}{\SideWS module}
{
Пусть $\Base$ - \Algebra.
Пусть $\Basis e$ - квазибазис \SideRu\From $\Base$\Hyph \VectorSetRuB $V$.
Пусть
\DrawEq[ce]{wi vi=0}{we \SideWS \Cols}
линейная зависимость векторов квазибазиса $\Basis e$.
Тогда
\StartLabelItem
\begin{enumerate}
\item
$\Base_{\BaseExt}$\Hyph число
\ShowEq{ci i in I}
не имеет обратного элемента
в \ShortAlgebraRuDWS $\Base_{\BaseExt}$.
\item
Множество $V'$ матриц
\ShowEq{c=ci i in I}
порождает \SideRuTo $\Base$\Hyph модуль $V'$.
\end{enumerate}
}

\DefProof{linear dependence between vectors of basis}
{
Допустим существует матрица
\ShowEq{c=ci i in I}
такая, что равенство
\eqRef{wi vi=0}{we \SideWS \Cols}
верно и существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}c.
Если мы положим, что $\Base$\Hyph число
\ACol cj
имеет обратный, то равенство
\ShowEq{\SideWS vj=sum vi}ec
является следствием равенства
\eqRef{wi vi=0}{we \SideWS \Cols}.
Следовательно вектор
\ARow ej{}
является линейной комбинацией остальных векторов множества $\Basis e$
и множество $\Basis e$ не является квазибазисом.
Следовательно, наше предположение неверно,
и $\Base_{\BaseExt}$\Hyph число
\ACol cj
не имеет обратного.

Пусть матрицы
\ShowEq{b in D'}b,
\ShowEq{b in D'}c.
Из равенств
\DrawEq[be]{wi vi=0}{}
\DrawEq[ce]{wi vi=0}{}
следует
\ShowEq{(b+c)*e, \SideWS module}
Следовательно, множество $\Base'$ является абелевой группой.

Пусть матрица
\ShowEq{b in D'}c{}
и $a\in\Base$.
Из равенства
\DrawEq[ce]{wi vi=0}{}
следует
\ShowEq{(ac)*e, \SideWS module}
Следовательно, абелевая группа $\Base'$ является \SideRu\What $\Base$\Hyph модулем.
}

\DefLabeledTheorem{coordinates of vector with linear dependence}{\SideWS module}
{
Пусть \SideRuTo $\Base$\Hyph модуль $V$
имеет квазибазис $\Basis e$ такой, что в равенстве
\DrawEq[ce]{wi vi=0}{2 we \SideWS \Cols}
существует индекс
\ShowEq{i=j}
такой, что
\ShowEq{wj ne 0}c.
Тогда
\StartLabelItem
\begin{enumerate}
\item
Матрица
\ShowEq{c=ci i in I}
определяет координаты вектора $0\in V$ относительно квазибазиса $\Basis e$.
\labelItem{coordinates of vector 0 with linear dependence, \SideWS module}
\item
Координаты вектора $\Vector v$ относительно квазибазиса $\Basis e$
определены однозначно с точностью до выбора координат вектора $0\in V$.
\labelItem{coordinates of vector with linear dependence, \SideWS module}
\end{enumerate}
}

\DefProof{coordinates of vector with linear dependence}
{
Утверждение
\RefItem{coordinates of vector 0 with linear dependence, \SideWS module}
является следствием равенства
\eqRef{wi vi=0}{2 we \SideWS \Cols}
и определения
\refDefinition{coordinates of vector}{\SideWS \VectorSetNS}.

Пусть вектор $\Vector v$ имеет разложение
\DrawEq{vv=ve \SideWS module}{2}
относительно квазибазиса $\Basis e$.
Равенство
\ShowEq{v=v+0, \SideWS module}
является следствием равенств
\eqRef{wi vi=0}{2 we \SideWS \Cols},
\eqRef{vv=ve \SideWS module}{2}.
Утверждение
\RefItem{coordinates of vector with linear dependence, \SideWS module}
является следствием равенств
\eqRef{vv=ve \SideWS module}{2},
\EqRef{v=v+0, \SideWS module}
и определения
\refDefinition{coordinates of vector}{\SideWS \VectorSetNS}.
}

\DefLabeledTheorem{quasibasis of module is basis}{\SideWS \VectorSetNS}
{
Пусть множество векторов квазибазиса \eV
\SideRu\From $\Base$\Hyph модуля $V$
линейно независимо.
Тогда квазибазис \eV является
базисом \SideRu\From $\Base$\Hyph модуля $V$.
}

\DefProof{quasibasis of module is basis}
{
Теорема является следствием определения
\RefDefinition{basis of representation}
и теоремы
\refTheorem{coordinates of vector with linear dependence}{\SideWS module}.
}

\DefLabeledDefinitionNote{free module over ring}{\SideNS}
{
\SideRuCTo $\Base$\Hyph модуль $V$ -
\AddIndex{свободный \SideRuTo $\Base$\Hyph модуль}{free module},\,\footnotemark
если \SideRuTo $\Base$\Hyph модуль $V$ имеет базис.
}
{
Я следую
определению в \citeBib{Serge Lang}, страница 103.
}

\DefProof{coordinates of vector of free module}
{
Теорема является следствием теоремы
\refTheorem{coordinates of vector with linear dependence}{\SideWS module}
и определений
\refDefinition{linearly independent vectors}{\SideNS},
\refDefinition{free module over ring}{\SideNS}.
}

\DefTheoremNote{standard representation of map A->A, associative algebra}
{
Пусть $A$ - конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis F$
- базис\,\footnotemark
левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f in L(A->B)}DAA{}
имеет следующее разложение
\labelItem{map f generated by basis F, associative algebra}
\DrawEq{map f generated by basis F}{associative algebra}
где
\ShowEq{fk= in AxA}
\item
Линейное отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, associative algebra}
\ShowEq{standard representation of map A->A, o, associative algebra}
\end{enumerate}
}{
Если $D$\Hyph модуль $A$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\ShowEq{f:A->B}fAA
порождённого множеством линейных отображений $\Basis F$.
}

\DefProof{standard representation of map A->A, associative algebra}
{
Поскольку $\Basis F$ является базисом левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA,
то согласно определению
\refDefinition{free module over ring}{\SideNS},
существует разложение
\DrawEq[A]{expansion of linear map with respect to basis}A
линейного отображения $f$ относительно базиса $\Basis F$.
Согласно определению
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{associative algebra}
Равенство
\eqRef{map f generated by basis F}{associative algebra}
является следствием равенств
\eqRef{expansion of linear map with respect to basis}A,
\eqRef{f=fkxfk}{associative algebra}.
Согласно теореме
\RefTheorem{standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A->A, associative algebra}
следует из равенств
\eqRef{map f generated by basis F}{associative algebra},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheoremNote{set FoG generates left module L(A;B), n<m}
{
Пусть $A$ - $D$\Hyph модуль,
\ShowEq{n=dim A}nA.
Пусть $B$ - ассоциативная $D$\Hyph алгебра,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{gi n<m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}1
порождает левый \BoxB{B}модуль\,\footnotemark
\ShowEq{L(A->B)}DAB.
}{
Я не утверждаю, что это множество является базисом,
так как отображения
\ShowEq{FijG}
могут быть линейно зависимыми.
}

\DefProof{set FoG generates left module L(A;B), n<m}
{
Пусть
\ShowEq{f:A->B}gAB
линейное отображение.
Пусть $\Basis e_A$ - базис $D$\Hyph модуля $A$.
Пусть $\Basis e_B$ - базис $D$\Hyph модуля $B$.
Согласно теореме
\ShowEq{ref linear map of D1 D2 module, coordinates}
линейное отображение $G$ имеет координаты
\ShowEq{matrix amn}Gmn
относительно базисов $\Basis e_A$, $\Basis e_B$
и линейное отображение $g$ имеет координаты
\ShowEq{matrix amn}gmn
относительно базисов $\Basis e_A$, $\Basis e_B$.
Строка $G_{\gii}$ матрицы $G$,
также как строка $g_{\gii}$ матрицы $g$,
является координатами линейной формы
\DrawEq[AD.]{A->B}{}
Поскольку матрица $G$ имеет максимальный ранг,
то строки матрицы $G$ порождают $D$\Hyph модуль
\ShowEq{L(A->B)}DAD{}
и строки матрицы $g$ являются линейной комбинацией строк матрицы $G$
\ShowEq{g=CG}
Поскольку мы можем рассматривать матрицу $C$
как координаты линейного отображения
\ShowEq{f:A->B}CBB
то равенство
\ShowEq{g=(cF)G}
является следствием равенства
\EqRef{g=CG}
и равенства
\ShowEq{C=cF}
Поскольку
\ShowEq{Gkj in D}
то равенство
\ShowEq{g=c(FG)}
является следствием равенства
\EqRef{g=(cF)G}.
Следовательно, отображение $g$ принадллежит
линейной оболочке множества отображений
\eqRef{F o G}1.
}

\DefTheorem{set FoG generates left module L(A;B), n>m}
{
Пусть
\ShowEq{n=dim A}nA,
\ShowEq{n=dim A}mB.
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{gi n>m}
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B), n>m}
{
Доказательство теоремы похоже на доказательство теоремы
\RefTheorem{set FoG generates left module L(A;B), n<m}.
Однако, так как число строк матрицы $G$ меньше размерности
$D$\Hyph модуля $A$, то строки матрицы $G$ не порождают $D$\Hyph модуль
\ShowEq{L(A->B)}DAD{}
и отображение $G$ имеет нетривиальное ядро.
В частности, строки матрицы $g$ линейно зависят от строк матрицы $G$
тогда и только тогда, когда
\ShowEq{ker G in ker g}g.
}

\DefTheorem{set FoG generates left module L(A;B)}
{
Пусть $\Basis F$ - базис левого \BoxB{B}модуля
\ShowEq{L(A->B)}DBB.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга.
Множество
\DrawEq{F o G}{}
порождает множество отображений
\ShowEq{set ker G in ker g}
}

\DefProof{set FoG generates left module L(A;B)}
{
Нетрудно убедиться, что теорема
\RefTheorem{set FoG generates left module L(A;B), n<m}
является частным случаем теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
так как в теореме
\RefTheorem{set FoG generates left module L(A;B), n>m}
$\ker G=\emptyset$.
}

\AddEq{remark: set FoG generates left module L(A;B), n>m}
{
Из теоремы
\RefTheorem{set FoG generates left module L(A;B), n>m},
следует, что
выбор отображения $G$ зависит от отображения $g$.
}

\DefTheorem{basis D module L(D->A)}
{
%Пусть тождественное отображение
%\ShowEq{f:A->B}IDD
%является базисом $D$\Hyph модуля
%\ShowEq{L(A->B)}DDD.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Тогда множество отображений
\ShowEq{d->dei}i
является базисом $D$\Hyph модуля
\ShowEq{L(A->B)}DDA.
}

\DefProof{basis D module L(D->A)}
{
Теорема является следствием равенства
\ShowEq{f(t)=fit ei}
}

\DefDefinition{component of linear map}
{
Выражение
\ShowEq{component of linear map}
в равенстве
\EqRef{fk= in AxA}
называется
\AddIndex{компонентой линейного отображения}
{component of linear map} $f$.
Выражение
\ShowEq{standard component of linear map}
в равенстве
\EqRef{standard representation of map A->A, associative algebra}
называется
\AddIndex{стандартной компонентой линейного отображения}
{standard component of linear map} $f$.
}

\DefTheorem{endomorphism of module from product}
{
Представление
\ShowEq{endomorphism of module from product}
$D$\Hyph модуля $A$ в $D$\Hyph модуле $A$
эквивалентно структуре $D$\Hyph алгебры $A$.
}

\DefLabeledConvention{sum av() convention}{\SideNS}
{
Мы будем пользоваться соглашением о сумме,
в котором повторяющийся индекс
в линейной комбинации
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av()\SideNS}
Я буду явно указывать множество индексов, если это необходимо.
}

\DefConvention{av=sum av convention}
{
Мы будем пользоваться соглашением Эйнштейна о сумме,
в котором повторяющийся индекс (один вверху и один внизу)
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av}cd
Я буду явно указывать множество индексов, если это необходимо.
}

\DefLabeledTheorem{effective representation of the ring}{\SideWS \Base-\VectorsSetNS}
{
Представление
\ShowEq{f:A->*B}f{\Base}V
\algebrae $\Base$
в абелевой группе $V$
\AddIndex{эффективно}{effective representation}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
}

\DefProof{effective representation of the ring}
{
Если $a$, $b\in \Base$
порождают одно и то же преобразование, то
\DrawEq{representation of ring, 1}{\Base}
для любого $m\in V$.
Из равенств
\eqRef{sum of transformations of Abelian group, 1}{\Base},
\eqRef{representation of ring, 1}{\Base}
следует, что
\DrawEq{representation of ring, 2}{\Base}
Равенство
\ShowEq{f(a-b)=0}
является следствием равенств
\eqRef{0ov=0}{\Base},
\eqRef{representation of ring, 2}{\Base}.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
}

\DefLabeledTheorem{Representation of ring f(0)=v0}{\SideWS \Base-\VectorsSetNS}
{
Представление
\ShowEq{f:A->*B}f{\Base}V
\algebrae $\Base$
в абелевой группе $V$
удовлетворяет равенству
\DrawEq{f(0)=v0}{\Base}
где
\ShowEq{0:V->V}
отображение такое, что
\DrawEq{0ov=0}{\Base}
}

\DefProof{Representation of ring f(0)=v0}
{
Равенство
\DrawEq{fa=fa+f0}{\Base}
является следствием равенства
\eqRef{sum of transformations of Abelian group, 1}{\Base}.
Равенство
\DrawEq{f0x=0}{\Base}
является следствием равенства
\eqRef{fa=fa+f0}{\Base}.
Равенство
\eqRef{0ov=0}{\Base}
является следствием равенств
\eqRef{f(0)=v0}{\Base},
\eqRef{f0x=0}{\Base}.
}

\DefText{sum of transformations of Abelian group}
{
Согласно теореме
\refTheorem{monoid-homomorphism, sum}{+},
рассматривая представление
\ShowEq{f:A->*B}f{\Base}V
\algebrae $\Base$ в абелевой группе $V$, мы полагаем
\DrawEq{f(a)+f(b)=}{\Base}
Согласно определению
\RefDefinition{representation of algebra},
отображение $f$ является гомоморфизмом \algebrae $\Base$.
Следовательно
\DrawEq{f(a+b)=f(a)+f(b)}{\Base}
Равенство
\DrawEq{sum of transformations of Abelian group, 1}{\Base}
является следствием равенств
\eqRef{f(a)+f(b)=}{\Base},
\eqRef{f(a+b)=f(a)+f(b)}{\Base}.
}

\AddEq{remark: we do not have definition of determinant for division algebra}
{
Согласно
\citeBib{q-alg-9705026},
\citeBib{math.QA-0208146},
у нас нет определения
детерминанта в случае алгебры с делением.\,\footnote{
В алгебре кватернионов профессор Кирчей
пользуется двойным определителем
(смотри определение в разделе
\citeBib{1812.03397}\Hyph 2.2)
для решения системы линейных уравнений
и для решения задачи о собственных значениях
(смотри раздел
\citeBib{1812.03397}\Hyph 2.5).
Я ограничился рассмотрением квазидетерминантов,
так как меня интересует более широкий класс алгебр.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOn

\FrameCiteBib{1812.03397}
\fi
}
Тем не менее, мы можем определить квазидетерминант,
который в конечном итоге даёт похожую картину.
В определении
\RefDefinition{RC-quasideterminant},
я следую определению
\citeBib{math.QA-0208146}-\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=9}{1.2.2}.
\ePrints{2020.06.01,2204.06320,2022.01.05}
\ifx\Semafor\ValueOn

\FrameCiteBib{q-alg-9705026}
\FrameCiteBib{math.QA-0208146}
\fi
}

\DefConvention{basis of algebra as basis of module}
{
Согласно определениям
\refDefinition{free module over ring}{},
\RefDefinition{algebra over ring}
свободная $D$\Hyph алгебра $A$ - это
$D$\Hyph модуль $A$,
который имеет базис \eV[][.]
Однако, вообще говоря, \eV не является
базисом $D$\Hyph алгебры $A$,
так как в $D$\Hyph алгебре $A$ определено произведение.
Например, в алгебре кватернионов произвольный кватернион
\ShowEq{any quaternion}
может быть представлен в виде
\ShowEq{any quaternion i j ij}
Однако при решении большинства задач
использование базиса $D$\Hyph модуля $A$ проще, чем
использование базиса $D$\Hyph алгебры $A$.
Например, легче определить координаты $H$\Hyph числа относительно базиса
$(1,i,j,k)$
$R$\Hyph векторного пространства $H$,
чем определить координаты $H$\Hyph числа относительно базиса
$(1,i,j)$
$R$\Hyph алгебры $H$.
Поэтому фраза "мы рассматриваем базис $D$\Hyph алгебры $A$"
означает, что мы рассматриваем $D$\Hyph алгебру $A$
и базис $D$\Hyph модуля $A$.
}

\DefConvention{we use separate color for index of element}
{
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
}

\DefTheorem{direct sum of n Abelian groups}
{
Прямая сумма абелевых групп
\ShowEq{a1n}An{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}A
}

\AddEq{remark: direct sum of n Abelian groups}
{
Пусть
\ShowEq{a1o+.n}An
прямая сумма абелевых групп
\ShowEq{a1n}An.
Согласно доказательству теоремы
\RefTheorem{direct sum of Abelian groups},
произвольное $A$\Hyph число $a$ имеет вид
$(a_1,...,a_n)$
где $a_i\in A_i$.
Мы также будем пользоваться записью
\ShowEq{a=a1 o+ an}
}

\DefLabeledTheorem{direct sum of n modules}{\SideWS \Base-\VectorsSetNS}
{
Прямая сумма \SideRu\TO $\Base$\Hyph \VectorsSetRuB
\ShowEq{a1n}{\Module}n{}
совпадает с их прямым произведением
\ShowEq{A1o+An=A1xAn}{\Module}
}

\DefLabeledTheorem{foa=fi ai}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\Module}n{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\Module}n
Представим $\VNumber$\Hyph число
\ShowEq{A 1o+.n}{\VNumber}n
как вектор столбец
%\ePrints{8525-2526}
%\ifx\Semafor\ValueOn
%\newpage
%\fi
\DrawEq[{\VNumber}n]{a=(a1.n col)}{}
Представим линейное отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
как вектор строку
\DrawEq[fn]{a=(a1.n row)}{}
\ShowEq{f:A->B}{\aD fi}{\aU {\Module}i}{\ModuleA}
Тогда значение отображения $f$ в $\Module$\Hyph числе $\VNumber$
можно представить как произведение матриц
\DrawEq[{\VNumber}{}]{foa=fi ai}{\SideWS \Base-\VectorsSetNS}
}

\DefProof{foa=fi ai}
{
Теорема является следствием определений
\ShowEq{def left}
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS},
\ShowEq{def right}
\eqRef{fxi,i=sum fxi}{\SideWS \Base-\VectorSetNS}.
}

\DefLabeledTheorem{foa=fi a}{\SideWS \Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\ModuleA}m{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\ModuleA}m
Представим $\ModuleA$\Hyph число
\ShowEq{A 1o+.n}{\VNumberA}m
как вектор столбец
\DrawEq[{\VNumberA}m]{a=(a1.n col)}{}
Тогда линейное отображение
\ShowEq{f:A->B}f{\Module}{\ModuleA}
имеет представление как вектор столбец отображений
\DrawEq[fm]{a=(a1.n col)}{}
таким образом, что если
\ShowEq{b=foa}{\VNumberA}{\VNumber}
то
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{}
}

\DefProof{foa=fi a}
{
Теорема является следствием теоремы
\RefTheorem{map from product into product}.
}

\DefTheorem{standard component of tensor, module}
{
Тензорное произведение $\Tensor A$ свободных
конечномерных модулей
$A_1$, ..., $A_n$
над коммутативным кольцом $D$ является свободным
конечномерным модулем.

Пусть \eV[i]
- базис модуля $A_i$ над кольцом $D$.
Произвольный тензор $a\in\Tensor A$ можно представить в виде
\ShowEq{standard component of tensor}
\ShowEq{tensor canonical representation, algebra}
Выражение
$\ShowSymbol{standard component of tensor}{}$
определено однозначно и называется
\AddIndex{стандартной компонентой тензора}{standard component of tensor}.
}

\DefLabeledTheorem{map of direct sum of modules}{\Base-\VectorsSetNS}
{
Пусть
\ShowEq{A 1n}{\Module}n,
\ShowEq{A 1n}{\ModuleA}m{}
- $\Base$\Hyph \VectorsSetRuA и
\ShowEq{A 1o+.n}{\Module}n
\ShowEq{A 1o+.n}{\ModuleA}m
Представим $\Module$\Hyph число
\ShowEq{A 1o+.n}{\VNumber}n
как вектор столбец
\DrawEq[{\VNumber}n]{a=(a1.n col)}{v,\SideWS \Base-\VectorsSetNS}
Представим $\ModuleA$\Hyph число
\ShowEq{A 1o+.n}{\VNumberA}m
как вектор столбец
\DrawEq[{\VNumberA}m]{a=(a1.n col)}{w,\SideWS \Base-\VectorsSetNS}
Тогда линейное отображение
\ShowEq{f:A->B}fVW
имеет представление как матрица отображений
\DrawEq[fnm]{a=(a11.nm matrix)}{f,\SideWS \Base-\VectorsSetNS}
таким образом, что если
\ShowEq{b=foa}{\VNumberA}{\VNumber}
то
\DrawEq[f{\VNumberA}{\VNumber}nm]{b=f rco a}{\SideWS \Base-\VectorsSetNS}
Отображение
\ShowEq{fij:->}{\Module}{\ModuleA}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}
}

\DefProof{map of direct sum of modules}
{
Согласно теореме
\refTheorem{foa=fi a}{\SideWS \Base-\VectorsSetNS},
существует множество линейных отображений
\ShowEq{fi:->}
таких, что
\DrawEq[{\VNumberA}{\VNumber}]{foa=fi a}{\SideWS \Base-\VectorsSetNS}
Согласно теореме
\refTheorem{foa=fi ai}{\SideWS \Base-\VectorsSetNS},
для каждого $\gii$,
существует множество линейных отображений
\ShowEq{fij:->}{\Module}{\ModuleA}
таких, что
\DrawEq{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}
Если мы отождествим матрицы
\ShowEq{fij=(fi)j}
то равенство
\eqRef{b=f rco a}{\SideWS \Base-\VectorsSetNS}
является следствием равенств
\eqRef{foa=fi a}{\SideWS \Base-\VectorsSetNS},
\eqRef{fioa=fij aj}{\SideWS \Base-\VectorsSetNS}.
}

\DefDefinition{Matrix of tensors}
{
Пусть $a$ - матрица и
\ShowEq{a in Aoxn}{\aUD aij}n.
Матрица $a$ называется матрицей тензоров
\ShowEq{Aoxn}n.
Если $n=2$, то матрица $a$ также называется
матрицей отображений.
}

\AddEq{remark: map of direct sum of modules}
{
Пусть
\ShowEq{aU A1n}Bm{}
- $D$\Hyph алгебры.
Тогда мы можем записать линейное отображение $\aUD fij$
с помощью \BoxB{\aU Bi}чисел.
}

\DefText{Free Algebra over Ring}
{
Пусть $D$ - коммутативное кольцо и $A$ - абелевая группа.
%Мы сперва рассматриваем вертикальное представление,
%а затем горизонтальные.
Диаграмма представлений
\DrawEq[{}{}{}g]{diagram of representations of D algebra}{}
порождает структуру $D$\Hyph алгебры $A$.
}

\DefText{Coordinates of Linear Map}
{
\section{Общее определение}

\ShowText{def Coordinates of Linear Map}111222{h(p)}{(g\circ a)}

\section{Линейное отображение, когда кольца
\ShowEq{A1=A2 pdf}D}

\ShowText{def Coordinates of Linear Map}{}11{}22p{(g\circ a)}

\section{Линейное отображение, когда \texorpdfstring{$D$}{D}-алгебры
\ShowEq{A1=A2 pdf}A}

\ShowText{def Coordinates of Linear Map}{}{}1{}{}2pa
}

\DefLabeledTheorem[7]{linear map of A module, coordinates}{\SideNS-\Cols(#1#2#3)}
{
Линейное отображение\,\refFootnote{Coordinates of Linear Map}{\SideNS-\Cols(#1#2#3)}
\newline
\FrameEqRef[{\Vector g}{\Vector f}{}]{homomorphism A module #1#2#3}{linear \SideNS}
\newline
имеет представление
\ShowText{g:A1->A2, D module(#1#2#3)}{ 0}
\ShowText{f:V1->V2, A module}{#1}{#2}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowText{homomorphism of vector space, algebra(#2)}{#1}{#2}{#3}{#4}{#5}{#6}{ 0}
\ShowText{homomorphism of vector space, algebra 1}{#1}{#2}{#3}{#4}{#5}{#6}
%\ShowEq{coordinates of the linear map}a{\Base}ghiI{D_2}{}b
%\ShowEq{coordinates of the linear map}v{\Module}fgkK{\Base_\DT}{\SideWS}w
\end{itemize}
Отображение
\ShowEq{fij:-> \SideWS A}
является линейным отображением и называется
\AddIndex{частным линейным отображением}{partial linear map}.
}

\AddEq [9]{coordinates of the linear map}
{
\item $#1$ - координатная матрица $#2_1$\Hyph числа
$\Vector #1$
относительно базиса
\ShowEq{basis e}{#2_1}{}
\DrawEq [#1{#2_1}]{va=ae1, #8module}{#1 \DFDT\SideWS module}
\def\Temp{D1 D2 }
\ifx\DFDT\Temp
\item
\ShowEq{h(a)=...}{#1}{#4}{#5}{#6}
- матрица $#7$\Hyph чисел.
\fi
\item $#9$ - координатная матрица вектора
\DrawEq[#1#9#3]{vb=f(va)}{#1 \DFDT\SideWS \VectorSetNS}
относительно базиса
\ShowEq{basis e}{#2_2}{}
\DrawEq [#9{#2_2}]{va=ae1, #8module}{#9 \DFDT\SideWS module}
\item $#3$ - координатная матрица множества векторов
\ShowEq{Vector f(e1) module}#3#2#5#6
относительно базиса
\ShowEq{basis e}{#2_2}.
Мы будем называть матрицу $#3$
\AddIndex{матрицей линейного отображения}{matrix of linear map}
$\Vector #3$ относительно базисов
\ShowEq{basis e}{#2_1}{}
и
\ShowEq{basis e}{#2_2}.
}

\DefText[6]{Proof, linear map of A module(1)}
{
Согласно определениям
\ShowRef{Proof, linear map of A module}{#1}{#2}{#3}%
отображение
\DrawEq[{\Vector g}A]{homomorphism D algebra #1#2}{\SideNS-\Cols}
\begin{sloppypar}
\noindent
явлется гомоморфизмом
$D_{#1}$\Hyph алгебры $A_{#2}$
в $D_{#4}$\Hyph алгебру $A_{#5}$.
Следовательно, равенства
\ShowRef{Proof, linear map of A module 1}{#1}{#2}{#3}%
следуют из равенств
\ShowRef{Proof, homomorphism of vector space 2}{#1}{#2}{#3}{#4}%
Из теоремы
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
следует что матрица $g$ определена однозначно.
\end{sloppypar}

}

\DefText[6]{Proof, linear map of A module()}
{%
}

\DefProof[6]{linear map of A module, coordinates}
{
\ShowText{Proof, linear map of A module(#2)}{#1}{#2}{#3}{#4}{#5}{#6}%

\ShowEq{module as direct sum}1kK
\ShowEq{module as direct sum}2lL
Равенство
\eqRef{linear map, A module (#2)}{\SideWS \Cols(#1#2)}
является следствием теоремы
\refTheorem{map of direct sum of modules}{\Base-\VectorsSetNS}.
}

\AddEq [3]{module as direct sum}
{
$A_{#1}$\Hyph модуль $V_{#1}$ является прямой суммой
\DrawEq[#1#2#3AV]{V=o+Ae}{}
}

\DefTheorem{representation of algebra An in LAnA}
{
Рассмотрим $D$\Hyph алгебру $A$.
Представление
\ShowEq{representation An in LAnA}DA
алгебры \AOn
в модуле \LAnA,
определённое равенством
\DrawEq[DA]{representation An in LAnA, 1}{}
позволяет отождествить тензор
\ShowEq{product in algebra An 1}
и перестановку $\sigma\in S^n$
с отображением
\DrawEq[DA]{product in algebra An 2}{DA}
где
\ShowEq{product in algebra AA 3}DA{\delta}
- тождественное отображение.
}

\DefDefinition{linear map from A1 to A2, algebra}
{
Пусть $A_1$ и
$A_2$ - алгебры над коммутативным кольцом $D$.
Линейное отображение
$D_{\DF}$\Hyph модуля $A_\VF$
в $D_{\DT}$\Hyph модуль $A_\VT$
называется
\AddIndex{линейным отображением}{linear map}
$D_{\DF}$\Hyph алгебры $A_\VF$ в $D_{\DT}$\Hyph алгебру $A_\VT$.

Обозначим
\ShowEq{set linear maps, module}D{A_1}{A_2}
множество линейных отображений
$D$\Hyph алгебры
$A_\VF$
в $D$\Hyph алгебру
$A_\VT$.
}

\DefText[4]{notation for linear map}
{
Если отображение
\eqRef{homomorphism D algebra #1#2}{module}
является линейным отображением $D_{#1}$\Hyph модуля $V_{#2}$ в $D_{#3}$\Hyph модуль $V_{#4}$,
то, согласно определению
\refDefinition[\RefRepresentation]{side representation of group}{left},
я пользуюсь обозначением
\DrawEq{f circ a =}{}
для образа отображения $f$.
}

\DefTheorem{linear map times constant, algebra}
{
Пусть отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
является линейным отображением $D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$.
Тогда отображения
\ShowEq{linear map times constant, algebra}
определённые равенствами
\ShowEq{linear map times constant, 0, algebra}
также являются линейными.
}

\DefTheorem{linear map AA LAA}
{
\ePrints{1502.04063}
\ifx\Semafor\ValueOn
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
\else
Для заданного отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
$D$\Hyph алгебры $A_1$ в $D$\Hyph алгебру $A_2$
\fi
существует линейное отображение
\ShowEq{linear map AA LAA}
определённое равенством
\ShowEq{linear map AA LAA, 1}
\ShowEq{linear map AA LAA, 2}
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{conjugation transformation}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.
Для любого отображения
\ShowEq{Ik in I}
существует множество линейных отображений
\ShowEq{conjugation transformation}
\ShowEq{conjugation transformation:}
$D$\Hyph модуля
$A_1\otimes A_1$
в $D$\Hyph модуль
$A_2\otimes A_2$
таких, что
\ShowEq{conjugation transformation =}
Отображение
\ShowEq{show conjugation transformation}
называется
\AddIndex{преобразованием сопряжения}{conjugation transformation}.
\end{ShadedTheorem}
}
{theorem: conjugation transformation}
%\DefEq

\DefProof{conjugation transformation}
{
Согласно теореме
\RefTheorem{product of linear map, algebra},
для произвольного тензора
$a\in A_1\otimes A_1$,
отображение
\ShowEq{x->Ik a x}
является линейным.
Согласно утверждению
\RefItem{map f generated by basis F},%, associative algebra},
существует разложение
\ShowEq{expansion Ik a x}
Положим
\ShowEq{b=Ikl a}
Равенство
\EqRef{conjugation transformation =}
является следствием равенств
\EqRef{expansion Ik a x},
\EqRef{b=Ikl a}.
Из равенств
\ShowEq{Ikl a1+a2}
\ShowEq{Ikl d a}
следует, что отображение $I_k^l$ является линейным.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps}
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$, $A_3$ - свободные ассоциативные $D$\Hyph алгебры.
Пусть $\Basis F$ - базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.
Пусть $\Basis G$ - базис левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_2}{A_3}.
\StartLabelItem
\begin{enumerate}
\item
Множество отображений
\labelItem{basis of composition of linear maps}
\DrawEq{JlIk}{linear map}
является базисом левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
\item
Пусть линейное отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
имеет разложение
\ShowEq{expansion of f with respect to basis I}
относительно базиса $\Basis I$.
Пусть линейное отображение
\ShowEq{f:A->B}g{A_2}{A_3}
имеет разложение
\ShowEq{expansion of g with respect to basis J}
относительно базиса $\Basis J$.
Тогда линейное отображение
\DrawEq{h=g o f}{123}
имеет разложение
\labelItem{hlk=glfk}
\ShowEq{expansion of h with respect to basis K}
относительно базиса $\Basis K$, где
\ShowEq{hlk=glfk}
\end{enumerate}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps}
%\DefEq

\DefProof{representation of composition of linear maps}
{
Равенство
\ShowEq{h(a)1}
является следствием равенств
\EqRef{expansion of f with respect to basis I},
\EqRef{expansion of g with respect to basis J},
\eqRef{h=g o f}{123}.
Равенство
\ShowEq{h(a)2}
является следствием равенств
\eqRef{JlIk}{linear map},
\EqRef{h(a)1}
и теоремы
\RefTheorem{conjugation transformation}.
Из равенства
\EqRef{h(a)2}
следует, что множество отображений $\Basis K$ порождает
левый \BoxB{A_3}модуля\newline
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
Из равенства
\ShowEq{aK=aJI}
следует, что
\ShowEq{aJ=0}
и, следовательно, $a^{lk}=0$.
Следовательно, множество $\Basis K$ является базисом
левого \BoxB{A_3}модуля
\ShowEq{L(A->B)}D{A_1\rightarrow A_2}{A_3}.
}

\DefDefinition{similar A numbers}
{
$A$\Hyph числа $a$ и $b$ называются подобными,
если существует $A$\Hyph число $c$ такое, что
\ShowEq{similar A numbers}
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation of composition of linear maps A->A}
Пусть $A$ - свободная ассоциативная $D$\Hyph алгеба.
Пусть левый \BoxB{A}модуль
\ShowEq{L(A->B)}DAA{}
порождён тождественным отображением $F_0=\delta$.
Пусть линейное отображение
\ShowEq{f:A->B}fAA
имеет разложение
\ShowEq{expansion of f A->A}
Пусть линейное отображение
\ShowEq{f:A->B}gAA
имеет разложение
\ShowEq{expansion of g A->A}
Тогда линейное отображение
\DrawEq{h=g o f}{A}
имеет разложение
\ShowEq{expansion of h A->A}
где
\ShowEq{hlk=glfk 01}
\end{ShadedTheorem}
}
{theorem: representation of composition of linear maps A->A}
%\DefEq

\DefEq
{
\begin{proof}
Равенство
\ShowEq{h(a)}
является следствием равенств
\EqRef{expansion of f A->A},
\EqRef{expansion of g A->A},
\eqRef{h=g o f}{A}.
Равенство
\EqRef{hlk=glfk 01}
является следствием равенства
\EqRef{h(a)}.
\end{proof}
}
{proof: representation of composition of linear maps A->A}
%\DefEq

\DefTheorem{h generated by f, associative algebra}
{
Рассмотрим $D$\Hyph алгебру $A_1$
и ассоциативную $D$\Hyph алгебру $A_2$.
Рассмотрим представление алгебры $\ATwo$
в модуле
\ShowEq{L(A->B)}D{A_1}{A_2}.
Отображение
\ShowEq{h:A1->A2}
порождённое отображением
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
имеет вид
\ShowEq{h generated by f, associative algebra}
}

\DefTheorem{coordinates of map A->A, algebra}
{
Пусть $A$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A$.
Пусть $\Basis F$ - базис
левого \BoxB{A}модуля
\ShowEq{L(A->B)}DAA{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}DAA{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq{coordinates of map A->A, 2}{associative algebra}
}

\DefProof{coordinates of map A->A, algebra}
{
Относительно базисов
$\Basis e$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f, associative algebra}
\ShowEq{coordinates of map Fk, associative algebra}
Равенство
\ShowEq{coordinates of map A->A, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A->A, associative algebra},
\EqRef{coordinates of map f, associative algebra},
\EqRef{coordinates of map Fk, associative algebra}.
Так как векторы $\aD ek$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A->A, 2}{associative algebra}
следует из равенства
\EqRef{coordinates of map A->A, 3, associative algebra}.
}

\DefTheorem{coordinates of map A1 A2 FoG, algebra}
{
Пусть $\Basis e_1$ - базис конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{f in L(A->B)}D{A_1}{A_2}.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_2}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базиса $\Basis e_2$.
Пусть
\ShowEq{f:A->B}GAB
линейное отображение максимального ранга такое, что
\ShowEq{ker G in ker g}f{}
и
\ShowEq{coordinates of map G}
- координаты отображения $G$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения $f$
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, FoG, associative algebra}f
}

\AddEq[1]{theorem: maps of conjugation as basis}
{
\begin{ShadedTheorem}
\labelTheorem{maps of conjugation as basis, algebra #1}
Множество линейных отображений
\ShowEq{vI=EI}
является базисом
левого $#1$\Hyph векторного пространства
\ShowEq{L(A->B)}R{#1}{#1}
и линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где
$#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq[1]{theorem: linear map, maps of conjugation, algebra}
{
\begin{ShadedTheorem}
\labelTheorem{linear map, maps of conjugation, algebra #1}
Линейное отображение
\ShowEq{f in L(A->B)}R{#1}{#1}{}
имеет разложение
\ShowEq{linear map of algebra #1, structure, 1}
\ShowEq{linear map of algebra #1, structure, 2}
где
\ShowEq{vI=... #1}
и $#1$\Hyph числа
\ShowEq{a... #1}
определены равенством
\ShowEq{a...= #1}
\end{ShadedTheorem}
}

\AddEq [1]{proof: L is left vector space}
{
\begin{proof}
Согласно теореме
\RefTheorem{linear map, maps of conjugation, algebra #1},
разложение
\EqRef{linear map of algebra #1, structure, 1}
линейного отображения $f$
существует и единственно.
Следовательно, множество
\ShowEq{I=(E,I)}{#1}{}
является базисом левого $#1$\Hyph векторного пространства
\ShowEq{L(A->B)}R{#1}{#1}.
\end{proof}
}

\DefTheorem{f=.E+.I+.J+.K}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}H
кватернионы, представленные строками матрицы $f$.
\ShowEq{fi=fij ej H}
Тогда
\ShowEq{f=.E+.I+.J+.K}
}

\DefProof{f=.E+.I+.J+.K}
{
Равенства
\ShowEq{a0=f03}
\ShowEq{a1=f03}
\ShowEq{a2=f03}
\ShowEq{a3=f03}
являются следствием равенства
\EqRef{a...= H}.
Равенство
\EqRef{f=.E+.I+.J+.K}
является следствием равенств
\ShowEq{f=.E+.I+.J+.K ref}
}

\DefTheorem{f=.I0.7}
{
Пусть
\ShowEq{f:H->H ij}
линейное отображение алгебры кватернионов.
Пусть
\DrawEq{fi=fij ej}O
Тогда
\ShowEq{f=.I0.7}
}

\DefProof{f=.I0.7}
{
Равенства
\ShowEq{a0=f0.7}
являются следствием равенства
\EqRef{a...= O}.
Равенство
\EqRef{f=.I0.7}
является следствием равенств
\ShowEq{f=.I0.7 ref}
}

\DefDefinition{maps of conjugation, complex field}
{
\ShowEq{C maps of conjugation}
Поле комплексных чисел имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{C list maps of conjugation}
}

\DefTheorem{HE is algebra isomorphic to quaternion algebra}
{
Множество
\ShowEq{HE set}
является $R$\Hyph алгеброй, изоморфной алгебре кватернионов.
}

\DefProof{HE is algebra isomorphic to quaternion algebra}
{
Теорема является следствием равенств
\ShowEq{aE+bE=(a+b)E}
\ShowEq{aE o bE=(ab)E}
опирающихся на теорему
\RefTheorem{linear map, maps of conjugation, algebra H}.
}

\DefDefinition{algebra, left and right action on L}
{
Пусть $A$ - $D$\Hyph модуль
и $B$ - $D$\Hyph алгебра.
Для произвольного отображения
\ShowEq{f in L(A->B)}DAB{}
и $b\in B$,
мы определим левосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b o f =}
и правосторонее преобразование отображения $f$, пользуясь равенством
\ShowEq{b * f =}
}

\DefDefinition{projection maps, complex field}
{
Следующие отображения проекции определены в поле комплексных чисел
\ShowEq{projection maps, complex field}
}

\DefTheorem{Expansion of projection maps relative E,I}
{
Разложение отображений проекции относительно базиса
\ShowEq{e=(E,I)}{}
имеет вид
\ShowEq{projection mappings 1, complex field}
}

\DefProof{Expansion of projection maps relative E,I}
{
Теорема является следствием теоремы
\RefTheorem{linear map, maps of conjugation, algebra C}
и определения
\RefDefinition{projection maps, complex field}.
}

\DefTheorem{f=.E+.I}
{
Пусть
\DrawEq[fCC{}]{f: A->B}{}
линейное отображение поля комплексных чисел.
Пусть
\DrawEq{fi=fij ej}C
Тогда
\ShowEq{f=.E+.I}
}

\DefProof{f=.E+.I}
{
Равенства
\ShowEq{a0=f01}
\ShowEq{a1=f01}
являются следствием равенства
\EqRef{a...= C}.
Равенство
\EqRef{f=.E+.I}
является следствием равенств
\ShowEq{f=.E+.I ref}
}

\DefDefinition{polylinear map of algebras}
{
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph алгебры.
Полилинейное отображение
\ShowEq{f:A->B}f{\Times}S
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$,
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph алгебр
$A_1$, ..., $A_n$
в $D$\Hyph алгебру $S$.
Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}DAS
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefTheorem{sum of linear maps, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество
$\mathcal L(D;A_1;A_2)$
является абелевой группой
относительно суммы отображений.
}

\DefTheorem{sum of polylinear maps, module}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,polylinear}
\ShowEq{sum of maps, 1, polylinear}
определённое равенством
\ShowEq{sum of  maps, polylinear}
называется
\AddIndex{суммой полилинейных отображений}{sum of maps}
$f$ и $g$
и является полилинейным отображением.
Множество
\ShowEq{module of polylinear maps}
является абелевой группой
относительно суммы отображений.
}

\DefCorollary{sum of linear maps, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{sum of maps,,D module}
\ShowEq{sum of maps, 1, D module}
определённое равенством
\ShowEq{sum of maps, D module}
называется
\AddIndex{суммой отображений}{sum of maps}
$f$ и $g$
и является линейным отображением.
Множество \LAB D{A_1}{A_2}
является абелевой группой
относительно суммы отображений.
}

\DefDefinition{linear map A module}
{
\ShowText{algebra over ring (11)}
Пусть
\ShowEq{Ai, i=}V
- $A_i$\Hyph \VectorSetRuANS.
Морфизм диаграммы представлений
\ShowEq{A module diagram for linear}1
в диаграмму представлений
\ShowEq{A module diagram for linear}2
называется
\AddIndex{линейным отображением}{linear map}
$A_1$\Hyph \VectorSetRuB $V_1$ в
$A_2$\Hyph \VectorSetRuA $V_2$.
Обозначим
\ShowEq{set linear maps, V12 module}
множество линейных отображений
$A_1$\Hyph \VectorSetRuB $V_1$ в
$A_2$\Hyph \VectorSetRuA $V_2$.
}

\DefText[7]{homomorphism of A module 1}
{
\subsection{Гомоморфизм \SideRu вого \texorpdfstring{$A$}{A}-\VectorSetRuB \ColsNA}
\ShowText{homomorphism of A module 2}{#1}{#2}{#3}{#4}{#5}{#6}{#7}
}

\DefText{homomorphism A module}
{
\section{Общее определение}

\ShowText{def homomorphism A module}111222{h(p)}{(g\circ a)}

\section{Гомоморфизм, когда кольца
\ShowEq{A1=A2 pdf}D}

\ShowText{def homomorphism A module}{}11{}22p{(g\circ a)}

\def\Temp{module}%
\ifx\Temp\VectorSetNS
\ProveTheorem{da in DA->da in D1A}

\ShowConvention{da in DA->da in D1A}
\fi

\section{Гомоморфизм, когда \texorpdfstring{$D$}{D}-алгебры
\ShowEq{A1=A2 pdf}A}

\ShowText{def homomorphism A module}{}{}1{}{}2pa
}

\DefText{algebra over ring (11)}
{
Пусть
\ShowEq{Ai, i=}A
- алгебра\DivisionRu над коммутативным кольцом $D_i$.%
}

\DefText{algebra over ring (1)}
{
Пусть
\ShowEq{Ai, i=}A
- алгебра\DivisionRu над коммутативным кольцом $D$.%
}

\DefText{algebra over ring ()}
{
Пусть $A$
- алгебра\DivisionRu над коммутативным кольцом $D$.%
}

\DefText{module over algebra (11)}
{
Пусть
\ShowEq{Ai, i=}V
- \SideRuTo $A_i$\Hyph модуль.
}

\DefText{module over algebra (1)}
{
Пусть
\ShowEq{Ai, i=}V
- \SideRuTo $A$\Hyph \VectorSetRuANS.
}

\DefLabeledDefinition[6]{homomorphism A module}{\SideNS(#1#2#3)}
{
Пусть
\DrawEq[{#1}{#2}{#3}{1.}]{diagram of representations, \SideWS module}{->1(#1#2#3)}
диаграмма представлений, описывающая
\SideRuTo $A_{#2}$\Hyph \VectorSetRuA $V_{#3}$.
Пусть
\DrawEq[{#4}{#5}{#6}{2.}]{diagram of representations, \SideWS module}{->2(#4#5#6)}
диаграмма представлений, описывающая
\SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
Морфизм
\DrawEq[gf]{homomorphism A module #1#2#3}{\SideNS}
диаграммы представлений
\eqRef{diagram of representations, \SideWS module}{->1(#1#2#3)}
в диаграмму представлений
\eqRef{diagram of representations, \SideWS module}{->2(#4#5#6)}
называется
\AddIndex{гомоморфизмом}{homomorphism}
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
Обозначим
\ShowEq{set homomorphisms, A module #1#2#3 \SideNS}
множество гомоморфизмов
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
%\ShowEq{set homomorphisms, \SideWS A12 module}
%множество гомоморфизмов
%\ShowEq{\SideWS column module}{A_1}
%модуля $V_1$ в
%\ShowEq{\SideWS column module}{A_2}
%модуль $V_2$.
}

\DefText[8]{homomorphism A module 1 111}
{
Отображение
\DrawEq[h{D_1}{D_2}{}{}]{f: A->B}{}
является гомоморфизмом колец и удовлетворяет равенствам
\ShowRef{define homomorphism of A module 111}
\ShowText{homomorphism A module 1 11}{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
}

\DefText[8]{homomorphism A module 1 11}
{
Отображение
\DrawEq[g{A_1}{A_2}{}{}]{f: A->B}{}
является гомоморфизмом $D_{#1}$\Hyph алгебры $A_1$ в $D_{#4}$\Hyph алгебру $A_2$
и удовлетворяет равенствам
\ShowRef{define homomorphism of A module 11}{#1}{#2}{#7}
\ShowText{homomorphism A module 1 1}{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
}

\DefText[8]{homomorphism A module 1 1}
{
Отображение
\DrawEq[f{V_1}{V_2}{}{}]{f: A->B}{}
является гомоморфизмом абелевой группы
\newline
(равенство
\ShowRef{define homomorphism of A module 1}{#1}{#2}
и согласовано с представлением
\newline
(равенство
\ShowRef{define homomorphism of A module 2}{#1}{#2}{#8}
}

\DefLabeledSummary[8]{homomorphism A module}{\SideNS(#1#2#3)}
{
Пусть
\ShowRef{diagram of representations of module}{#1}{#2}{#3}1
диаграмма представлений, описывающая
\SideRuTo $A_{#2}$\Hyph \VectorSetRuA $V_{#3}$.
Пусть
\ShowRef{diagram of representations of module}{#4}{#5}{#6}2
диаграмма представлений, описывающая
\SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
Гомомрфизм
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$.
- это отображение
\ShowRef{homomorphism A module}{#1}{#2}{#3}gf
каждая компонента которого
является гомоморфизмом соответствующей алгебры
и эти гомоморфизмы согласованы.
\ShowText{homomorphism A module 1 #1#2#3}{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
}

\DefLabeledSummary[8]{homomorphism associative A module}{\SideNS(#1#2#3)}
{
\ShowEq{\DefCol}
\ShowEq{prolog homomorphism of vector space(#1#2#3)}{#1}{#2}{#3}{#4}{#5}{#6}
\ShowText{matrices of numbers(#2#3)}{#4}{#5}{#1}{#2}
\ShowText{matrix generates A module homomorphism}{#1}{#2}{#3}{#4}{#5}{#6}{}
Гомоморфизм
\ShowRef{homomorphism A module}{#1}{#2}{#3}{\Vector g}{\Vector f}
который имеет%
\ShowText{define homomorphism by given matrix(#2)}%
определён однозначно.

Если $D_2$\Hyph алгебра $A_2$ ассоциативна,
то из равенства
\eqRef{f o (ae)=ga o f e, vector space \Product-\Cols}{\SideNS(111)}
следует равенство
\begin{equation}%
\aU{(\Vector{f}\circ(v\CRstar e_{V_1}))}j=(\Vector g\circ \aU vi)\CRstar \aUD fji
\end{equation}%

Обратное утверждение также верно.
Пусть квазибазис \eV[V_2] является базисом.
\ShowText{matrix of homomorphism relative bases #2#3}{#1}{#2}{#3}{#5}
}

\DefLabeledTheorem[8]{define homomorphism A module}{\SideNS(#1#2#3)}
{
Гомоморфизм
\newline
\FrameEqRef[gf]{homomorphism A module #1#2#3}{\SideNS}
\newline
\SideRu вого $A_{#2}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$
удовлетворяет следующим равенствам
\ShowEq{define homomorphism of A module #1#2#3}{#1}{#2}{#3}{#7}{#8}{}
}

\DefProof[7]{define homomorphism A module}
{
\ShowText{define homomorphism of vector space(#2)}{#1}{#2}{#4}{#5}{#7}
Равенство
\eqRef{homomorphism, f v+w=}{f(#1#2)\SideWS A module#7}
является следствием определения
\refDefinition{homomorphism A module}{\SideNS(#1#2#3)},
так как, согласно определению
\RefDefinition{morphism of representations of universal algebra},
отображение $f$ является гомоморфизмом абелевой группы.
Равенство
\eqRef{\SideWS homomorphism, f av=}{(#1#2)\SideWS A module#7}
является следствием равенства
\EqRef{morphism of representations of universal algebra},
так как отображение
\ShowEq{homomorphism A module, 1#7}{#1}{#2}{#3}
является морфизмом представления $g_{1.34}$
в представление $g_{2.34}$.
}

\DefTheorem{L(An;B) is free D module}
{
Пусть $A_1$, ..., $A_n$, $B$ - свободные модули над коммутативным кольцом $D$.
$D$\Hyph модуль
\ShowEq{L(A->B)}D{A_1\times...\times A_n}B{}
является свободным $D$\Hyph модулем.
}

\DefLabeledTheoremNote[5]{linear map of D module}{#1#2}
{
Линейное отображение
\newline
\FrameEqRef[fV]{homomorphism D algebra #1#2}{module}
\newline
$D_{#1}$\Hyph модуля $V_{#2}$
в $D_{#3}$\Hyph модуль $V_{#4}$
удовлетворяет равенствам\,\footnotemark
\ShowEq{define homomorphism of D module #1#2}{#1}{#2}{#5}
}
{\,
В некоторых книгах
(например, на странице \citeBib{Serge Lang}\Hyph 94) теорема
\refTheorem{linear map of D module}{#1#2}
рассматривается как определение.
}

\DefText{linear map of D module (11)}
{
Согласно определению
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
отображение $h$
явлется гомоморфизмом кольца $D_1$
в кольцо $D_2$.
Равенства
\ShowEq{ref linear map of D module 1}
являются следствием этого утверждения.
}

\DefText{linear map of D module (1)}
{
}

\DefProof[2]{linear map of D module}
{
\ShowText{linear map of D module (#1#2)}
Из определения
\RefDefinition[\RefRepresentation]{morphism of representations of universal algebra},
следует, что
отображение $f$ является гомоморфизмом абелевой группы $V_1$
в абелеву группу $V_2$ (равенство
\eqRef{homomorphism, f v+w=}{f D module #1#2}).
Равенство
\eqRef{left homomorphism, f av=}{f D module #1#2}
является следствием равенства
\EqRef[\RefRepresentation]{morphism of representations of universal algebra}.
}

\DefDefinition{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Приведенный полиморфизм $D$\Hyph модулей
$A_1$, ..., $A_n$ в $D$\Hyph модуль $S$
\ShowEq{f:A->B}f{\Times}S
называется
\AddIndex{полилинейным отображением}{polylinear map} $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$.

Обозначим
\ShowEq{set polylinear maps}
множество полилинейных отображений
$D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль
$S$.
Обозначим
\ShowEq{set polylinear maps An}DAS
множество $n$\hyph линейных отображений
$D$\Hyph модуля $A$ ($A_1=...=A_n=A$)
в $D$\Hyph модуль
$S$.
}

\DefTheorem{polylinear map of modules}
{
Пусть $D$ - коммутативное кольцо.
Полилинейное отображение $D$\Hyph модулей
$A_1$, ..., $A_n$
в $D$\Hyph модуль $S$
\ShowEq{f:A->B}f{\Times}S
удовлетворяет равенствам
\DrawEq[f]{f(ai+bi)=fai+fbi}{}
\DrawEq[f]{f(pai)=pfai}{}
\ShowEq{polylinear map of algebras, 1}{A_i}D
}

\DefTheorem{there exists tensor product of modules}
{
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
\AddIndex{Тензорное произведение}{tensor product}
\ShowEq{tensor product of modules}
\ShowEq{f:xA->oxA}
$D$\Hyph модулей $A_1$, ..., $A_n$ существует и единственно.
Мы пользуемся обозначением
\ShowEq{fxa=oxa}
для образа отображения $f$.
}

\DefTheorem{tensor product and polylinear map}
{
Пусть $A_1$, ..., $A_n$ -
модули над коммутативным кольцом $D$.
Пусть
\ShowEq{map f, 1, tensor product}
полилинейное отображение,
определённое равенством
\ShowEq{map f, tensor product}
Пусть
\ShowEq{map g, tensor product}
полилинейное отображение в $D$\Hyph модуль $V$.
Существует линейное отображение
\ShowEq{map h, tensor product}
такое, что диаграмма
\ShowEq{map gh, tensor product}
коммутативна.
Отображение \(h\) определено равенством
\ShowEq{g=h, tensor product}
}

\DefProof{polylinear map of modules}
{
Теорема является следствием определений
\RefDefinition[\RefRepresentation]{reduced polymorphism of representations},
\refDefinition{linear map of D module}1,
\RefDefinition{polylinear map of modules}
и теоремы
\refTheorem{linear map of D module}1.
}

\DefProof{sum of polylinear maps, module}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{sum of maps f}
\DrawEq[f]{f(pai)=pfai}{sum of maps f}
\DrawEq[g]{f(ai+bi)=fai+fbi}{sum of maps g}
\DrawEq[g]{f(pai)=pfai}{sum of maps g}
Равенство
\ShowEq{sum of maps, 31, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps f},
\eqRef{f(ai+bi)=fai+fbi}{sum of maps g}.
Равенство
\ShowEq{sum of maps, 32, polylinear}
является следствием равенств
\EqRef{sum of maps, polylinear},
\eqRef{f(pai)=pfai}{sum of maps f},
\eqRef{f(pai)=pfai}{sum of maps g}.
Из равенств
\EqRef{sum of maps, 31, polylinear},
\EqRef{sum of maps, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{sum of maps, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Пусть
\ShowEq{module of polylinear maps, 1}
Для любого
\ShowEq{module of polylinear maps, 2}
Следовательно, сумма полилинейных отображений коммутативна и ассоциативна.

Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{0:A1n->S}
является нулём операции сложения
\ShowEq{0+f=f 1n}
Из равенства
\EqRef{sum of maps, polylinear}
следует, что отображение
\ShowEq{-f:A1n->S}
является отображением, обратным отображению \(f\)
\ShowEq{f-f=0}
так как
\ShowEq{f-f=0 1n}
Из равенства
\ShowEq{sum of maps, 4, polylinear}
следует, что сумма отображений коммутативно.
Следовательно, множество $\\$
\ShowEq{module of polylinear maps}
является абелевой группой.
}

\DefTheorem{module of polylinear maps}
{
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,polylinear}
\ShowEq{product of map over scalar, 1, polylinear}
определённое равенством
\ShowEq{product of map over scalar, polylinear}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является полилинейным отображением.
Представление
\ShowEq{a:LA1n->LA1n}
кольца $D$ в абелевой группе
\ShowEq{module of polylinear maps}
порождает структуру $D$\Hyph модуля.
}

\DefProof{module of polylinear maps}
{
Согласно теореме
\RefTheorem{polylinear map of modules}
\DrawEq[f]{f(ai+bi)=fai+fbi}{product of map over scalar}
\DrawEq[f]{f(pai)=pfai}{product of map over scalar}
Равенство
\ShowEq{product of map over scalar, 31, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(ai+bi)=fai+fbi}{product of map over scalar}.
Равенство
\ShowEq{product of map over scalar, 32, polylinear}
является следствием равенств
\EqRef{product of map over scalar, polylinear},
\eqRef{f(pai)=pfai}{product of map over scalar}.
Из равенств
\EqRef{product of map over scalar, 31, polylinear},
\EqRef{product of map over scalar, 32, polylinear}
и теоремы
\RefTheorem{polylinear map of modules}
следует, что отображение
\EqRef{product of map over scalar, 1, polylinear}
является полилинейным отображением $D$\Hyph модулей.

Равенство
\DrawEq{(p+q)f=pf+qf}{polylinear}
является следствием равенства
\ShowEq{(p+q)f=pf+qf 1}
Равенство
\DrawEq{p(qf)=(pq)f}{polylinear}
является следствием равенства
\ShowEq{p(qf)=(pq)f 1}
Из равенств
\eqRef{(p+q)f=pf+qf}{polylinear},
\eqRef{p(qf)=(pq)f}{polylinear},
следует, что отображение
\EqRef{a:LA1n->LA1n}
является представлением кольца $D$
в абелевой группе
\ShowEq{module of polylinear maps}.
Так как указанное представление эффективно,
то, согласно определению
\refDefinition{module over algebra}{\SideWS \VectorSetNS}
и теореме
\RefTheorem{sum of polylinear maps, module},
абелевая группа
\ShowEq{L(A->B)}D{A_1}{A_2}{}
является $D$\Hyph модулем.
}

\DefCorollary{product of linear map over scalar, D module}
{
Пусть $A_1$, $A_2$ - $D$\Hyph модули.
Отображение
\ShowEq{product of map over scalar,,D module}
\ShowEq{product of map over scalar, 1, D module}
определённое равенством
\ShowEq{product of map over scalar, D module}
называется
\AddIndex{произведением отображения $f$ на скаляр}
{product of map over scalar} $d$
и является линейным отображением.
Представление
\ShowEq{a:LA12->LA12}
кольца $D$ в абелевой группе
\ShowEq{L(A->B)}D{A_1}{A_2}{}
порождает структуру $D$\Hyph модуля.
}

\DefLabeledTheorem[8]{linear map of A module}{#1#2#3, \SideNS}
{
Линейное отображение
\DrawEq[gf]{homomorphism A module #1#2#3}{linear \SideNS}
\SideRu\From $A_{#5}$\Hyph \VectorSetRuB $V_{#3}$
в \SideRuTo $A_{#5}$\Hyph \VectorSetRuA $V_{#6}$
удовлетворяет равенствам
\ShowEq{define homomorphism of A module #1#2#3}{#1}{#2}{#3}{#7}{#8}{ 0}
}

\DefTheorem{complex field over real field}
{
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
}

\DefProof{complex field over real field}
{
Равенства
\EqRef{product of complex field} и
\EqRef{structural constants of complex field}
следуют из равенства $i^2=-1$.
}

\DefLabeledTheorem[1]{maps of conjugation antilinear}{#1}
{
Отображения сопряжения
\ShowEq{I... #1}
\DoVerb являются антилинейными гомоморфизмами.
}

\DefProof[1]{maps of conjugation antilinear}
{
Произведение $#1$\Hyph чисел
\ShowEq{#1 number Ea}a
и
\ShowEq{#1 number Ea}b
имеет вид
\DrawEq[ab]{#1 product aEx}{ab}
\ShowText{maps of conjugation antilinear #1}
}

\DefText{maps of conjugation antilinear H}
{
\ShowEq{H items maps of conjugation antilinear}
}

\DefText{maps of conjugation antilinear O}
{
Для доказательства теоремы достаточно рассмотреть отображение $\aU I1$,
так как доказательство аналогично для остальных отображений.
\ShowEq{item maps of conjugation antilinear}O1
}

\DefTheorem{coordinates of map A1 A2, algebra}
{
Пусть $\Basis e_1$ - базис свободного конечно мерного
$D$\Hyph модуля $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть
\ShowEq{structural constants, algebra}
- структурные константы алгебры $A_2$.
Пусть $\Basis F$ - базис
левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}{}
и
\ShowEq{coordinates of map Ik}
- координаты отображения $F_k$ относительно базисов $\Basis e_1$ и $\Basis e_2$.
Координаты
\ShowEq{Coordinates of map f}
отображения
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
и его стандартные компоненты
\ShowEq{standard components of map f}k
связаны равенством
\DrawEq[f-]{coordinates of map A1 A2, 2, associative algebra}f
}

\DefProof{coordinates of map A1 A2, algebra}
{
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $I_k$ имеют вид
\ShowEq{coordinates of map f 18, associative algebra}
\ShowEq{coordinates of map Ik, associative algebra}
Равенство
\ShowEq{coordinates of map A1 A2, 3, associative algebra}
является следствием равенств
\EqRef{standard representation of map A1 A2, associative algebra},
\EqRef{coordinates of map f 18, associative algebra},
\EqRef{coordinates of map Ik, associative algebra}.
Так как векторы $e_{2\cdot\gik}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\eqRef{coordinates of map A1 A2, 2, associative algebra}f
следует из равенства
\EqRef{coordinates of map A1 A2, 3, associative algebra}.
}

\DefTheorem{linear map in L(A,A), associative algebra}
{
Пусть $A_1$ - $D$\Hyph алгебра.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Левый \BoxB{A_2}модуль
\ShowEq{L(A->B)}D{A_1}{A_2}{}
имеет конечный
\AddIndex{базис}{basis of algebra L(A,A)} $\Basis I$.
\StartLabelItem
\begin{enumerate}
\item
Линейное отображение
\ShowEq{f in L(A->B)}D{A_1}{A_2}{}
имеет вид
\labelItem{f in L(A,A), 1, associative algebra}
\ShowEq{f in L(A,A), 1, associative algebra}
\item
Его стандартное представление имеет вид
\labelItem{f in L(A,A), 2, associative algebra}
\ShowEq{f in L(A,A), 2, associative algebra}
\end{enumerate}
}

\DefTheoremNote{standard representation of map A1 A2, associative algebra}
{
Пусть $A_1$ - свободный $D$\Hyph модуль.
Пусть $A_2$ - свободная конечно мерная ассоциативная $D$\Hyph алгебра.
Пусть $\Basis e$ - базис $D$\Hyph модуля $A_2$.
Пусть $\Basis F$
- базис левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2}.\,\footnotemark
\StartLabelItem
\begin{enumerate}
\item
Отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
имеет следующее разложение
\labelItem{map f generated by basis F}
\DrawEq{map f generated by basis F}{expansion}
где
\ShowEq{fk= in A2xA2}
\item
Отображение $f$ имеет стандартное представление
\labelItem{standard representation of map A1 A2, associative algebra}
\ShowEq{standard representation of map A1 A2, associative algebra}
\end{enumerate}
}{
Если $D$\Hyph модуль $A_1$ или $D$\Hyph модуль $A_2$
не является свободным $D$\Hyph модулем,
то мы будем рассматривать множество
\ShowEq{Ik 1n}
линейно независимых линейных отображений. Теорема верна для любого линейного отображения
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
порождённого множеством линейных отображений $\Basis F$.
}

\DefProof{standard representation of map A1 A2, associative algebra}
{
Поскольку $\Basis F$ является базисом левого \BoxB{A_2}модуля
\ShowEq{L(A->B)}D{A_1}{A_2},
то согласно определению
\ShowEq{ref definition: basis of representation}
и теореме
\ShowEq{RefTheorem set of vectors generated by set of vectors, module}
%существует разложение
\DrawEq[{A_2}]{expansion of linear map with respect to basis}{A2}
линейного отображения $f$ относительно базиса $\Basis I$.
Согласно определению
\ShowEq{ref map j, representation, tensor product}
\DrawEq{f=fkxfk}{module}
Равенство
\eqRef{map f generated by basis F}{expansion}
является следствием равенств
\eqRef{expansion of linear map with respect to basis}{A2},
\eqRef{f=fkxfk}{module}.
Согласно теореме
\RefTheorem{standard component of tensor, algebra},
стандартное представление тензора $f^k$ имеет вид
\ShowEq{standard representation of map A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of map A1 A2, associative algebra}
следует из равенств
\eqRef{map f generated by basis F}{expansion},
\EqRef{standard representation of map A1 A2, 3, associative algebra}.
}

\DefTheorem{map > bullet map}
{
Пусть $A$ - $D$\Hyph алгебра.
Для любого $A$\Hyph числа $a$, отображение
\ShowEq{f->ao f}
определённое равенством
\ShowEq{ao f=a f o}
является эндоморфизмом $D$\Hyph модуля
\ShowEq{L(A->B)}DAA.
}

\DefProof{map > bullet map}
{
}

\DefTheorem{a > a bullet}
{
$D$\Hyph модуль
\ShowEq{L(A->B)}DAA
является левым $A$\Hyph модулем, порождённым представлением
\ShowEq{a > a bullet}
}

\DefProof{a > a bullet}
{
}

\AddEq[3]{theorem: ao Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map ao}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2{#3}
\DrawEq[{#1}{#2}]{a o, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number Ea}a
и
\ShowEq{#2 number #1a}x
имеет вид
\DrawEq[ax]{#2 product a#1x}{}
Следовательно, отображение
\eqRef{map ao}{#1#2}
имеет матрицу Якоби
\eqRef{a o, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq [2]{item maps of conjugation antilinear}
{

Равенство
\ShowEq{#1#2 product ab}
является следствием равенств
\EqRef{#2x= #1},
\eqRef{#1 product aEx}{ab}.
Из равенства
\eqRef{#1 product aEx}{ab}
следует, что произведение $#1$\Hyph чисел
\ShowEq{#1 number #2a}b
и
\ShowEq{#1 number #2a}a
имеет вид
\ShowEq{#1 #2b*#2a}
Из равенств
\EqRef{#1#2 product ab},
\EqRef{#1 #2b*#2a}
следует, что отображение $\aU I#2$
\DoVerb является линейным антигомоморфизмом.
}

\AddEq[2]{theorem: ao Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a#1, #2, Jacobian matrix 1}
\DrawEq[#1]{ao, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: ao Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{ao, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{a#1, #2 matrix 2}
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix}
Отображение
\DrawEq[{#1}{#2}]{map a*}{#1#2}
имеет матрицу
\ShowEq{maps of conjugation, Jacobian matrix}#1#2r
\DrawEq[{#1}{#2}]{a *, Jacobian matrix}{#1#2}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix}
{
\begin{proof}
Произведение $#2$\Hyph чисел
\ShowEq{#2 number #1a}x
и
\ShowEq{#2 number Ea}a
имеет вид
\ShowEq{#2 product #1xa}
Следовательно, отображение
\eqRef{map a*}{#1#2}
имеет матрицу Якоби
\eqRef{a *, Jacobian matrix}{#1#2}.
\end{proof}%
}

\AddEq[2]{theorem: a* Jacobian matrix 1}
{
\begin{ShadedTheorem}
\labelTheorem{a*#1, #2, Jacobian matrix 1}
\DrawEq[#1]{a*, #2 matrix 1}{#1}
\end{ShadedTheorem}
}

\AddEq[2]{proof: a* Jacobian matrix 1}
{
\begin{proof}
Равенство
\eqRef{a*, #2 matrix 1}{#1}
следует из цепочки равенств
\ShowEq{#1a, #2 matrix 2}
\end{proof}%
}

\DefDefinition{antilinear homomorphism}
{
Отображение
\ShowEq{f in L(A->B)}DAA{}
называется
\AddIndex{антилинейным гомоморфизмом}{antilinear homomorphism}
если отображение $f$ удовлетворяет равенству
\ShowEq{fab=fbfa}
}

\DefDefinition{quaternion maps of conjugation}
{
\ShowEq{H maps of conjugation}
Алгебра кватернионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{H list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\DefDefinition{octonion maps of conjugation}
{
\ShowEq{O maps of conjugation}
Алгебра октонионов имеет следующие
\AddIndex{отображения сопряжения}{map of conjugation}
\ShowEq{O list maps of conjugation}
Мы также будем пользоваться обозначением
\ShowEq{I0=E}
}

\AddEq[1]{theorem: L is left vector space}
{
\begin{ShadedTheorem}
\labelTheorem{L(#1->#1) is left #1-vector space}
$#1\otimes #1$\Hyph модуль
\ShowEq{L(A->B)}R{#1}{#1}
является левым $#1$\Hyph векторным пространством
и имеет базис
\ShowEq{I=(E,I)}{#1}.
\end{ShadedTheorem}
}

\DefText{let i=12}
{
Пусть
\ShowEq{i=1,2}.
}

\DefText[6]{Let be quasibasis of module}
{
Пусть множество векторов
\DrawEq[{#1_i}{#2}{#3}]{basis ei of module #5}{#6}
является квазибазисом \SideRu вого $#4$\Hyph \VectorSetRuB $#1_i$.%
}

\DefText[6]{Let be basis of vector space}
{
Пусть множество векторов
\DrawEq[{#1_i}{#2}{#3}]{basis ei of module #5}{#6}
является базисом \SideRu вого $#4$\Hyph \VectorSetRuB $#1_i$.%
}

\AddEq [9]{Let be basis of vector space}
{%
Пусть множество векторов
\DrawEq[{#1}{#2}{#3}]{basis e of module #8}{#9}
является базисом \SideRu вого $#4_{#5}$\Hyph \VectorSetRuB $#6_{#7}$.%
}%

\AddEq [3]{Let be Basis of vector space}
{%
Пусть \eV[#1]
базис \SideRu вого $#2$\Hyph векторного пространства $#3$.%
}%

\AddEq [9]{Let be basis of module}
{%
Пусть
\DrawEq[{#1_{#2}}{#3}{#4}]{basis e of module \Cols}-
базис #5 $#6_{#7}$\Hyph \VectorSetRuB \ColsA $#8_{#9}$.
}

\AddEq [9]{Let be basis of algebra}
{%
Пусть множество векторов
\DrawEq[{#1_{#2}}{#3}{#4}]{basis e of module \Cols}{#9}
является базисом $#5_{#6}$\Hyph алгебры \ColsA $#7_{#8}$.%
}

\DefText[5]{Let be basis of algebra and C}
{
Пусть множество векторов
\DrawEq[{#1_i}{#2}{#3}]{basis ei of module \Cols}{#5}
является базисом и
\ShowEq{structural constants of algebra}ikij,
\ShowEq{kij in I}{#3}i
- структурные константы $#4$\Hyph алгебры \ColsA $#1_i$.%
}

\AddEq [9]{Let be basis of algebra and C}
{%
Пусть множество векторов
\DrawEq[{#1}{#3}{#4}]{basis e of module \Cols}{#9}
является базисом и
\ShowEq{structural constants of algebra}{#2}kij,
\ShowEq{kij in I}{#4}{}
- структурные константы $#5_{#6}$\Hyph алгебры \ColsA $#7_{#8}$.%
}

\AddEq [5]{Let e be basis 1n}
{
Пусть
\ShowEq{basis e of module 1n}{#1}{#2}
базис в #3 $#4$\Hyph модуле $#5$.
}

\DefText[5]{coordinates of the linear map 1}
{
\item $#1$ - координатная матрица $#2_1$\Hyph числа
$\Vector #1$
относительно базиса \eV[#3](\Base)
\def\Temp{D}
\ifx\Temp\Base
\DrawEq [{#1}{#3}{}]{va=ae1, module (#5)(\Cols)}{\SideNS-\VectorSet #1 #4}
\else
\DrawEq [{#1}{#3}]{va=ae1, module (#5)(\Cols)}{}
\fi
}

\DefText[5]{coordinates of the linear map 2(1)}
{
\item
\ShowEq{h(a)=...}{#1}{#2}{#3}{#4}
- матрица $#5$\Hyph чисел.
}

\DefText[5]{coordinates of the linear map 2()}
{
}

\DefText[7]{coordinates of the linear map 3}
{
\item $#6$ - координатная матрица $#2_2$\Hyph числа
\DrawEq[#1#6#4]{vb=f(va)}{}%{#1 #7(\Cols)\SideNS-\VectorSetNS}
относительно базиса \eV[#3]
\def\Temp{D}
\ifx\Temp\Base
\DrawEq [{#6}{#3}]{va=ae1, module (#5)(\Cols)}{#6 #7\SideNS-\VectorSetNS}
\else
\DrawEq [{#6}{#3}]{va=ae1, module (#5)(\Cols)}{}
\fi
}

\DefText[6]{coordinates of the linear map 4}
{
\item $#1$ - координатная матрица множества $#2_2$\Hyph чисел
\ShowEq{Vector f(e1) module}#1{#3}#5#6
относительно базиса \eV[#4][.]
}

\DefText[4]{Let be module of}
{
Пусть  $#1_{#2}$ является \SideRu\What $#3_{#4}$\Hyph \VectorSetRuE \ColsNA.
}

\DefText[2]{we identify linear map and matrix}
{
На основании теорем
\refTheorem{linear map of D module, coordinates}{#1#2cols},
\refTheorem{matrix generates D module homomorphism}{cols(#1#2)},
а также на основании теорем
\refTheorem{linear map of D module, coordinates}{#1#2rows},
\refTheorem{matrix generates D module homomorphism}{rows(#1#2)},
мы идентифицируем линейное отображение
\DrawEq[{\Vector f}V]{homomorphism D algebra #1#2}{}
и матрицу $f$ его представления.
}

\DefLabeledFootnote[4]{homomorphism of d algebra}{#1#2\Cols}
{
В теоремах
\refTheorem{homomorphism of d algebra, coordinates}{#1#2\Cols},
\refTheorem{matrix generates D algebra homomorphism}{\Cols(#1#2)},
мы опираемся на следующее соглашение.
\ShowEq{Let be basis of algebra and C}11iID{#1}A{#2}-
\ShowEq{Let be basis of algebra and C}22jJD{#3}A{#4}-
}

\DefLabeledTheorem[5]{homomorphism of d algebra, coordinates}{#1#2\Cols}
{
Гомоморфизм\refFootnote{homomorphism of d algebra}{#1#2\Cols}
\DrawEq[{\Vector f}A]{homomorphism D algebra #1#2}{}
$D_{#1}$\Hyph алгебры \ColsA $A_{#2}$
в $D_{#3}$\Hyph алгебру \ColsA $A_{#4}$ имеет представление
\DrawEq[f{#5}{}]{f:V1->V2, D module \Cols}{algebra(#1#2)}
\DrawEq[hf{#2}{#4}a]{f o ea=efa i (#1#2)}{(\Cols)algebra}
\DrawEq[hf12]{f o ea=efa (#1#2)(\Cols)}{algebra}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowText{coordinates of the linear map 1}aA1{(#1)(#2)}{}
\ShowText{coordinates of the linear map 2(#1)}ahiI{D_{#3}}
\ShowText{coordinates of the linear map 3}aA2f{}b{(#1)(#2)}
\ShowText{coordinates of the linear map 4}fA{#2}{#4}iI
\ShowText{Morphism of D algebra}{#1}{#2}f{}
\end{itemize}
}

%\DefProofRef[4]{homomorphism of d algebra, coordinates}{#1#2\Cols}
\DefProof[4]{homomorphism of d algebra, coordinates}
{
Равенства
\ShowRef{homomorphism of d algebra, coordinates}{#1}{#2}{#4}
являются следствием теорем
\refTheorem{linear map of D module, coordinates}{#1#2\Cols},
\refTheorem{homomorphism from A1 to A2, D algebra}{#1#2}.

Равенство
\DrawEq{algebra, homomorphism and product eiej(#1#2)}{\Cols}
является следствием равенств
\ShowRef{algebra, homomorphism and product eiej}{#1}{#2}{#3}
Равенство
\DrawEq{algebra, homomorphism and product eiej 4(#1#2)}{\Cols}
является следствием равенства
\ShowRef{algebra, homomorphism and product eiej 1}{#1}{#2}
и равенства
\eqRef{algebra, homomorphism and product eiej(#1#2)}{\Cols}.
Равенство
\DrawEq{algebra, homomorphism and product eiej 5}{(#1#2)\Cols}
является следствием равенства
\ShowRef{homomorphism, f vw=}{#1}{#2}
Равенство
\DrawEq{algebra, homomorphism and product eiej 2(#1#2)}{\Cols}
является следствием равенства
\ShowEq{algebra, homomorphism and product, 1}
и равенства
\eqRef{algebra, homomorphism and product eiej 5}{(#1#2)\Cols}.
Равенство
\DrawEq{algebra, homomorphism and product eiej 3(#1#2)}{\Cols}
является следствием равенств
\eqRef{algebra, homomorphism and product eiej 4(#1#2)}{\Cols},
\eqRef{algebra, homomorphism and product eiej 2(#1#2)}{\Cols}.
Равенство
\ShowRef{algebra, homomorphism and product}{#1}{#2}f
следует из равенства
\eqRef{algebra, homomorphism and product eiej 3(#1#2)}{\Cols}
и теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
}

\DefLabeledTheorem[5]{linear map of D module, coordinates}{#1#2\Cols}
{
Линейное отображение\refFootnote{homomorphism of D module}{\Cols(#1#2)}
\DrawEq[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
$D_{#1}$\Hyph модуля \ColsA $A_{#2}$
в $D_{#3}$\Hyph модуль \ColsA $A_{#4}$ имеет представление
\DrawEq[hf{#2}{#4}{}]{f o ea=efa (#1#2)(\Cols)}{module}
\DrawEq[hf{#2}{#4}a]{f o ea=efa i (#1#2)}{(\Cols)module}
\DrawEq[f{#5}{}]{f:V1->V2, D module \Cols}{#1#2}
относительно заданных базисов. Здесь
\begin{itemize}
\ShowText{coordinates of the linear map 1}aV1{(#1)(#2)}{}
\ShowText{coordinates of the linear map 2(#1)}ahiI{D_{#3}}
\ShowText{coordinates of the linear map 3}aV2f{}b{(#1)(#2)}
\ShowText{coordinates of the linear map 4}fV{#2}{#4}iI
\end{itemize}
}

\DefProofRef[5]{linear map of D module, coordinates}{#1#2\Cols}
{
Так кaк
\newline
\FrameEqRef[{\Vector f}V]{homomorphism D algebra #1#2}{Vector module, coordinates \Cols}
\newline
линейное отображение, то равенство
\ShowEq{vb=h(e1)a (#1)(#2)(\Cols)\SideNS}
является следствием равенств
\ShowRef{vb=h(e1)a}{#1}{#2}{#5}
$V_2$\Hyph число
\ShowEq{f(e1)(\Cols)\SideNS}
имеет разложение
\DrawEq{f(e1)=(\Cols)\SideNS}{(#1)(#2)}
относительно базиса $\Basis e_2$.
Комбинируя \EqRef{vb=h(e1)a (#1)(#2)(\Cols)\SideNS}
и \eqRef{f(e1)=(\Cols)\SideNS}{(#1)(#2)}, мы получаем
\ShowEq{vb=a f e (#1)(#2)(\Cols)\SideNS}
\eqRef{f:V1->V2, D module \Cols}{#1#2}
следует из сравнения
\newline
\FrameEqRef[b2]{va=ae1, module ()(\Cols)}{b (#1)(#2)\SideNS-\VectorSetNS}
\newline
и \EqRef{vb=a f e (#1)(#2)(\Cols)\SideNS} и
теоремы
\refTheorem{coordinates of vector}{\SideNS-\Cols}.
}

\DefDefinitionNote{algebra over ring}
{
Пусть $D$ - коммутативное кольцо.
$D$\Hyph модуль $A$ называется
\AddIndex{алгеброй над кольцом}{algebra over ring} $D$
или
\AddIndex{$D$\Hyph алгеброй}{D algebra},
если определена операция произведения\,\footnotemark
в $A$
\DrawEq{product in D algebra}{definition}
где $C$ - билинейное отображение
\ShowEq{product in algebra, definition 1}
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
}
{
Я следую определению,
приведенному в
\citeBib{Richard D. Schafer}, страница 1,
\citeBib{0105.155}, страница 4. Утверждение,
верное для произвольного $D$\Hyph модуля,
верно также для $D$\Hyph алгебры.
}

\DefText{algebra inherits type of module}
{
$D$\Hyph алгебра $A$ наследует тип $D$\Hyph модуля $A$.
}

\DefLabeledDefinition{type of algebra}{\Cols}
{
$D$\Hyph алгебра $A$ называется
$D$\Hyph алгеброй \ColsNA,
если $D$\Hyph модуль $A$
является $D$\Hyph модулем \ColsNA.
}

\DefLabeledTheorem{associative product in algebra}{\Cols}
{
Если алгебра $A$ коммутативна, то
\DrawEq{commutative product in algebra, 1}{\Cols}
Если алгебра $A$ ассоциативна, то
\DrawEq{associative product in algebra, 1}{\Cols}
}

\DefProof{associative product in algebra}
{
Для коммутативной алгебры,
равенство
\eqRef{commutative product in algebra, 1}{\Cols}
следует из равенства
\ShowEq{commutative product in algebra}
\begin{sloppypar}
\noindent
Для ассоциативной алгебры,
равенство
\eqRef{associative product in algebra, 1}{\Cols}
следует из равенства
\end{sloppypar}
\ShowEq{associative product in algebra}
}

\DefLabeledTheorem{product in algebra}{\Cols}
{
\ShowEq{Let be basis of algebra}{}{}iID{}A{}-
Пусть
\ShowEq{a b in basis of algebra}
Произведение $a$, $b$ можно получить согласно правилу
\DrawEq{product in algebra}{\Cols}
где
\ShowEq{structural constants of algebra symb}
- \AddIndex{структурные константы}{structural constants}
алгебры $A$ над кольцом $D$.
Произведение базисных векторов в алгебре $A$ определено согласно правилу
\DrawEq{product of basis vectors, algebra}{\Cols}
}

\DefProofSloppy{product in algebra}
{
Равенство
\eqRef{product of basis vectors, algebra}{\Cols}
является следствием утверждения, что \eV
является базисом $D$\Hyph алгебры $A$.
Так как произведение в алгебре является билинейным отображением,
то произведение $a$ и $b$ можно записать в виде
\DrawEq{product in algebra, 1}{\Cols}
Из равенств
\eqRef{product of basis vectors, algebra}{\Cols},
\eqRef{product in algebra, 1}{\Cols},
следует
\DrawEq{product in algebra, 2}{\Cols}
Так как \eV является базисом алгебры $A$, то равенство
\eqRef{product in algebra}{\Cols}
следует из равенства
\eqRef{product in algebra, 2}{\Cols}.
}

\DefText{D-module type}
{
Организацию координат вектора в матрице
мы будем называть типом $D$\Hyph модуля.

В этом разделе мы рассмотрим вектор\Hyph столбец
и вектор\Hyph строку.
Очевидно, что существуют и другие формы представления вектора.
Например, мы можем записать координаты вектора в виде
\nmTimes nm матрицы или в виде треугольной матриц.
Формат представления зависит от рассматриваемой задачи.
}

\DefText{D-module type 1}
{
Если утверждение зависит от формата представления вектора,
мы будем указывать либо тип $D$\Hyph модуля,
либо формат представления базиса.
Оба способа указания типа $D$\Hyph модуля эквивалентны.
}

\DefText{Morphism of D algebra, injection 11}
{
(а следовательно,
\ShowEq{Morphism of D algebra, injection}
}

\DefText{Morphism of D algebra, injection 1}
{
}

\DefText[4]{Morphism of D algebra}
{
\item Матрица гомоморфизма
и структурные константы связаны соотношением
\DrawEq[{#3}{}]{algebra, homomorphism and product (#1#2)}{\Cols(\SideNS)#4}
}

\DefText{algebra, homomorphism and product 11}
{
Поскольку отображение $h$ является гомоморфизмом колец,
то равенство
\DrawEq{algebra, homomorphism and product, 4}{\Cols}
является следствием равенства
\eqRef{algebra, homomorphism and product eiej(11)}{\Cols}.
Равенство
\DrawEq{algebra, homomorphism and product, 5 11}{\Cols}
является следствием теоремы
\refTheorem{homomorphism of d algebra, coordinates}{11\Cols}
и равенства
\eqRef{algebra, homomorphism and product, 4}{\Cols}.
}

\DefText{algebra, homomorphism and product 1}
{
Равенство
\DrawEq{algebra, homomorphism and product, 5 1}{\Cols}
является следствием теоремы
\refTheorem{homomorphism of d algebra, coordinates}{1\Cols}
и равенства
\eqRef{algebra, homomorphism and product eiej(1)}{\Cols}.
}

\DefDefinition{commutator of algebra}
{
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
}

\DefDefinitionNote{nucleus of algebra}
{
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это
множество\,\footnotemark
\ShowEq{nucleus of algebra}
}
{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13.}

\DefDefinition{associator of algebra}
{
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
\ShowEq{associator of algebra =}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
}

\DefTheorem{associator of algebra = A}
{
Пусть $\Basis e$ - базис $D$\Hyph алгебры $A$. Тогда
\ShowEq{associator of algebra = A}
где
\AddIndex{координаты ассоциатора}{coordinates of associator}
определены равенством
\ShowEq{coordinates of associator}
\ShowEq{coordinates of associator =}
}

\DefProof{associator of algebra = A}
{
Равенство
\ShowEq{associator of algebra = Ae}
является следствием равенства
\EqRef{associator of algebra =}.
Равенство
\EqRef{coordinates of associator =}
является следствием равенства
\EqRef{associator of algebra = Ae}.
}

\DefDefinitionNote{center of algebra}
{
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это
множество\,\footnotemark
\ShowEq{center of algebra}
}{
Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, страница 14.
}

\DefDefinition{otimes -}
{
Билинейное отображение
\ShowEq{otimes -}
определено равенством
\ShowEq{otimes -, 1}
}


==> Stmt.Representation.Russian.tex <==
%auto-ignore
\input{Stmt.Representation.Eq}

\DefDefinition{morphism of representations of universal algebra}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Для
\ShowEq{i=1,2},
пусть отображение
\ShowEq{ri:A->B}
является гомоморфизмом $\Omega_i$\Hyph алгебры.
Кортеж отображений
\ShowEq{map r12}r{}
таких, что
\ShowEq{morphism of representations of universal algebra, definition, 2}
называется
\AddIndex{морфизмом представлений из $f$ в $g$}
{morphism of representations from f into g}.
Мы также будем говорить, что определён
\AddIndex{морфизм представлений $\Omega_1$\Hyph алгебры
в $\Omega_2$\Hyph алгебре}
{morphism of representations of Omega1 algebra in Omega2 algebra}.
}

\DefRemark{morphism of representations of universal algebra}
{
Мы можем интерпретировать
\eqRef{morphism of representations of universal algebra, 2m}{representation}
двумя способами
\begin{itemize}
\item Пусть преобразование $\BlueText{f(a)}$ отображает $m\in A_2$
в $\BlueText{f(a)}(m)$.
Тогда преобразование
\ShowEq{g(r1(a))}
отображает
\ShowEq{r2(m)in B2}
в
\ShowEq{r2(f(a,m))}
\item Мы можем представить морфизм представлений из $f$ в $g$,
пользуясь диаграммой
\DrawEq{morphism of representations of universal algebra, 2m 1}{ShadedDefinition}
Из \EqRef{morphism of representations of universal algebra, definition, 2}
следует, что диаграмма $(1)$ коммутативна.
\end{itemize}
Мы будем также пользоваться диаграммой
\ShowEq{morphism of representations of universal algebra, definition, 2m 2}
вместо диаграммы
\eqRef{morphism of representations of universal algebra, 2m 1}{ShadedDefinition}.
}

\DefRemark{morphism of representations of universal algebra as map}
{
Мы можем рассматривать пару отображений $r_1$, $r_2$ как отображение
\ShowEq{F:A1+A2->B1+B2}
такое, что
\ShowEq{F:A1+A2->B1+B2 1}
Поэтому в дальнейшем кортеж отображений
\ShowEq{map r12}r{}
мы будем также называть отображением
и пользоваться записью
\ShowEq{f:A->B}rfg
Пусть
\ShowEq{a=a12}
- кортеж $A$\Hyph чисел.
Мы будем пользоваться записью
\ShowEq{r(a)12}
для образа кортежа $A$\Hyph чисел
при морфизме представлений $r$.
}

\DefTheorem{unique morphism of representations of universal algebra}
{
Если представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$ однотранзитивно
и представление
\ShowEq{f:A->*B}g{B_1}{B_2}
$\Omega_1$\Hyph алгебры $B_1$ однотранзитивно,
то для заданного гомоморфизма $\Omega_1$\Hyph алгебры
\ShowEq{f:A->B}{r_1}{A_1}{B_1}
гомоморфизм $\Omega_2$\Hyph алгебры
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
такой, что
\ShowEq{map r12}r{}
является морфизмом
представлений из $f$ в $g$,
определён однозначно
с точностью до выбора образа
\ShowEq{n=r2(m)}
заданного элемента $m\in A_2$.
}

\DefLabeledFootnote[1]{iso end aut morphism}{#1}
{
Я следую определению на
странице \citeBib{Cohn: Universal Algebra}\Hyph 63.
}

\DefConvention[2]{A number}
{
Элемент $#1$\Hyph #2 $A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph числом, а кватернион называется $H$\Hyph числом.
}

\DefTheorem{map is reduced morphism of representations iff}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{f:A->B}{r_2}{A_2}{B_2}
является приведенным морфизмом представлений тогда и только тогда, когда
\DrawEq{reduced morphism representation =}{definition}
}

\DefDefinition{morphism of representation f}
{
Если представления $f$ и $g$ совпадают, то морфизм представлений
\ShowEq{map r12}r{}
называется
\AddIndex{морфизмом представления $f$}{morphism of representation f}.
}

\DefRemark{notation for morphism of representations}
{
Рассмотрим морфизм представлений
\ShowEq{r12:A->B}rAB
Мы можем обозначать элементы множества $B_1$, пользуясь буквой по образцу $b\in B_1$.
Но если мы хотим показать, что $b$ является образом элемента
\ShowEq{a in A1},
мы будем пользоваться обозначением $\RedText{r_1(a)}$.
Таким образом, равенство
\ShowEq{r1(a)=r1(a)}
означает, что $\RedText{r_1(a)}$ (в левой части равенства)
является образом
\ShowEq{a in A1}{}
(в правой части равенства).
Пользуясь подобными соображениями, мы будем обозначать
элемент множества $B_2$ в виде $\BlueText{r_2(m)}$.
Мы будем следовать этому соглащению, изучая соотношения
между гомоморфизмами $\Omega_1$\Hyph алгебр
и отображениями между множествами,
где определены соответствующие представления.
}

\DefTheorem{Tuple of maps is morphism of representations iff}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений тогда и только тогда, когда
\DrawEq{morphism of representations of universal algebra, 2m}{representation}
}

\DefDefinition{tower of representations}
{
Рассмотрим множество $\Omega_k$\Hyph алгебр $A_k$, \Kn1.
Положим $A=(A_1,...,A_n)$.
Положим $f=(f_{1\,2},...,f_{n-1\,n})$.
Множество представлений $f_{k\,k+1}$, \Kn1, 
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_{k+1}$\Hyph алгебре $A_{k+1}$
называется
\AddIndex{башней $(f,A)$ представлений $\Omega$\Hyph алгебр}
{tower of representations of algebras}.
}

\DefDefinition{diagram of representations}
{
\AddIndex{Диаграмма $(f,A)$ представлений универсальных алгебр}
{diagram of representations of algebras}
- это такой ориентированный граф, что
\StartLabelItem
\begin{enumerate}
\item
вершина $A_k$, \Kn1, является $\Omega_k$\Hyph алгеброй;
\item
ребро $f_{kl}$ является представлением
$\Omega_k$\Hyph алгебры $A_k$ в
$\Omega_l$\Hyph алгебре $A_l$;
\end{enumerate}
Мы будем требовать, чтобы этот граф
был связным и не содержал циклов.
Мы будем полагать, что $A_{[0]}$ - это множество начальных вершин графа.
Мы будем полагать, что $A_{[k]}$ - это множество вершин графа,
для которых максимальный путь от начальных вершин равен $k$.
}

\DefRemark{diagram of representations}
{
Так как в разных вершинах графа
может быть одна и таже алгебра,
то мы обозначим
\ShowEq{A=A1n}A{}
множество универсальных алгебр, которые попарно различны.
Из равенства
\ShowEq{A=A(1n)1n}A
следует, что для любого индекса $(i)$
существует по крайней мере один индекс $i$ такой, что
\ShowEq{A(i)=Ai}i.
Если даны два набора множеств
\ShowEq{A=A1n}A,
\ShowEq{A=A1n}B
и определено отображение
\ShowEq{hi:Ai->Bi}
для некоторого индекса $(i)$,
то также определено отображение
\ShowEq{f:A->B}{h_i}{A_i}{B_i}
для любого индекса $i$ такого, что
\ShowEq{A(i)=Ai}i{}
и в этом случае $h_i=h_{(i)}$.
}

\DefTheorem{diagram of representations}
{
{\bf(}\AddIndex{Индукция по диаграмме представлений}{induction over diagram of representations}{\bf)}.
Пусть теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[0]}$
диаграммы $(f,A)$ представлений универсальных алгебр.
Пусть из утверждения, что теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[k]}$
диаграммы $(f,A)$ представлений, следует утверждение,
что теорема $\mathcal T$ верна для множества
универсальных алгебр $A_{[k+1]}$
диаграммы $(f,A)$ представлений.
Тогда теорема $\mathcal T$ верна для множества
универсальных алгебр
диаграммы $(f,A)$ представлений.
}

\DefDefinitionNote{commutative diagram of representations}
{
Диаграмма $(f,A)$ представлений универсальных алгебр
называется
\AddIndex{коммутативной}{commutative diagram of representations},
если выполнено следующее условие.
для каждой пары представлений
\ShowEq{f:A->*B}{f_{ik}}{A_i}{A_k}
\ShowEq{f:A->*B}{f_{jk}}{A_j}{A_k}
следующее равенство верно\,\footnotemark
\ShowEq{fik fjk = fjk fik}
}
{
Образно говоря,
представления $f_{ik}$ и $f_{jk}$
прозрачны друг для друга.
}

\DefTheoremNote{diagram of representations, define map fik}
{
Пусть
\ShowEq{f:i->*j}ij
представление $\Omega_i$\Hyph алгебры $A_i$
в $\Omega_j$\Hyph алгебре $A_j$.
Пусть
\ShowEq{f:i->*j}jk
представление $\Omega_j$\Hyph алгебры $A_j$
в $\Omega_k$\Hyph алгебре $A_k$.
Мы можем описать фрагмент\,\footnotemark
\DrawEq[ijk]{Ai->*Aj->*Ak}{}
диаграмы представлений с помощью диаграммы
%\ePrints{8525-2526}
%\ifx\Semafor\ValueOn
%\newpage
%\fi
\ShowEq{tower of representations, 1 2 3}
Отображение
\ShowEq{f:A->End 2 3}
определено равенством
\ShowEq{define map f13}
где
\ShowEq{a in A}i,
\ShowEq{a in A}j.
Если представление $f_{jk}$ эффективно
и представление $f_{ij}$ свободно,
то отображение $f_{ijk}$ является свободным представлением
\ShowEq{f:1->*3}
$\Omega_i$\Hyph алгебры $A_i$
в $\Omega_j$\Hyph алгебре
\ShowEq{End Ak}Ak.
}
{
Теорема
\RefTheorem{diagram of representations, define map fik}
утверждает, что преобразования в башне представлений согласованы.
}

\DefDefinition{Morphism of Diagram of Representations}
{
Пусть
$(f,A)$
- диаграмма представлений, где
\ShowEq{A=A1n}A{}
- множество универсальных алгебр.
Пусть
$(B,g)$
- диаграмма представлений, где
\ShowEq{A=A1n}B{}
- множество универсальных алгебр.
Множество отображений
\ShowEq{A=A1n}h{}
\ShowEq{hi:Ai->Bi}
называется \AddIndex{морфизмом из диаграммы представлений
$(f,A)$ в диаграмму представлений $(B,g)$}
{morphism from diagram of representations into diagram of representations},
если для любых индексов $(i)$, $(j)$, $i$, $j$ таких, что
\ShowEq{A(i)=Ai}i,
\ShowEq{A(i)=Ai}j,
и для каждого представления
\ShowEq{f:A->*B}{f_{ji}}{A_j}{A_i}
пара отображений $(h_j\ \ h_i)$ является
морфизмом представлений из $f_{ji}$ в $g_{ji}$.
}

\AddEq{remark: Morphism of Diagram of Representations}
{
Для любого представления $f_{ij}$,
\Kn[i]1, \Kn[j]1,
мы имеем диаграмму
\ShowEq{morphism of diagram of representations of F algebra, level k, diagram}
Равенства
\ShowEq{morphism of diagram of representations, level k}
\ShowEq{morphism of diagram of representations, levels k k+1}
выражают коммутативность диаграммы (1).
}

\DefTheorem{reduced polymorphism of representations}
{
Пусть отображение $r_2$ - приведенный полиморфизм
эффективных представлений $f_1$, ..., $f_n$ в эффективное представление $f$.
\begin{itemize}
\item
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, ak}
\item
Для любого
\ShowEq{kl,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, akl}
\item
Пусть $\omega_2\in\Omega_2(p)$.
Для любого
\ShowEq{k,1n}
отображение $r_2$ удовлетворяет равенству
\ShowEq{reduced polymorphism of representation, omega2}
\end{itemize}
}

\AddEq{remark: morphism of representation of Omega group}
{
\begin{remark}
\labelRemark{morphism of \SideWS representation of Omega group}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть отображение
\ShowEq{f:A->*B}g{B_1}{B_2}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $B_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Пусть отображение
\ShowEq{r12:A->B}rAB
является морфизмом представлений.
Мы будем пользоваться записью
\ShowEq{r2a=r2 o a}
для образа $A_2$\Hyph числа $a_2$
при отображении $r_2$.
Тогда мы можем записать равенство
\eqRef{morphism of representations of universal algebra, 2m}{representation}
следующим образом
\ShowEq{morphism of \SideWS representation of Omega group}
\qed
\end{remark}
}

\DefTheorem{proper definition of orbit}
{
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является левосторонним представлением
мультипликативной $\Omega$\Hyph группы $A_1$.
Если
\ShowEq{orbit, proposition}
то
\ShowEq{A1a2=A1b2}
}

\AddEq{definition: orbit of representation}
{
\begin{ShadedDefinition}
\labelDefinition{orbit of \SideNS-side representation}
Пусть $A_1$ является $\Omega$\Hyph группоидом с произведением
\ShowEq{(ab)->ab}
Пусть отображение
\ShowEq{f:A->*B}f{A_1}{A_2}
является \SideRu восторонним представлением
$\Omega$\Hyph группоида $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Для любого
\ShowEq{a in A}2,
мы определим
\AddIndex{орбиту представления}{orbit of representation}
$\Omega$\Hyph группоида $A_1$ как множество
\ShowEq{orbit of \SideNS-side representation}
\end{ShadedDefinition}
}

\AddEq{Let A->*AB2 be representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
}

\AddEq{Let XY be generating sets}
{
Пусть $X$ - множество образующих представления
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $Y$ - множество образующих представления
\ShowEq{f:A->*B}g{A_1}{B_2}
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
}

\DefDefinitionNote{product in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ShowEq{product in category}
и множество морфизмов
\ShowEq{set f:A->B}fP{B_i}
называется
\AddIndex{произведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{product in category}\,\footnotemark,
если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}gR{B_i}
существует единственный морфизм
\ShowEq{f:A->B}hRP
такой, что диаграмма
\ShowEq{product in category diagram}
коммутативна для всех $i\in I$.

Если $|I|=n$, то для произведения множества объектов
$\{B_i,\iI\}$ в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{product in category, 1 n}
}
{
Определение дано согласно \citeBib{Serge Lang},
страница 45.
}

\DefExample{Cartesian product of sets}
{
Пусть \(\mathcal S\) - категория множеств.\,\footnote{Смотри
также пример в
\citeBib{Serge Lang},
страница 45.
}
Согласно определению
\ShowEq{ref product in category}
декартово произведение
\ShowEq{Cartesian product of sets}
семейства множеств
\ShowEq{Ai iI}A{}
и семейство проекций на \(i\)\Hyph й множитель
\ShowEq{projection on i factor}
являются произведением в категории \(\mathcal S\).
}

\DefTheorem{product of effective representations}
{
В категории
\ShowEq{A1(mA2)}
существует произведение
эффективных представлений $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре
и это произведение является
эффективным представлением $\Omega_1$\Hyph алгебры $A_1$.
}

\DefTheoremNote{structure of subrepresentations}
{
Пусть\,\footnotemark
\ShowEq{f:A->*B}g{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть $X\subset A_2$.
Определим подмножество $X_k\subset A_2$ индукцией по $k$.
\ShowEq{structure of subrepresentations}
Тогда
\ShowEq{structure of subrepresentations, 1}
}{
Утверждение теоремы аналогично
утверждению теоремы 5.1, \citeBib{Cohn: Universal Algebra}, страница 94.
}

\DefFootnote{direct sum of Abelian groups}
{
Определение дано согласно \citeBib{Serge Lang}, страница 55.
}

\DefLabeledDefinition{direct sum of Abelian groups}{\GroupLbl}
{
Копроизведение в категории \GroupType тивных абелевых групп
\ShowEq{category Ab(\GroupLbl)}
называется
\AddIndex{прямой суммой}{direct sum}.\,\RefFootnote{direct sum of Abelian groups}
Мы будем пользоваться записью
\ShowEq{direct sum of Abelian groups}
для прямой суммы абелевых групп $A$ и $B$.
}

\DefDefinitionNote{coproduct in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Пусть
\ShowEq{category A[Bi]}
- категория,
объектами которой являются кортежи $(P,f)$,
где $P$ - объект категории $\mathcal A$
и $f$ - множество морфизмов
\ShowEq{set f:A->B}f{B_i}P
Универсально отталкивающий объект категории
\ShowEq{category A[Bi]}
\ShowEq{coproduct in category}
называется
\AddIndex{копроизведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{coproduct in category}.\,\footnotemark

Если $|I|=n$, то для копроизведения множества объектов
\ShowEq{set Bi}B
в $\mathcal A$
мы так же будем пользоваться записью
\ShowEq{coproduct in category, 1 n}
}
{
Определение дано согласно определению на странице
\citeBib{Serge Lang}\Hyph 46.
}

\DefFootnote{free Abelian group}
{
Смотри также определение в \citeBib{Serge Lang}, страницы 56, 57.
}

\DefLabeledDefinition{free Abelian group}{\GroupLbl}
{
Пусть $S$ - множество и\,\RefFootnote{free Abelian group}
\ShowEq{category AbS(\GroupLbl)}
- категория, объектами которой являются отображения
\ShowEq{f:A->B}fSG
множества $S$ в \GroupType тивные абелевые группы.
Если
\ShowEq{f:A->B}fSG
\ShowEq{f:A->B}{f'}S{G'}
объекты категории
\ShowEq{category AbS(\GroupLbl)},
то морфизм из $f$ в $f'$
- это гомоморфизм групп
\ShowEq{f:A->B}gG{G'}
такой, что диаграмма
\DrawEq{AbS ff'g}{}
коммутативна.
}

\DefFootnote{theorem free Abelian group}
{
Смотри аналогичное утверждение в \citeBib{Serge Lang}, страница 57.
}

\DefLabeledTheorem{free Abelian group}{\GroupLbl}
{
Универсально отталкивающий объект $G$ категории
\ShowEq{category AbS(\GroupLbl)}
существует.\,\RefFootnote{theorem free Abelian group}
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{S in G}
\item
Множество $S$ порождает \GroupType вную абелевую группу $G$.
\labelItem{set generates Abelian group (\GroupLbl)}
\end{enumerate}
Абелевая группа $G$ называется
{\bf free Abelian group},
порождённой множеством $S$.
}

\DefProof{free Abelian group}
{
Пусть $G$
- множество отображений
\ShowEq{f:A->B}hSZ
таких, что множество
\ShowEq{x in -> h(x)}{}
конечно.

\begin{ShadedLemma}
Определим на множестве $G$ операцию
\ShowEq{h1h2=}
Множество $G$ является \GroupType тивной абелевой группой.
\end{ShadedLemma}
{\sc Доказательство.}
Пусть
\ShowEq{h12 in G}
Согласно определению, множества
\ShowEq{x in -> h(x)}1
\ShowEq{x in -> h(x)}2
конечны.
Тогда конечно множество
\ShowEq{H1vH2}
Следовательно,
\ShowEq{h1+h2 in G}
Свойства абелевой группы очевидны.
\hfill\(\odot\)

Пусть $k\in Z$, $x\in S$.
Рассмотрим отображение $h=k*x$, определённое равенством
\ShowEq{k*x=k}
Отображение
\ShowEq{f:S->G}
инъективно и позволяет отождествить $S$ и образ $f(S)\subseteq G$
(утверждение
\RefItem{S in G (\GroupLbl)})
и пользоваться записью
\ShowEq{kx=k*x(\GroupLbl)}
Согласно определению множества $G$,
любое отображение $h\in G$ может быть записано в виде
\ShowEq{h=k*x(\GroupLbl)}
где
\ShowEq{k in Z x in S}
и множество
\ShowEq{|kx ne 0|}
конечно.
Утверждение
\RefItem{set generates Abelian group (\GroupLbl)}
является следствием теоремы
\refTheorem{structure of Abelian group}{\GroupLbl}.

\begin{ShadedLemma}
{\it
Представление
\EqRef{h=k*x(\GroupLbl)}
отображения $h$ единственно.
}
\end{ShadedLemma}
{\sc Доказательство.}
Если отображение $h$ допускает представления
\ShowEq{h=k12*x i(\GroupLbl)}
то равенство
\ShowEq{k1-k2 *x(\GroupLbl)}
является следствием равенства
\EqRef{h=k12*x i(\GroupLbl)}.
\ShowEq{k1=k2 i}
следует из равенства
\EqRef{k1-k2 *x(\GroupLbl)}.
\hfill\(\odot\)

Пусть
\ShowEq{f:A->B}{f'}S{G'}
отображение множества $S$ в абелевую группу $G'$.
Мы определим гомоморфизм
\ShowEq{f:A->B}gG{G'}
таким образом, чтобы диаграмма
\DrawEq{AbS ff'g}{\GroupLbl}
была коммутативной.
Из диаграммы
\eqRef{AbS ff'g}{\GroupLbl}
следует, что
\DrawEq{g(1x)=f'(x)}{\GroupLbl}
Согласно теореме
\refTheorem{homomorphism f(na)=nf(a)}{\GroupLbl},
так как отображение $g$ - гомоморфизм абелевой группы, то равенство
\ShowEq{g(x)=(\GroupLbl)}
для любого отображения $h\in G$
является следствием равенств
\eqRef{g(1x)=f'(x)}{\GroupLbl},
\EqRef{h=k*x(\GroupLbl)}.
Следовательно, гомоморфизм $g$ определён однозначно.
Согласно определениям
\RefDefinition{universally repelling object of category},
\refDefinition{free Abelian group}{\GroupLbl},
абелевая группа $G$ является свободной группой.
}

\DefLabeledTheorem{homomorphism f(na)=nf(a)}{\GroupLbl}
{
Гомоморфизм
\ShowEq{f:A->B}fG{G'}
удовлетворяет равенству
\ShowEq{f(na)=nf(a) (\GroupLbl)}
}

\DefTheoremNote{coproduct in category}
{
Пусть $\mathcal A$ - категория.
Пусть
\ShowEq{set Bi}B
- множество объектов из $\mathcal A$.
Объект
\ShowEq{coproduct in category}
и множество морфизмов
\ShowEq{set f:A->B}f{B_i}P
называется
\AddIndex{копроизведением множества объектов
\ShowEq{set Bi}B
в категории $\mathcal A$}
{coproduct in category},\,\footnotemark
если для любого объекта $R$ и множество морфизмов
\ShowEq{set f:A->B}g{B_i}R
существует единственный морфизм
\ShowEq{f:A->B}hPR
такой, что диаграмма
\ShowEq{coproduct in category diagram}
коммутативна для всех $i\in I$.
}{Определение дано согласно \citeBib{Serge Lang}, страница 46.}

\DefProof{coproduct in category}
{
Теорема является следствием определений
\RefDefinition{universally repelling object of category},
\RefDefinition{coproduct in category}.
}

\DefFootnote{Theorem direct sum of Abelian groups}
{
Смотри также предложение \citeBib{Serge Lang}-10, страница 55.
}

\DefLabeledTheorem{direct sum of Abelian groups}{\GroupLbl}
{
Пусть
\ShowEq{set Bi}A
- семейство \GroupType тивных абелевых групп.
Пусть
\ShowEq{A in xAi}
такое множество, что
\ShowEq{(xi)in A}
Тогда\,\RefFootnote{Theorem direct sum of Abelian groups}
\ShowEq{A=o+Ai}A
}

\DefProof{direct sum of Abelian groups}
{
Согласно теореме
\RefTheorem[\RefRepresentation]{product exists in category of Omega algebras},
существует абелевая группа
\ShowEq{B=prod Ai}
%\begin{sloppypar}
Согласно утверждению
\RefItem[\RefRepresentation]{tuple represent A number},
мы можем представить $B$\Hyph число $a$ в виде кортежа
\ShowEq{set Bi}a
$A_i$\Hyph чисел.
Согласно утверждению
\RefItem[\RefRepresentation]{operation is defined componentwise},
\GroupOpName в группе $B$ определен\OpEndS равенством
%\end{sloppypar}
\DrawEq{(ai)+(bi)=(ai+bi)}{\GroupLbl}

Согласно построению
$A$ является подгруппой абелевой группы $B$.
Отображение
\ShowEq{f:A->B}{\lambda_j}{A_j}A
определённое равенством
\DrawEq{lj(x)=0x0}{\GroupLbl}
является инъективным гомоморфизмом.

Пусть
\ShowEq{set f:A->B}f{A_i}\GroupLbl
семейство гомоморфизмов в \GroupType тивную абелевую группу $C$.
Мы определим отображение
\ShowEq{f:A->B}fAC
пользуясь равенством
\ShowEq{fxi,i=sum fxi(\GroupLbl)}
\GroupOpNameC в правой части равенства
\EqRef{fxi,i=sum fxi(\GroupLbl)}
конечн\OpEnd, так как все \ArgsOfOp, кроме конечного числа, равны $\UnitId$.
Из равенства
\ShowEq{fi(x+y)=}
и равенства
\EqRef{fxi,i=sum fxi(\GroupLbl)}
следует, что
\ShowEq{f(x+y)i=}
Следовательно, отображение $f$ является гомоморфизмом абелевой группы.
Равенство
\ShowEq{flj=fj}
является следствием равенств
\eqRef{lj(x)=0x0}{\GroupLbl},
\EqRef{fxi,i=sum fxi(\GroupLbl)}.
Так как отображение $\lambda_i$ инъективно,
то отображение $f$ определено однозначно.
Следовательно, теорема является следствием определений
\RefDefinition{coproduct in category},
\refDefinition{direct sum of Abelian groups}{\GroupLbl}.
}

\AddEq{remark: Non-commutative Sum}
{
С детства мы знаем, что от перестановки мест слагаемых сумма не меняется.
Поэтому, когда услышал о некоммутативном сложении
(\citeBib{Alain Connes 1994}),
я слегка растерялся.
Однако мне недавно повезло встретить геометрию, где сумма векторов некоммутативна.

В школе я увлекался многими вещами: физикой, химией, черчением.
Математика была немного в стороне.
Я не любил арифметику, но мне нравились алгебра и геометрия.
Я тогда ещё не знал, что все пути ведут в математику.

Черчение было моим любим предметом. Мой учитель,
Габис Сергей Александрович, подарил мне сборник задач по черчению,
и я добросовестно все их перерешал.
А потом придумал свою собственную задачу и решил её.
К моему удивлению, первая теорема, которую мы доказывали на
уроке геометрии на следующий год, была именно решением этой задачи.

Я понимал, что после школы мне будет сложно поступить в институт.
Поэтому после восьмого класса я решил что я буду поступать в техникум.
Бела Марковна предложила позаниматься со мной летом,
посмотреть насколько я готов к экзамену по математике.
Один из уроков остался в моей памяти.
Когда мы рассматривали графики прямой и параболы,
Бела Марковна сказала: нарисовать прямую или параболу легко,
а как быть с кардиограммой?
И я загорелся идеей найти аналитическое выражение 
для кардиограммы.

Мой товарищ предложил мне на протяжении лета
вместе изучать математический анализ.
В нашем доме жили мальчики, которые учились в техникуме,
и они одолжили мне свой учебник по математическому анализу.
К этому времени мой товарищ потерял интерес к своей идее,
и я стал изучать математический анализ самостоятельно.

Первая глава учебника была посвящена аналитической геометрии.
И я понял, что это то что мне нужно для анализа кривых кардиограммы.
Аналитическая геометрия решила моё будущее.
Я понял, что буду готовиться в университет на механико-математический факультет.

Я перечитал много книг по математическому анализу.
Но в какой-то момент у меня сложилось впечатление
что один автор списывает у другого.
Я стал искать другие книги.
Не помню откуда у меня появился первый том Фихтенгольца.
Но эта книга произвела на меня неизгладимое впечатление.
Ближе к весне я почувствовал, что книга становится трудной,
но продолжал читать.
В марте у меня был грипп с необычайно высокой температурой.
Но я сомневаюсь, что это был грипп,
так как после этого первый том Фихтенгольца стал для меня понятен.

Изучение математического анализа отразилось
на моих попытках восстановить функциональную
зависимость с графика. Я тогда ещё не понимал,
что не всякое отображение может быть представлено аналитически.
Я рисовал графики, составлял таблицы приращения функции
в зависимости от приращения аргумента.
Но вскоре эта затея мне надоела,
и я сменил занятие.

Когда мне в руки попала книга по тензорному исчислению,
я обнаружил, что сложные построения аналитической геометрии
по классификации кривых второго порядка
можно заменить простыми теоремами линейной алгебры.
После этого, мой интерес к аналитической геометрии
заметно стал меньше.

Прошло почти полвека.
И неожиданно аналитическая геометрия преподнесла мне
два приятных сюрприза.
Сперва я обнаружил, что аналитическая геометрия
является интересной структурой с точки зрения
теории представлений универсальных алгебр.
Точнее, я отождествляю аналитическую и аффинную геометрии,
но я думаю, что это небольшая ошибка.

Второй сюрприз связан с тем, что я понял,
что я могу построить модель аффинной геометрии
в римановом пространстве.
Так как я очень долго занимался метрико\Hyph аффинными многообразиями,
то оставался один шаг, чтобы увидеть модель аффинной геометрии,
где сумма некоммутативна.
С этого момента некоммутативное сложение перестало быть для меня
абстрактной концепцией.
}

\DefText{side representation of group}
{
Из равенства
\eqRef{* \SideNS-side representation of group}{def}
следует, что
\DrawEq{o \SideNS-side representation of group}{def}
Мы можем рассматривать равенство
\eqRef{o \SideNS-side representation of group}{def}
как
\AddIndex{закон ассоциативности}{associative law},

\begin{sloppypar}
\begin{example}
Пусть
\ShowEq{f:A->B}f{A_2}{A_2}
\ShowEq{f:A->B}g{A_2}{A_2}
эндоморфизмы $\Omega_2$\Hyph алгебры $A_2$.
Пусть произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
является композицией эндоморфизмов.
Так как произведение отображений $f$ и $g$ определено в том же порядке,
как эти отображения действуют на $A_2$\Hyph число,
то мы можем рассматривать равенство
\ShowEq{fga= o \SideNS}
как
закон ассоциативности,
который позволяет записывать равенство
\EqRef{fga= o \SideNS}
без использования скобок
\ShowEq{fga= 1 \SideNS}
а также записать равенство
\eqRef{\SideNS-side representation of group}{def}
в виде
\DrawEq{\SideNS-side 1 representation of group}{def}
\qed
\end{example}
\end{sloppypar}
}

\AddEq[4]{theorem: select second basis of representation}
{
\begin{ShadedTheorem}
\labelTheorem{select second basis of representation, #4}
Пусть $#2$ - пассивное преобразование
многообразия базисов #3 $#4$.
Пусть $\Basis e_1$ - базис #3 $#4$,
\ShowEq{e2=e1 o S}{#2}21
Пусть для базиса $\Basis e_3$ существует активное преобразование $#1$ такое, что
\ShowEq{e3=R o e1}{#1}31
Положим
\ShowEq{e3=R o e1}{#1}42
Тогда
\ShowEq{e2=e1 o S}{#2}43
\end{ShadedTheorem}
}

\AddEq[3]{proof: select second basis of representation}
{
\begin{proof}
Согласно равенству
\eqRef{active transformation}{#3},
активное преобразование координат базиса $\Basis e_3$ имеет вид
\DrawEq{active transformation, 1}{#3}
Пусть
\ShowEq{e2=e1 o S}{#2}53
Из равенства
\eqRef{passive transformation}{#3}
следует, что
\DrawEq{passive transformation, 1}{#3}
Из совпадения выражений в равенствах
\eqRef{active transformation, 1}{#3},
\eqRef{passive transformation, 1}{#3}
следует, что
\ShowEq{Basis e4=Basis e5}
Следовательно,
коммутативна диаграмма
\ShowEq{passive and active maps}{#1}{#2}
\end{proof}
}

\AddEq[2]{definition: basis manifold}
{
Множество
\ShowEq{basis manifold}
базисов #1 $#2$ называется
\AddIndex{многообразием базисов}{basis manifold}
#1 $#2$.
}

\AddEq{ref active representation, representation}
{
Согласно теоремам
\RefTheorem{superposition of coordinates, representation},
\RefTheorem{Automorphism of representation maps a basis into basis},
}

\AddEq{ref active representation, diagram of representations}
{
Согласно теореме
\RefTheorem{Automorphism of diagram of representations maps a basis into basis}
и определению
\RefDefinition{superposition of coordinates and words, diagram of representations},
}

\AddEq[4]{definition: active representation in basis manifold}
{
\begin{ShadedDefinition}
\labelDefinition{active representation in basis manifold, #1}
\ShowEq{ref active representation, #1}
автоморфизм $#4$ #2 $#3$
порождает преобразование
\DrawEq[{#4}]{active transformation}{#1}
многообразия базисов #2.
Это преобразование называется
\AddIndex{активным}{active transformation of basis}.
Согласно теореме
\RefTheorem{group of automorphisms of #1},
определено левостороннее представление
\ShowEq{active representation in basis manifold}
\ShowEq{active representation in basis manifold def}
группы $GA(f)$
в многообразии базисов $\mathcal B[f]$.
Представление $A(f)$ называется
\AddIndex{активным представлением}{active representation in basis manifold}.
Согласно следствию
\RefCorollary{automorphism uniquely defined by image of basis, #1},
это представление однотранзитивно.
\qed
\end{ShadedDefinition}
}

\AddEq[4]{remark: active representation}
{
\begin{remark}
\labelRemark{active representation, #1}
Согласно замечанию
\RefRemark{X is quasibasis of #1},
могут существовать базисы #2 $#3$,
не связанные активным преобразованием.
В этом случае мы в качестве многообразия базисов будем рассматривать
орбиту выбранного базиса.
Следовательно, #4 $#3$ может иметь различные многообразия базисов.
Мы будем предполагать, что мы выбрали многообразие базисов.
\end{remark}
}

\AddEq[6]{theorem: Coordinate transformation does not depend}
{
\begin{ShadedTheorem}
\labelTheorem{Coordinate transformation does not depend, #1}
Допустим пассивное преобразование $#2\in GA(f)$ отображает
базис $\Basis e_1\in\mathcal{B}[f]$
в базис $\Basis e_2\in\mathcal{B}[f]$
\DrawEq[{#2}]{passive transformation S}{#1}
Допустим #6 $#3$ имеет #5
\DrawEq[1{#3}]{Omega_2 word, basis e}{1 #1}
относительно базиса $\Basis e_1$ и имеет #5
\DrawEq[2{#3}]{Omega_2 word, basis e}{2 #1}
относительно базиса $\Basis e_2$.
Преобразование координат
\DrawEq[{#3}{#2}]{coordinate transformation}{#1}
не зависит от #4 $#3$ или базиса $\Basis e_1$, а
определенно исключительно координатами #4 $#3$
относительно базиса $\Basis e_1$.
\end{ShadedTheorem}
}

\AddEq[3]{proof: Coordinate transformation does not depend}
{
\begin{proof}
Из \eqRef{passive transformation S}{#1}
и
\eqRef{Omega_2 word, basis e}{2 #1}
следует, что
\DrawEq[{#2}{#3}]{Omega word in representation, basis Y, 1}{#1}
Сравнивая \eqRef{Omega_2 word, basis e}{1 #1}
и
\eqRef{Omega word in representation, basis Y, 1}{#1}
получаем, что
\DrawEq[{#2}{#3}]{coordinate transformation in representation, 1}{#1}
Так как $#2$ - автоморфизм представления, то равенство
\eqRef{coordinate transformation}{#1}
следует из
\eqRef{coordinate transformation in representation, 1}{#1}
и теоремы
\RefTheorem{coordinates of inverse transformation, #1}.
\end{proof}
}

\AddEq[3]{remark: active and passive transformation}
{
Активное преобразование изменяет базис #1 и
#2 согласовано
и координаты #3 относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к изменению
координат #3 относительно базиса.
}

\AddEq[2]{theorem: Coordinate transformations form right-side representation}
{
\begin{ShadedTheorem}
\labelTheorem{Coordinate transformations form right-side representation, #1}
Преобразования координат
\eqRef{coordinate transformation}{#1}
порождают эффективное контравариантное
правостороннее представление группы $GA(f)$, называемое
\AddIndex{координатным представлением}{coordinate representation}
в #2.
\end{ShadedTheorem}
}

\AddEq[8]{proof: Coordinate transformations form right-side representation}
{
\begin{proof}
Согласно следствию
\RefCorollary{map of coordinates of #1},
преобразование
\eqRef{coordinate transformation}{#1}
является эндоморфизмом #4\,\footnote{Это преобразование
не порождает эндоморфизма #4 $#6$. Координаты меняются, поскольку меняется
базис, относительно которого мы определяем координаты. Однако
#7, координаты которого мы рассматриваем, не меняется.}
#5

Допустим мы имеем два последовательных пассивных преобразования
$#2$ и $#8$. Преобразование координат
\DrawEq[{#3}{#2}]{coordinate transformation}{#2 #1}
соответствует пассивному преобразованию $#2$.
Преобразование координат
\DrawEq[{#3}{#8}]{coordinate transformation}{#8 #1}
соответствует пассивному преобразованию $#8$.
Согласно теореме
\RefTheorem{passive representation in basis manifold, #1},
произведение преобразований координат
\eqRef{coordinate transformation}{#2 #1}
и
\eqRef{coordinate transformation}{#8 #1}
имеет вид
\ShowEq{coordinate transformation in representation, TS}{#3}{#2}{#8}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\ShowEq{coordinate transformation in representation, TS 1}{#8}{#2}
Согласно теоремам
\RefTheorem{coordinates of inverse transformation, #1},
\RefTheorem{coordinates of product of inverse transformation, #1}
и определению
\RefDefinition{Left side contravariant representation}
преобразования координат
порождают
правостороннее контравариантное представление группы $GA(f)$.

Если координатное преобразование не изменяет координаты выбранного базиса,
то ему соответствует единица группы $GA(f)$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
\end{proof}
}

\AddEq[5]{remark: geometric object}
{
Пассивное представление $P(g)$ согласовано
с пассивным представлением $P(f)$,
если существует гомоморфизм $h$ группы $GA(f)$ в группу $GA(g)$.
Рассмотрим диаграмму
\ShowEq{passive representation coordinated with passive representation}
Так как отображения $P(f)$, $P(g)$ являются изоморфизмами группы,
то отображение $H$ является гомоморфизмом групп.
Следовательно, отображение $f'$ является представлением группы $GA(f)$
в многообразии базисов $\mathcal B(g)$.
Согласно построению, пассивному преобразованию $#2$ многообразии базисов $\mathcal B(f)$
соответствует пассивное преобразование $H(#2)$ многообразия базисов $\mathcal B(g)$
\DrawEq[{#2}]{passive transformation of representation g}{#1}
Тогда координатное преобразование в #3 $#4$ принимает вид
\DrawEq[{#5}{#2}]{coordinate transformation g}{#1}
}

\AddEq[5]{definition: coordinate of geometric object}
{
\begin{ShadedDefinition}
\labelDefinition{coordinate of geometric object, #1}
Мы будем называть
орбиту
\ShowEq{coordinates of geometric object}{#3}%
\ShowEq{show coordinates of geometric object}{#2}{#3}
\AddIndex{координатами геометрического объекта}{coordinates of geometric object},
определёнными в #4 $#5$.
Для любого базиса
\ShowEq{geometric object 1}{#2}
соответствующая точка
\eqRef{coordinate transformation g}{#1}
орбиты  определяет
\AddIndex{координаты геометрического объекта}{coordinates of geometric object}
относительно базиса
\ShowEq{geometric object 2}
\qed
\end{ShadedDefinition}
}

\AddEq[1]{remark: 2 views on geometric object}
{
Так как геометрический объект - это орбита представления,
то согласно теореме
\RefTheorem{proper definition of orbit}
определение геометрического объекта корректно.

Определение
\RefDefinition{coordinate of geometric object, #1}
строит геометрический объект в координатном пространстве.
Определение \RefDefinition{geometric object, #1} предполагает,
что мы выбрали базис представления $g$.
Это позволяет использовать представитель геометрического объекта
вместо его координат.
}

\AddEq[7]{definition: geometric object}
{
\begin{ShadedDefinition}
\labelDefinition{geometric object, #1}
Мы будем называть
орбиту
\ShowEq{geometric object}{#3}%
\ShowEq{show geometric object}{#2}{#3}%
\AddIndex{геометрическим объектом}{geometric object},
определённым в #4 $#5$.
Мы будем также говорить, что $#3$ - это
\AddIndex{геометрический объект типа $H$}{type of geometric object}.
Для любого базиса
\ShowEq{geometric object 1}{#2}
соответствующая точка 
\eqRef{coordinate transformation g}{#1}
орбиты  определяет #6
\ShowEq{geometric object 2, g}{#3}%
#7 мы называем
\AddIndex{представителем геометрического объекта}{representative of geometric object}
в #4 $#5$.
\qed
\end{ShadedDefinition}
}

\AddEq[1]{theorem: invariance principle}
{
\begin{ShadedTheorem}[принцип инвариантности]
\AddIndex{}{invariance principle}
\labelTheorem{invariance principle, #1}
Представитель геометрического объекта не зависит от выбора
базиса $\Basis e_f$.
\end{ShadedTheorem}
}

\AddEq[6]{proof: invariance principle}
{
\begin{proof}
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $\Basis e_f$ #2 $#3$,
базис $\Basis e_g$ #2 $#4$
и координаты геометрического объекта
\ShowEq{invariance principle 4}{#5}
Соответствующий представитель геометрического
объекта имеет вид
\ShowEq{invariance principle 1}{#5}
Базис $\Basis e_{f1}$ связан с базисом
$\Basis e_f$ пассивным преобразованием
\ShowEq{invariance principle 2 passive}{#6}
Согласно построению это порождает пассивное преобразование
\eqRef{passive transformation of representation g}{#1}
и координатное преобразование
\eqRef{coordinate transformation g}{#1}.
Соответствующий
представитель геометрического объекта имеет вид
\ShowEq{invariance principle 3 algebra}{#5}{#6}
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
\end{proof}
}

\AddEq[1]{theorem: passive representation in basis manifold}
{
\begin{ShadedTheorem}
\labelTheorem{passive representation in basis manifold, #1}
Существует однотранзитивное правостороннее представление
\ShowEq{passive representation in basis manifold}
\ShowEq{passive representation in basis manifold def}
группы $GA(f)$
в многообразии базисов $\mathcal B[f]$.
Представление $P(f)$ называется
\AddIndex{пассивным представлением}{passive representation in basis manifold}.
\end{ShadedTheorem}
}

\DefProof{passive representation in basis manifold}
{
Поскольку $A(f)$ - однотранзитивное левостороннее представление группы $GA(f)$,
то однотранзитивное правостороннее представление $P(f)$
определено однозначно
согласно теореме
\RefTheorem{two representations of group}.
}

\AddEq[1]{theorem: passive transformation is automorphism of A(f)}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation is automorphism of A(f), #1}
Пассивное преобразование многообразия базисов
является автоморфизмом представления $A(f)$.
\end{ShadedTheorem}
}

\DefProof{passive transformation is automorphism of A(f)}
{
Теорема является следствием теоремы
\RefTheorem{twin representations of group, automorphism}.
}

\AddEq[3]{theorem: passive transformation}
{
\begin{ShadedTheorem}
\labelTheorem{passive transformation, #1}
Преобразование представления $P(f)$
называется
\AddIndex{пассивным преобразованием многообразия базисов}
{passive transformation of basis}
#2.
Мы будем пользоваться записью
\ShowEq{passive transformation of basis}{#3}
\ShowEq{passive transformation of basis def}{#3}
для обозначения образа базиса $\Basis e$ при пассивном преобразовании $#3$.
Пассивное преобразование базиса имеет вид
\DrawEq[#3]{passive transformation}{#1}
\end{ShadedTheorem}
}

\AddEq[1]{proof: passive transformation}
{
\begin{proof}
Согласно равенству
\eqRef{active transformation}{#1},
активное преобразование действует на координаты
базиса слева.
Равенство
\eqRef{passive transformation}{diagram of representations}
следует из теорем
\RefTheorem{shift is automorphism of representation},
\RefTheorem{two representations of group},
\RefTheorem{twin representations of group, automorphism},
согласно которым
пассивное преобразование действует на координаты
базиса справа.
\end{proof}
}

\DefLabeledDefinitionNote{side representation of group}{\SideNS}
{
Пусть
\ShowEq{End O2}{A_2}{}
- мультипликативная $\Omega$\Hyph группа с произведением\,\footnotemark
\ShowEq{(fg)->fg}
Пусть эндоморфизм $f$ действует на $A_2$\Hyph число $a$ с\SideRu ва.
Мы будем пользоваться записью
\ShowEq{f(a)=o \SideNS}
Пусть $A_1$ - мультипликативная $\Omega$\Hyph группа с произведением
\ShowEq{(ab)->ab}
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{\SideNS-side}
\AddIndex{\SideRu восторонним представлением}{\SideNS-side representation}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{\SideRu восторонним $A_1$\Hyph представлением}{\SideNS-side A representation}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{\SideNS-side representation of group}{def}
Мы будем отождествлять
$A_1$\Hyph число $a_1$ с его образом $f(a_1)$
и записывать \SideRu востороннее преобразование,
порождённое $A_1$\Hyph числом $a_1$,
в форме
\ShowEq{\SideNS-side representation}
В этом случае равенство
\eqRef{\SideNS-side representation of group}{def}
принимает вид
\DrawEq{* \SideNS-side representation of group}{def}
Отображение
\ShowEq{A12->A2 1 \SideNS}
порождённое \SideRu восторонним представлением $f$, называется
\AddIndex{\SideRu восторонним произведением}{\SideNS-side product}
$A_2$\Hyph числа $a_2$ на $A_1$\Hyph число $a_1$.
}
{
Очень часто произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
совпадает с суперпозицией эндоморфизмов
\ShowEq{Act=circ}
Однако произведение
в мультипликативной $\Omega$\Hyph группе
\ShowEq{End O2}{A_2}{}
может отличаться от суперпозиции эндоморфизмов.
}

\DefDefinition{reduced morphism of representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$ и 
\ShowEq{f:A->*B}g{A_1}{B_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $B_2$.
Пусть
\ShowEq{id:A1->A1 A2->B2}
морфизм представлений.
В этом случае мы можем отождествить морфизм
\ShowEq{map r,R}{\id}{r_2}{}
представлений $\Omega_1$\Hyph алгебры и соответствующий гомоморфизм $r_2$ $\Omega_2$\Hyph алгебры
и будем называть гомоморфизм $r_2$
\AddIndex{приведенным морфизмом представлений}
{reduced morphism of representations}.
Мы будем пользоваться диаграммой
\ShowEq{morphism id,R of representations}
для представления приведенного морфизма $r_2$ представлений
$\Omega_1$\Hyph алгебры.
Из диаграммы следует
\ShowEq{morphism of representations of universal algebra}
Мы будем также пользоваться диаграммой
\ShowEq{morphism id,R of representations 2}
вместо диаграммы
\EqRef{morphism id,R of representations}.
}

\DefLabeledDefinition{action of rational integers in Abelian group}{\GroupLbl}
{
Мы определим действие кольца целых чисел $Z$
в \GroupType тивной абелевой группе $G$
согласно правилу
\ShowEq{action of rational integers in Abelian group (\GroupLbl)}
}

\DefLabeledTheorem{action of ring of rational integers in Abelian group}{\GroupLbl}
{
Действие кольца целых чисел $Z$
в \GroupType тивной абелевой группе $G$,
рассмотренное в определении
\refDefinition{action of rational integers in Abelian group}{\GroupLbl},
является представлением.
Верны следующие равенства
\ShowEq{representation of Z in G (\GroupLbl)}
}

\DefProof{action of ring of rational integers in Abelian group}
{
Равенство
\EqRef{1a=a (\GroupLbl)}
является следствием равенства
\EqRef{0g=0 (\GroupLbl)}
и равенства
\EqRef{(n+1)g= (\GroupLbl)},
когда $n=0$.

\ShowEq{step of proof: action in Abelian group}{(m+n)a=ma+na}

Равенство
\ShowEq{(k+n)a-na=ka (\GroupLbl)}
является следствием равенства
\EqRef{(m+n)a=ma+na (\GroupLbl)}.
Равенство
\EqRef{(m-n)a=ma-na (\GroupLbl)}
является следствием равенства
\EqRef{(k+n)a-na=ka (\GroupLbl)},
если мы положим
$m=k+n$, $k=m-n$.

\ShowEq{step of proof: action in Abelian group}{(nm)a=n(ma)}

\ShowEq{step of proof: action in Abelian group}{n(a+b)=na+nb}

Из равенства
\EqRef{n(a+b)=na+nb (\GroupLbl)}
следует, что отображение
\ShowEq{phi(n):G->G (\GroupLbl)}
является эндоморфизмом абелевой группы $G$.
Из равенств
\EqRef{(m+n)a=ma+na (\GroupLbl)},
\EqRef{(nm)a=n(ma) (\GroupLbl)}
следует, что отображение
\ShowEq{phi:Z->End(G)}
является гомоморфизмом кольца $Z$.
Согласно определению
\RefDefinition[\RefRepresentation]{representation of algebra},
отображение $\varphi$ является представлением
кольца целых чисел $Z$
в абелевой группе $G$.
}

\DefDefinitionNote{tensor product of representations}
{
Пусть $A$ является абелевой мультипликативной $\Omega_1$\Hyph группой.
Пусть
\ShowEq{a1n}An{}
- $\Omega_2$\Hyph алгебры.\,\footnotemark
Пусть для любого
\ShowEq{k,1n}
\ShowEq{representation A Ak 1}
эффективное представление мультипликативной $\Omega_1$\Hyph группы $A$
в $\Omega_2$\Hyph алгебре $A_k$.
Рассмотрим категорию $\mathcal A$ объектами которой являются
приведенные полиморфизмы представлений $f_1$, ..., $f_n$
\ShowEq{polymorphisms category}
где $S_1$, $S_2$ - $\Omega_2$\Hyph алгебры и
\ShowEq{representation of algebra in S1 S2}
эффективные представления мультипликативной $\Omega_1$\Hyph группы $A$.
Мы определим морфизм
\ShowEq{r1->r2}
как приведенный морфизм представлений $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{polymorphisms category, diagram}
Универсальный объект
\ShowEq{tensor product of representations}
категории $\mathcal A$ называется
\AddIndex{тензорным произведением}{tensor product}
представлений
\ShowEq{a1n}An.
}
{
Я определяю
тензорное произведение представлений универсальной алгебры
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
}

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{tensor product of representations}
Если существует полиморфизм представлений,
то тензорное произведение представлений существует.
\end{ShadedTheorem}
}
{theorem: tensor product of representations}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{representation, tensor product}
Пусть
\ShowEq{equivalence, 1, representation, tensor product}
Тензорное произведение дистрибутивно относительно операции $\omega$
\ShowEq{tensors 1, representation, tensor product}
Представление мультипликативной $\Omega_1$\Hyph группы $A$
в тензорном произведении определено равенством
\ShowEq{tensors 2, representation, tensor product}
\end{ShadedTheorem}
}
{theorem: representation, tensor product}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{tensor product and polymorphism}
Пусть $B_1$, ..., $B_n$ -
$\Omega_2$\Hyph алгебры.
Пусть
\ShowEq{map f, 1, representation, tensor product}
приведенный полиморфизм, определённый равенством
\ShowEq{map f, representation, tensor product}
Пусть
\ShowEq{map g, representation, tensor product}
приведенный полиморфизм в $\Omega_2$\Hyph алгебру $V$.
Существует морфизм представлений
\ShowEq{map h, representation, tensor product}
такой, что диаграмма
\ShowEq{map gh, representation, tensor product}
коммутативна.
\end{ShadedTheorem}
}
{theorem: tensor product and polymorphism}
%DefEq

\DefEq
{
\begin{ShadedTheorem}
\labelTheorem{B times->B otimes}
Отображение
\ShowEq{B times->B otimes}
является полиморфизмом.
\end{ShadedTheorem}
}
{theorem: B times->B otimes}
%DefEq

\DefTheorem{|a-b|>|a|-|b|}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Тогда
\ShowEq{|a-b|>|a|-|b|}
}

\DefDefinitionNote{free representation of algebra}
{
Мы будем называть представление
\ShowEq{f:A->*B}f{A_1}{A_2}
$\Omega_1$\Hyph алгебры $A_1$
\AddIndex{свободным}{free representation},\,\footnotemark
если из утверждения
\ShowEq{faa=fba}
для любого
\ShowEq{a in A}2{}
следует, что
\ShowEq{a=b}.
}
{
Аналогичное определение свободного представления группы смотри в
\citeBib{Postnikov: Differential Geometry}, страница 16.
\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn
Смотри также теорему
\RefTheorem{free representation of group}.
\fi
}

\DefDefinition{continuous map, Omega group}
{
Отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{|x'-x|<delta}
влечёт
\ShowEq{|f(x)-f(x')|<epsilon}
}

\DefTheorem{continuous map, open set}
{
Отображение
\DrawEq[f{A_1}{A_2}{}]{f: A->B}{}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
непрерывно тогда и только тогда, когда
прообраз открытого множества
является открытым множеством.
}

\DefTheorem{image of interval is interval, real field}
{
Пусть
\ShowEq{f:A->B}fRR
непрерывное отображение поля действительных чисел.
Тогда образ интервала является интервалом.
}

\DefDefinition{norm of operation}
{
Пусть $A$
- нормированн\WhatA $\Omega$\Hyph \Algebrab.
Для $n$\Hyph арной операции $\omega$, величина
\ShowEq{norm of operation}
\ShowEq{norm of operation, definition}
называется
\AddIndex{нормой операции}{norm of operation} $\omega$.
}

\DefTheorem{|fx|<|f||x|1n}
{
Пусть $A$ - нормированн\WhatA $\Omega$\Hyph \Algebrab.
Для $n$\Hyph арной операции $\omega$,
\ShowEq{|a omega|<|omega||a|1n}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{norm of representation}
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление\
\ePrints{1305.4547}
\ifx\Semafor\ValueOn
\footnote{
Смотри определение
\ShowEq{ref definition: left-side representation of algebra}{}
представления универсальной алгебры.
Согласно определению
\xRef[1211.6965]{definition: module over ring},
модуль - это представление кольца в абелевой группе.
Так как кольцо и абелева группа являются $\Omega$\Hyph группами,
то модуль - это представление $\Omega$\Hyph группы.
}
\fi
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Величина
\ShowEq{norm of representation}
\ShowEq{norm of representation, definition}
называется
\AddIndex{нормой представления}{norm of representation} $f$.
\qed
\end{ShadedDefinition}
}
{definition: norm of representation}
%\DefEq

\DefTheorem{|fab|<|f||a||b|}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Тогда
\ShowEq{|fab|<|f||a||b|}
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{open set}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Множество
$U\subset A$
называется
\AddIndex{открытым}{open set},\,\footnote{
В топологии
обычно сперва определяют открытое множество,
а затем базу топологии.
В случае метрического или нормированного пространства,
удобнее дать определение открытого множества,
опираясь на определение базы топологии.
В этом случае определение основано на одном из свойств
базы топологии. Непосредственная проверка
позволяет убедиться, что определённое таким образом
открытое множество удовлетворяет основным свойствам.
}
если для любого $A$\Hyph числа
\ShowEq{a in U}{}
существует
\ShowEq{epsilon in R}
такое, что
\ShowEq{B(a) subset U}
\qed
\end{ShadedDefinition}
}
{definition: open set}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{compact set}
Множество $T$ топологического пространства называется
\AddIndex{компактным}{compact set},
если любое его открытое покрытие содержит
конечное подпокрытие.\,\footnote{
Смотри также определение в
\citeBib{Kolmogorov Fomin}, страница 98.
}
\qed
\end{ShadedDefinition}
}
{definition: compact set}
%\DefEq

\DefTheorem{c1+c2 in B}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Для
\ShowEq{c1 c2 in A}cA,
пусть
\ShowEq{c1 c2 in B}
Тогда
\ShowEq{c1+c2 in B}
}

\DefLabeledDefinition{limit of sequence}{normed \AlgebraLabel}
{
Пусть $\Module$
- нормированн\EndC $\Base$\Hyph \Algebrab.
$\Module$\Hyph число $a$ называется 
\AddIndex{пределом последовательности}{limit of sequence}
\ShowEq{[an] in A}
\ShowEq{limit of sequence}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|an-a|<epsilon}{-}
для любого $n>n_0$.
Мы будем также говорить, что
\AddIndex{последовательность $a_n$ сходится}{sequence converges}
к $a$.
}

\DefLabeledTheorem{limit of sequence}{\AlgebraLabel}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
$\Module$\Hyph число $a$ является 
пределом последовательности
\ShowEq{[an] in A}
\DrawEq{a=lim an}{}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{an in B(a)}{}
для любого $n>n_0$.
}

\DefProof{limit of sequence}
{
Следствие определений
\RefDefinition{open ball},
\refDefinition{limit of sequence}{normed \AlgebraLabel}.
}

\DefLabeledDefinition{fundamental sequence}{normed \AlgebraLabel}
{
Пусть $\Module$
- нормированн\EndC $\Base$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
называется 
\AddIndex{фундаментальной}{fundamental sequence}
или \AddIndex{последовательностью Коши}{Cauchy sequence},
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|ap-aq|<epsilon}{-}
для любых $p$, $q>n_0$.
}

\AddEq{theorem: fundamental sequence}
{
\begin{ShadedTheorem}
\labelTheorem{fundamental sequence, normed \Algebrac}
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Последовательность
\ShowEq{[an] in A}
является фундаментальной последовательностью,
тогда и только тогда, когда для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\ShowEq{aq in B(ap)}
для любых $p$, $q>n_0$.
\end{ShadedTheorem}
}

\DefProof{fundamental sequence}
{
Следствие определений
\RefDefinition{open ball},
\refDefinition{fundamental sequence}{normed \Algebrac}.
}

\DefTheorem{norm of compact set is bounded}
{
Пусть $C$ - компактное множество
нормированной $\Omega$\Hyph группы $A$.
Тогда норма
\ShowEq{|x in C|}
ограничена сверху и снизу.
}

\DefTheorem{lim a=lim b}
{
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть $a_n$, $b_n$, $n=1$, ..., - фундаментальные последовательности.
Пусть
\DrawEq{lim a-b=0}{limit}
Если последовательность $a_n$ сходится, то
последовательность $b_n$ сходится и
\ShowEq{lim a=lim b}
}

\DefDefinition{complete Omega group}
{
Нормированн\WhatA $\Omega$\Hyph \AlgebrabWS $A$ называется 
\AddIndex{полн\WhatB}{complete Omega \IndexAlgebra}
если любая фундаментальная последовательность элементов
$\Omega$\Hyph \AlgebradWS $A$ сходится, т. е.
имеет предел в этой $\Omega$\Hyph \Algebrae.
}

\DefText{complete D algebra}
{
Если полное $\Omega$\Hyph кольцо $A$
является $D$\Hyph алгеброй,
то $D$\Hyph алгебра $A$ называется
\AddIndex{банаховой}{Banach algebra}.
}

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{limit of sequence, map to Omega group}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
Отображение
\ShowEq{f M(X,A)}
называется
\AddIndex{пределом последовательности}{limit of sequence}
$f_n$, если для любого $x\in X$
\DrawEq{f(x)=lim}{}
Мы будем также говорить, что
\AddIndex{последовательность $f_n$ сходится}{sequence converges}
к отображению $f$.
\qed
\end{ShadedDefinition}
}
{definition: limit of sequence, map to Omega group}
%\DefEq

\DefEq
{
\begin{ShadedDefinition}
\labelDefinition{sequence converges uniformly}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
\AddIndex{Последовательность $f_n$ сходится равномерно}
{sequence converges uniformly}
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{fn(x) - f(x)}
для любого $n>N$.
\qed
\end{ShadedDefinition}
}
{definition: sequence converges uniformly}
%\DefEq

\DefTheorem{sequence converges uniformly, fn-fm}
{
Последовательность отображений
\ShowEq{fn M(X,A)}
в нормированную
$\Omega$\Hyph группу $A$ сходится равномерно
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{|fn(x)-fm(x)|<e}
для любых \(n\), \(m>N\).
}

\DefDefinition{quasibasis of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$
и
\ShowEq{Gen f =}
Если для множества $X\subset A_2$ верно
\ShowEq{in Gen}Xf,
то для любого множества $Y$, $X\subset Y\subset A_2$,
также верно
\ShowEq{in Gen}Yf.
Если существует минимальное множество
\ShowEq{in Gen}Xf,
то множество $X$ называется
\AddIndex{квазибазисом}{quasibasis}
представления $f$.
}

\DefTheorem{X is quasibasis of representation}
{
Если множество $X$ является квазибазисом представления $f$,
то для любого $m\in X$
множество $X\setminus\{m\}$ не является
множеством образующих представления $f$.
}

\DefRemark{X is quasibasis of representation}
{
Доказательство теоремы
\RefTheorem{X is quasibasis of representation}
даёт нам эффективный метод построения квазибазиса представления $f$.
Выбрав произвольное множество образующих, мы шаг за шагом
исключаем те элементы множества, которые имеют координаты
относительно остальных элементов множества.
Если множество образующих представления бесконечно,
то рассмотренная операция может не иметь последнего шага.
Если представление имеет конечное множество образующих,
то за конечное число шагов мы можем построить квазибазис этого представления.
}

\AddEq{remark: representation in form of Omega2-word is ambiguous}
{
Мы ввели $\Omega_2$\Hyph слово элемента $x\in A_2$ относительно множества образующих $X$
в определении
\RefDefinition{word of element relative to set, representation}.
Из теоремы
\RefTheorem{X is quasibasis of representation}
следует, что если множество образующих $X$ не является квазибазисом,
то выбор $\Omega_2$\Hyph слова относительно множества образующих $X$ неоднозначен.
Но даже если множество образующих $X$ является квазибазисом,
то представление $m\in A_2$ в виде $\Omega_2$\Hyph слова неоднозначно.
}

\DefDefinitionNote{word of element relative to set, representation}
{
Пусть $X\subset A_2$.
Для любого
\ShowEq{x in JX}m{}
существует
\AddIndex{$\Omega_2$\Hyph слово}
{word of element relative to generating set, representation}
\ShowEq{word of element relative to generating set, representation},
определённое согласно следующему правилам.
\StartLabelItem
\begin{enumerate}
\item Если $m\in X$, то $m$ - $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, m in X}
\item Если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова и
$\omega\in\Omega_2(n)$, то $m_1...m_n\omega$
- $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, omega}
\item Если $m$ - $\Omega_2$\Hyph слово и
\ShowEq{a in A1},
то $f(a)(m)$
- $\Omega_2$\Hyph слово.
\labelItem{word of element relative to set, representation, am}
\end{enumerate}
Мы будем отождествлять элемент
\ShowEq{x in JX}m{}
и соответствующее ему $\Omega_2$\Hyph слово, выражая это равенством
\ShowEq{identify element jf(X) and word}
Аналогично, для произвольного множества
\ShowEq{subset of representation}{}
рассмотрим множество $\Omega_2$\Hyph слов\,\footnotemark
\ShowEq{subset of words of representation}
Мы будем также пользоваться записью
\ShowEq{subset of words of representation, 1}
Обозначим
\ShowEq{word set of representation}
\AddIndex{множество $\Omega_2$\Hyph слов представления $J[f,X]$}
{word set of representation}.
}{
Выражение $\wXm$
является частным случаем
выражения $\wXm[B]$, а именно
\ShowEq{subset of words of representation, 2}
}

\DefRemark{three reasons of ambiguity in Omega2-word}
{
Существует три источника неоднозначности в записи
$\Omega_2$\Hyph слова.
\StartLabelItem
\begin{enumerate}
\item
В $\Omega_i$\Hyph алгебре $A_i$, $i=1$, $2$,
могут быть определены равенства.
Например, если $e$ - единица мультипликативной группы $A_i$,
то верно равенство
\[ae=a\]
для любого $a\in A_i$.
\item
\begin{sloppypar}
Неоднозначность выбора $\Omega_2$\Hyph слова
может быть связана со свойствами представления.
Например, если $m_1$, ..., $m_n$ - $\Omega_2$\Hyph слова,
$\omega\in\Omega_2(n)$ и
\ShowEq{a in A1},
то\,\footnote{
Например, пусть
$\{e_1,e_2\}$
- базис векторного пространства над полем $k$.
Равенство \EqRef{ambiguity of coordinates 1}
принимает форму закона дистрибутивности
\ShowEq{ambiguity of coordinates 1, vector}
}
\ShowEq{ambiguity of coordinates 1}
В тоже время, если $\omega$ является операцией
$\Omega_1$\Hyph алгебры $A_1$ и операцией
$\Omega_2$\Hyph алгебры $A_2$, то мы можем потребовать,
что $\Omega_2$\Hyph слова
\ShowEq{a1n omega x}
и
\ShowEq{a1n x omega}
описывают один и тот же
элемент $\Omega_2$\Hyph алгебры $A_2$.\,\footnote{Для векторного пространства
это требование принимает форму закона дистрибутивности
\ShowEq{(a+b)e=ae+be}
}
\DrawEq{ambiguity of coordinates 2}{representation}
\end{sloppypar}
\item
Равенства вида
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
сохраняются при морфизме представления.
Поэтому мы можем игнорировать эту
форму неоднозначности записи $\Omega_2$\Hyph слова.
Однако возможна принципиально другая форма неоднозначности,
пример которой можно найти
в теоремах
\refTheorem[\RefRepresentation]{linear dependence between vectors of basis}{\SideWS module},
\refTheorem[\RefRepresentation]{coordinates of vector with linear dependence}{\SideWS module}.
\end{enumerate}
Таким образом, мы видим, что на множестве $\Omega_2$\Hyph слов
можно определить различные отношения эквивалентности.\,\footnote{
Очевидно, что каждое из равенств
\EqRef{ambiguity of coordinates 1},
\eqRef{ambiguity of coordinates 2}{representation}
порождает некоторое отношение эквивалентности.
}
Наша задача - найти максимальное отношение эквивалентности
на множестве $\Omega_2$\Hyph слов, которое
сохраняется при морфизме представления.
}

\DefTheoremNote{equivalence generated by basis}
{
Пусть $X$ - квазибазис представления
\ShowEq{f:A->*B}f{A_1}{A_2}
Для любого множества образующих $X$ представления $f$
существует отношение эквивалентности
\ShowEq{l fX in w fX}
которое порождено исключительно следующими утверждениями.
\StartLabelItem
\begin{enumerate}
\item
%\labelItem{w1 w2 in l fX}
Если в $\Omega_2$\Hyph алгебре $A_2$ существует равенство
\ShowEq{w1[]=w2[]}
определяющее структуру $\Omega_2$\Hyph алгебры, то
\ShowEq{w1 w2 in l fX}
\item
%\labelItem{fw1m fw2m in l fX}
Если в $\Omega_1$\Hyph алгебре $A_1$ существует равенство
\ShowEq{w1[]=w2[]}
определяющее структуру $\Omega_1$\Hyph алгебры, то
\ShowEq{fw1m fw2m in l fX}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l}
Для любой операции
\ShowEq{omega n ari}{}1n,
\ShowEq{(f(a1n)a2,f(a)a2) in l}
\item
%\labelItem{(fa1(a21n),fa1(a2)) in l}
Для любой операции
\ShowEq{omega n ari}{}2n,
\ShowEq{(fa1(a21n),fa1(a2)) in l}
\item
%\labelItem{(f(a1n)a2,f(a)a2) in l 1}
Пусть
\ShowEq{omega in O1AO2}12.
Если представление $f$ удовлетворяет равенству\,\footnotemark
\ShowEq{f(a1n)a2=f(a)a2}
то мы можем предположить, что верно равенство
\ShowEq{(f(a1n)a2,f(a)a2) in l 1}
\end{enumerate}
}
{
Рассмотрим представление коммутативного кольца $D$
в $D$\Hyph алгебре $A$. Мы будем пользоваться записью
\ShowEq{f(a)(v)=av}
В обеих алгебрах определены операции сложения и умножения.
Однако равенство
\ShowEq{f(a+b)v=}
верно, а равенство
\ShowEq{f(ab)v=}
является ошибочным.
}

\DefDefinition{basis of representation}
{
Квазибазис $\Basis e$ представления $f$ такой, что
\ShowEq{rho=lambda}
называется
\AddIndex{базисом представления}{basis of representation} $f$.
}

\DefDefinition{equivalence on the set of Omega2-words}
{
Множество образующих $X$ представления $f$
порождает отношение эквивалентности
\ShowEq{rho fX=}
на множестве $\Omega_2$\Hyph слов.
}

\DefTheorem{h=f+g, converges uniformly}
{
Пусть последовательность отображений
\ShowEq{fn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $f$.
Пусть последовательность отображений
\ShowEq{gn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $g$.
Тогда последовательность отображений
\ShowEq{hn=fn+gn}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению
\DrawEq{h=f+g}{converges uniformly}
}

\DefTheorem{representation f generates representation fX}
{
Представление
\ShowEq{f:A->*B}g{A_1}{A_2}
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$
порождает представление
\ShowEq{f:A->*B}{f_X}{M(X,A_1)}{M(X,A_2)}
$\Omega_1$\Hyph группы
\ShowEq{M(X,A1)}
в $\Omega_2$\Hyph группе
\ShowEq{M(X,A2)}
где (
\ShowEq{g1 in M(X,A1)},
\ShowEq{g2 in M(X,A2)}
)
\ShowEq{f(x)g(x):X->A2}
}

\DefTheorem{fX(g1)(g2), converges uniformly}
{
Пусть
\ShowEq{f:A->*B}g{A_1}{A_2}
представление
полной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в полной $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть последовательность отображений
\ShowEq{g1n M(X,A1)}
сходится равномерно
к отображению $g_1$.
Пусть последовательность отображений
\ShowEq{g2n M(X,A2)}
сходится равномерно
к отображению $g_2$.
Пусть множество значений отображения $g_i$, $i=1$, $2$,
компактно.
Тогда последовательность отображений
\ShowEq{f(g1n)(g2n)}
сходится равномерно
к отображению
\ShowEq{fX(g1)(g2)}.
}

\DefTheorem{set of maps to Omega group}
{
Пусть
\ShowEq{set of maps to Omega group}
- множество отображений множества $X$ в $\Omega$\Hyph группу $A$.
Мы можем определить структуру $\Omega$\Hyph группы на множестве
\EqParm{M(X,A)}{=.}
}

\DefEq
{
Так как $X$ - произвольное множество, мы не можем определить
норму в $\Omega$\Hyph группе
\EqParm{M(X,A)}{=.}
Однако мы можем определить сходимость последовательности в
\EqParm{M(X,A)}{=.c}
следовательно, мы можем определить топологию в
\EqParm{M(X,A)}{=.}
}
{remark: set of maps to Omega group}
%\DefEq

\DefDefinition{closed ball}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{closed ball}
называется
\AddIndex{замкнутым шаром}{closed ball}
с центром в $a$.
}

\DefDefinition{open ball}
{
Пусть $\Module$
- нормированн\WhatA $\Base$\Hyph \Algebrab.
Пусть $a\in \Module$.
Множество
\ShowEq{open ball}
называется
\AddIndex{открытым шаром}{open ball}
с центром в $a$.
}

\DefDefinition{reduced polymorphism of representations}
{
Пусть
\ShowEq{set of universal algebras 1}
- универсальные алгебры.
Пусть, для любого
\ShowEq{k,1n}
\ShowEq{f:A->*B}{f_k}A{B_k}
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B_k$.
Пусть
\ShowEq{f:A->*B}fAB
эффективное представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
Отображение
\ShowEq{reduced polymorphism of representation}
называется
\AddIndex{приведенным полиморфизмом представлений}
{reduced polymorphism of representations}
$f_1$, ..., $f_n$ в представление $f$,
если для любого
\ShowEq{k,1n}
при условии, что все переменные кроме переменной $x_k\in B_k$
имеют заданное значение, отображение $r_2$
является приведенным морфизмом представления $f_k$ в представление $f$.

Если $f_1=...=f_n$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f_1$ в представление $f$.

Если $f_1=...=f_n=f$, то мы будем говорить, что отображение $r_2$
является приведенным полиморфизмом представления $f$.
}

\DefConvention{Einstein summation}
{
Мы будем пользоваться соглашением Эйнштейна о сумме.
Это означает, что, когда индекс присутствует в
выражении дважды (один вверху и один внизу) и множество индексов известно,
это выражение подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av}av
Я буду явно указывать множество
индексов, если это необходимо.
}

\DefText{in this section G is group}
{
В этом разделе $G$ - \GroupType тивная абелевая группа.
}

\DefLabeledTheorem{structure of Abelian group}{\GroupLbl}
{
Множество $G$\Hyph чисел, порождённое множеством
\ShowEq{S=si},
имеет вид
\ShowEq{J(S)=gi si (\GroupLbl)}
где множество
\ShowEq{|gi ne 0|}g
конечно.
}

\DefProof{structure of Abelian group}
{
Мы докажем теорему по индукции, опираясь на теоремы
\citeBib{Cohn: Universal Algebra}\Hyph 5.1, страница 94, и
\RefTheorem[\RefRepresentation]{structure of subrepresentations}.

Для произвольного $\aD sk\in S$,
положим
\ShowEq{gi=dik}
Тогда
\ShowEq{sk=sum si (\GroupLbl)}
\ShowEq{sk in JS}
следует из
\EqRef{J(S)=gi si (\GroupLbl)},
\EqRef{sk=sum si (\GroupLbl)}.

Пусть
\ShowEq{w12 in Jv}gS
Так как $G$ является абелевой группой,
то, согласно утверждению
\RefItem[\RefRepresentation]{x1n omega in Xk+1},
\ShowEq{w1+w2 in Jv (\GroupLbl)}gS
Согласно равенству
\EqRef{J(S)=gi si (\GroupLbl)},
существуют $Z$\Hyph числа
\ShowEq{gi12}g
такие, что
\DrawEq[g]{w12= (\GroupLbl)}{group}
где множества
\DrawEq[g]{|ci12 ne 0|}{group(\GroupLbl)}
конечны.
Из равенства
\eqRef{w12= (\GroupLbl)}{group}
следует, что
\DrawEq[g]{w1+w2= (\GroupLbl)}{group}
Равенство
\DrawEq[g]{w1+w2= 1 (\GroupLbl)}{group}
является следствием равенств
\EqRef{(m+n)a=ma+na (\GroupLbl)},
\eqRef{w1+w2= (\GroupLbl)}{group}.
Из равенства
\eqRef{|ci12 ne 0|}{group(\GroupLbl)}
следует, что
множество
\ShowEq{|gi 1+2 ne 0| (\GroupLbl)}g
конечно.
Из равенства
\eqRef{w1+w2= 1 (\GroupLbl)}{group}
следует, что
\ShowEq{w1+w2 in Jv (\GroupLbl)}gS
}

\DefConvention{Einstein summation convention ()}
{
Мы будем пользоваться соглашением о произведении,
в котором повторяющийся индекс (один в основании и один в экспоненте)
подразумевает произведение по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса произведения и знак произведения опускается
\ShowEq{av=prod av}gs
}

\DefConvention{Einstein summation convention (+)}
{
Мы будем пользоваться соглашением Эйнштейна о сумме,
в котором повторяющийся индекс (один вверху и один внизу)
подразумевает сумму по повторяющемуся индексу.
В этом случае предполагается известным множество
индекса суммирования и знак суммы опускается
\ShowEq{av=sum av}gs
}

\AddEq [1]{step of proof: action in Abelian group}
{
Из равенства
\EqRef{0g=0  (\GroupLbl)}
следует, что равенство
\EqRef{#1 (\GroupLbl)}
верно, когда $n=0$.
\def\TempA{(nm)a=n(ma)}
\def\TempC{product Z bilinear 1}
\def\TempD{product Z bilinear 2}
\def\TempB{#1}
\begin{itemize}
\item
Пусть равенство
\EqRef{#1 (\GroupLbl)}
верно, когда $n=k\ge 0$.
Тогда
\ShowEq{#1,n=k (\GroupLbl)}
Равенство
\ShowEq{#1,n=k+1 (\GroupLbl)}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n+1)g= (\GroupLbl)},
\EqRef{(m+n)a=ma+na (\GroupLbl)}.
\else
\ifx\TempC\TempB
равенств
\EqRef{(n+1)g= (\GroupLbl)},
\EqRef{(a+b)c=distributive}.
\else
\ifx\TempD\TempB
равенств
\EqRef{(n+1)g= (\GroupLbl)},
\EqRef{a(b+c)=distributive}.
\else
равенства
\EqRef{(n+1)g= (\GroupLbl)}.
\fi
\fi
\fi
Следовательно, равенство
\EqRef{#1 (\GroupLbl)}
верно, когда $n=k+1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1 (\GroupLbl)}
верно для любого $n\ge 0$.
\item
Пусть равенство
\EqRef{(m+n)a=ma+na (\GroupLbl)}
верно, когда $n=k\le 0$.
Тогда
\ShowEq{#1,n=k (\GroupLbl)}
Равенство
\ShowEq{#1,n=k-1 (\GroupLbl)}
является следствием
\ifx\TempA\TempB
равенств
\EqRef{(n-1)g= (\GroupLbl)},
\EqRef{(m-n)a=ma-na (\GroupLbl)}.
\else
\ifx\TempC\TempB
равенств
\EqRef{(n+1)g= (\GroupLbl)},
\EqRef{(a+b)c=distributive}.
\else
\ifx\TempD\TempB
равенств
\EqRef{(n+1)g= (\GroupLbl)},
\EqRef{a(b+c)=distributive}.
\else
равенства
\EqRef{(n-1)g= (\GroupLbl)}.
\fi
\fi
\fi
Следовательно, равенство
\EqRef{#1 (\GroupLbl)}
верно, когда $n=k-1$.
Согласно принципу математической индукции,
равенство
\EqRef{#1 (\GroupLbl)}
верно для любого $n\le 0$.
\item
Следовательно, равенство
\EqRef{#1 (\GroupLbl)}
верно для любого $n\in Z$.
\end{itemize}
}

\DefDefinition{category of representations A1(mA2)}
{
Пусть $A_1$ - $\Omega_1$\Hyph алгебра.
Пусть $\mathcal A_2$ - категория $\Omega_2$\Hyph алгебр.
Мы определим \AddIndex{категорию
\ShowEq{A1(mA2) symb}
представлений}
{category of representations}
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Объектами этой категории являются представления
$\Omega_1$\Hyph алгебры $A_1$ в $\Omega_2$\Hyph алгебре.
Морфизмами этой категории являются приведенные морфизмы соответствующих представлений.
}

\DefProofRef{cr transpose}{}
{
Мы можем доказать \eqRef{cr transpose}{Theorem} в случае матриц тем же
образом, что мы
доказали \eqRef{rc transpose}{Theorem}. Тем не менее для нас более
важно показать, что \eqRef{cr transpose}{Theorem}
следует непосредственно из \eqRef{rc transpose}{Theorem}.

Применяя \EqRef{double transpose} к каждому слагаемому в левой части
\eqRef{cr transpose}{Theorem}, мы получим
\ShowEq{cr transpose, 1}
Из \EqRef{cr transpose, 1} и \eqRef{rc transpose}{Theorem}
следует, что
\ShowEq{cr transpose, 2}
\eqRef{cr transpose}{Theorem} следует из \EqRef{cr transpose, 2}
и \EqRef{double transpose}.
}

\DefProofRef{rc transpose}{}
{
Цепочка равенств
\ShowEq{rc transpose, 1}
следует из \EqRef{transpose of matrix, 1},
\EqRef{rc-product of matrices} и
\EqRef{cr-product of matrices}.
Равенство \eqRef{rc transpose}{Theorem} следует из
\EqRef{rc transpose, 1}.
}

\DefText{matrix operations 1}
{
Согласно традиции произведение
матриц $a$ и $b$ определено как произведение
строк матрицы $a$ и столбцов матрицы $b$.
\ePrints{1908.04418,6860-2955,2020.06.01,2204.06320,2022.01.05}
\Items{8428-0408,8525-2526,2207.06506,2024.10.11}%
\ifx\Semafor\ValueOn
В некоммутативной алгебре этой операции умножения
недостаточно для решения некоторых задач.
\ePrints{8428-0408,8525-2526,2207.06506}
\ifx\Semafor\ValueOff
\ShowExample{matrix in right vector space}

\ShowExample{matrix in left vector space}

Из примеров
\RefExample{matrix in right vector space},
\RefExample{matrix in left vector space}
\else
\TwoColText
{
\ShowEq{def left}
\ShowEq{def AVector}%
\ShowEq{\DefCol}
\ShowExample{matrix in vector space}
}
{
\ShowEq{def right}
\ShowEq{def AVector}%
\ShowEq{\DefCol}
\ShowExample{matrix in vector space}
}

Из примеров
\refExample{matrix in vector space}{left},
\refExample{matrix in vector space}{right}
\fi
следует, что
\else
Если произведение в
\ePrints{5284-0163,1801.01628}
\ifx\Semafor\ValueOn
$D$\Hyph алгебре
\else
$\Omega$\Hyph кольце
\fi
некоммутативно,
\fi
мы не можем ограничиться традиционным произведением матриц
и нам нужно определить два вида произведения матриц.
Чтобы различать эти произведения, мы вводим
новые обозначения.
}

\DefText{matrix operations 2}
{
Мы так же определим следующие операции на множестве матриц.
}

\DefExample{matrix in left vector space}
{
Мы представим базис $\Basis e$
левого векторного пространства $V$
\ePrints{2020.06.01,2204.06320,2022.01.05,2024.10.11}
\ifx\Semafor\ValueOff
над $D$\Hyph алгеброй $A$
(смотри определение
\ShowEq{def left}%
\ShowEq{def AVector}%
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS}
и теорему
\refTheorem{basis over division algebra}{left})
\fi
как строку матрицы
\DrawEq[en]{a=(a1.n row)}{left basis}
Мы можем представить координаты вектора
\ShowEq{w=w*e left-cols}v{}
как вектор столбец
\DrawEq[vn]{a=(a1.n col)}{left basis}
Однако мы не можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(v)(e)}
так как это произведение не определено.
\ePrints{2020.06.01,2204.06320,2022.01.05,2024.10.11}
\ifx\Semafor\ValueOff
Линейный гомоморфизм
левого векторного пространства $V$
может быть представлен с помощью матрицы
\ShowEq{v'=vf}
Равенство
\EqRef{v'=vf}
не может быть выражено как традиционное произведение матриц $v$ и $f$.
\fi
}

\AddEq{define basis for example}
{
Мы представим множество векторов
\ShowEq{\RowN() 1n}en{}
базиса $\Basis e$
\SideRu вого векторного пространства $V$
над $D$\Hyph алгеброй $A$
(смотри определение
\ShowRef{\SideWS module over algebra}
и теорему
\refTheorem{basis over division algebra}{left})
в виде
\RowA матрицы
\DrawEq[en]{a=(a1.n \RowN)}{\SideWS basis}
Мы представим координаты
\ShowEq{\ColNS() 1n}vn{}
вектора
\ShowEq{w=w*e left-cols}v{}
в виде \ColA матрицы
\DrawEq[vn]{a=(a1.n \ColNS)}{vn \SideNS-\Cols}
}

\AddEq{vector as matrix product left}
{
Поэтому мы можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(e)(v)}
}

\AddEq{vector as matrix product right}
{
Однако мы не можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(v)(e)}
так как это произведение не определено.
}

\DefLabeledExample{matrix in vector space}{\SideNS}
{
\ShowEq{define basis for example}
\ShowEq{vector as matrix product \SideNS}
}

\DefExample{matrix in right vector space}
{
Мы представим базис $\Basis e$
правого векторного пространства $V$
\ePrints{2020.06.01,2204.06320,2022.01.05,2024.10.11}
\ifx\Semafor\ValueOff
над $D$\Hyph алгеброй $A$
(смотри определение
\ShowEq{def right}%
\ShowEq{def AVector}%
\refDefinition{module over associative algebra}{\SideWS \VectorSetNS}
и теорему
\refTheorem{basis over division algebra}{right})
\fi
как строку матрицы
\DrawEq[en]{a=(a1.n row)}{right basis}
Мы можем представить координаты вектора
\ShowEq{w=w*e right-cols}v{}
как вектор столбец
\DrawEq[vn]{a=(a1.n col)}{right basis}
Поэтому мы можем представить вектор $\Vector v$
как традиционное произведение матриц
\ShowEq{v=(e)(v)}
\ePrints{2020.06.01,2204.06320,2022.01.05,2024.10.11}
\ifx\Semafor\ValueOff
Линейный гомоморфизм
правого векторного пространства $V$
может быть представлен с помощью матрицы
\ShowEq{v'=fv}
Равенство
\EqRef{v'=fv}
выражает традиционное произведение матриц $f$ и $v$.
\fi
}

\DefDefinition{row over column product}
{
Пусть число столбцов матрицы $a$ равно числу строк матрицы $b$.
\AddIndex{\RC произведение}{rc-product}
матриц $a$ и $b$ имеет вид
\ShowEq{rc-product}
\ShowEq{rc-product of matrices}
\ShowEq{entry rc-product of matrices}
\ShowEq{rc-product, matrices}
\RC произведение может быть выражено как произведение строк матрицы $a$
и столбцов матрицы $b$.
}

\DefDefinition{column over row product}
{
Пусть число строк матрицы $a$ равно числу столбцов матрицы $b$.
\AddIndex{\CR произведение}{cr-product}
матриц $a$ и $b$ имеет вид
\ShowEq{cr-product}
\ShowEq{cr-product of matrices}
\ShowEq{entry cr-product of matrices}
\ShowEq{cr-product, matrices}
\CR произведение может быть выражено как произведение столбцов матрицы $a$
и строк матрицы $b$.
}

\DefDefinition{transpose of matrix}
{
Транспонирование $a^T$ матрицы $a$
меняет местами строки и столбцы
\ShowEq{transpose of matrix, 1}
}

\DefDefinition{sum of matrices}
{
Сумма матриц $a$ и $b$ определена равенством
\ShowEq{(a+b)=}
}

\DefDefinition{rc power}
{
Мы определим \AddIndex{\RC степень}{rc power}
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph числа
\else
матрицы
\fi
$a$,
пользуясь рекурсивным правилом
\ShowEq{rc power}
\DrawEq{rc power, 0}1
\DrawEq{rc-power, n}1
}

\DefDefinition{cr power}
{
Мы определим \AddIndex{\CR степень}{cr power}
$\mathcal{A}$\Hyph числа $a$,
пользуясь рекурсивным правилом
\ShowEq{cr power}
\DrawEq{cr power, 0}1
\DrawEq{cr-power, n}1
}

\DefDefinitionNote{Hadamard inverse of matrix}
{
Пусть
\DrawEq[ann]{a=(a11.nm matrix)}{}
матрица $A$\Hyph чисел.
Мы называем матрицу\,\footnotemark
\ShowEq{Hadamard inverse of matrix}
\ShowEq{Hadamard inverse of matrix 2}
\ShowEq{Hadamard inverse of matrix 2 entry}
\AddIndex{обращением Адамара матрицы}{Hadamard inverse of matrix} $a$
(\citeBib{q-alg-9705026}-\href{https://arxiv.org/pdf/math/9705026.pdf\#Page=4}{page 4}).
}{
Запись в равенстве
\EqRef{Hadamard inverse of matrix 2 entry}
означает, что
при обращении Адамара столбцы и строки меняются местами.
\label{footnote: index of inverse element}
Мы можем
формально записать правую часть равенства
\EqRef{Hadamard inverse of matrix 2 entry}
следующим образом
\ShowEq{Hadamard inverse of matrix 3}
}

\DefDefinition{transformation coordinated with equivalence}
{
Пусть на множестве $A_2$ определена эквивалентность $S$.
Преобразование $f$ называется
\AddIndex{согласованным с эквивалентностью}{transformation coordinated with equivalence} $S$,
если из условия
\ShowEq{m1 m2 modS}{}
следует
\ShowEq{fm1 fm2 modS}.
}

\DefTheorem{transformation correlated with equivalence}
{
Пусть на множестве $A_2$ определена эквивалентность $S$.
Пусть на множестве
\ShowEq{End O2}{A_2}{}
определена $\Omega_1$\Hyph алгебра.
Если любое преобразование
\ShowEq{f in End A2},
согласованно с эквивалентностью $S$,
то мы можем определить структуру $\Omega_1$\Hyph алгебры
на множестве
\ShowEq{End A2/S}S.
}

\DefTheorem{decompositions of morphism of representations}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$,
\ShowEq{f:A->*B}g{B_1}{B_2}
представление $\Omega_1$\Hyph алгебры $B_1$.
Пусть
\ShowEq{r12:A->B}tAB
морфизм представлений из $f$ в $g$.
Тогда для отображений $t_1$, $t_2$ существуют разложения,
которые можно описать диаграммой
\ShowEq{decompositions of morphism of representations, diagram}
\StartLabelItem
\begin{enumerate}
\item
Ядро гомоморфизма
\ShowEq{kernel of homomorphism i}
является конгруэнцией на $\Omega_i$\Hyph алгебре $A_i$,
\ShowEq{i=1,2}.
\labelItem{kernel of homomorphism i}
\item
Существует разложение гомоморфизма $t_i$,
\ShowEq{i=1,2},
\ShowEq{morphism of representations of algebra, homomorphism, 1}
\labelItem{exists decomposition of homomorphism}
\item
Отображения
\ShowEq{morphism of representations of algebra, p1=}
\ShowEq{morphism of representations of algebra, p2=}
являются естественными гомоморфизмами.
\labelItem{p12 are natural homomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, q1=}
\ShowEq{morphism of representations of algebra, q2=}
являются изоморфизмами.
\labelItem{q12 are isomorphisms}
\item
Отображения
\ShowEq{morphism of representations of algebra, r1=}
\ShowEq{morphism of representations of algebra, r2=}
являются мономорфизмами.
\labelItem{r12 are monomorphisms}
\item $F$ - представление $\Omega_1$\Hyph алгебры $A_1/s$ в $A_2/s_2$
\item $G$ - представление $\Omega_1$\Hyph алгебры $t_1A_1$ в $t_2A_2$
\item Отображение
\ShowEq{map r12}p{}
является морфизмом представлений $f$ и $F$
\labelItem{(p12) is morphism of representations}
\item Отображение
\ShowEq{map r12}q{}
является изоморфизмом представлений $F$ и $G$
\labelItem{(q12) is isomorphism of representations}
\item Отображение
\ShowEq{map r12}r{}
является морфизмом представлений $G$ и $g$
\labelItem{(r12) is morphism of representations}
\item Существует разложение морфизма представлений
\labelItem{exists decompositions of morphism of representations}
\ShowEq{decompositions of morphism of representations}
\end{enumerate} 
}

\DefDefinition{stable set of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Множество
\ShowEq{B2 subset A2}
называется
\AddIndex{стабильным множеством представления}
{stable set of representation} $f$,
если
\ShowEq{fam in B2}
для любых
\ShowEq{a in A1},
$m\in B_2$.
}

\DefTheorem{subrepresentation of representation}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
представление $\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Пусть множество
\ShowEq{B2 subset A2}
является подалгеброй $\Omega_2$\Hyph алгебры $A_2$
и стабильным множеством представления $f$.
Тогда существует представление
\ShowEq{representation of algebra A in algebra B}
такое, что
\ShowEq{fB2(a)=}
Представление $f_{B_2}$ называется
\AddIndex{подпредставлением}{subrepresentation}
представления $f$.
}

\DefTheoremNote{lattice of subrepresentations}
{
Множество\,\footnotemark
\ShowEq{lattice of subrepresentations}
всех подпредставлений представления $f$ порождает
систему замыканий на $\Omega_2$\Hyph алгебре $A_2$
и, следовательно, является полной структурой.
}{
Это определение
аналогично определению структуры подалгебр
(\citeBib{Cohn: Universal Algebra}, стр. 93, 94).
\ePrints{1908.04418,6860-2955}
\ifx\Semafor\ValueOn%
Вообще говоря, в этой и последующих теоремах 
этой главы необходимо рассмотреть структуру универсальных алгебр
$A_1$ и $A_2$.
Так как основная задача этой главы -
это изучение структуры представления,
я сознательно упростил теоремы, чтобы детали не заслоняли
основные утверждения.
Более подробно эта тема будет раскрыта в главе
\RefChapter{Basis of Diagram of Representations of Universal Algebra},
где теоремы будут сформулированы в общем виде.
\fi
}

\AddEq{remark: closure operator, representation}
{
Обозначим соответствующий оператор замыкания через
\ShowEq{closure operator, representation}
Таким образом,
\ShowEq{subrepresentation generated by set}
является пересечением всех подалгебр
$\Omega_2$\Hyph алгебры $A_2$,
содержащих $X$ и стабильных относительно представления $f$.
}

\DefDefinition{generating set of representation}
{
\ShowEq{show closure operator, representation}
называется
\AddIndex{подпредставлением}{subrepresentation},
порождённым множеством $X$,
а $X$ -
множеством образующих
подпредставления $J[f,X]$.
В частности,
\AddIndex{множеством образующих}{generating set}
представления $f$
будет такое подмножество $X\subset A_2$, что
\ShowEq{generating set of representation}
}

\DefTheoremNote{map of words of representation}
{
\ShowEq{Let A->*AB2 be representations}
Пусть $X$ - множество образующих представления $f$.
Пусть
\ShowEq{f:A->B}R{A_2}{B_2}
приведенный морфизм представления\,\footnotemark
и $X'=R(X)$.
Приведенный морфизм $R$ представления
порождает отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation}
такое, что
\StartLabelItem
\begin{enumerate}
\item Если
\ShowEq{map of words of representation, m in X, 1}
то
\ShowEq{map of words of representation, m in X}
\item Если
\ShowEq{map of words of representation, omega, 1}
то для операции
$\omega\in\Omega_2(n)$ справедливо
\ShowEq{map of words of representation, omega}
\item Если
\ShowEq{map of words of representation, am, 1}
то
\ShowEq{map of words of representation, am}
\end{enumerate}
}{
Я рассмотрел морфизм представления в теореме
\RefTheorem[\RefRepresentation]{map of words of diagram of representations}.
}

\DefTheorem{Representation is single transitive iff}
{
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in A_2$
существует одно и только одно $g\in A_1$ такое, что $a=f(g)(b)$.
}

\DefProof{Representation is single transitive iff}
{
Следствие определений \RefDefinition{free representation of algebra}
и \RefDefinition{transitive representation of algebra}.
}

\DefTheorem{single transitive representation generates algebra}
{
Пусть
\ShowEq{f:A->*B}f{A_1}{A_2}
однотранзитивное представление
$\Omega_1$\Hyph алгебры $A_1$
в $\Omega_2$\Hyph алгебре $A_2$.
Существует структура $\Omega_1$\Hyph алгебры на множестве $A_2$.
}

\AddEq{theorem: automorphism uniquely defined by image of basis}
{
\begin{ShadedTheorem}
\labelTheorem{automorphism uniquely defined by image of basis}
Пусть $\Basis e$ - базис представления $f$.
Пусть
\ShowEq{R1 X->}{\Basis e}
произвольное отображение множества $\Basis e$.
Рассмотрим отображение $\Omega_2$\Hyph слов
\ShowEq{map of words of representation, W}{\Basis e}
удовлетворяющее условиям
\RefItem{map of words of representation, m in X},
\RefItem{map of words of representation, omega},
\RefItem{map of words of representation, am},
и такое, что
\ShowEq{map of words of representation, W in X}e{\Basis e}
Существует единственный эндоморфизм представлнения $f$\,\footnotemark
\ShowEq{R:A2->A2}
определённый правилом
\ShowEq{endomorphism based on map of words of representation}{\Basis e}
\end{ShadedTheorem}
\footnotetext{\,
Это утверждение
похоже на теорему \citeBib{Serge Lang}-1, с. 104.
}
}

\DefDefinition{parity of permutation}
{
Отображение
\ShowEq{sigma->+-}
определённое равенством
\def\permutation{перестановка }
\def\even{чётная}
\def\odd{не\even}
\ShowEq{parity of permutation}
называется
\AddIndex{чётностью перестановки}{parity of permutation}.
}

\DefText{passive representation of vector space 1}
{
\ShowText{coordinates of vector with respect to basis (1,2) \Cols}v3
Тогда
\ShowEq{v=vi ei 123, \SideNS-\Cols}
Пусть пассивное преобразование $g_1$ отображает базис
\ShowEq{Basis e in BVG}1
в базис
\ShowEq{Basis e in BVG}2
\DrawEq[12g1]{e2i=aij e1j \Product-\Cols}{12}
Пусть пассивное преобразование $g_2$ отображает базис
\ShowEq{Basis e in BVG}2
в базис
\ShowEq{Basis e in BVG}3
\DrawEq[23g2]{e2i=aij e1j \Product-\Cols}{23}
}

\DefText{passive representation of vector space 2}
{
Преобразование
\ShowEq{e3=g12 cr e1 \SideNS-\Cols}
является произведением преобразований
\eqRef{e2i=aij e1j \Product-\Cols}{12},
\eqRef{e2i=aij e1j \Product-\Cols}{23}.
Преобразование координат
\DrawEq[v2v1g1{\SideNS}{\Cols}]{v2=v1g-}{1 \SideNS-\Cols}
соответствует пассивному преобразованию $g_1$
и является следствием равенств
\EqRef{v=vi ei 123, \SideNS-\Cols},
\eqRef{e2i=aij e1j \Product-\Cols}{12}
и теоремы
\refTheorem{passive transformation of vector space}{\SideNS-\Cols}.
}

\DefText{passive representation of vector space 3}
{
Аналогично,
\ePrints{1908.04418,6860-2955}%
\ifx\Semafor\ValueOff%
согласно теореме
\refTheorem{passive transformation of vector space}{\SideNS-\Cols},
\fi
преобразование координат
\DrawEq[v3v2g2{\SideNS}{\Cols}]{v2=v1g-}{23 \SideNS-\Cols}
соответствует пассивному преобразованию $g_2$
и является следствием равенств
\EqRef{v=vi ei 123, \SideNS-\Cols},
\eqRef{e2i=aij e1j \Product-\Cols}{23}.
Произведение преобразований координат
\eqRef{v2=v1g-}{1 left-cols},
\eqRef{v2=v1g-}{23 left-cols}
имеет вид
\ShowEq{v3=v1 cr g1- cr g2- \SideNS-\Cols}
и является координатным преобразованием,
соответствующим пассивному преобразованию
\EqRef{e3=g12 cr e1 \SideNS-\Cols}.
Равенство
\ShowEq{v3=v1 cr g21- \SideNS-\Cols}
является следствием равенств
\EqRef{cr-inverse matrix of product},
\EqRef{v3=v1 cr g1- cr g2- \SideNS-\Cols}.
}

\DefText{passive representation of left vector space}
{
\ShowText{passive representation of vector space 1}
\ShowText{passive representation of vector space 2}
\ShowText{passive representation of vector space 3}
}

\DefDefinition{Left side contravariant representation}
{
Левостороннее представление
\ShowEq{f:A->*B}f{A_1}{A_2}
называется
\AddIndex{контравариантным}{contravariant representation},
если равенство
\ShowEq{Left side contravariant representation}
верно.
}

\DefDefinition{Left side covariant representation}
{
Левостороннее представление
\ShowEq{f:A->*B}f{A_1}{A_2}
называется
\AddIndex{ковариантным}{covariant representation},
если равенство
\ShowEq{Left side covariant representation}
верно.
}

\DefDefinition{cr-inverse matrix}
{
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph число
\else
Матрица
\fi
\ShowEq{cr-inverse element}
- это \AddIndex{\CR обратный элемент}{cr-inverse element}
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
$\mathcal{A}$\Hyph числа
\else
матрицы
\fi
$a$, если
\DrawEq{cr-inverse matrix}1
\ePrints{2020.06.01}
\ifx\Semafor\ValueOn
Матрица $a$ называется
\CR невырожденной,
если существует \CR обратная матрица.
\fi
}

\DefDefinition{delta=Matrix}
{
Матрица
\ShowEq{delta=Matrix}
является единицей для обоих произведений.
}

\DefRemark{pronunciation of product}
{
Мы будем пользоваться символом \RC\,\, или \CR\,\,  в имени свойств
каждого произведения и в обозначениях.
Мы можем читать символ
$\RCstar$ как
$rc$\hyph произведение (произведение строки на столбец)
и символ $\CRstar$ как
$cr$\hyph произведение (произведение столбца на строку).
Для совместимости
обозначений с существующими мы будем иметь
в виду \RC произведение, когда
нет явных обозначений.
\ePrints{2020.06.01}
\ifx\Semafor\ValueOff
Это правило мы распространим на последующую терминологию.
Символ произведения
сформирован из двух символов операции произведения, которые записываются на
месте индекса суммирования.
Например, если произведение $A$\Hyph чисел имеет вид
$a\circ b$,
то \RC произведение
матриц $a$ и $b$ имеет вид
$a\RCcirc b$
и \CR произведение
матриц $a$ и $b$ имеет вид
$a\CRcirc b$.
\fi
}

\DefTheorem{quasideterminant rc cr, matrix 2x2}
{
\ShowEq{quasideterminant matrix 2x2 def}
Рассмотрим матрицу
\ShowEq{inverse matrix 2x2, 0}
Тогда
\ShowEq{quasideterminant rc, matrix 2x2}
\ShowEq{quasideterminant cr, matrix 2x2}
\ShowEq{rc inverse matrix 2x2}
}

\DefDefinition{RC-quasideterminant}
{
\AddIndex{$(\aUD{}ji)$\hyph \RC квазидетерминант}{j i RC-quasideterminant}
\nTimes матрицы $a$
- это формальное выражение
\ShowEq{j i RC-quasideterminant definition}
\ShowEq{j i RC-quasideterminant =}
Мы можем рассматривать $\aUD (ji)$\hyph \RC квазидетерминант
как элемент матрицы
\ShowEq{RC-quasideterminant definition}
\ShowEq{RC-quasideterminant definition=}
которую мы будем называть
\AddIndex{\RC квазидетерминантом}{RC-quasideterminant}.
}

\DefDefinition{biring}
{
\AddIndex{Бикольцо}{biring} $\mathcal A$ - это множество,
на котором мы определили унарную операцию, называемую транспозицией,
и три бинарных операции,
называемые \RC произведение, \CR произведение и сумма, такие что
\begin{itemize}
\item \RC произведение и сумма определяют структуру кольца на $\mathcal A$
\item \CR произведение и сумма определяют структуру кольца на $\mathcal A$
\item оба произведения имеют общую единицу $\delta$
\item произведения удовлетворяют равенству
\DrawEq{rc transpose}{}
\item транспозиция единицы есть единица
\DrawEq{transpose of identity}E
\item двойная транспозиция есть исходный элемент
\ShowEq{double transpose}
\end{itemize}
}

\DefTheorem{double transpose is original matrix}
{
Двойная транспозиция есть исходная матрица
\ShowEq{double transpose}
}

\DefProof{double transpose is original matrix}
{
Теорема является следствием определения
\RefDefinition{transpose of matrix}.
}

\DefEq
{
\begin{ShadedTheorem}[принцип двойственности для бикольца]
\AddIndex{}{duality principle for biring}
\labelTheorem{duality principle for biring}
Пусть $\mathcal{A}$ - истинное утверждение о
бикольце $A$.
Если мы заменим одновременно
\begin{itemize}
\item $a\in A$ и $a^T$
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{ShadedTheorem}
}
{theorem: duality principle for biring}
%\DefEq

\DefEq
{
\begin{ShadedTheorem}[принцип двойственности для бикольца матриц]
\AddIndex{}{duality principle for biring of matrices}
\labelTheorem{duality principle for biring of matrices}
Пусть $A$ является бикольцом матриц.
Пусть $\mathcal{A}$ - истинное утверждение о матрицах.
Если мы заменим одновременно
\begin{itemize}
\item строки и столбцы всех матриц
\item \RC произведение и \CR произведение
\end{itemize}
то мы снова получим истинное утверждение.
\end{ShadedTheorem}
\begin{proof}
Непосредственное следствие
теоремы \RefTheorem{duality principle for biring}.
\end{proof}
}
{theorem: duality principle for biring of matrices}
%\DefEq

\DefEq
{
\begin{remark}
\labelRemark{reducible biring}
Если произведение в $\Omega$\Hyph кольце коммутативно, то
\ShowEq{reducibility of products}
\AddIndex{Приводимое бикольцо}{reducible biring}
- это бикольцо, в котором выполняется
\AddIndex{условие приводимости произведений}
{condition of reducibility of products}
\EqRef{reducibility of products}.
Поэтому в приводимом бикольце достаточно рассматривать только
\RC произведение. Однако в тех случаях, когда
порядок сомножителей существенен,
мы будем пользоваться также \CR произведением.
\qed
\end{remark}
}
{remark: reducible biring}
%\DefEq

\DefEq
{
Так как левостороннее представление и правостороннее представление
опирается на гомоморфизм $\Omega$\Hyph группы,
то верно следующее утверждение.

\begin{ShadedTheorem}[принцип двойственности для представления мультипликативной $\Omega$\Hyph группы]
\labelTheorem{duality principle, algebra representation}
Любое утверждение, справедливое для
левостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$,
будет справедливо для правостороннего представления мультипликативной $\Omega$\Hyph группы $A_1$, если
мы будем пользоваться правосторонним произведением на $A_1$\Hyph число $a_1$ вместо
левостороннего произведения на $A_1$\Hyph число $a_1$.
\qed
\end{ShadedTheorem}
}
{theorem: duality principle, algebra representation}
%\DefEq

\DefTheorem{left right shift}
{
Произведение
\ShowEq{(ab)->ab}
в мультипликативной $\Omega$\Hyph группе $A$
определяет два различных представления.
\begin{itemize}
\EqParm{associative shift}{def left}
\EqParm{associative shift}{def right}
\end{itemize}
}

\AddEq{non associative shift}
{
\item
\SideRuC вый сдвиг
\ShowEq{\SideWS shift}
является представлением
$\Omega$\Hyph алгебры $A$
в $\Omega$\Hyph алгебре $A$.
}

\AddEq{associative shift}
{
\item
\AddIndex{\SideRuC вый сдвиг}{\SideWS shift}
\ShowEq{\SideWS shift =}
\ShowEq{\SideWS shift}
является \SideRu восторонним представлением
мультипликативной $\Omega$\Hyph группы $A$
в $\Omega$\Hyph алгебре $A$
\ShowEq{\SideWS shift, product}
}

\DefDefinition{representation of algebra}
{
Пусть множество $A_2$ является $\Omega_2$\Hyph алгеброй.
Пусть
на множестве преобразований
\ShowEq{End O2}{A_2}{}
определена структура $\Omega_1$\Hyph алгебры.
Гомоморфизм
\ShowEq{representation of algebra}
$\Omega_1$\Hyph алгебры $A_1$ в
$\Omega_1$\Hyph алгебру
\ShowEq{End O2}{A_2}{}
называется
\AddIndex{представлением $\Omega_1$\Hyph алгебры}
{representation of algebra}
$A_1$ или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$.
}

\DefEq
{
Если мультипликативная $\Omega$\Hyph группа $A_1$ - абелевая,
то нет разницы между левосторонним и правосторонним представлениями.

\begin{ShadedDefinition}
\labelDefinition{representation of Abelian group} 
Пусть $A_1$ - абелевая мультипликативная $\Omega$\Hyph группа.
Мы будем называть гомоморфизм мультипликативной $\Omega$\Hyph группы
\DrawEq{representation of group, map}{Abelian group}
\AddIndex{представлением}{representation of algebra}
мультипликативной $\Omega$\Hyph группы $A_1$
или
\AddIndex{$A_1$\Hyph представлением}{A representation of algebra}
в $\Omega_2$\Hyph алгебре $A_2$, если отображение $f$ удовлетворяет условиям
\DrawEq{left-side representation of group}{Abelian}
\end{ShadedDefinition}

Обычно мы отождествляем представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и левостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
Однако, если это необходимо нам,
мы можем отождествить представление абелевой мультипликативной $\Omega$\Hyph группы $A_1$
и правостороннее представление мультипликативной $\Omega$\Hyph группы $A_1$.
}
{definition: representation of Abelian group}
%\DefEq

\DefTheorem{two representations of group}
{
Пусть $A_1$ - мультипликативная $\Omega$\Hyph группа.
Пусть левостороннее $A_1$\Hyph представление $f$
на $\Omega_2$\Hyph алгебре $A_2$ однотранзитивно.
Тогда мы можем однозначно определить однотранзитивное правостороннее $A_1$\Hyph представление $h$
на $\Omega_2$\Hyph алгебре $A_2$
такое, что диаграмма
%\ePrints{8525-2526}
%\ifx\Semafor\ValueOn
%\newpage
%\fi
\ShowEq{two representations of group}
коммутативна для любых $a_1$, $b_1\in A_1$.
}

\AddEq{definition: twin representations}
{
Мы будем называть представления $f$ и $h$
\AddIndex{парными представлениями}{twin representations}
мультипликативной $\Omega$\Hyph группы $A_1$.
}

\DefRemark{one representation of group}
{
Очевидно, что преобразования $L(a)$ и $R(a)$
отличаются, если мультипликативная $\Omega$\Hyph группа $A_1$ неабелева.
Тем не менее, они являются отображениями на.
Теорема \RefTheorem{two representations of group} утверждает, что, если оба
представления правого и левого сдвига существуют на множестве $A_2$,
то мы можем определить два перестановочных представления на множестве $A_2$.
Только правый или левый сдвиг не может представлять оба типа представления.
Чтобы понять почему это так, мы можем изменить диаграмму
\EqRef{Diagram: two representations of group}
и предположить
\ShowEq{haa=Laa}
вместо
\ShowEq{haa=aRa}
и проанализировать, какое выражение $h(a_1)$ имеет в
точке $c_2$. Диаграмма
\ShowEq{Diagram: two representations of group 1}
эквивалентна диаграмме
\ShowEq{Diagram: two representations of group 2}
и мы имеем
\ShowEq{d2=...c2 1}
Следовательно
\ShowEq{d2=...c2}
Мы видим, что представление $h$
зависит от его аргумента.
}

\DefTheorem{single transitive representation of group}
{
Если существует однотранзитивное представление
\ShowEq{f:A->*B}f{A_1}{A_2}
мультипликативной $\Omega$\Hyph группы $A_1$
в $\Omega_2$\Hyph алгебре $A_2$,
то мы можем однозначно определить координаты на $A_2$, пользуясь $A_1$\Hyph числами.

Если $f$ - левостороннее однотранзитивное однотранзитивное представление,
то $f(a)$ эквивалентно левому сдвигу $L(a)$ на группе $A_1$.
Если $f$ - правостороннее однотранзитивное представление, то $f(a)$ эквивалентно
правому сдвигу $R(a)$ на группе $A_1$.
}

\DefDefinition{algebra of sets}
{
Непустая система множеств $\mathcal R$ называется
\AddIndex{кольцом множеств}{ring of sets},\,\footnote{
Смотри так же определение
\citeBib{Kolmogorov Fomin}\Hyph 1, страница 41.}
если условие
\ShowEq{A, B in R}
влечёт
\ShowEq{A, B in R 1}
Множество
\ShowEq{E in R}
называется
\AddIndex{единицей кольца множеств}{unit of ring of sets},
если
\ShowEq{A cap E=A}
Кольцо множеств с единицей называется
\AddIndex{алгеброй множеств}{algebra of sets}.
}

\DefEq
{
\begin{remark}
\labelRemark{A cup/minus B}
Для любых
\ShowEq{A cup/minus B}
Следовательно, если
\ShowEq{A, B in R},
то
\ShowEq{A cup/minus B R}
\qed
\end{remark}
}
{remark: A cup/minus B}
%\DefEq

\DefDefinition{sigma algebra of sets}
{
Кольцо множеств $\mathcal R$ называется
\AddIndex{\(\sigma\)\Hyph кольцом множеств}{sigma ring of sets},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, страница 45, определение 3.}
если условие
\ShowEq{Ai in R}
влечёт
\ShowEq{Ai in R 1}
\(\sigma\)\Hyph Кольцо множеств с единицей называется
\AddIndex{\(\sigma\)\Hyph алгеброй множеств}{sigma algebra of sets}.
}

\DefDefinition{Borel algebra}
{
Минимальная \(\sigma\)\Hyph алгебра
\ShowEq{Borel algebra}
над совокупностью всех открытых шаров нормированной $\Omega$\Hyph группы $A$,
называется
\AddIndex{алгеброй Бореля}{Borel algebra}.\,\footnote{
Смотри определение в
\citeBib{Kolmogorov Fomin}, с. 46.
Согласно замечанию
\ref{remark: A cup/minus B},
алгебра Бореля может быть также порождена множеством
замкнутых шаров.
}
Множество,
принадлежащее алгебре Бореля,
называется
\AddIndex{борелевским множеством}{Borel set}
или
\AddIndex{$B$\Hyph множеством}{B set}.
}

\DefDefinition{C_X C_Y measurable}
{
Пусть $\mathcal C_X$ -
\(\sigma\)\Hyph алгебра множеств множества $X$.
Пусть $\mathcal C_Y$ -
\(\sigma\)\Hyph алгебра множеств множества $Y$.
Отображение
\ShowEq{f:A->B}fXY
называется
$(\mathcal C_X,\mathcal C_Y)$\Hyph измеримым,\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282.}
если для всякого множества
\ShowEq{CX CY measurable map}
}

\DefEq
{
\begin{example}
\labelExample{measurable map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{algebra of sets measurable with respect to measure}
- \(\sigma\)\Hyph алгебра измеримых относительно меры $\mu$ множеств.
Пусть
$\mathcal B(A)$
- алгебра Бореля
нормированной $\Omega$\Hyph группы $A$.
Отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{$\mu$\Hyph измеримым}{mu measurable map},\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282, определение 1.
Если мера $\mu$ на множестве $X$ определена в контексте,
мы также будем называть отображение
\ShowEq{f:A->B}fXA
\AddIndex{измеримым}{measurable map}.
}
если для всякого множества
\ShowEq{measurable map}
\qed
\end{example}
}
{example: measurable map}
%\DefEq

\DefDefinition{simple map}
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Отображение
\ShowEq{f:A->B}fXA
в нормированную $\Omega$\Hyph группу $A$ называется
\AddIndex{простым отображением}{simple map},
если это отображение $\mu$\Hyph измеримо и
принимает не более, чем счётное множество значений.
}

\DefTheorem{measurable simple map}
{
Пусть отображение
\ShowEq{f:A->B}fXA
принимает не более, чем счётное множество значений
\ShowEq{range f}
.
Отображение $f$ $\mu$\Hyph измеримо тогда и только тогда, когда
все множества
\DrawEq{Fn=}{}
$\mu$\Hyph измеримы.\,\footnote{
Смотри аналогичную теорему в
\citeBib{Kolmogorov Fomin}, страница 292, теорема 1.}
}

\DefDefinition{measure}
{
Пусть \(\mathcal C_m\) - полукольцо множеств.\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 265.}
Отображение
\ShowEq{f:A->B}f{\mathcal C_m}R
называется
\AddIndex{мерой}{measure},
если
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{m(A)>0}
\item
Отображение \(m\) аддитивно.
Если множество
\ShowEq{A in Cm}
имеет конечное разлоение
\DrawEq{A=+Ai Cm}{}
где
\ShowEq{Ai*Aj=0},
то
\ShowEq{m A=+m Ai}
\end{enumerate}
}

\DefDefinition{complete measure}
{
Мера \(\mu\) называется
\AddIndex{полной}{complete measure},
если из условий
\ShowEq{B in A, mu(A)=0}
следует,
что множество \(B\) измеримо.
}

\DefDefinition{sigma-additive measure}
{
Пусть $\mathcal C_{\mu}$ -
\(\sigma\)\Hyph алгебра множеств множества $F$.\,\footnote{
Смотри аналогичные определения в
\citeBib{Kolmogorov Fomin}, определение 1 на странице 265
и определение 3 на странице 268.}
Отображение
%\ShowEq{mu:CF->A}
%в нормированную $\Omega$\Hyph группу $A$ называется
\ShowEq{f:A->B}{\mu}{\mathcal C_{\mu}}R
в поле действительных чисел $R$ называется
\AddIndex{\(\sigma\)\Hyph аддитивной мерой}{sigma-additive measure},
если для любого множества
\ShowEq{X in Cmu}
выполнены следующие условия.
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{muX>0}
\item
Пусть
\DrawEq{X=+Xi}{}
конечное или счётное объединение множеств
\ShowEq{Xn in Cmu}
Тогда
\DrawEqParm{mu(X=+Xi)}X{}
где ряд в правой части сходится абсолютно.
\labelItem{mu(X=+Xi)}
\end{enumerate}
}

\DefEq
{
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть определено эффективное представление поля действительных чисел \(R\)
в полной абелевой \(\Omega\)\Hyph группе \(A\).\,\footnote{
Другими словами,
\(\Omega\)\Hyph группа \(A\) является
\(R\)\Hyph векторным пространством.}
}
{remark - measure - effective representation of real field}
%\DefEq

\DefDefinition{series converges normally}
{
Пусть \(a_i\) - последовательность \(A\)\Hyph чисел.
Если
\ShowEq{sum |ai|<infty}
то мы будем говорить, что {\bf ряд}
\ShowEq{sum ai}
\AddIndex{сходится нормально}
{series converges normally}.\,\footnote{Смотри также
определение нормальной сходимости ряда
на странице \citeBib{Cartan differential form}-12.}
}

\DefDefinition{Integral of Map over Set of Finite Measure}
{
\(\mu\)\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),\,\footnote{
Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 3, страницы 294, 295.
}
если существует последовательность
простых  отображений
\ShowEq{f:A->B}{f_n}XA
сходящаяся равномерно к \(f\).
Если отображение \(f\) интегрируемо,
то предел
\ShowEq{integral of map}
\ShowEq{integral of measurable map}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\).
}

\DefDefinition{integrable map}
{
Для простого отображения
\ShowEq{f:A->B}fXA
рассмотрим ряд
\DrawEq{sum mu(F) f}{integral}
где
\begin{itemize}
\item
Множество
\ShowEq{f1...}
является областью определения отображения \(f\)
\item
Если \(n\ne m\), то
\ShowEq{fn ne fm}
\item
\DrawEq{Fn=}{-}
\end{itemize}
Простое отображение
\ShowEq{f:A->B}fXA
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),
если ряд
\eqRef{sum mu(F) f}{integral}
сходится нормально.\,\footnote{
Смотри аналогичное определение в
\citeBib{Kolmogorov Fomin}, определение 2, с. 293.}
Если отображение \(f\) интегрируемо,
то сумма ряда
\eqRef{sum mu(F) f}{integral}
называется
\AddIndex{интегралом Лебега}{Lebesgue integral}
отображения \(f\) по множеству \(X\)
\ShowEq{integral of map}
\ShowEq{integral of simple map}
}

\DefTheorem{|int f|<int|f|}
{
Пусть
\ShowEq{f:A->B}fXA
измеримое отображение.
Интеграл
\ShowEq{int f X}
существует
тогда и только тогда, когда
интеграл
\ShowEq{int |f| X}
существует.
Тогда
\DrawEq{|int f|<int|f|}{measurable}
}

\DefTheorem{int |f|<M mu}
{
Пусть $\mu$\Hyph измеримое отображение
\ShowEq{f:A->B}fXA
удовлетворяет условию
\DrawEq{|f(x)|<M}{}
Если мера множества \(X\) конечна, то
\DrawEq{int |f|<M mu}{measurable}
}

\DefTheorem{int f+g X}
{
Пусть
\ShowEq{f:A->B}fXA
\ShowEq{f:A->B}gXA
$\mu$\Hyph измеримые отображения
с компактным множеством значений.
Если существуют интегралы
\ShowEq{int f X}
\ShowEq{int g X}
то существует интеграл
\ShowEq{int f+g X}
и
\DrawEq{int f+g X =}{measurable}
}


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {прямая сумма}%
   {direct sum}%
   {0}{0}%
\Symb%
   {единичный интервал}%
   {unit interval}%
   {0}{0}%

\SetIndexSpace%A%0
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
   {A}{0}%
\Symb%
   {активное представление в многообразии базисов}%
   {active representation in basis manifold}%
   {A}{0}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
   {A}{0}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
   {A}{0}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
   {A}{0}%
\Symb%
   {аффинное пространство}%
   {An}%
   {A}{0}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
   {A}{0}%
\Symb%
   {категория левосторонних представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of left-side representations of Omega1 algebra}%
   {A}{0}%
\Symb%
   {категория представлений}%
   {category of representations}%
   {A}{0}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
   {A}{0}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
   {A}{0}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
   {A}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
   {A}{0}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
   {A}{0}%
\Symb%
   {координаты ассоциатора}%
   {coordinates of associator}%
   {A}{0}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
   {A}{0}%
\Symb%
   {\crd вектор}%
   {crd vector}%
   {A}{0}%
\Symb%
   {\CR обратная матрица}%
   {cr-inverse matrix}%
   {A}{0}%
\Symb%
   {\CR произведение}%
   {cr-product}%
   {A}{0}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
   {A}{0}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
   {A}{0}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
   {A}{0}%
\Symb%
   {\drc вектор}%
   {drc vector}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
   {A}{0}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
   {A}{0}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
   {A}{0}%
\Symb%
   {изоморфны}%
   {isomorphic}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {левая дробь}%
   {left fraction}%
   {A}{0}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
   {A}{0}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
   {A}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {A}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
   {A}{0}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
   {A}{0}%
\Symb%
   {минорная матрица}%
   {minor matrix}%
   {A}{0}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
   {A}{0}%
\Symb%
   {$\Omega$\Hyph алгебра}%
   {Omega-algebra}%
   {A}{0}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
   {A}{0}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear map}%
   {A}{0}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
   {A}{0}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
   {A}{0}%
\Symb%
   {главный идеал}%
   {principal ideal}%
   {A}{0}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
   {A}{0}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
   {A}{0}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
   {A}{0}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
   {A}{0}%
\Symb%
   {\RC обратная матрица}%
   {rc-inverse matrix}%
   {A}{0}%
\Symb%
   {\RC произведение}%
   {rc-product}%
   {A}{0}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
   {A}{0}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
   {A}{0}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
   {A}{0}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
   {A}{0}%
\Symb%
   {множество аддитивных отображений}%
   {set additive maps}%
   {A}{0}%
\Symb%
   {множество однородных многочленов}%
   {set of homogeneous polynomials}%
   {A}{0}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
   {A}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {A}{0}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
   {A}{0}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
   {A}{0}%
\Symb%
   {симплекс}%
   {simplex}%
   {A}{0}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
   {A}{0}%
\Symb%
   {пространство орбит левостороннего представления}%
   {space of orbits of left side representation}%
   {A}{0}%
\Symb%
   {пространство орбит представления}%
   {space of orbits of representation}%
   {A}{0}%
\Symb%
   {пространство орбит эффективного правостороннего представления}%
   {space of orbits of right-side representation}%
   {A}{0}%
\Symb%
   {квадратный корень}%
   {square root}%
   {A}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {A}{0}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
   {A}{0}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
   {A}{0}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
   {A}{0}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
   {A}{0}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
   {B}{0}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
   {B}{0}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
   {B}{0}%
\Symb%
   {каноническое частное от деления}%
   {canonical remainder of the division}%
   {B}{0}%
\Symb%
   {декартова степень}%
   {Cartesian power}%
   {B}{0}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
   {B}{0}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
   {B}{0}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
   {B}{0}%
\Symb%
   {замыкание множества}%
   {closure of set}%
   {B}{0}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {B}{0}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
   {B}{0}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
   {B}{0}%
\Symb%
   {структура подпредставлений}%
   {lattice of subrepresentations}%
   {B}{0}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
   {B}{0}%
\Symb%
   {открытый шар}%
   {open ball}%
   {B}{0}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {B}{0}%
\Symb%
   {правая дробь}%
   {right fraction}%
   {B}{0}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
   {B}{0}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
   {C}{0}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
   {C}{0}%
\Symb%
   {класс непрерывности}%
   {class Cn}%
   {C}{0}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
   {C}{0}%
\Symb%
   {косинус}%
   {cosine}%
   {C}{0}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of maps}%
   {C}{0}%
\Symb%
   {гиперболический косинус}%
   {hyperbolic cosine}%
   {C}{0}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
   {C}{0}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
   {C}{0}%
\Symb%
   {структурные константы}%
   {structural constants}%
   {C}{0}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
   {D}{0}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
   {D}{0}%
\Symb%
   {компонента производной отображения $f(x)$}%
   {component of derivative}%
   {D}{0}%
\Symb%
   {компонента производной второго порядка отображения $f(x)$}%
   {component of derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
   {D}{0}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
   {D}{0}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
   {D}{0}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
   {D}{0}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
   {D}{0}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
   {D}{0}%
\Symb%
   {координатное векторное расслоение}%
   {coordinate vector bundle}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map}%
   {D}{0}%
\Symb%
   {производная отображения $f$}%
   {derivative of map inline}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n}%
   {D}{0}%
\Symb%
   {производная порядка $n$}%
   {derivative of Order n inline}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная второго порядка}%
   {derivative of Second Order inline}%
   {D}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
   {D}{0}%
\Symb%
   {дифференциал независимой переменной}%
   {differential of independent variable}%
   {D}{0}%
\Symb%
   {дифференциал отображения $f$}%
   {differential of map}%
   {D}{0}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
   {D}{0}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
   {D}{0}%
\Symb%
   {внешний дифференциал}%
   {exterior differential}%
   {D}{0}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
   {D}{0}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
   {D}{0}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
   {D}{0}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
   {D}{0}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
   {D}{0}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
   {D}{0}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
   {D}{0}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
   {D}{0}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
   {D}{0}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
   {D}{0}%
\Symb%
   {матрица Якоби отображения}%
   {Jacobi matrix of map}%
   {D}{0}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
   {D}{0}%
\Symb%
   {производная Картана}%
   {overbrace D}%
   {D}{0}%
\Symb%
   {производная}%
   {overline D}%
   {D}{0}%
\Symb%
   {частная производная}%
   {partial derivative}%
   {D}{0}%
\Symb%
   {частная производная второго порядка}%
   {partial derivative of second order}%
   {D}{0}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
   {D}{0}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
   {D}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {D}{0}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
   {D}{0}%
\Symb%
   {стандартная компонента производной}%
   {standard component of derivative}%
   {D}{0}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
   {D}{0}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%
   {D}{0}%

\SetIndexSpace%E%0
\Symb%
   {аффинный базис}%
   {Affine Basis}%
   {E}{0}%
\Symb%
   {базис}%
   {Basis}%
   {E}{0}%
\Symb%
   {базис модуля}%
   {basis for module}%
   {E}{0}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
   {E}{0}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
   {E}{0}%
\Symb%
   {многообразие базисов}%
   {basis manifold}%
   {E}{0}%
\Symb%
   {базис векторного пространства}%
   {basis of vector space}%
   {E}{0}%
\Symb%
   {базис \crd векторного пространства}%
   {basis, crd vector space}%
   {E}{0}%
\Symb%
   {базис \dcr векторного пространства}%
   {basis, dcr vector space}%
   {E}{0}%
\Symb%
   {базис \drc векторного пространства}%
   {basis, drc vector space}%
   {E}{0}%
\Symb%
   {базис \rcd векторного пространства}%
   {basis, rcd vector space}%
   {E}{0}%
\Symb%
   {базис в векторного расслоения}%
   {basis, vector bundle}%
   {E}{0}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
   {E}{0}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
   {E}{0}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
   {E}{0}%
\Symb%
   {\CR экспонента}%
   {CR exponent}%
   {E}{0}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
   {E}{0}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
   {E}{0}%
\Symb%
   {экспонента}%
   {exponent}%
   {E}{0}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
   {E}{0}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
   {E}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
   {E}{0}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
   {E}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {E}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
   {E}{0}%
\Symb%
   {образ базиса $\Basis e$ при пассивном преобразовании $S$}%
   {passive transformation of basis}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
   {E}{0}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
   {E}{0}%
\Symb%
   {квазиэкспонента}%
   {quasiexponent}%
   {E}{0}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
   {E}{0}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
   {E}{0}%
\Symb%
   {\RC экспонента}%
   {RC exponent}%
   {E}{0}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
   {E}{0}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
   {E}{0}%
\Symb%
   {множество \CR собственных значений}%
   {set of cr-eigenvalues}%
   {E}{0}%
\Symb%
   {множество эндоморфизмов}%
   {set of endomorphisms}%
   {E}{0}%
\Symb%
   {множество \RC собственных значений}%
   {set of rc-eigenvalues}%
   {E}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {множество преобразований универсальной алгебры}%
   {set of transformations}%
   {E}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
   {E}{0}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
   {E}{0}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
   {E}{0}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
   {E}{0}%
\Symb%
   {вектор базиса}%
   {vector of basis}%
   {E}{0}%

\SetIndexSpace%F%0
\Symb%
   {альтернация полилинейного отображения}%
   {alternation of polylinear map}%
   {F}{0}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
   {F}{0}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
   {F}{0}%
\Symb%
   {преобразование сопряжения}%
   {conjugation transformation}%
   {F}{0}%
\Symb%
   {внешнее произведение}%
   {exterior product}%
   {F}{0}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
   {F}{0}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
   {F}{0}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
   {F}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
   {F}{0}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
   {F}{0}%
\Symb%
   {норма функционала}%
   {norm of functional}%
   {F}{0}%
\Symb%
   {норма отображения}%
   {norm of map}%
   {F}{0}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
   {F}{0}%
\Symb%
   {норма представления}%
   {norm of representation}%
   {F}{0}%
\Symb%
   {орбита представления группы}%
   {orbit of representation}%
   {F}{0}%
\Symb%
   {ортонормированный базис}%
   {Orthonormal Basis, division ring}%
   {F}{0}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
   {F}{0}%
\Symb%
   {система отсчёта}%
   {reference frame}%
   {F}{0}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
   {F}{0}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
   {F}{0}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
   {F}{0}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
   {F}{0}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
   {F}{0}%
\Symb%
   {сумма отображений}%
   {sum of maps}%
   {F}{0}%
\Symb%
   {симметрирование полилинейного отображения}%
   {symmetrization of polylinear map}%
   {F}{0}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
   {G}{0}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, 1 n}%
   {G}{0}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
   {G}{0}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
   {G}{0}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
   {G}{0}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
   {G}{0}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
   {G}{0}%
\Symb%
   {неопределённый интеграл}%
   {indefinite integral}%
   {G}{0}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {алгебра Ли группы Ли}%
   {Lie algebra of Lie group}%
   {G}{0}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
   {G}{0}%
\Symb%
   {малая группа}%
   {little group}%
   {G}{0}%
\Symb%
   {орбита эффективного	\Ts представления группы}%
   {orbit of effective starT representation of fibered group}%
   {G}{0}%
\Symb%
   {орбита эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar representation of fibered group}%
   {G}{0}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
   {G}{0}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
   {G}{0}%
\Symb%
   {группа стабилизации}%
   {stability group}%
   {G}{0}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
   {H}{0}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
   {H}{0}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
   {H}{0}%
\Symb%
   {алгебра кватернионов}%
   {quaternion algebra}%
   {H}{0}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
   {H}{0}%
\Symb%
   {множество гомоморфизмов}%
   {set of homomorphisms}%
   {H}{0}%

\SetIndexSpace%I%0
\Symb%
   {образ отображения}%
   {image of map}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
   {I}{0}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
   {I}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {I}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {I}{0}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
   {I}{0}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
   {I}{0}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%
   {I}{0}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
   {J}{0}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
   {J}{0}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
   {J}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {J}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {J}{0}%
\Symb%
   {подпредставление, порождённое множеством образующих $X$}%
   {subrepresentation generated by set}%
   {J}{0}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
   {J}{0}%

\SetIndexSpace%K%0
\Symb%
   {ядро гомоморфизма}%
   {kernel of homomorphism}%
   {K}{0}%
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%
   {K}{0}%
\Symb%
   {ядро отображения}%
   {kernel of map}%
   {K}{0}%
\Symb%
   {отображение сопряжения}%
   {map of conjugation}%
   {K}{0}%
\Symb%
   {матрица Якоби отображения сопряжения}%
   {maps of conjugation, Jacobian matrix}%
   {K}{0}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
   {L}{0}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
   {L}{0}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
   {L}{0}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
   {L}{0}%
\Symb%
   {левый сдвиг}%
   {left shift}%
   {L}{0}%
\Symb%
   {левое векторное пространство алгебры $A$}%
   {left vector space of algebra A}%
   {L}{0}%
\Symb%
   {левое векторное пространство отображений}%
   {left vector space of maps B->A}%
   {L}{0}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
   {L}{0}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
   {L}{0}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
   {L}{0}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
   {L}{0}%
\Symb%
   {линейная комбинация}%
   {linear combination}%
   {L}{0}%
\Symb%
   {модуль косо симметричных полилинейных отображений}%
   {module of skew symmetric polylinear maps}%
   {L}{0}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
   {L}{0}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
   {L}{0}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
   {L}{0}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
   {L}{0}%
\Symb%
   {множество линейных отображений}%
   {set linear maps}%
   {L}{0}%
\Symb%
   {множество обратных матриц}%
   {set of inverse matrices}%
   {L}{0}%
\Symb%
   {множество левосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of left-side nonsingular transformations}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
   {L}{0}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
   {L}{0}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
   {L}{0}%

\SetIndexSpace%M%0
\Symb%
   {множество левосторонних преобразований универсальной алгебры $M$}%
   {set of left-side transformations}%
   {M}{0}%
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
   {M}{0}%
\Symb%
   {множество правосторонних преобразований универсальной алгебры $M$}%
   {set of right-side transformations}%
   {M}{0}%
\Symb%
   {пространство орбит \Ts{G}представления}%
   {space of orbits of G* representation}%
   {M}{0}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
   {N}{0}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
   {N}{0}%

\SetIndexSpace%O%0
\Symb%
   {координаты геометрического объекта}%
   {coordinates of geometric object}%
   {O}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {O}{0}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
   {O}{0}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
   {O}{0}%
\Symb%
   {тензорное произведение}%
   {tensor product}%
   {O}{0}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
   {P}{0}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
   {P}{0}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
   {P}{0}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
   {P}{0}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {пассивное представление группы $GA(f)$ в многообразии базисов $\mathcal B[f]$}%
   {passive representation in basis manifold}%
   {P}{0}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
   {P}{0}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
   {P}{0}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%
   {P}{0}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
   {R}{0}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
   {R}{0}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
   {R}{0}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
   {R}{0}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
   {R}{0}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
   {R}{0}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
   {R}{0}%
\Symb%
   {произведение колец множеств}%
   {product of rings of sets}%
   {R}{0}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of maps}%
   {R}{0}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
   {R}{0}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
   {R}{0}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
   {R}{0}%
\Symb%
   {правый сдвиг}%
   {right shift}%
   {R}{0}%
\Symb%
   {правое векторное пространство алгебры $A$}%
   {right vector space of algebra A}%
   {R}{0}%
\Symb%
   {правое векторное пространстао отображений}%
   {right vector space of maps B->A}%
   {R}{0}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
   {R}{0}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
   {R}{0}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
   {R}{0}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
   {R}{0}%
\Symb%
   {множество обратных матриц}%
   {set of inverse matrices}%
   {R}{0}%
\Symb%
   {множество правосторонних невырожденных преобразований универсальной алгебры $M$}%
   {set of right-side nonsingular transformations}%
   {R}{0}%
\Symb%
   {сферические координаты}%
   {spherical coordinates}%
   {R}{0}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
   {S}{0}%
\Symb%
   {гиперболический синус}%
   {hyperbolic sine}%
   {S}{0}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
   {S}{0}%
\Symb%
   {интеграл Лебега}%
   {Lebesgue integral}%
   {S}{0}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
   {S}{0}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of permutations}%
   {S}{0}%
\Symb%
   {множество перестановок}%
   {set of transpositions}%
   {S}{0}%
\Symb%
   {синус}%
   {sine}%
   {S}{0}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%
   {S}{0}%

\SetIndexSpace%T%0
\Symb%
   {категория левосторонних представлений}%
   {category of left-side representations}%
   {T}{0}%
\Symb%
   {касательная плоскость к группе Ли $G$}%
   {tangent plane to Lie group}%
   {T}{0}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%
   {T}{0}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
   {V}{0}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
   {V}{0}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
   {V}{0}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
   {V}{0}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
   {V}{0}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
   {V}{0}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
   {V}{0}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
   {V}{0}%
\Symb%
   {линейная комбинация векторов}%
   {linear composition of vectors}%
   {V}{0}%
\Symb%
   {множество векторов, порождённых вектором $v$}%
   {set of vectors generated by vector}%
   {V}{0}%
\Symb%
   {векторное пространство}%
   {V}%
   {V}{0}%
\Symb%
   {векторное пространство начальных значений системы дифференциальных уравнений}%
   {vector space of initial values}%
   {V}{0}%
\Symb%
   {векторное пространство решений системы дифференциальных уравнений}%
   {vector space of solutions}%
   {V}{0}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
   {V}{0}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%
   {V}{0}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
   {W}{0}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
   {W}{0}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
   {W}{0}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates relative to set}%
   {W}{0}%
\Symb%
   {геометрический объект}%
   {geometric object}%
   {W}{0}%
\Symb%
   {множество кортежей $\Omega$\Hyph слов}%
   {set of tuples of Omega words}%
   {W}{0}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
   {W}{0}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
   {W}{0}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
   {W}{0}%
\Symb%
   {суперпозиция координат}%
   {superposition of coordinates}%
   {W}{0}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
   {W}{0}%
\Symb%
   {кортеж $\Omega$\Hyph слов}%
   {tuple of Omega words}%
   {W}{0}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
   {W}{0}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
   {W}{0}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
   {W}{0}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%
   {W}{0}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
   {X}{0}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
   {X}{0}%
\Symb%
   {матрица Вронского}%
   {Wronskian matrix}%
   {X}{0}%
\Symb%
   {неголономная координата}%
   {x(k)}%
   {X}{0}%

\SetIndexSpace%Z%0
\Symb%
   {центр $A$\Hyph числа}%
   {center of A number}%
   {Z}{0}%
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
   {Z}{0}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%
   {Z}{0}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
   {Delta}{1}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
   {Delta}{1}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
   {Delta}{1}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%
   {Delta}{1}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
   {Gamma}{1}%
\Symb%
   {связность}%
   {conection overline}%
   {Gamma}{1}%
\Symb%
   {связность}%
   {connection}%
   {Gamma}{1}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
   {Gamma}{1}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
   {Gamma}{1}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
   {Gamma}{1}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%
   {Gamma}{1}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
   {Lambda}{1}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%
   {Lambda}{1}%

\SetIndexSpace%Mu%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
   {Mu}{1}%
\Symb%
   {степень меры}%
   {power of measure}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures}%
   {Mu}{1}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%
   {Mu}{1}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%
   {Omega}{1}%
\Symb%
   {определённый интеграл}%
   {definite integral}%
   {Omega}{1}%
\Symb%
   {интеграл дифференциальной $1$\Hyph формы вдоль пути}%
   {integral of differential 1 form along path}%
   {Omega}{1}%
\Symb%
   {норма операции}%
   {norm of operation}%
   {Omega}{1}%
\Symb%
   {область операторов}%
   {operator domain}%
   {Omega}{1}%
\Symb%
   {множество дифференциальных $p$\Hyph форм}%
   {set of differential p forms}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операций $\Omega$\Hyph алгебры}%
   {set of n-ary operations}%
   {Omega}{1}%
\Symb%
   {множество $n$\Hyph арных операторов}%
   {set of n-ary operators}%
   {Omega}{1}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
   {Psi}{1}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%
   {Psi}{1}%

\SetIndexSpace%Sigma%1
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
   {Sigma}{1}%
\Symb%
   {чётность перестановки}%
   {parity of permutation}%
   {Sigma}{1}%
\Symb%
   {подрасслоение}%
   {subbundle}%
   {Sigma}{1}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
   {Nabla}{2}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%
   {Nabla}{2}%

\SetIndexSpace%Phi%1
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%
   {Phi}{1}%
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
   {Phi}{1}%

\SetIndexSpace%Pi%1
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_i$, $i\in I$}%
   {Cartesian product of groups}%
   {Pi}{1}%
\Symb%
   {декартово произведение групп $G_1$, ..., $G_n$}%
   {Cartesian product of groups, i 1 n}%
   {Pi}{1}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
   {Pi}{1}%
\Symb%
   {копроизведение в категории}%
   {coproduct in category}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
   {Pi}{1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
   {Pi}{1}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
   {Pi}{1}%
\Symb%
   {произведение в категории}%
   {product in category}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
   {Pi}{1}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%
   {Pi}{1}%

\CloseIndex

